Decompositions and statistics for beta(1,0)-trees and nonseparable permutations

The subject of pattern avoiding permutations has its roots in computer science, namely in the problem of sorting a permutation through a stack. A formula for the number of permutations of length n that can be sorted by passing it twice through a stack (where the letters on the stack have to be in increasing order) was conjectured by West, and later proved by Zeilberger. Goulden and West found a bijection from such permutations to nonseparable planar maps, and later, Jacquard and Schaeffer presented a bijection from these planar maps to certain labeled plane trees, called beta(1,0)-trees. Using generating trees, Dulucq, Gire and West showed that nonseparable planar maps are equinumerous with permutations avoiding the (classical) pattern 2413 and the barred pattern 41\bar{3}52; they called these permutations nonseparable. We give a new bijection between beta(1,0)-trees and permutations avoiding the dashed patterns 3-1-4-2 and 2-41-3. These permutations can be seen to be exactly the reverse of nonseparable permutations. Our bijection is built using decompositions of the permutations and the trees, and it translates seven statistics on the trees into statistics on the permutations. Among the statistics involved are ascents, left-to-right minima and right-to-left maxima for the permutations, and leaves and the rightmost and leftmost paths for the trees. In connection with this we give a nontrivial involution on the beta(1,0)-trees, which specializes to an involution on unlabeled rooted plane trees, where it yields interesting results. Lastly, we conjecture the existence of a bijection between nonseparable permutations and two-stack sortable permutations preserving at least four permutation statistics.

==> pgfbaseimage.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfbaseimage.code.tex,v 1.7 2007/05/31 10:31:50 tantau Exp $


% Declare an image
%
% #1 = optional argument: width, height, page specification
% #2 = name of the image for later use
% #4 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF and .ps, .eps, .epsi for postscript.
%
% Description:
%
% This command declares an image file for later use. Even if the image
% is used several times in the document, in PDF it will only be stored
% once. 
%
% Example:
%
% \pgfdeclareimage[width=2cm,page=2]{myimage}{imagefilename}

\def\pgfdeclareimage{\pgfutil@ifnextchar[{\pgf@declareimage}{\pgf@declareimage[]}}
\def\pgf@declareimage[#1]#2#3{%
  \setkeys{pgfimage}{height=,width=,page=,interpolate=false,mask=}% defaults
  \setkeys{pgfimage}{#1}%
  % Try to find the file
  \gdef\pgf@filename{}%
  % If page= parameter is not empty, try that file first:
  \ifx\pgf@imagepage\pgfutil@empty%
  \else%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3.page\pgf@imagepage}%
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \else%
    \setkeys{pgfimage}{page=}% make page empty     
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \PackageWarning{pgf}%
    {File "#3" not found when defining image "#2".\MessageBreak
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
    \pgf@declaredraftimage{#2}%
  \else%
    \ifpgf@draftmode%
      \pgf@declaredraftimage{#2}%
    \else%
      \pgfsys@defineimage%
    \fi%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@image@#2!\endcsname=\pgf@image%
}

\define@key{pgfimage}{width}{\edef\pgf@imagewidth{#1}}
\define@key{pgfimage}{height}{\edef\pgf@imageheight{#1}}
\define@key{pgfimage}{page}{\edef\pgf@imagepage{#1}}
\define@key{pgfimage}{interpolate}[true]{\edef\pgf@imageinterpolate{/Interpolate #1}}
\define@key{pgfimage}{mask}{%
  \edef\pgf@imagemask{#1}%
  \ifx\pgf@imagemask\pgfutil@empty%
  \else%
    \pgfutil@ifundefined{pgf@mask@#1}%
    {\PackageError{pgf}{Undefined mask "#1".}{}%
      \edef\pgf@imagemask{}}%
    {\edef\pgf@imagemask{\csname pgf@mask@#1\endcsname}%
      \ifx\pgf@imagemask\pgfutil@empty%
      \else
      \edef\pgf@imagemask{/SMask \pgf@imagemask\space 0 R}%
      \fi}%
    \fi}

\def\pgf@findfile#1:#2+#3{%
  \pgfutil@IfFileExists{#3.#1}%
  {\xdef\pgf@filename{#3.#1}}%
  {\def\pgf@mightbeempty{#2}%
    \ifx\pgf@mightbeempty\pgfutil@empty\else%
    \pgf@findfile#2+{#3}%
    \fi}}

\def\pgf@declaredraftimage#1{%
  \ifx\pgf@imagewidth\pgfutil@empty%
    \PackageWarning{pgf}{Missing width for image "#1" in draft mode.\MessageBreak  Using 1cm instead}%
    \edef\pgf@imagewidth{1cm}%
  \fi%
  \ifx\pgf@imageheight\pgfutil@empty%
    \PackageWarning{pgf}{Missing height for image "#1" in draft mode.\MessageBreak Using 1cm instead}%
    \edef\pgf@imageheight{1cm}%
  \fi%  
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepagetext{ page \pgf@imagepage}\fi%
  \edef\pgf@image{%
    \hbox to \pgf@imagewidth{%
      \vrule\kern-0.4pt%
      \vbox to \pgf@imageheight{%
        \hrule\vfil%
        \hbox to \pgf@imagewidth{\hskip-10cm\hfil\noexpand\tiny#1\pgf@imagepage\hfil\hskip-10cm}%
        \vfil\hrule}%
      \kern-0.4pt\vrule}%
  }%
}



% Declare a soft mask
%
% #1 = optional argument: matte specification. default matte is
%      white. 
% #2 = name of the mask for later use
% #3 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF. Postscript is not supported.
%
% Description:
%
% This command declares a soft mask for later masking an image. The
% declared mask should be used together with an image of exactly the
% same height/width if matte is defined. Matte should be the
% preblended background color (see pdf spec for details).
%
% Example:
%
% \pgfdeclaremask[matte=white]{maskname}{maskfilename}
% \pgfdeclareimage[mask=maskname]{image}{imagefilename}

\def\pgfdeclaremask{\pgfutil@ifnextchar[\pgf@declaremask{\pgf@declaremask[]}}
\def\pgf@declaremask[#1]#2#3{%
  \setkeys{pgfmask}{matte={1 1 1}}% defaults
  \setkeys{pgfmask}{#1}%
  \def\pgf@mask{}%
  % Try to find the file
  \gdef\pgf@filename{}%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \ifx\pgf@filename\pgfutil@empty%
    \PackageWarning{pgf}%
    {File "#3" not found when defining mask "#2".\MessageBreak
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
  \else%
    \pgfsys@definemask%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@mask@#2\endcsname=\pgf@mask%
}

\define@key{pgfmask}{matte}{\edef\pgf@maskmatte{#1}}




% Create an alias name for an image
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfdeclareimage{image}{1cm}{1cm}{filename
% \pgfaliasimage{alias}{image}
% \pgfuseimage{alias}

\def\pgfaliasimage#1#2{%
  \expandafter\global\expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@image@#2!\endcsname%
  \expandafter\global\expandafter\let\csname pgf@image@#1!\endcsname=\pgf@temp%
  }

  
% Use an image
%
% #1 = name of a previously declared image
%
% Example:
%
% \pgfputat{\pgforigin}{\pgfbox[left,base]{\pgfuseimage{myimage}}}

\def\pgfuseimage#1{%
  \def\pgf@imagename{pgf@image@#1}%
  \pgf@tryextensions{\pgf@imagename}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@imagename}%
  {\PackageError{pgf}{Undefined image "#1"}{}}%
  {{\leavevmode\csname\pgf@imagename\endcsname}}}

\def\pgf@tryextensions#1#2{%
  \edef\pgf@args{[#2!]}\expandafter\pgf@@tryextensions\pgf@args{#1}}
\def\pgf@@tryextensions[#1!#2]#3{%
  \expandafter\pgfutil@ifundefined\expandafter{#3.#1!#2}%
  {\def\pgf@temp{#2}%
    \ifx\pgf@temp\pgfutil@empty%
    \edef#3{#3!}%
    \else%
    \pgf@@tryextensions[#2]{#3}%
    \fi}%
  {\edef#3{#3.#1!#2}}}


% Alternate image
%
% Description:
%
% When an image is used, pgf first attempts to use the image with the
% alternate extension added. If this fails, the original image is
% used. If the alternate extension contains ``!'', then the text up to
% the ! is successively removed and the remainder is tried as an
% alternate extension.
%
% Example:
%
% \def\pgfalternateextension{20!white}

\def\pgfalternateextension{}



% Directly insert an image
%
% #1 = optional argument: width, height, page specification
% #2 = file name
%
% Description:
%
% Directly inserts an image without declaration. You can, however,
% still access this image using the name pgflastimage. By using
% pgfaliasimage, you can also save this image for later.
%
% Example:
%
% \pgfimage[height=2cm]{filename}

\def\pgfimage{\pgfutil@ifnextchar[\pgf@imagecom{\pgf@imagecom[]}}
\def\pgf@imagecom[#1]#2{%
  \pgfdeclareimage[#1]{pgflastimage}{#2}%
  \pgfuseimage{pgflastimage}}








% The external read/write mechanism is used as follows:
%
% In your document, you put a number or all of your pgfpicture (or
% tikzpicture) environments inside a pair of \beginpgfexternal and
% \endpgfexternal. The \beginpgfexternal gets one parameter called the
% graphics name.
%
% Once this is done, the next step is to declare the names of your
% graphics in the document at the beginning using the
% \pgfdeclaregraphicname command.
%
% Now, when you typeset your document, each time a \beginpgfexternal
% command is encountered, it will be checked whether the corresponding
% graphics file exists. If this is the case, it will be included and
% the code between \beginpgfexternal and \endpgfexternal is
% ignored. Otherwise, the code is executed normally.
%
% Things change when you run tex on your file with the \jobname set to
% the name of a decalred graphics name. In this case, only your
% graphic will be typeset, the rest of the document will be "thrown away". 
% To be more precise, everything is gobbled up to the beginning
% of the first \beginpgfexternal with the given graphics name. Then,
% the content of the "environment" is put in a box (this "environment"
% need not contain a graphics, it may contain anything that can be put
% in a box). Then a single page is output whose size is exactly the
% size of the picture.
%
% So, once you have run tex repeatedly, each time with the jobname set
% to each of the graphics, you can then run tex on the whole document
% and this will cause all graphics to be included rather than begin
% typeset.
%
% Finally, once all the graphics have been created, you can also say
% \input pgfexternal.tex instead of including pgf/TikZ.



% Tells pgf which jobname is the name of the real file
%
% #1 = name
%
% Description:
%
% This command is used to tell pgf that the file named #1 should be
% typeset normally. If \jobname is not equal to #1, only
% the graphic called \jobname will be typeset. 
%
% Example:
%
% \pgfrealjobname{survey}

\def\pgfrealjobname#1{%
  \edef\pgf@tempa{\expandafter\string\csname #1\endcsname}%
  \edef\pgf@tempb{\expandafter\string\csname\jobname\endcsname}%
  \ifx\pgf@tempa\pgf@tempb%
  \else%
    \pgf@external@grabshipouttrue
  \fi%
}


\newif\ifpgf@external@grabshipout
\newbox\pgfexternal@startupbox

\AtBeginDocument{%
  \ifpgf@external@grabshipout
    \global\let\pgfexternal@originalshipout=\shipout%
    \global\def\shipout{\setbox\pgfpic=}
    \maxdeadcycles=10000%
    % Ok, gather everything we have seen up to now in a box. This box
    % will contain any specials that have been used.
    {%
      \output{\global\setbox\pgfexternal@startupbox=\vbox{\csname @begindvi\endcsname\unvbox255}}%
      \hbox{}\eject%
    }%
  \fi%
}


% "Environment" for an external graphic.
%
% #1 = graphic name
%
% Example:
%
% \beginpgfgraphicnamed{main-graphic2}
%   \begin{tikzpicture}
%     ...
%   \end{tikzpicture}
% \endpgfgraphicnamed

\def\pgf@externalbegin#1{%
  % First, check whether we wish to grab this graphic:
  \let\pgf@next=\pgf@external@normal%
  \ifpgf@external@grabshipout
    \edef\pgf@tempa{\expandafter\string\csname #1\endcsname}%
    \edef\pgf@tempb{\expandafter\string\csname\jobname\endcsname}%
    \ifx\pgf@tempa\pgf@tempb%
      \let\pgf@next=\pgf@external@grab%
    \fi%
  \fi%
  \pgf@next{#1}%
}


\AtBeginDocument{
  \let\beginpgfgraphicnamed=\pgf@externalbegin% overwrite definition of pgfexternal.tex if necessary   
  \let\endpgfgraphicnamed=\unskip
}


% Normal operation: Include an external graphic instead of the
% picture, if such an external picture exists.
\def\pgf@external@normal#1{%
  \let\pgf@filename=\pgfutil@empty%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#1}%
  \ifx\pgf@filename\pgfutil@empty%
    % Ok, no such image... Just typeset the picture normally.
    \let\pgf@next=\relax%
  \else%
    \let\pgf@next=\pgf@replacepicturebygraphic%
  \fi%
  \pgf@next%  
}

\long\def\pgf@replacepicturebygraphic#1\endpgfgraphicnamed{\includegraphics{\pgf@filename}\unskip}


% Grab operation: If jobname matches the graphic name, typeset this
% picture normall.

\def\pgf@external@grab#1{%
  \setbox\pgfpic=\hbox\bgroup\bgroup%
    \let\endpgfgraphicnamed=\pgf@externalend%
}

\def\pgf@externalend{%
  \unskip\egroup\egroup%
  {%
    \parindent0pt%
    \leftmargin0pt%
    \rightmargin0pt%
    \dimen0\ht\pgfpic%
    \advance\dimen0\dp\pgfpic%
    \pgfsys@papersize{\the\wd\pgfpic}{\the\dimen0}%
    \setbox0=\vbox{%
      \kern -1truein%
      \hbox{%
        \kern -1truein%
        \hbox to0pt{%
          \wd\pgfexternal@startupbox=0pt%
          \ht\pgfexternal@startupbox=0pt%
          \dp\pgfexternal@startupbox=0pt%
          \box\pgfexternal@startupbox%
          \pgfsys@atbegindocument\hss}%
        \box\pgfpic%
        \kern 1truein}%
      \kern1truein}%
    \pgfexternal@originalshipout\box0%
  }%
}


\endinput


==> pgfbaselayers.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfbaselayers.code.tex,v 1.5 2006/10/16 22:32:58 tantau Exp $


% Creates a new pgf layer
%
% #1 = layer name
%
% Declares a new layer for pgf.
%
% Example:
%
% \pgfdeclarelayer{background}

\def\pgfdeclarelayer#1{%
  \expandafter\pgf@newbox\csname pgf@layerbox@#1\endcsname%
  \expandafter\pgf@newbox\csname pgf@layerboxsaved@#1\endcsname%
}
\let\pgf@newbox=\newbox % avoid plain TeX outer problem

% Sets the layers that compose the picture
%
% #1 = List of layers
%
% Description:
%
% Sets the list of layers that make up the picture. The layers will be
% put on top of each other in the order given. 
%
% Example:
%
% \pgfsetlayers{background,main}

\def\pgfsetlayers#1{\edef\pgf@layerlist{#1}}
\pgfsetlayers{main}



% Adds code to a layer
%
% #1 = layer name
%
% Note:
%
% You cannot anything to the ``main'' layer using this command.
%
% Example:
%
% \begin{pgfonlayer}{background}
%   \fill[red] (0,0) -- (1,1);
% \end{pgfonlayer}

\def\pgfonlayer#1{%
  \expandafter\global\expandafter%
  \setbox\csname pgf@layerbox@#1\endcsname=\hbox to 0pt%
    \bgroup%
      \expandafter\box\csname pgf@layerbox@#1\endcsname%
      \begingroup%
}
\def\endpgfonlayer{%
      \endgroup%
      \hss
    \egroup%
}




% Hooks into the scoping:

\def\pgf@insertlayers{%
  \expandafter\pgf@dolayer\pgf@layerlist,,\relax%
}
\def\pgf@maintext{main}%
\def\pgf@dolayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
    \box\pgf@layerbox@main%
  \else%
    \pgfsys@beginscope%
      \expandafter\box\csname pgf@layerbox@#1\endcsname%
    \pgfsys@endscope%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dolayer#2,\relax%
  \fi%
}

\def\pgf@savelayers{%
  \expandafter\pgf@dosavelayer\pgf@layerlist,,\relax%
}
\def\pgf@dosavelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
  \else%
    \setbox\csname pgf@layerboxsaved@#1\endcsname=\box\csname pgf@layerbox@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosavelayer#2,\relax%
  \fi%
}

\def\pgf@restorelayers{%
  \expandafter\pgf@dorestorelayer\pgf@layerlist,,\relax%
}
\def\pgf@dorestorelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
  \else%
    \global\setbox\csname pgf@layerbox@#1\endcsname=\box\csname pgf@layerboxsaved@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dorestorelayer#2,\relax%
  \fi%
}

\endinput


==> pgfbasematrix.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfbasematrix.code.tex,v 1.11 2007/03/09 17:49:32 tantau Exp $


\newif\ifpgfmatrix
\newif\ifpgf@matrix@correct@call

\newif\ifpgf@matrix@fixed

\newcount\pgfmatrixcurrentrow

\newcount\pgfmatrixcurrentcolumn
\newcount\pgf@matrix@numberofcolumns

\let\pgf@matrix@cell=\pgfnodeparttextbox % alias
\let\pgf@matrix@box=\pgf@matrix@cell % alias


% Sets the default row or column sep
%
% #1 = default row or column sep list
%
% Description:
%
% Sets the macro \pgfmatrixrowsep or \pgfmatrixcolumnsep to #1.
%
% Example:
%
% \pgfsetmatrixrowsep{5pt}

\def\pgfsetmatrixrowsep#1{\def\pgfmatrixrowsep{#1}}
\def\pgfsetmatrixcolumnsep#1{\def\pgfmatrixcolumnsep{#1}}

\def\pgfmatrixrowsep{0pt}
\def\pgfmatrixcolumnsep{0pt}



% The pgfmatrix command creates a node that contains a matrix. Like
% the \pgfnode command, it is to be used inside a pgfpicture
% environment. 
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
% #5 = inner shift
% #6 = startup code
% #7 = the matrix code (may contain verbatim stuff)
%
% Description:
%
% This command creates a node that contains a matrix. For 
% each cell of the matrix, drawing commands may be given. These
% commands will create a cell picture and a bounding box is computed
% for each cell picture. The cell picture is then placed inside the
% cell. The position inside the cell is computed according to the
% following rules: 
%
% 1. In each column, the origins of the cell pictures are all on a
%    vertical line.
% 2. In each row, the origins of the cell pictures are all on a
%    horizontal line.
% 3. All cells in the same row have the same height and depth.
% 4. All cells in the same column have the same width.
% 5. The size of cells are chosen minimal such that the boxes fit into
%    the cells and still meet the above requirement.
%
% Next, the whole resulting matrix, which is given as #7, is placed
% inside a node whose name is given as #3, whose shape is #1, and
% whose anchor is #1. This means that the resulting node is shifted
% such that the given anchor lies at the origin. Then, as for a normal
% node, the #4 path usage command is used for the node. 
%
% The parameter #5 is an additional negative shift for the node. Normally, such
% a shift could be given beforehand (that is, the shift could be
% preapplied to the current transformation matrix). However, when #5
% is evaluated, you can refer to temporary positions of nodes inside
% the matrix. In detail, the following happens: When the matrix has
% been typeset, all nodes in the matrix temporarily get assigned their
% positions in the matrix box. The origin of this coordinate system is
% at the left baseline end of the matrix box, which corresponds to the
% text anchor. The position #5 is then interpreted inside this
% coordinate system and then used for shifting. 
%
% The idea behind using the parameter #5 is the following: If you
% specify "text" as anchor #2 and specify \pgfpointanchor{inner
% node}{some anchor} for parameter #5, where inner node is a node that
% is created in the matrix, then the whole matrix will be shifted such
% that inner node.some anchor lies at the origin of the whole picture.
%
% At the beginning and at the end of each cell, the macros
% \pgfmatrixbegincode and \pgfmatrixendcode are called. Inside these
% macros you can use \pgfmatrixcurrentcolumn and \pgfmatrixcurrentrow
% to access the current row and column.
%
% Before each column except for the first, an extra space given by the
% macro \pgfmatrixcolumnsep is added. Additionally, an extra space
% given by the optional argument of the \pgfmatrixnextcell commands in
% the first line are added, which may vary between columns. Between
% rows, an extra space given by the macro \pgfmatrixrowsep is
% added. You can also change this value for each row by using a \gdef.
%
% Inside the matrix, \\ must be used to end every line ***including
% the last***. You can pass an optional parameter to \\ as in \\[2pt]
% to give an additional space after this particular line.
%
% The usage of \\ at the end of the matrix is imporant since this
% command is used to find the end of the matrix. What happens is that
% \\ followed by a closing brace ends the matrix. 
%
% Inside the matrix, you must use \pgfmatrixnextcell to separate
% columns. The reason is that two columns are used internally for
% every single column shown. The macro \pgfmatrixnextcell is yields
% (more or less) two && (and some further trickery).
%
% The parameter #6 is executed at the beginning of the matrix
% group. It is inside the protecting group of the matrix, but outside
% the matrix itself. It can be used for different purposes: 1) It can be
% used to simplify the next cell macro. 2) It can be used to issue an
% \aftergroup command. 3) It can be used to setup local settings. For
% example, by setting #6 to \let\&=\pgfmatrixnextcell you can use \&
% instead of \pgfmatrixnextcell. You can also set the catcode of & to
% active.
%
%
% Example:
%
% \begin{tikzpicture}
%
%   \draw (0,0) circle (1mm);  % b.north will lie on the center of this circle
%
%   \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{\let\&=\pgfmatrixnextcell}
%   {
%     \draw (0,0) circle (1cm); \& \node (a) [draw] {Hallo}; \\
%     \node (b) [draw] {Welt};  \& \draw (0,0) circle (5mm); \\
%   }
%
%   \draw [->] (a) -- (b);
%
% \end{tikzpicture}

\def\pgfmatrix#1#2#3#4#5#6{%
  \ifpgfmatrix%
    \PackageError{pgf}{You cannot nest pgfmatrix environments, yet}{}
  \fi%
  \bgroup%  
    #6%
    \def\pgf@matrix@par@shape{#1}%
    \def\pgf@matrix@par@anchor{#2}%
    \def\pgf@matrix@par@name{#3}%
    \def\pgf@matrix@par@usage{#4}%
    \def\pgf@matrix@par@shift{#5}%
    % the matrix must have a name:
    \ifx\pgf@matrix@par@name\pgfutil@empty%
      \def\pgf@matrix@par@name{pgf@matrix@internal}%
    \fi%
    \pgfmatrixcurrentrow=0\relax%
    \pgfmatrixcurrentcolumn=0\relax%
    \pgf@matrix@numberofcolumns=0\relax%
    \let\\=\pgf@matrix@eol%
    \tabskip=0pt%
    \offinterlineskip%
    \pgfmatrixtrue%
    \let\pgf@matrix@node@list=\pgfutil@empty%
    \expandafter\let\csname pgf@matrix@column@finish@1\endcsname=\pgfutil@empty%
    \let\pgf@matrix@row@finish=\pgfutil@empty%
    % 
    % Get rid of bgroup
    %
    \afterassignment\pgf@matrix@cont\let\pgf@next=%
}
\def\pgf@matrix@cont{%  
    \setbox\pgf@matrix@box=\hbox\bgroup\vbox\bgroup%
    \halign\bgroup%
    \pgf@matrix@init@row%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }%
    &%
    ##\pgf@matrix@padding&&%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }&%
    ##\pgf@matrix@padding%
    \cr%
}

\def\pgf@end@matrix{%
      \egroup\egroup%
    \egroup%
    %
    % If there are named nodes, we must adjust their coordinates.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      % Ok, this means we got a lot of work to do...
      \pgf@matrix@compute@origin%
      \pgf@matrix@shift@nodes@initial%
    \fi%
    %
    % Compute additional shift
    %
    \pgftransformresetnontranslations%
    \pgftransformshift{\pgf@process{\pgftransformreset\pgf@matrix@par@shift\pgf@x=-\pgf@x\pgf@y=-\pgf@y}}%
    %
    % Create node
    %
    \pgfmultipartnode{\pgf@matrix@par@shape}{\pgf@matrix@par@anchor}{\pgf@matrix@par@name}{\pgf@matrix@par@usage}%
    %
    % If there are named nodes, we must adjust their coordinates, again.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      {%
        \pgftransformreset%
        \pgf@process{\pgfpointanchor{\pgf@matrix@par@name}{text}}%
        \xdef\pgf@matrix@offset{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
        \pgf@matrix@shift@nodes@secondary{\pgf@matrix@offset}%
      }%
    \fi%
}




% Ending a cell
%
% #1 = (optional) spacing between previous and next column. This
%      parameter only has an effect in the first row.
%
% Description:
%
% This command ends a cell of a matrix.
%
% Example:
%
% \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{}
% {
%   \draw (0,0) circle (1cm); \pgfmatrixnextcell[1cm] \node (a) [draw] {Hallo}; \\
%   \node (b) [draw] {Welt};  \pgfmatrixnextcell \draw (0,0) circle (5mm); \\
% }

\def\pgfmatrixnextcell{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end%
  \pgfutil@ifnextchar[{\pgf@matrix@cell@cont}{\pgf@matrix@cell@cont[0pt]}}%}

\def\pgf@matrix@cell@cont[#1]{%
  \ifnum\pgfmatrixcurrentcolumn<\pgf@matrix@numberofcolumns%
  \else%
  {%
    \global\pgf@matrix@fixedfalse%
    \pgf@x=0pt%
    \pgf@matrix@addtolength{\pgf@x}{\pgfmatrixcolumnsep}%
    \pgf@matrix@addtolength{\pgf@x}{#1}%
    \ifpgf@matrix@fixed%
      \expandafter\pgfutil@g@addto@macro\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
        {\global\pgf@picmaxx=0pt}%
    \fi%
    \advance\pgfmatrixcurrentcolumn by1\relax % only temporary for the following:
    \expandafter\xdef\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@x}%
    \ifpgf@matrix@fixed%
      \expandafter\gdef\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname{\global\pgf@picminx=0pt}%
    \else%
      \expandafter\global\expandafter\let\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname=\pgfutil@empty%
    \fi%
  }%
  \fi%
  &\pgf@matrix@correct@calltrue&%
}%


\def\pgf@matrix@fixed@text{between origins}
\def\pgf@matrix@natural@text{between borders}

\def\pgf@matrix@addtolength#1#2{\edef\pgf@temp{#2}\expandafter\pgf@matrix@addtolength@\expandafter#1#2,\pgf@stop}
\def\pgf@matrix@addtolength@#1#2,#3\pgf@stop{%
  \def\pgf@temp{#2}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \ifx\pgf@temp\pgf@matrix@fixed@text%
      \global\pgf@matrix@fixedtrue%
    \else%
      \ifx\pgf@temp\pgf@matrix@natural@text%
        \global\pgf@matrix@fixedfalse%
      \else%
        \pgfmathaddtolength{#1}{#2}%
      \fi%
    \fi%
  \fi%
  \def\pgf@temp{#3}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \pgf@matrix@addtolength@#1#3\pgf@stop%
  \fi%
}



% Init a line

\def\pgf@matrix@init@row{%
  \relax%
  \global\advance\pgfmatrixcurrentrow by 1\relax%
  \global\pgfmatrixcurrentcolumn=0\relax%
  \expandafter\gdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{0pt}%
  \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
}



% Step the row column number

\def\pgf@matrix@step@column{%
  \relax%
  \global\advance\pgfmatrixcurrentcolumn by1\relax%
}



% Start a cell

\def\pgf@matrix@startcell{%
  %
  % Step 1: Init the list of nodes for this cell
  %
  \let\pgf@nodecallback=\pgf@matrix@nodecallback%
  %
  % Step 2: Setup the bounding box
  %
  \pgfinterruptboundingbox%
  %
  % Step 3: Reset the transformation matrix
  %
  \pgftransformreset%
  %
  % Step 4: Collect everything in a cell box
  %
  \setbox\pgf@matrix@cell=\hbox\bgroup\bgroup%
    \pgfsys@beginpicture%
    \normalbaselines%
    % Find out whether the cell is empty:
    \pgfutil@ifnextchar\let%
    {% ok, candidate, check following symbol
      \afterassignment\pgf@matrix@empty@check\let\pgf@next=% get rid of \let
    }%
    {% no, not empty
      \pgf@matrix@empty@cell@false%
      \pgfmatrixbegincode%
    }%
}

\def\pgf@matrix@empty@check{%
  \pgfutil@ifnextchar\pgf@matrix@signal@cell@end%
  {% Bingo!
    \pgf@matrix@empty@cell@true%
    \pgfmatrixemptycode%
    \let% reinserted
  }%
  {% Nope!
    \pgf@matrix@empty@cell@false%
    \pgfmatrixbegincode%
    \let% reinserted
  }
}%

\newif\ifpgf@matrix@empty@cell@


% End a  cell

\def\pgf@matrix@endcell{%
    \ifpgf@matrix@empty@cell@%
    \else%
      \expandafter\pgfmatrixendcode%
    \fi
    \pgfsys@endpicture%
    \csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
    \pgf@matrix@row@finish%
  \egroup\egroup%
  % Special case of the empty picture
  \ifdim\pgf@picmaxx=-16000pt\relax%
    \pgf@picmaxx=0pt\relax%
    \pgf@picminx=0pt\relax%
    \pgf@picmaxy=0pt\relax%
    \pgf@picminy=0pt\relax%
  \fi%
  %
  % Step 5: Horizontal gap
  %
  \ifnum\pgfmatrixcurrentcolumn>1\relax%
    \pgf@y=\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname\relax%
    \advance\pgf@picminx by-\pgf@y%
  \fi%
  % 
  % Step 6: Protocol and adjust height and depth
  %
  % Step 6.1: Protocol...
  %
  \ifdim\pgf@picmaxy>\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picmaxy}%
  \fi%  
  \ifdim\pgf@picminy<\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picminy}%
  \fi%  
  %
  % Step 6.2: and setup.
  %  
  \ht\pgf@matrix@cell=\pgf@picmaxy%
  \dp\pgf@matrix@cell=-\pgf@picminy%
  %
  % Step 7: Protocol and adjust left and right width
  %
  % Step 7.1: Protocol...
  %
  \ifnum\pgfmatrixcurrentcolumn>\pgf@matrix@numberofcolumns\relax%
    \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \global\pgf@matrix@numberofcolumns=\pgfmatrixcurrentcolumn\relax%
  \else%
    \ifdim\pgf@picmaxx>\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \fi%  
    \ifdim\pgf@picminx<\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \fi%  
  \fi%
  %
  % Step 7.2: and setup.
  %  
  \xdef\pgf@matrix@paddingskip{\the\pgf@picmaxx}%
  % 
  % Step 8: Put in the box now
  %
  \hfil\hskip-\pgf@picminx%
  \wd\pgf@matrix@cell=0pt%
  \box\pgf@matrix@cell%
  %
  % Step 9: End bounding box
  \endpgfinterruptboundingbox%
}

% Default code for the start and end code
\let\pgfmatrixbegincode=\relax
\let\pgfmatrixendcode=\relax
\let\pgfmatrixemptycode=\relax


% The following callback is called for every node that is produced
% inside a cell

\def\pgf@matrix@nodecallback#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \xdef\pgf@matrix@node@list{\pgf@matrix@node@list,{#1}}%
    \expandafter\xdef\csname pgf@matrix@node@location@#1\endcsname{{\the\pgfmatrixcurrentrow}{\the\pgfmatrixcurrentcolumn}}%
  \fi%
}



% Padding code

\def\pgf@matrix@padding{%
  \ifpgf@matrix@correct@call%
  \else%
    \PackageError{pgfbasematrix}{Single ampersand used with wrong
      catcode}{}%
  \fi%
  \hskip\pgf@matrix@paddingskip\hfil%
}


% Compute the real positions of the origins

% We must now compute the real positions of the origins of all the
% small pictures. To this end, we need to compute prefix sums. After
% the procedure is done, the minx and the maxy will contain the origin
% positions. 

\def\pgf@matrix@compute@origin{%
  %
  % Inverse prefix sum on the vertical positions
  %
  {%
    \ifnum\pgfmatrixcurrentrow>0\relax%
      \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
    \fi
    \c@pgf@counta=\pgfmatrixcurrentrow\relax%
    \loop%
    \ifnum\c@pgf@counta>1\relax%
      \pgf@y=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by\csname pgf@matrix@maxy\the\c@pgf@counta\endcsname\relax
      \advance\c@pgf@counta by-1\relax%
      \pgf@ya=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by-\pgf@ya\relax%
      \expandafter\xdef\csname pgf@matrix@miny\the\c@pgf@counta\endcsname{\the\pgf@y}%
    \repeat%
  }%
  %
  % Prefix sum on the horizontal positions
  %
  {%
    \ifnum\pgf@matrix@numberofcolumns>0\relax%
      \pgf@x=\csname pgf@matrix@minx1\endcsname\relax%
      \pgf@x=-\pgf@x%
      \expandafter\xdef\csname pgf@matrix@minx1\endcsname{\the\pgf@x}%
    \fi
    \c@pgf@counta=1\relax%
    \loop%
    \ifnum\c@pgf@counta<\pgf@matrix@numberofcolumns\relax%
      \pgf@x=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by\csname pgf@matrix@maxx\the\c@pgf@counta\endcsname\relax%
      \advance\c@pgf@counta by1\relax%
      \pgf@xa=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by-\pgf@xa\relax%
      \expandafter\xdef\csname pgf@matrix@minx\the\c@pgf@counta\endcsname{\the\pgf@x}%
    \repeat%
  }%
}


% Shift the nodes to their origins

% The following procedure shifts all nodes in
% \pgf@matrix@node@list to their location inside a temporary
% picture. This picture will later be shifted again to its final
% position in the real picture.

\def\pgf@matrix@shift@nodes@initial{%
  {%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{%
          \pgf@x=\csname pgf@matrix@minx%
            \expandafter\expandafter\expandafter\pgfutil@secondoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          \pgf@y=\csname pgf@matrix@miny%
            \expandafter\expandafter\expandafter\pgfutil@firstoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          }%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
  }%
}


% The second shifting, done in the following procedure, shifts all
% nodes to their real positions inside the real picture.

\def\pgf@matrix@shift@nodes@secondary#1{%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{#1}%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
}


% End of line
\def\pgf@matrix@eol{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end%
  &\pgf@matrix@correct@calltrue%
  \global\pgf@matrix@fixedfalse%
  \pgf@y=0pt%
  \pgf@matrix@addtolength\pgf@y{\pgfmatrixrowsep}%
  \pgfutil@ifnextchar[{\pgf@matrix@eol@skip}{\pgf@matrix@finish@line}%
}

\def\pgf@matrix@signal@cell@end{\pgf@matrix@signal@cell@end}
% exact definition does not matter, only needs to be unique.

\def\pgf@matrix@eol@skip[#1]{%
  \pgf@matrix@addtolength\pgf@y{#1}%
  \pgf@matrix@finish@line%
}

\def\pgf@matrix@finish@line{%
  \global\pgf@y=\pgf@y%
  \pgf@ya=-\pgf@y%
  \global\advance\pgf@ya by\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
  \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@ya}%
  \@ifnextchar\egroup{\cr\pgf@end@matrix}{\pgf@matrix@no@eom@found}%
}

\def\pgf@matrix@eom@found{%
  \cr%
  \pgf@end@matrix%
}

\def\pgf@matrix@no@eom@found{%
  \cr%
  \noalign{\vskip\pgf@y%
  \ifpgf@matrix@fixed%
    \vskip\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname% unskip
    \vskip\pgf@y%
    \pgf@y=-\pgf@y%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@y}%
    \gdef\pgf@matrix@row@finish{\global\pgf@picmaxy=0pt}%
  \else%
    \global\let\pgf@matrix@row@finish=\pgfutil@empty%
  \fi%
  }%
}


\endinput


==> pgfbasepatterns.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfbasepatterns.code.tex,v 1.10 2007/02/05 11:23:22 tantau Exp $


% Creates a new uncolored pattern
%
% #1 = pattern name
% #2 = lower left of bounding box
% #3 = upper right of bounding box
% #4 = step vector
% #5 = pattern code
%
% Description:
%
% Declares a new uncolored pattern. An uncolored pattern is a pattern
% that has no inherent color. When the pattern is used, a color for
% the pattern must be supplied.
%
% See the pdf-manual for more details on uncolored patterns.
%
% The bounding box must be a bounding box of the pattern cell.
%
% The step vector must provide the x- and y-step by which the cells
% are spaced.
%
% The pattern code should be pgf code that can be protocolled.
%
% The transformation matrix will be reset prior to invoking the
% pattern code.
%
% Example:
%
% \pgfdeclarepatternformonly{stars}{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% {\pgfpoint{1cm}{1cm}}{
%   \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
%   \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{144}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{288}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{72}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{216}{4mm}}
%   \pgfpathclose%
%   \pgfusepath{stroke}
% }

\def\pgfdeclarepatternformonly#1#2#3#4#5{\pgf@declarepattern{#1}{#2}{#3}{#4}{#5}{0}}

% Creates a new colored pattern
%
% #1 = pattern name
% #2 = lower left of bounding box
% #3 = upper right of bounding box
% #4 = step vector
% #5 = pattern code
%
% Description:
%
% Declares a new colored pattern. Such patterns have a one or more
% fixed inherent colors. See the pdf-manual for more details on
% uncolored patterns.
%
% The parameters have the same effect as for uncolored patterns.
%
% Example:
%
% \pgfdeclarepatterninherentlycolored{red stars}{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% {\pgfpoint{1cm}{1cm}}{
%   \pgfsetfillcolor{red}
%   \pgfsetstrokecolor{black}
%   \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
%   \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{144}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{288}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{72}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{216}{4mm}}
%   \pgfpathclose%
%   \pgfusepath{stroke,fill}
% }

\def\pgfdeclarepatterninherentlycolored#1#2#3#4#5{\pgf@declarepattern{#1}{#2}{#3}{#4}{#5}{1}}

\def\pgf@declarepattern#1#2#3#4#5#6{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
  \pgfsysprotocol@getcurrentprotocol\pgf@pattern@temp%
  {%
    \pgfinterruptpath%
      \pgfpicturetrue%
      \pgf@relevantforpicturesizefalse%
      \pgftransformreset%
      \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
      \pgfsysprotocol@bufferedtrue%
      \pgfsys@beginscope%
      #5%
      \pgfsys@endscope%
      \pgfsysprotocol@getcurrentprotocol\pgf@pattern@code%
      \global\let\pgf@pattern@code=\pgf@pattern@code%
    \endpgfinterruptpath%
    \pgf@process{#2}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#3}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#4}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    % Now, build a name for the pattern
    \pgfutil@tempcnta=\pgf@pattern@number%
    \advance\pgfutil@tempcnta by1\relax%
    \xdef\pgf@pattern@number{\the\pgfutil@tempcnta}%
    \expandafter\xdef\csname pgf@pattern@name@#1\endcsname{\the\pgfutil@tempcnta}%
    \expandafter\gdef\csname pgf@pattern@type@#1\endcsname{#6}%
    \xdef\pgf@marshal{\noexpand\pgfsys@declarepattern
      {\csname pgf@pattern@name@#1\endcsname}
      {\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xb}{\the\pgf@yb}{\the\pgf@xc}{\the\pgf@yc}{\pgf@pattern@code}{#6}}%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgf@pattern@temp%
  \expandafter\global\expandafter\let\csname pgf@pattern@instantiate@#1\endcsname=\pgf@marshal%
  }
  {%
    \PackageError{pgfbasepatterns}{Pattern `#1' already defined}{}%
  }%
}

\def\pgf@pattern@number{0}%

\def\pgf@ifpatternisinherentlycolored#1#2#3{%
  \expandafter\ifnum\csname pgf@pattern@type@#1\endcsname=1\relax#2\else#3\fi%
}



% Set an pattern as fill color
%
% #1 = Name of the pattern
% #2 = Color to be used for the pattern. If the pattern is already
%      colored, this parameter is ignored.
%
% Description:
%
% Sets the pattern for subsequent filling operations.
%
% Example:
%
% \pgfsetfillpattern{stars}{red}

\def\pgfsetfillpattern#1#2{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
    \PackageError{pgfbasepatterns}{Undefined pattern `#1'}{}}
  {%
    \csname pgf@pattern@instantiate@#1\endcsname%
    \expandafter\global\expandafter\let\csname pgf@pattern@instantiate@#1\endcsname=\relax%
    \pgf@ifpatternisinherentlycolored{#1}{%
      \pgfsys@setpatterncolored{\csname pgf@pattern@name@#1\endcsname}%
    }{%
      \pgfutil@colorlet{pgf@tempcolor}{#2}%
      \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
      \pgfutil@extractcolorspec{pgf@tempcolor}{\pgf@tempcolor}%
      \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
      \expandafter\pgf@set@fill@patternuncolored\pgf@rgbcolor\relax{#1}%
    }%
  }%
}
\def\pgf@set@fill@patternuncolored#1,#2,#3\relax#4{%
  \pgfsys@setpatternuncolored{\csname pgf@pattern@name@#4\endcsname}{#1}{#2}{#3}%
}




\endinput


==> pgfbaseplot.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfbaseplot.code.tex,v 1.7 2007/05/02 14:08:27 tantau Exp $


% PGF's plotting interface works as follows:
%
% In order to plot something, two things need to be done. First, you
% need to provide the coordinates (obviously) of the points that
% should be plotted. The coordinates are given via a long stream of
% commands. These commands are \pgfplotstreamstart, which is
% given exactly once at the beginning, \pgfplotstreampoint, of which there
% are numerous in the middle, \pgfplotstreamspecial, of which there may be
% numerous in the middle, and \pgfplotstreamend, which must be given
% at the end. Between these commands arbitrary other commands may be
% given. Here is an example:
%
% ...
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampoint{\pgfpointxy{3}{9}}
% \pgfplotstreamspecial{some handler-dependent special stuff}
% \pgfplotstreamend
%
% By themselves, the \pgfplotstreamxxxx commands do not do anything by
% default. Rather, the ``use'' such a stream, you must first install a
% stream handler. For example, the ``lineto'' handler will simply
% translate every \pgfplotstreampoint into a \pgfpathlineto.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
%
% \pgfplothandlerlineto
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampoint{\pgfpointxy{3}{9}}
% \pgfplotstreamend


% The stream commands actually call their ``internal'' versions, which
% are set by the handlers:
\def\pgfplotstreamstart{\pgf@plotstreamstart}
\def\pgfplotstreampoint#1{\gdef\pgfplotlastpoint{#1}\pgf@plotstreampoint{#1}}
\def\pgfplotstreamspecial{\pgf@plotstreamspecial}
\def\pgfplotstreamend{\pgf@plotstreamend}




% Sets the action taken for the first point of a plot to a lineto.
%
% Description:
%
% For certain handlers it makes sense either the start a plot by
% moving to the first point of the plot or to do a lineto to that
% first point. Using this command this action can be set to a lineto. 
%
% Example:
%
% \pgfsetlinetofirstplotpoint

\def\pgfsetlinetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathlineto}


% Sets the action taken for the first point of a plot to a moveto.
%
% Example:
%
% \pgfsetmovetofirstplotpoint

\def\pgfsetmovetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathmoveto}

\let\pgf@plot@first@action=\pgfpathmoveto



%
% Handlers
%


% This handler converts each plot stream command into a lineto
% command, except for the first, which is converted to the action that
% has previously been specified using \pgfsetlinetofirstplotpoint or
% \pgfsetmovetofirstplotpoint. 
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotxyfile{mytable}

\def\pgfplothandlerlineto{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@line@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@line@handler#1{%
  \pgf@plot@first@action{#1}%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}



% More handlers are defined in pgflibraryplothandlers





% This handler discards the plot.
%
% Example:
%
% \pgfplothandlerdiscard
% \pgfplotxyfile{mytable}

\def\pgfplothandlerdiscard{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgfutil@gobble%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}




% This handler records each plot stream command to a macro. This is
% useful if plot commands are difficult to generate and need to be
% ``recylced'' later on.
%
% Example:
%
% \pgfplothandlerrecord{\myplot}
% \pgfplotxyfile{mytable}  % stored in \myplot now
% \pgfplothandlerline
% \myplot
% \pgftransformxshift{1cm}
% \myplot

\def\pgfplothandlerrecord#1{%
  \def\pgf@plot@recordto{#1}%
  \gdef#1{\pgfplotstreamstart}%
  \def\pgf@plotstreamstart{%
    \gdef\pgf@plotstreampoint####1{\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreampoint{####1}}}%
    \gdef\pgf@plotstreamspecial####1{\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamspecial{####1}}}%
    \gdef\pgf@plotstreamend{\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamend}}%
  }%
}



% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Each line of the file should begin with two numbers separated by a
% space. Such a line with number #1 and #2 is converted to a
% \pgfplotstreampoint{\pgfpointxy{#1}{#2}}. Extra characters following
% on the line are ignored.
%
% Lines starting with ``%'' and ``#'' are ignored.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyfile#1{%
  \begingroup%
    \pgfplotstreamstart%
    \openin1=#1
    \ifeof1
      \PackageWarning{pgf}{Plot data file `#1' not found.}
     \else
      \catcode`\#=14
      \pgf@readxyfile%
    \fi
    \pgfplotstreamend%    
  \endgroup%
}

\let\pgf@savedpar=\par%
\def\pgf@partext{\par}
\def\pgf@readxyfile{%
  \read1 to \pgf@temp%
  \let\par=\pgf@savedpar%
  \edef\pgf@temp{\pgf@temp}%
  \ifx\pgf@temp\pgfutil@empty%
  \else\ifx\pgf@temp\pgf@partext%
  \else%
    \expandafter\pgf@parsexyline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof1\else\expandafter\pgf@readxyfile\fi%
}

\def\pgf@parsexyline#1 #2 #3\pgf@stop{%
  \pgfplotstreampoint{\pgfpointxy{#1}{#2}}%
}





% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Like xy, except that each line contains three numbers, which are
% converted to xyz coordiantes.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyzfile#1{%
  \begingroup%
    \pgfplotstreamstart%
    \openin1=#1
    \ifeof1
      \PackageWarning{pgf}{Plot data file `#1' not found.}
    \else
      \catcode`\#=14
      \pgf@readxyzfile%
    \fi
    \pgfplotstreamend%    
  \endgroup%
}

\def\pgf@readxyzfile{%
  \read1 to \pgf@temp%
  \ifx\pgf@temp\pgfutil@empty%
  \else\ifx\pgf@temp\pgf@partext%
  \else%
    \expandafter\pgf@parsexyzline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof1\else\expandafter\pgf@readxyzfile\fi%
}

\def\pgf@parsexyzline#1 #2 #3 #4\pgf@stop{%
  \pgfplotstreampoint{\pgfpointxyz{#1}{#2}{#3}}%
}




% Render a function using gnuplot.
%
% #1 = filename prefix for .gnuplot and .table files (optional,
%      default is \jobname)
% #2 = gnuplot function text
%
% Description:
%
% This command will write a file called #1.gnuplot that sets up
% some gnuplot commands to write output to a file called
% #1.table. Then it calls gnuplot (using the \write18 mechanism)
% to execute the file. Then it reads #2.table using \pgfplotxyfile.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotgnuplot[\jobname]{plot [x=0:5] x*sin(x)}

{
  \catcode`\%=12
  \catcode`\"=12
  \xdef\pgf@gnuplot@head#1{set terminal table; set output "#1.table"; set format "%.5f"}
}

\newwrite\pgf@plotwrite
\newif\ifpgf@resample@plot

\def\pgfplotgnuplot{\pgfutil@ifnextchar[{\pgf@plotgnuplot}{\pgf@plotgnuplot[\jobname]}}%}
\def\pgf@plotgnuplot[#1]#2{%
  \pgf@resample@plottrue%
  % Check, whether it is up-to-date
  \openin\pgfutil@inputcheck=#1.gnuplot
  \ifeof\pgfutil@inputcheck%
  \else%
    \read\pgfutil@inputcheck to\pgf@temp% ignored
    \read\pgfutil@inputcheck to\pgf@plot@line%
    \edef\pgf@plot@code{#2\space}%
    \ifx\pgf@plot@code\pgf@plot@line%
      \openin\pgfutil@inputcheck=#1.table
      \ifeof\pgfutil@inputcheck%
      \else%
        \pgf@resample@plotfalse%
      \fi%
    \fi%
  \fi
  \ifpgf@resample@plot%  
    \immediate\openout\pgf@plotwrite=#1.gnuplot
    \immediate\write\pgf@plotwrite{\pgf@gnuplot@head{#1}}%
    \immediate\write\pgf@plotwrite{#2}%
    \immediate\closeout\pgf@plotwrite%
    \immediate\write18{gnuplot #1.gnuplot}
  \fi%
  \pgfplotxyfile{#1.table}
}



% This producer handler plots a function using pgf's mathematical engine.
%
% #1 = variable
% #2 = domain for the variable
% #3 = point, typically defined in terms of the value of the variable
%
% Description:
%
% This producer will iterate the variable #1 over all variables in #2
% (using the \foreach statement). For each value, a plot coordinate
% #3  is created.
%
% Note that this command is pretty slow.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotfunction{\x}{0,0.1,...,3.141}{\pgfpointxy{\x}{sin(\x)}}

\def\pgfplotfunction#1#2#3{%
  \pgfplotstreamstart%
  \foreach#1in{#2}%
  {%
    \pgf@process{#3}%
    \edef\pgf@marshal{\noexpand\pgfplotstreampoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
    \pgf@marshal%
  }
  \pgfplotstreamend%
}




\endinput


==> pgfbaseshapes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfbaseshapes.code.tex,v 1.19 2007/06/07 07:41:10 tantau Exp $


\newbox\pgfnodeparttextbox


% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% When this command is called, the shape-specific TeX boxes of the
% node must have been setup correctly.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfmultipartnode{rectangle}{center}{hellonode}{\pgfusepath{stroke}}

\def\pgfmultipartnode#1#2#3#4{%
  \pgfutil@ifundefined{pgf@sh@s@#1}%
  {\PackageError{pgf}{Unknown shape ``#1''}{}}%
  {%
    {%
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \csname pgf@sh@s@#1\endcsname%
      \pgf@sh@savedpoints%
      \pgftransformshift{%
        \pgf@sh@reanchor{#1}{#2}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@test{#3}%
      \ifx\pgf@test\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@#3\endcsname{#1}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@#3\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \pgfgettransform\pgf@temp
        \expandafter\xdef\csname pgf@sh@nt@#3\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@#3\endcsname{\pgfpictureid}%
      \fi%
      \pgfutil@ifundefined{pgf@sh@bbg@#1}{}
      {{\pgfscope\csname pgf@sh@bbg@#1\endcsname\endpgfscope}}%
      \pgfutil@ifundefined{pgf@sh@bg@#1}{}%
      {\csname pgf@sh@bg@#1\endcsname#4}%
      \pgfutil@ifundefined{pgf@sh@fbg@#1}{}
      {{\pgfscope\csname pgf@sh@fbg@#1\endcsname\endpgfscope}}%
      {%
        \expandafter\pgfutil@for\expandafter\pgf@shape@com\expandafter:\expandafter=\csname pgf@sh@boxes@#1\endcsname\do{%
          {%
            \pgftransformshift{\pgf@sh@reanchor{#1}{\pgf@shape@com}}%
            \expandafter\pgfqboxsynced\expandafter{\csname pgfnodepart\pgf@shape@com box\endcsname}%
          }%
        }%
      }%
      \pgfutil@ifundefined{pgf@sh@bfg@#1}{}%
      {{\pgfscope\csname pgf@sh@bfg@#1\endcsname\endpgfscope}}%
      \pgfutil@ifundefined{pgf@sh@fg@#1}{}%
      {\csname pgf@sh@fg@#1\endcsname#4}%
      \pgfutil@ifundefined{pgf@sh@ffg@#1}{}%
      {{\pgfscope\csname pgf@sh@ffg@#1\endcsname\endpgfscope}}%
      \pgf@nodecallback{#3}%
    }%
  }%
}


\def\pgf@shift@node#1#2{%
  % This internal command shifts the recorded coordinates for node #1
  % by the vector #2. It is used to
  % correct the position of the node if the recorded coordinate
  % happens to be wrong
  {%
    \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
    \pgf@process{#2}%
    \advance\pgf@pt@x by\pgf@x%
    \advance\pgf@pt@y by\pgf@y%
    \pgfgettransform{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  }%
}

\let\pgf@nodecallback=\pgfutil@gobble



% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = normal TeX text
% #4 = name for later reference
% #5 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfnode{rectangle}{center}{Hello}{hellonode}{\pgfusepath{stroke}}

\def\pgfnode#1#2#3#4#5{%
  {%
    \setbox\pgfnodeparttextbox=\hbox%
    {%
      \pgfinterruptpicture%
        {#3}%
      \endpgfinterruptpicture%
    }%
    \pgfmultipartnode{#1}{#2}{#4}{#5}%
  }
}  

\def\pgf@sh@resavedanchor#1#2{%
  \pgf@process{#2}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    }}%
  \pgf@sh@marshal%
}


\def\pgf@sh@resaveddimen#1#2{%
  {#2\global\pgf@x=\pgf@x}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\the\pgf@x}%
    }}%
  \pgf@sh@marshal%
}

% Invoke an anchor
\def\pgf@sh@reanchor#1#2{%
  \pgfutil@ifundefined{pgf@anchor@#1@#2}%
  {%
    \pgfmathsetcounter{pgf@counta}{#2}%
    \csname pgf@anchor@#1@border\endcsname{\pgfqpointpolar{\c@pgf@counta}{1pt}}%
  }%
  {\csname pgf@anchor@#1@#2\endcsname}%
}



% Retrieves an anchor of a shape
%
% #1 = name
% #2 = anchor or a number (corresponding to a degree)
%
% Description:
%
% This command yields a point at the anchor of the given named shape.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointanchor{hellonode}{center}}

\def\pgfpointanchor#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\PackageError{pgf}{No shape named #1 is known}{}%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname
      \pgf@sh@reanchor{\csname pgf@sh@ns@#1\endcsname}{#2}%
      {%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform{\pgf@x}{\pgf@y}%
        \global\pgf@x=\pgf@x%
        \global\pgf@y=\pgf@y%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }%
}

\def\pgf@shape@interpictureshift#1{%
  \expandafter\ifx\csname pgf@sh@pi@#1\endcsname\pgfpictureid%
  \else%
    \pgfsys@getposition{\csname pgf@sh@pi@#1\endcsname}\pgf@shape@original@pos%
    \pgfsys@getposition{\pgfpictureid}\pgf@shape@current@pos%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@current@pos}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@original@pos}%
    \advance\pgf@xa by\pgf@x%
    \advance\pgf@ya by\pgf@y%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
  \fi%
}



% Retrieves a border point of a shape
%
% #1 = name
% #2 = another point
%
% Description:
%
% This command yields a point on the border of the shape that is on a
% straight line from the center to the point #2.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointshapeborder{hellonode}{\pgfpoint{2cm}{1cm}}
% \pgfpathlineto{\pgfpoint{2cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfpointshapeborder#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\PackageError{pgf}{No shape named #1 is known}{}%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname%
      {%
        \pgf@process{\pgfpointtransformed{#2}}%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgftransforminvert%
        \pgf@pos@transform{\pgf@x}{\pgf@y}%
        \pgf@xa=\pgf@x%
        \pgf@ya=\pgf@y%
        \pgf@process{\csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @center\endcsname}%
        \pgf@process{\pgf@shape@interpictureshift{#1}}%%
        \advance\pgf@xa by-\pgf@x%
        \advance\pgf@ya by-\pgf@y%
        \csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @border\endcsname{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform{\pgf@x}{\pgf@y}%
        \global\pgf@x=\pgf@x%
        \global\pgf@y=\pgf@y%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }%
}



% Declares a shape type
%
% #1 = shape type
% #2 = shape specification
%
% Description:
%
% This command declares a new shape type. The shape specification
% should contain the following commands:
%
% - \savedanchor
%   This command takes two arguments: a name and some code. The point
%   specified by the code (the \pgf@x and \pgf@y values resulting from
%   executing the code, to be precise), will be stored under the given
%   name. Whenever, later on, an anchor is invoked these stored points
%   will be available. The \saveddimen works like \savedanchor, only a
%   single dimension is stored (taken from \pgf@x).
%   When a savedanchor is calculated, the height/width/depth of the
%   boxes mentioned in \nodeparts can be used.
%
% - \anchor
%   Specifies an anchor. This command takes two arguments: an anchor
%   name and some code for computing the anchor. When the anchor
%   computation starts, all shape points and shape dimension will be
%   setup.
%
% - \anchorborder
%   This command should compute a point on the border of the
%   shape. When the code is called, \pgf@x and \pgf@y will have been
%   preinitialised with a direction.
%
% - \behindbackgroundpath
%   Some things to be draw behind everything.
%
% - \backgroundpath
%   A path that is drawn behind the main box. How this path is used
%   depends on how \pgfshape is called.
%
% - \beforebackgroundpath
%   Some things to be draw before the background path, but behind the
%   main box.
%
% - \behindforegroundpath
%   Some things to be draw on top of the main box.
%
% - \foregroundpath
%   A path that is drawn on top of all of the above. How this path is
%   used depends on how \pgfshape is called.
%
% - \beforeforegroundpath
%   Some things to be draw before everything.
%
% - \nodeparts
%   List of node parts that make up the shape. For each entry XYZ in
%   the list there must be a box named \pgfnodepartXYZbox (possibly
%   ``redirected'' to some different box using \let). Each such box
%   will be placed at the anchor XYZ.
%   By default, \nodeparts is just {text}. Thus, there will be one
%   node part box named \pgfnodeparttextbox and this node will be
%   placed at the anchor text. 
%   
%
% Example:
%
% See the definition of rectangle, below.

\long\def\pgfdeclareshape#1#2{%
  {
    \def\shape@name{#1}
    \let\savedanchor=\pgf@sh@savedanchor
    \let\saveddimen=\pgf@sh@saveddimen
    \let\anchor=\pgf@sh@anchor
    \let\anchorborder=\pgf@sh@anchorborder
    \let\behindbackgroundpath=\pgf@sh@behindbgpath
    \let\backgroundpath=\pgf@sh@bgpath
    \let\beforebackgroundpath=\pgf@sh@beforebgpath
    \let\behindforegroundpath=\pgf@sh@behindfgpath
    \let\foregroundpath=\pgf@sh@fgpath
    \let\beforeforegroundpath=\pgf@sh@beforefgpath
    \let\nodeparts=\pgf@sh@boxes
    \let\inheritsavedanchors=\pgf@sh@inheritsavedanchors
    \let\inheritanchor=\pgf@sh@inheritanchor
    \let\inheritanchorborder=\pgf@sh@inheritanchorborder
    \let\inheritbehindbackgroundpath=\pgf@sh@inheritbehindbgpath
    \let\inheritbackgroundpath=\pgf@sh@inheritbgpath
    \let\inheritbeforebackgroundpath=\pgf@sh@inheritbeforebgpath
    \let\inheritbehindforegroundpath=\pgf@sh@inheritbehindfgpath
    \let\inheritforegroundpath=\pgf@sh@inheritfgpath
    \let\inheritbeforeforegroundpath=\pgf@sh@inheritbeforefgpath
    \let\inheritnodeparts=\pgf@sh@inheritboxes
    \anchorborder{\csname pgf@anchor@#1@center\endcsname}%
    \anchor{text}{\pgfpointorigin}%
    \nodeparts{text}%
    \expandafter\global\expandafter\let\csname pgf@sh@s@\shape@name\endcsname=\pgfutil@empty%
    #2
  }
}

\def\pgf@sh@savedanchor#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\shape@name\endcsname{\pgf@sh@resavedanchor{#1}{#2}}}
\def\pgf@sh@saveddimen#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\shape@name\endcsname{\pgf@sh@resaveddimen{#1}{#2}}}
\def\pgf@sh@anchor#1#2{\expandafter\gdef\csname pgf@anchor@\shape@name @#1\endcsname{#2}}
\def\pgf@sh@anchorborder#1{\expandafter\gdef\csname pgf@anchor@\shape@name @border\endcsname##1{\pgf@process{##1}#1}}
\long\def\pgf@sh@behindbgpath#1{\expandafter\gdef\csname pgf@sh@bbg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@bgpath#1{\expandafter\gdef\csname pgf@sh@bg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@beforebgpath#1{\expandafter\gdef\csname pgf@sh@fbg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@behindfgpath#1{\expandafter\gdef\csname pgf@sh@bfg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@fgpath#1{\expandafter\gdef\csname pgf@sh@fg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@beforefgpath#1{\expandafter\gdef\csname pgf@sg@ffg@\shape@name\endcsname{#1}}
\def\pgf@sh@boxes#1{\expandafter\gdef\csname pgf@sh@boxes@\shape@name\endcsname{#1}}

\def\pgf@sh@inheritsavedanchors[from=#1]{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\shape@name\endcsname{\csname pgf@sh@s@#1\endcsname}}
\def\pgf@sh@inheritanchor[from=#1]#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\shape@name @#2\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@#2\endcsname}%
  \pgf@marshal%
}
\def\pgf@sh@inheritanchorborder[from=#1]{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\shape@name @border\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@border\endcsname}%
  \pgf@marshal%
}
\def\pgf@sh@inheritor#1#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@sh@#1@\shape@name\endcsname=\expandafter\noexpand\csname
    pgf@sh@#1@#2\endcsname}%
  \pgf@marshal%
}
\def\pgf@sh@inheritbehindbgpath[from=#1]{\pgf@sh@inheritor{bbg}{#1}}
\def\pgf@sh@inheritbgpath[from=#1]{\pgf@sh@inheritor{bg}{#1}}
\def\pgf@sh@inheritbeforebgpath[from=#1]{\pgf@sh@inheritor{fbg}{#1}}
\def\pgf@sh@inheritbehindfgpath[from=#1]{\pgf@sh@inheritor{bfg}{#1}}
\def\pgf@sh@inheritfgpath[from=#1]{\pgf@sh@inheritor{fg}{#1}}
\def\pgf@sh@inheritbeforefgpath[from=#1]{\pgf@sh@inheritor{ffg}{#1}}
\def\pgf@sh@inheritboxes[from=#1]{\pgf@sh@inheritor{boxes}{#1}}



% 
% Coordinate. This shape is special: It is only used to reference a
% point for later usage. Nothing is drawn, all anchors are identical
% to the center. 
%

\pgfdeclareshape{coordinate}
{
  \savedanchor\centerpoint{%
    % x
    \pgf@x=.5\wd\pgfnodeparttextbox%
    % y
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by -.5\dp\pgfnodeparttextbox%
  }
  
  \anchor{center}{\centerpoint}
  \anchor{north}{\centerpoint}
  \anchor{north west}{\centerpoint}
  \anchor{north east}{\centerpoint}
  \anchor{center}{\centerpoint}
  \anchor{west}{\centerpoint}
  \anchor{east}{\centerpoint}
  \anchor{mid}{\centerpoint}
  \anchor{mid west}{\centerpoint}
  \anchor{mid east}{\centerpoint}
  \anchor{base}{\centerpoint}
  \anchor{base west}{\centerpoint}
  \anchor{base east}{\centerpoint}
  \anchor{south}{\centerpoint}
  \anchor{south west}{\centerpoint}
  \anchor{south east}{\centerpoint}
  \anchorborder{\centerpoint}

  \nodeparts{}% no text
}


% Set the recommended inner x separation
%
% #1 = size
%
% Example:
%
% \pgfsetshapeinnerxsep{2pt}

\def\pgfsetshapeinnerxsep#1{\def\pgfshapeinnerxsep{#1}}
\pgfsetshapeinnerxsep{.3333em}


% Set the recommended inner y separation
%
% #1 = size
%
% Example:
%
% \pgfsetshapeinnerxsep{2pt}

\def\pgfsetshapeinnerysep#1{\def\pgfshapeinnerysep{#1}}
\pgfsetshapeinnerysep{.3333em}


% Set the recommended outer x separation
%
% #1 = size
%
% Example:
%
% \pgfsetshapeouterxsep{2pt}

\def\pgfsetshapeouterxsep#1{\def\pgfshapeouterxsep{#1}}
\pgfsetshapeouterxsep{.5\pgflinewidth}


% Set the recommended outer y separation
%
% #1 = size
%
% Example:
%
% \pgfsetshapeouterxsep{2pt}

\def\pgfsetshapeouterysep#1{\def\pgfshapeouterysep{#1}}
\pgfsetshapeouterysep{.5\pgflinewidth}


% Set the recommended minimum width
%
% #1 = size
%
% Example:
%
% \pgfsetshapeminwidth{1cm}

\def\pgfsetshapeminwidth#1{\def\pgfshapeminwidth{#1}}
\pgfsetshapeminwidth{1pt}


% Set the recommended minimum height
%
% #1 = size
%
% Example:
%
% \pgfsetshapeminheight{1cm}

\def\pgfsetshapeminheight#1{\def\pgfshapeminheight{#1}}
\pgfsetshapeminheight{1pt}


% 
% Rectangle
%

\pgfdeclareshape{rectangle}
{
  \savedanchor\northeast{%
    % Calculate x
    %
    % First, is width < minimum width?
    \pgf@x=\the\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xc{\pgfshapeinnerxsep}%
    \advance\pgf@x by 2\pgf@xc%
    \pgfmathsetlength\pgf@xb{\pgfshapeminwidth}%
    \ifdim\pgf@x<\pgf@xb%
      % yes, too small. Enlarge...
      \pgf@x=\pgf@xb%
    \fi%
    % Now, calculate right border: .5\wd\pgfnodeparttextbox + .5 \pgf@x + outer sep
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xa{\pgfshapeouterxsep}%
    \advance\pgf@x by\pgf@xa%
    % Calculate y
    %
    % First, is height+depth < minimum height?
    \pgf@y=\ht\pgfnodeparttextbox%
    \advance\pgf@y by\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yc{\pgfshapeinnerysep}%
    \advance\pgf@y by 2\pgf@yc%
    \pgfmathsetlength\pgf@yb{\pgfshapeminheight}%
    \ifdim\pgf@y<\pgf@yb%
      % yes, too small. Enlarge...
      \pgf@y=\pgf@yb%
    \fi%
    % Now, calculate upper border: .5\ht-.5\dp + .5 \pgf@y + outer sep
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
    \advance\pgf@y by.5\ht\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@ya{\pgfshapeouterysep}%
    \advance\pgf@y by\pgf@ya%
  }
    
  \savedanchor\southwest{%
      % Calculate x
      %
      % First, is width < minimum width?
      \pgf@x=\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xc{\pgfshapeinnerxsep}%
      \advance\pgf@x by 2\pgf@xc%
      \pgfmathsetlength\pgf@xb{\pgfshapeminwidth}%
      \ifdim\pgf@x<\pgf@xb%
        % yes, too small. Enlarge...
        \pgf@x=\pgf@xb%
      \fi%
      % Now, calculate left border: .5\wd\pgfnodeparttextbox - .5 \pgf@x - outer sep
      \pgf@x=-.5\pgf@x%
      \advance\pgf@x by.5\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xa{\pgfshapeouterxsep}%
      \advance\pgf@x by-\pgf@xa%
      % Calculate y
      %
      % First, is height+depth < minimum height?
      \pgf@y=\ht\pgfnodeparttextbox%
      \advance\pgf@y by\dp\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@yc{\pgfshapeinnerysep}%
      \advance\pgf@y by 2\pgf@yc%
      \pgfmathsetlength\pgf@yb{\pgfshapeminheight}%
      \ifdim\pgf@y<\pgf@yb%
        % yes, too small. Enlarge...
        \pgf@y=\pgf@yb%
      \fi%
       % Now, calculate upper border: .5\ht-.5\dp - .5 \pgf@y - outer sep
      \pgf@y=-.5\pgf@y%
      \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
      \advance\pgf@y by.5\ht\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@ya{\pgfshapeouterysep}%
      \advance\pgf@y by-\pgf@ya%
  }

  %
  % Anchors
  % 
  \anchor{center}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \pgf@y=.5\pgf@y%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@y by \pgf@ya%
  }
  \anchor{mid}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base}{\pgf@anchor@rectangle@center\pgf@y=0pt}
  \anchor{north}{
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }
  \anchor{south}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }
  \anchor{west}{
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }
  \anchor{mid west}{\southwest\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base west}{\southwest\pgf@y=0pt}
  \anchor{north west}{
    \southwest
    \pgf@xa=\pgf@x
    \northeast
    \pgf@x=\pgf@xa}
  \anchor{south west}{\southwest}
  \anchor{east}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }
  \anchor{mid east}{\northeast\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base east}{\northeast\pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{south east}{
    \northeast
    \pgf@xa=\pgf@x
    \southwest
    \pgf@x=\pgf@xa
  }
  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }

  %
  % Background path
  %
  \backgroundpath{
    \pgfpathrectanglecorners
    {\pgfpointadd{\southwest}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}
    {\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfshapeouterxsep}{\pgfshapeouterysep}}}}
  }
}



% Special  current bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current bounding box\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
  \def\northeast{\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
}
\expandafter\def\csname pgf@sh@nt@current bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
\expandafter\def\csname pgf@sh@pi@current bounding box\endcsname{\pgfpictureid}


% Special  current path bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current path bounding box\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current path bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@pathminx}{\pgf@pathminy}}%
  \def\northeast{\pgfqpoint{\pgf@pathmaxx}{\pgf@pathmaxy}}%
}
\expandafter\def\csname pgf@sh@nt@current path bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
\expandafter\def\csname pgf@sh@pi@current path bounding box\endcsname{\pgfpictureid}


% Special  current page bounding box rectangle:
\expandafter\def\csname pgf@sh@ns@current page\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current page\endcsname{%
  \def\southwest{\pgfqpoint{0pt}{0pt}}%
  \def\northeast{\pgfqpoint{\paperwidth}{\paperheight}}%
}
\expandafter\def\csname pgf@sh@nt@current page\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
\expandafter\def\csname pgf@sh@pi@current page\endcsname{pgfpageorigin}



%
% Circle
%

\pgfdeclareshape{circle}
%
% Draws a circle around the text
%
{
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
  }
    
  \saveddimen\radius{%
    % 
    % Caculate ``height radius''
    % 
    \pgf@ya=.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfshapeinnerysep}%
    \advance\pgf@ya by\pgf@yb%
    % 
    % Caculate ``width radius''
    % 
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfshapeinnerxsep}%
    \advance\pgf@xa by\pgf@xb%
    % 
    % Calculate length of radius vector:
    % 
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \ifdim\pgf@x>\pgf@y%
        \c@pgf@counta=\pgf@x%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@xa=16\pgf@xa\relax%
          \divide\pgf@xa by\c@pgf@counta%
          \pgf@xa=16\pgf@xa\relax%
        \fi%
      \else%
        \c@pgf@counta=\pgf@y%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@ya=16\pgf@ya\relax%
          \divide\pgf@ya by\c@pgf@counta%
          \pgf@xa=16\pgf@ya\relax%
        \fi%
    \fi%
    \pgf@x=\pgf@xa%
    % 
    % If necessary, adjust radius so that the size requirements are
    % met: 
    % 
    \pgfmathsetlength{\pgf@xb}{\pgfshapeminwidth}%  
    \pgfmathsetlength{\pgf@yb}{\pgfshapeminheight}%  
    \ifdim\pgf@x<.5\pgf@xb%
        \pgf@x=.5\pgf@xb%
    \fi%
    \ifdim\pgf@x<.5\pgf@yb%
        \pgf@x=.5\pgf@yb%
    \fi%
    % 
    % Now, add larger of outer sepearations.
    % 
    \pgfmathsetlength{\pgf@xb}{\pgfshapeouterxsep}%  
    \pgfmathsetlength{\pgf@yb}{\pgfshapeouterysep}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgf@x by\pgf@yb%
    \else%
      \advance\pgf@x by\pgf@xb%
    \fi%
  }

  %
  % Anchors
  % 
  \anchor{center}{\centerpoint}
  \anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base}{\centerpoint\pgf@y=0pt}
  \anchor{north}{\centerpoint\advance\pgf@y by\radius}
  \anchor{south}{\centerpoint\advance\pgf@y by-\radius}
  \anchor{west}{\centerpoint\advance\pgf@x by-\radius}
  \anchor{east}{\centerpoint\advance\pgf@x by\radius}
  \anchor{mid west}{\centerpoint\advance\pgf@x by-\radius\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{mid east}{\centerpoint\advance\pgf@x by\radius\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base west}{\centerpoint\advance\pgf@x by-\radius\pgf@y=0pt}
  \anchor{base east}{\centerpoint\advance\pgf@x by\radius\pgf@y=0pt}
  \anchor{north west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }
  \anchor{south west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }
  \anchor{north east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }
  \anchor{south east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }
  \anchorborder{
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderellipse
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\radius}{\radius}}%
    }%
    \pgf@marshal%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \centerpoint%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }

  %
  % Background path
  %
  \backgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfshapeouterxsep}%  
    \pgfmathsetlength{\pgf@yb}{\pgfshapeouterysep}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
  }
}





\endinput


==> pgfbasesnakes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfbasesnakes.code.tex,v 1.11 2007/03/09 17:49:32 tantau Exp $

\newdimen\pgfsnakeremainingdistance
\newdimen\pgfsnakecompleteddistance


% Creates a new pgf snake
%
% #1 = snake name
% #1 = initial state
% #3 = states of the snake
%
%
% This command declares a new snake for later use. The second
% parameter specifies the states of the snake, see also the
% description of pgfpathsnake.
%
% Inside the code of #3 the command \state may be used. This command
% will only be defined while #3 is executed.
%
% Example:
%
% \pgfdeclaresnake{zig zag}{one zig zag}
% {
%   \state{one zig zag}[width=10pt]
%   {
%     \pgfpathlineto{\pgfpoint{2.5pt}{2.5pt}}
%     \pgfpathlineto{\pgfpoint{7.5pt}{-2.5pt}}
%     \pgfpathlineto{\pgfpoint{10pt}{0pt}}
%   }
%   \state{final}
%   {
%     \pgfpathlineto{\pgfpoint{\pgfsnakeremainingdistance}{0pt}}
%   }
% }

\long\def\pgfdeclaresnake#1#2#3{%
  \def\pgf@snake@name{#1}%
  \pgfutil@namedef{pgf@snake@@#1@initial}{#2}%
  \let\pgf@orig@state=\state%
  \let\state=\pgf@snake@state
  #3
  \let\state=\pgf@orig@state%
}


% Sets the additional transformation applied to every segment of a snake
%
% #1 = transformation
%
% Example:
%
% \pgfsetsnakesegmenttransformation{\pgftransformyshift{5pt}}

\def\pgfsetsnakesegmenttransformation#1{\def\pgf@snakeadditionaltransform{#1}}
\pgfsetsnakesegmenttransformation{}


% Declares a new state
%
% #1 = state name
% #2 = options
% #3 = path element
%
% Description:
%
% When a snake is drawn and the current state is #1, the following
% happens. First, the options are executed, which will possible change
% the state. If that does not happen, the path element is added to the
% path and the coordinate system is translated by the path element's
% width (which is specified using the width option).
%
% Example:
%
% \state{initial}[width=10pt]
% {
%   \pgfpathlineto{\pgfpoint{2.5pt}{2.5pt}}
%   \pgfpathlineto{\pgfpoint{7.5pt}{-2.5pt}}
%   \pgfpathlineto{\pgfpoint{10pt}{0pt}}
% }

\def\pgf@snake@state#1{\pgfutil@ifnextchar[{\pgf@@snake@start#1}{\pgf@@snake@start#1[]}}%}
\def\pgf@@snake@start#1[#2]#3{%
  \pgfutil@namedef{pgf@snake@@\pgf@snake@name @#1@options}{#2}%
  \pgfutil@namedef{pgf@snake@@\pgf@snake@name @#1@code}{#3}%
}



% Use multiple snakes
%
% #1 = list of snake names/length pairs
% #2 = point to which the snake leads
%
% This operation uses the snakes in parameter #1 to get to the point
% #4. The parameter #1 should contain pairs consisting of a snake name
% and a length for which this snake should be used. When the length is
% computed, the dimensions \pgfsnakeremainingdistance and
% \pgfsnakecompleteddistance will have been set to the length of the
% total distance to #2 that has already been covered/that still needs
% to be covered.
%
% Example:
%
% \pgfpathsnakesto{{lineto}{1cm},{zig zag}{\pgfsnakeremainingdistance}}{\pgfpoint{2cm}{3cm}}

\def\pgfpathsnakesto#1#2{%
  \begingroup%
    % compute target vector
    \pgfpointtransformed{#2}%
    \advance\pgf@x by-\pgf@path@lastx%
    \advance\pgf@y by-\pgf@path@lasty%
    % Ok, now normalize the vector...
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointnormalised{}}%
    % ok, now computer length (arghh...)
    % In theory that's easy: divide the larger of the values x or y by
    % the normalized x or y. Well...
    %
    % First, make xa and ya positive:
    \ifdim\pgf@xa<0pt%
      \pgf@xa=-\pgf@xa%
    \fi%
    \ifdim\pgf@ya<0pt%
      \pgf@ya=-\pgf@ya%
    \fi%
    % Now do division:
    \ifdim\pgf@xa>\pgf@ya%
      \c@pgf@counta=\pgf@x%
      \ifnum\c@pgf@counta=0\relax%
      \else%
        \divide\c@pgf@counta by 255\relax%
        \pgf@xa=16\pgf@xa\relax%
        \divide\pgf@xa by\c@pgf@counta%
        \pgf@xa=16\pgf@xa\relax%
      \fi%
    \else%
      \c@pgf@counta=\pgf@y%
      \ifnum\c@pgf@counta=0\relax%
      \else%
        \divide\c@pgf@counta by 255\relax%
        \pgf@ya=16\pgf@ya\relax%
        \divide\pgf@ya by\c@pgf@counta%
        \pgf@xa=16\pgf@ya\relax%
      \fi%
    \fi%
    % Make positive:
    \ifdim\pgf@xa<0pt%
      \pgf@xa=-\pgf@xa%
    \fi%
    % Ok, now we draw things...
    \edef\pgf@list{#1}%
    \pgfsnakeremainingdistance=\pgf@xa%
    \pgfsnakecompleteddistance=0pt%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgfutil@for\pgf@temp:=\pgf@list\do{%
      \ifx\pgf@temp\pgfutil@empty%
      \else%
        \expandafter\pgf@snake@invoke\pgf@temp%
      \fi%
    }%
  \endgroup%
}

\def\pgf@snake@invoke#1#2{%
  \pgfmathsetlength\pgf@xa{#2}%
  {%
    \edef\pgf@marshal{\noexpand\pgfpathsnakealongvector{#1}{\the\pgf@xa}{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}}%
    \pgf@marshal%
  }%
  \advance\pgfsnakecompleteddistance by\pgf@xa%
  \advance\pgfsnakeremainingdistance by-\pgf@xa%
}

% Use a snake
%
% #1 = snake name
% #2 = point to which the snake leads
%
% This operation mainly computes \pgfpathsnakealongvector for a vector
% appropriately choosen. See \pgfpathsnakealongvector for details.
%
% Example:
%
% \pgfpathsnaketo{zig zag}{\pgfpoint{2cm}{3cm}}

\def\pgfpathsnaketo#1#2{\pgfpathsnakesto{{#1}{\pgfsnakeremainingdistance}}{#2}}



% Use a snake
%
% #1 = snake name
% #2 = length of the snake
% #3 = vector along which the snake grows, should have unit length.
%
% This command draws a snake (more precisely, it adds a snake to the
% path). This works as follows:
%
% First, the coordinate system is transformed such that the vector #3
% points to the right.
%
% Next, the state `initial' of the snake is entered. Unless the
% options of this state cause it to switch to another state, the path
% element is added to the path. Then, the coordinate system is
% translated by the width of the path element as specified in the
% width option of the path element. The dimensions
% \pgfsnakeremainingdistance and \pgfsnakecompleteddistance are
% updated. 
%
% The process ends when the state `final' is entered. The code of the
% final state is executed and the process stops.
%
% Example:
%
% \pgfpathsnakealongvector{zig zag}{100pt}{\pgfpolar{30}{1pt}}

\def\pgfpathsnakealongvector#1#2#3{%
  \pgfutil@ifundefined{pgf@snake@@#1@initial}{\PackageError{pgf}{Undefined snake ``#1''}{}}
  { 
  \begingroup% keep things local
    \pgftransformreset%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgf@process{#3}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@xb=-\pgf@y%
    \pgf@yb=\pgf@x%
    \pgftransformcm
      {\pgf@sys@tonumber{\pgf@xa}}{\pgf@sys@tonumber{\pgf@ya}}
      {\pgf@sys@tonumber{\pgf@xb}}{\pgf@sys@tonumber{\pgf@yb}}
      {\pgfpointorigin}%
    % Now, setup the automaton
    \expandafter\let\expandafter\pgf@snake@current@state\expandafter=\csname pgf@snake@@#1@initial\endcsname%
    \def\pgf@snake@name{#1}%  
    \pgfsnakecompleteddistance=0pt%  
    \pgfmathsetlength\pgfsnakeremainingdistance{#2}%
    \pgf@snake@run%
    % Last step:
    {%
      \pgftransformxshift{\pgfsnakecompleteddistance}%
      \pgf@snakeadditionaltransform%
      \csname pgf@snake@@#1@final@code\endcsname%
    }%
  \endgroup%
  }%
}

\def\pgf@final@text{final}

\def\pgf@snake@run{%
  \let\pgf@snake@next=\pgf@snake@do@state%
  \ifx\pgf@snake@current@state\pgf@final@text%
    \let\pgf@snake@next=\relax%
  \fi%
  \pgf@snake@next%  
}

\def\pgf@snake@do@state{%
  \let\pgf@snake@next=\relax%
  \let\pgf@snake@next@state=\pgf@snake@current@state%
  % execute options
  \def\pgf@marshal{\setkeys{pgfsnake}}%
  \expandafter\expandafter\expandafter\pgf@marshal
  \expandafter\expandafter\expandafter{\csname pgf@snake@@\pgf@snake@name @\pgf@snake@current@state @options\endcsname}%
  \ifx\pgf@snake@next\relax%
    \let\pgf@snake@next=\pgf@snake@do@code%
  \fi%
  \pgf@snake@next%
}

\def\pgf@snake@do@code{%
  % Ok, execute code:
  {%
    \pgftransformxshift{\pgfsnakecompleteddistance}%
    \pgf@snakeadditionaltransform%
    \csname pgf@snake@@\pgf@snake@name @\pgf@snake@current@state @code\endcsname%
  }%
  % next, do transformation and update
  \pgfmathsetlength{\pgf@xa}{\pgf@snake@width}%
  \advance\pgfsnakeremainingdistance by-\pgf@xa%
  \advance\pgfsnakecompleteddistance by\pgf@xa%
  % Next iteration:
  \let\pgf@snake@current@state=\pgf@snake@next@state%
  \pgf@snake@run%
}

\define@key{pgfsnake}{width}{%
  \def\pgf@snake@width{#1}%
  \pgf@snake@switch@if#1 to final\pgf@stop%
}
\define@key{pgfsnake}{switch if less than}{%
  \pgf@snake@switch@if#1\pgf@stop%
}
\define@key{pgfsnake}{next state}{%
  \def\pgf@snake@next@state{#1}%
}

\def\pgf@snake@switch@if#1to #2\pgf@stop{%
  \ifx\pgf@snake@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgfsnakeremainingdistance<\pgf@x%
      \def\pgf@snake@current@state{#2}%
      \let\pgf@snake@next=\pgf@snake@run%
    \fi%
  \fi%
}



% lineto snake
%
% This snake simply adds a straight line. This snake is mainly useful
% in conjunction with other snakes.

\pgfdeclaresnake{lineto}{final}
{
  \state{final}
  { \pgfpathlineto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}} }
}



% moveto snake
%
% This snake simply jumps to the end. This snake, too, is mainly
% useful in conjunction with other snakes.

\pgfdeclaresnake{moveto}{final}
{
  \state{final}
  { \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}} }
}



\endinput


==> pgfcore.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcore.code.tex,v 1.5 2007/03/09 17:49:32 tantau Exp $

\newif\ifpgf@draftmode

\input pgfmath.code.tex

\input pgfcorepoints.code.tex
\input pgfcorepathconstruct.code.tex
\input pgfcorepathusage.code.tex
\input pgfcorescopes.code.tex
\input pgfcoregraphicstate.code.tex
\input pgfcoretransformations.code.tex
\input pgfcorequick.code.tex
\input pgfcoreobjects.code.tex
\input pgfcorepathprocessing.code.tex
\input pgfcorearrows.code.tex
\input pgfcoreshade.code.tex

\endinput


==> pgfcorearrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorearrows.code.tex,v 1.8 2007/06/07 07:41:10 tantau Exp $


% Sets the end arrow
%
% #1 = An arrow name
%
% Example:
%
% \pgfsetarrowsend{stealth}

\def\pgfsetarrowsend#1{\pgf@arrowset{end}{#1}}
\def\pgf@arrowset#1#2{%
  \pgfutil@ifundefined{pgf@arrow@code@#2}
  {\PackageError{pgf}{Arrow #1 type ``#2'' unknown}{}}
  {%
    \edef\pgf@arrow@temp{#2}%
    \ifx\pgf@arrow@temp\pgfutil@empty% ah. clear!
      \expandafter\let\csname pgf@#1arrow\endcsname=\pgfutil@empty%
      \expandafter\let\csname pgf@shorten@#1\endcsname=\pgfutil@empty%
    \else%
      %\pgf@arrow@prepare{#2}%
      \expandafter\def\csname pgf@#1arrow\endcsname{\pgf@arrow@call{#2}}%
      \expandafter\edef\csname pgf@shorten@#1\endcsname{\expandafter\noexpand\csname pgf@arrow@right@#2\endcsname}%
    \fi%
  }%
}


% Sets the start arrow
%
% #1 = An arrow name
%
% Example:
%
% \pgfsetarrowsstart{stealth}

\def\pgfsetarrowsstart#1{\pgf@arrowset{start}{\csname pgf@arrows@invert#1\endcsname}}

\def\pgf@arrows@invname#1#2{\expandafter\def\csname pgf@arrows@invert#1\endcsname{#2}}
\pgf@arrows@invname{}{}




% Sets arrows
%
% #1 = An arrow specification of the form ``left''-``right''. The last
%      and right should be arrow types that have been defined using
%      the \pgfarrowsdef command
%
% Example:
%
% \pgfsetarrows{-to}

\def\pgfsetarrows#1{\pgf@arrows#1\pgf@stop}
\def\pgf@arrows#1-#2\pgf@stop{%
  \pgfsetarrowsstart{#1}
  \pgfsetarrowsend{#2}
}

\def\pgf@arrows@checked#1#2#3{%
  \pgfutil@ifundefined{pgf@arrow@code@#2}%
  {%
    \PackageError{pgf}{Arrow end type ``#2'' unknown}{}}%
  {%
    \pgfutil@ifundefined{pgf@arrow@code@\csname pgf@arrows@invert#1\endcsname}
    {\PackageError{pgf}{Arrow start type ``#1'' unknown}{}}%
    {#3}%
  }%
}

\def\pgf@arrows@check@already#1#2#3{%
  \pgfutil@ifundefined{pgf@arrow@code@#2}
  {#3}%
  {\PackageError{pgf}{Arrow end type ``#2'' already defined}{}}%
}


% Called when an arrow needs to be rendered

\def\pgf@arrow@call#1{%
  \expandafter\ifx\csname pgf@arrow@prot@#1@\the\pgflinewidth\endcsname\relax%
    \pgfsysprotocol@getcurrentprotocol\pgf@arrow@temp%
    {%
      \pgfinterruptpath%
        \let\pgfusepath=\pgf@nousepath@here%
        \pgf@relevantforpicturesizefalse%
        \pgftransformreset%
        \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
        \pgfsysprotocol@bufferedtrue%
        \pgfsys@beginscope%
        \csname pgf@arrow@code@#1\endcsname%
        \pgfsys@endscope%
        \pgfsysprotocol@getcurrentprotocol\pgf@@arrow@temp%
        \global\let\pgf@@arrow@temp=\pgf@@arrow@temp%
      \endpgfinterruptpath%
      \expandafter\def\expandafter\pgf@temp\expandafter{\expandafter\pgfsys@invoke\expandafter{\pgf@@arrow@temp}}%
      \expandafter\global\expandafter\let\csname pgf@arrow@prot@#1@\the\pgflinewidth\endcsname=\pgf@temp%
    }%
    \pgfsysprotocol@setcurrentprotocol\pgf@arrow@temp%
  \fi%
  \csname pgf@arrow@prot@#1@\the\pgflinewidth\endcsname%
} 

\def\pgf@arrow@code@{} % dummy

\def\pgf@nousepath@here#1{%
  \PackageError{pgf}{The definition of an arrow may not use \string\pgfusepath}{}
}



% Define an arrow type.
%
% #1 = name or mnemonic for arrow when used at the start (examples: ``to'' or ``<'')
% #2 = name or mnemonic for arrow when used at the end (examples: ``to'' or ``>'')
% #3 = code to setup the left and right extend of the arrow. To set
%      the left extend, call \pgfarrowsleftextend, for the right \pgfarrowsrightextend.
% #4 = protocolable code
%
% Description:
%
% When you define an arrow using this command, you must give two
% names. The first is used for the arrow when it is ``at the start'',
% the other when it is at the end. For example, a simple arrow might
% have the names ``<'' and ``>'', though these particular names are
% not used by pgf and left for the user.
%
% The code should be ``protocolable'' code. This means that it uses
% only pretty simple commands. 
%
% The arrow code will be protocolled once for each line width at which
% the arrow is used. Thus, the code can (and often should) depend on
% the line width.
%
% The arrow should ``point right'' in the coordinate system. The end
% of the line at which the arrow should be drawn will be at the origin
% of the coordinate system. The coordinate system will be scaled and
% rotated appropriately before the arrow is drawn.
%
% The right extend of the arrow should be set to how much the arrow
% ``protrudes over the right''. Prior to drawing the arrow, the line
% will be shortened by this amount so that the arrow tip will exactly
% touch the original right end of the unshortened line.
%
% The left extend specifies the leftmost point of the arrow. This is
% important only if you use the swapping command, when this end is
% used to compute the shortening. 
%
% The definition of an arrow should normally take care of the fact
% that the line cap of the main line may be a butt cap, a round cap or
% a rect cap. In all cases, the arrow should ``cover'' the cap
% completely or not at all.
%
% Example:
%
% \pgfarrowsdeclare{stealth}{stealth}
% {
%   \pgfarrowsleftextend{-6\pgflinewidth}
%   \pgfarrowsrightextend{2\pgflinewidth}
% {
%   \pgfpathmoveto{\pgfpoint{2\pgflinewidth}{0pt}}
%   \pgfpathlineto{\pgfpoint{-6\pgflinewidth}{4\pgflinewidth}}
%   \pgfpathlineto{\pgfpoint{-3\pgflinewidth}{0pt}}
%   \pgfpathlineto{\pgfpoint{-6\pgflinewidth}{-4\pgflinewidth}}
%   \pgfusepathqfill
% }

\def\pgfarrowsdeclare#1#2#3#4{%
  \pgf@arrows@check@already{#1}{#2}
  {%
    \expandafter\def\csname pgf@arrow@code@#2\endcsname{#4}%
    \expandafter\def\csname pgf@arrow@left@#2\endcsname{#3\advance\pgf@x by-\pgf@xa}%
    \expandafter\def\csname pgf@arrow@right@#2\endcsname{#3\advance\pgf@x by\pgf@xb}%
    \pgf@arrows@invname{#1}{#2}%
  }%
}

\def\pgfarrowsleftextend#1{\pgfmathsetlength\pgf@xa{#1}}
\def\pgfarrowsrightextend#1{\pgfmathsetlength\pgf@xb{#1}}

\def\pgf@arrows@repeat#1#2{%
  \edef\pgf@arrows@marshal{\noexpand\let\expandafter\noexpand\csname#2\endcsname=\expandafter\noexpand\csname#1\endcsname}%
  \pgf@arrows@marshal}



% Declare a new arrow type to be the same as another one.
%
% #1 = name of new start
% #2 = name or new end
% #3 = name or old start
% #4 = name or old end
%
% Example:
%
% \pgfarrowsdeclarealias{<}{>}{to}{to}

\def\pgfarrowsdeclarealias#1#2#3#4{%
  \pgf@arrows@check@already{#1}{#2}
  {%
    \pgf@arrows@checked{#3}{#4}%
    {%
      \pgf@arrows@repeat{pgf@arrow@code@#4}{pgf@arrow@code@#2}%
      \pgf@arrows@repeat{pgf@arrow@left@#4}{pgf@arrow@left@#2}%
      \pgf@arrows@repeat{pgf@arrow@right@#4}{pgf@arrow@right@#2}%
      \pgf@arrows@invname{#1}{#2}%
    }%
  }%
}




% Creates a new arrows by ``swapping'' an existing arrow.
%
% #1 = name of new start
% #2 = name of new end
% #3 = name of old start
% #4 = name of old end
%
% Example:
%
% \pgfarrowsdeclarealias{]}{[}{[}{]}

\def\pgfarrowsdeclarereversed#1#2#3#4{%
  \pgf@arrows@check@already{#1}{#2}%
  {%
    \pgf@arrows@checked{#3}{#4}%
    {%
      \expandafter\def\csname pgf@arrow@code@#2\endcsname{%
        \pgflowlevel{\pgftransformxscale{-1}}%
        \csname pgf@arrow@code@#4\endcsname}%
      \pgf@arrows@repeat{pgf@arrow@right@#4}{pgf@arrow@left@#2}%
      \pgf@arrows@repeat{pgf@arrow@left@#4}{pgf@arrow@right@#2}%
      \pgf@arrows@invname{#1}{#2}%
    }%
  }%
}



% Creates new arrows by combining two existing arrows.
%
% #1 = optional additional space
% #2 = name of new start
% #3 = name of new end
% #4 = name of second (innermost) start
% #5 = name of second end
% #6 = name of first (outermost) start
% #7 = name of first end
%
% In the star form, the line will end at the innermost arrows,
% otherwise the line will end at the outermost arrows.
%
% Example:
%
% \pgfarrowsdeclarecombine*{|<}{>|}{|}{|}{<}{>}
% \pgfarrowsdeclarecombine{<<}{>>}{<}{>}{<}{>}

\def\pgfarrowsdeclarecombine{\pgfutil@ifnextchar*{\pgfarrowsdeclarecombine@star}{\pgf@@arrowsdeclarecombine}}

\def\pgf@@arrowsdeclarecombine{\pgfutil@ifnextchar[{\pgf@arrowsdeclarecombine}{\pgf@arrowsdeclarecombine[0pt]}}
\def\pgf@arrowsdeclarecombine[#1]#2#3#4#5#6#7{%
  \pgf@arrows@check@already{#2}{#3}%
  {%
    \pgf@arrows@checked{#4}{#5}%
    {%
      \pgf@arrows@checked{#6}{#7}%
      {%
        \expandafter\edef\csname pgf@arrow@code@#3\endcsname{%
          \noexpand\pgfscope%
          {\expandafter\noexpand\csname pgf@arrow@code@#7\endcsname}%
          \noexpand\endpgfscope%
          {%
            \noexpand\pgfmathsetlength\pgf@x{#1}%
            \noexpand\pgf@process{\expandafter\noexpand\csname pgf@arrow@left@#7\endcsname}%
            \noexpand\pgf@process{\expandafter\noexpand\csname pgf@arrow@right@#5\endcsname}%
            \pgf@x=-\pgf@x%
            \noexpand\pgflowlevel{\noexpand\pgftransformxshift{\pgf@x}}%
            \expandafter\noexpand\csname pgf@arrow@code@#5\endcsname}%
          }%
        \pgf@arrows@repeat{pgf@arrow@right@#7}{pgf@arrow@right@#3}%
        \expandafter\def\csname pgf@arrow@left@#3\endcsname{%
          \pgf@process{%
            \pgfmathsetlength\pgf@y{#1}%
            \advance\pgf@x by\pgf@y%
            \pgf@process{\csname pgf@arrow@left@#7\endcsname}%
            \pgf@process{\csname pgf@arrow@right@#5\endcsname}%
            \pgf@process{\csname pgf@arrow@left@#5\endcsname}%
          }%
        }%
        \pgf@arrows@invname{#2}{#3}%
      }%
    }%
  }%
}

\def\pgfarrowsdeclarecombine@star*{\pgfutil@ifnextchar[{\pgf@arrowsdeclarecombine@star}{\pgf@arrowsdeclarecombine@star[0pt]}}
\def\pgf@arrowsdeclarecombine@star[#1]#2#3#4#5#6#7{%
  \pgf@arrows@check@already{#2}{#3}%
  {%
    \pgf@arrows@checked{#4}{#5}%
    {%
      \pgf@arrows@checked{#6}{#7}%
      {%
        \expandafter\edef\csname pgf@arrow@code@#3\endcsname{%
          \noexpand\pgfscope%
            {%
              \noexpand\pgfmathsetlength\pgf@x{#1}%
              \pgf@process{\expandafter\noexpand\csname pgf@arrow@left@#7\endcsname}%
              \pgf@process{\expandafter\noexpand\csname pgf@arrow@right@#5\endcsname}%
              \noexpand\pgflowlevel{\noexpand\pgftransformxshift{\pgf@x}}%
            }%
            {\expandafter\noexpand\csname pgf@arrow@code@#7\endcsname}%
          \noexpand\endpgfscope%
          \expandafter\noexpand\csname pgf@arrow@code@#5\endcsname%
        }%
        \pgf@arrows@repeat{pgf@arrow@left@#7}{pgf@arrow@left@#3}%
        \expandafter\def\csname pgf@arrow@right@#3\endcsname{%
          \pgf@process{%
            \pgfmathsetlength\pgf@y{#1}%
            \advance\pgf@x by\pgf@y%
            \pgf@process{\csname pgf@arrow@left@#7\endcsname}%
            \pgf@process{\csname pgf@arrow@right@#5\endcsname}%
            \pgf@process{\csname pgf@arrow@right@#7\endcsname}%
          }%
        }%
        \pgf@arrows@invname{#2}{#3}%
      }%
    }%
  }%
}



% Creates new arrows by doubling/tripling existing arrows.
%
% #1 = optional additional space in multiples of line width
% #2 = name of new start
% #3 = name of new end
% #4 = name of old start
% #5 = name of old end
%
% Example:
%
% \pgfarrowsdeclaredouble{<<}{>>}{<}{>}

\def\pgfarrowsdeclaredouble{\pgfutil@ifnextchar[{\pgf@arrowsdeclaredouble}{\pgf@arrowsdeclaredouble[0pt]}}
\def\pgf@arrowsdeclaredouble[#1]#2#3#4#5{\pgfarrowsdeclarecombine[#1]{#2}{#3}{#4}{#5}{#4}{#5}}
\def\pgfarrowsdeclaretriple{\pgfutil@ifnextchar[{\pgf@arrowsdeclaretriple}{\pgf@arrowsdeclaretriple[0pt]}}
\def\pgf@arrowsdeclaretriple[#1]#2#3#4#5{%
  \pgfarrowsdeclarecombine[#1]{pgf@trip@#2}{pgf@trip@#3}{#4}{#5}{#4}{#5}%
  \pgfarrowsdeclarecombine[#1]{#2}{#3}{pgf@trip@#2}{pgf@trip@#3}{#4}{#5}%
}


% A stealth-fighter-like pointed arrow
%
% Example:
%
% \pgfsetarrows{-stealth}

\pgfarrowsdeclare{stealth}{stealth}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-3\pgfutil@tempdima}
  \pgfarrowsrightextend{+5\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{5\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqfill
}

\pgfarrowsdeclarereversed{stealth reversed}{stealth reversed}{stealth}{stealth}


% An arrow similar to the $\to$ arrow
%
% Example:
%
% \pgfsetarrow{-to}

\pgfarrowsdeclare{to}{to}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclare{to reversed}{to reversed}
{
  \pgfutil@tempdima=-0.21pt%
  \advance\pgfutil@tempdima by-0.475\pgflinewidth%
  \pgfutil@tempdimb=0.98pt%
  \advance\pgfutil@tempdimb by1.45\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{+0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{3.5\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{3.25\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{-0.25\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{0.5\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{3.25\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{3.5\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}



% LaTeX's orginal arrow type
%
% Example:
%
% \pgfsetarrows{-latex}

\pgfarrowsdeclare{latex}{latex}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-1\pgfutil@tempdima}
  \pgfarrowsrightextend{+9\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{6.3333\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{2\pgfutil@tempdima}{2\pgfutil@tempdima}}
  {\pgfqpoint{-1\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-1\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{2\pgfutil@tempdima}{-2\pgfutil@tempdima}}
  {\pgfqpoint{6.3333\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfusepathqfill
}
\pgfarrowsdeclarereversed{latex reversed}{latex reversed}{latex}{latex}



% A bar shaped arrow
%
% Example:
%
% \pgfsetarrows{-|}

\pgfarrowsdeclare{|}{|}
{
  \pgfarrowsleftextend{+-0.25\pgflinewidth}
  \pgfarrowsrightextend{+.75\pgflinewidth}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetrectcap
  \pgfpathmoveto{\pgfqpoint{0.25\pgflinewidth}{-\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.25\pgflinewidth}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}



\endinput


==> pgfcoregraphicstate.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoregraphicstate.code.tex,v 1.7 2007/03/09 17:49:32 tantau Exp $

% Globals

\newdimen\pgflinewidth


% Set the line width to #1.
% 
% #1 = new line width.
% 
% Example:
%
% \pgfsetlinewidth{3pt}

\def\pgfsetlinewidth#1{%
  \pgfmathsetlength\pgflinewidth{#1}%
  \global\pgflinewidth=\pgflinewidth%
  \pgfsys@setlinewidth{\the\pgflinewidth}%
  \ignorespaces}


% Set the miter limit to #1.
% 
% #1 = new miter limit factor.
% 
% Example:
%
% \pgfsetmiterlimit{3}

\def\pgfsetmiterlimit#1{%
  \pgfsys@setmiterlimit{#1}%
  \ignorespaces}


% Set the dash pattern to #1 with phase #2/
% 
% #1 = a row of numbers of length of ``on'' and ``off'' points.
% #2 = a phase
% 
% Example:
%
% \pgfsetdash{}          {0pt} % solid line
% \pgfsetdash{{.1cm}}    {0pt} % long dashes
% \pgfsetdash{{1pt}{1ex}}{0pt} % dotted

\def\pgfsetdash#1#2{%
  \def\pgf@temp{}%
  \def\pgf@next{\pgf@strip}%
  \pgf@strip#1{pgf@stop}%
  \pgfmathsetlength\pgf@x{#2}%
  \pgfsys@setdash{\pgf@temp}{\the\pgf@x}%
  \ignorespaces}

\def\pgf@strip#1{%
  \def\pgf@@temp{#1}%
  \ifx\pgf@@temp\pgf@stop%
    \let\pgf@next=\relax%
  \else%
    \pgfmathsetlength\pgf@x{#1}%
    \ifx\pgf@temp\pgfutil@empty%
      \edef\pgf@temp{\the\pgf@x}%
    \else%
      \edef\pgf@temp{\pgf@temp,\the\pgf@x}%
    \fi%
  \fi\pgf@next}

\def\pgf@stop{pgf@stop}


% Set color of strokes. This will overrule the normal color.
% 
% Example:
%
% \pgfsetstrokecolor{red}

\def\pgfsetstrokecolor#1{%
  \pgfutil@colorlet{pgf@tempcolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
  \expandafter\expandafter\expandafter\pgf@setstrokecolor\csname\string\color@pgf@tempcolor\endcsname%
}
\def\pgf@setstrokecolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4@stroke\endcsname\relax%
    \PackageError{pgfbase}{Unsupported color model `#4'. Sorry}{}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4@stroke\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}

\def\pgf@uncomma#1,{%
  \def\pgf@coltest{#1}%
  \ifx\pgf@coltest\pgfutil@empty%
    \let\pgf@colnext=\relax%
  \else%
    \expandafter\def\expandafter\pgf@colmarshal\expandafter{\pgf@colmarshal{#1}}%
    \let\pgf@colnext=\pgf@uncomma%
  \fi%
  \pgf@colnext%  
}


% Set color of fills. This will overrule the normal color.
% 
% Example:
%
% \pgfsetfillcolor{gray}

\def\pgfsetfillcolor#1{%
  \pgfutil@colorlet{pgf@tempcolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
  \expandafter\expandafter\expandafter\pgf@setfillcolor\csname\string\color@pgf@tempcolor\endcsname%
}
\def\pgf@setfillcolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4@fill\endcsname\relax%
    \PackageError{pgfbase}{Unsupported color model `#4'. Sorry}{}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4@fill\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}



% Sets both the stroke and fill color.
% 
% Example:
%
% \pgfsetcolor{blue}

\def\pgfsetcolor#1{%
  \pgfutil@colorlet{pgf@tempcolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
  \expandafter\expandafter\expandafter\pgf@setcolor\csname\string\color@pgf@tempcolor\endcsname%
}
\def\pgf@setcolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4\endcsname\relax%
    \PackageError{pgfbase}{Unsupported color model `#4'. Sorry}{}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}

% Code for ensuring the stroke/fill colors are correctly reset.
\def\XC@bcolor{\pgfsys@color@reset}

% Set a butt line cap.
% 
% Example:
%
% \pgfsetbuttcap

\def\pgfsetbuttcap{\pgfsys@buttcap\ignorespaces}


% Set a round line cap.
% 
% Example:
%
% \pgfsetroundcap

\def\pgfsetroundcap{\pgfsys@roundcap\ignorespaces}


% Set a rectangular line cap.
% 
% Example:
%
% \pgfsetrectcap

\def\pgfsetrectcap{\pgfsys@rectcap\ignorespaces}


% Set a miter line join.
% 
% Example:
%
% \pgfsetmiterjoin

\def\pgfsetmiterjoin{\pgfsys@miterjoin\ignorespaces}


% Set a bevel line join.
% 
% Example:
%
% \pgfsetbeveljoin

\def\pgfsetbeveljoin{\pgfsys@beveljoin\ignorespaces}


% Set a round line join.
% 
% Example:
%
% \pgfsetroundjoin

\def\pgfsetroundjoin{\pgfsys@roundjoin\ignorespaces}


% Sets the even-odd rule for filling and clipping.
% 
% Example:
%
% \pgfseteorule

\def\pgfseteorule{\pgfsys@eoruletrue\ignorespaces}


% Sets the non-zero winding number rule for filling and clipping.
% 
% Example:
%
% \pgfsetnonzerorule

\def\pgfsetnonzerorule{\pgfsys@eorulefalse\ignorespaces}


% Sets the opacity of stroking operations.
% 
% #1 = opacity, where 1 means fully opaque and 0 means fully
% transparent. 
%
% Example:
%
% \pgfsetstrokeopacity{0.5}

\def\pgfsetstrokeopacity#1{%
  \edef\pgf@temp{{#1}}%
  \expandafter\pgfsys@stroke@opacity\pgf@temp}


% Sets the opacity of stroking operations.
% 
% #1 = opacity, where 1 means fully opaque and 0 means fully
% transparent. 
%
% Example:
%
% \pgfsetfillopacity{0.5}

\def\pgfsetfillopacity#1{%
  \edef\pgf@temp{{#1}}%
  \expandafter\pgfsys@fill@opacity\pgf@temp}



\endinput


==> pgfcoreobjects.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoreobjects.code.tex,v 1.2 2006/10/11 15:22:25 tantau Exp $


% Object reuse


% Define a pgf object for reuse. Such objects will be stored
% efficiently internally.
%
% #1 = name for later reuse
% #2 = lower left corner point of bounding box
% #3 = upper right left corner point of bounding box
% #4 = pure pgf code (nothing too fancy!)
%
% Description:
% 
% Used to define reusable objects. The object must be composed of
% basic pgf graphic primitives. Nothing fancy can be used. The
% created object will be stored as an xform object in pdf or as a
% postscript procedure in postscript.
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfpathqmoveto{0pt}{0pt}
%  \pgfpathqmoveto{10pt}{0pt}
%  \pgfpathqmoveto{10pt}{10pt}
%  \pgfpathqmoveto{0pt}{10pt}
%  \pgfpathclose
%  \pgfusepath{stroke}}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgfuseobject{myrect}
% \end{pgfpicture}

\def\pgfdefobject#1#2#3#4{%
  \pgfinterruptpath%
    \pgf@relevantforpicturesizefalse%
    \pgfsys@defobject{#1}{#2}{#3}{#4}%
  \endpgfinterruptpath%
  \ignorespaces%
}


% Use an object that was previously defined using pgfdefobject
%
% #1 = name of previously defined object
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfqmoveto{0}{0}
%  \pgfqmoveto{10}{0}
%  \pgfqmoveto{10}{10}
%  \pgfqmoveto{0}{10}
%  \pgfclosestroke}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgfuseobject{myrect}
% \end{pgfpicture}

\def\pgfuseobject#1{\pgfsys@beginscope\pgfsys@useobject{#1}{}\pgfsys@endscope}


% Use an object that was previously defined using pgfdefobject, but
% magnify the object by the current x and y register values
%
% #1 = name of previously defined object
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfqmoveto{0}{0}
%  \pgfqmoveto{10}{0}
%  \pgfqmoveto{10}{10}
%  \pgfqmoveto{0}{10}
%  \pgfclosestroke}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgf@x=2pt% Scale by factor two in x-direction
%   \pgf@y=2pt% Scale by factor two in y-direction
%   \pgfuseobjectmagnify{myrect}
% \end{pgfpicture}

\def\pgfuseobjectmagnify#1{%
  \pgfsys@beginscope%
  \pgfsys@useobject{#1}{\pgfsys@transformxyscale{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}}%
  \pgfsys@endscope%
}


\endinput


==> pgfcorepathconstruct.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepathconstruct.code.tex,v 1.9 2007/06/07 07:41:10 tantau Exp $


\newdimen\pgf@path@lastx
\newdimen\pgf@path@lasty



% Replace corners by arcs.
%
% #1 = in-size of arc
% #2 = out-size of arc
% 
% Description:
% 
% This command influences path construction command like
% \pgfpathlineto or \pgfpatharc. It will cause the corners at the end
% of these commands to be replaced by little arcs. If the
% corner is a 90 degrees corner and if #1=#2, a quarter-circle of
% radius #1 is put in place of the corner. If #1 and #2 are different,
% the quarter circle will instead by a quarter ellipse. If the angle
% is different from 90 degrees, a deformed quarter circle will
% result, which may or may not be desirable. For a ``perfect'' arc you
% must use the \pgfpatharc command. 
% 
% 
% Example: One rounded corner.
%
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathlineto{\pgfpointxy{0}{1}}
% \pgfpathlineto{\pgfpointxy{1}{1}}
% \pgfstroke
%
% Example: A rounded rectangle
%
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% \pgfstroke
%
% Example: A rounded triangles
%
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{1cm}{0cm}}
% \pgfpathlineto{\pgfpoint{1cm}{1cm}}
% \pgfpathclose
% \pgfstroke

\newif\ifpgf@arccorners

\def\pgfsetcornersarced#1{%
  \pgf@process{#1}%
  \edef\pgf@corner@arc{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@arccornerstrue%
  \ifdim\pgf@x=0pt%
    \ifdim\pgf@y=0pt\relax%
      \pgf@arccornersfalse%
    \fi%
  \fi%
}

\def\pgf@roundcornerifneeded{%
  \ifpgf@arccorners\expandafter\pgfsyssoftpath@specialround\pgf@corner@arc\fi%
}


% Move current point to #1.
%
% #1 = new current point
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfstroke

\def\pgfpathmoveto#1{%
  \pgfpointtransformed{#1}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgfsyssoftpath@moveto{\the\pgf@x}{\the\pgf@y}%
  \global\pgf@path@lastx=\pgf@x%
  \global\pgf@path@lasty=\pgf@y%
}

\def\pgf@protocolsizes#1#2{%
  \ifpgf@relevantforpicturesize%
    \ifdim#1<\pgf@picminx\global\pgf@picminx#1\fi%
    \ifdim#1>\pgf@picmaxx\global\pgf@picmaxx#1\fi%
    \ifdim#2<\pgf@picminy\global\pgf@picminy#2\fi%
    \ifdim#2>\pgf@picmaxy\global\pgf@picmaxy#2\fi%
  \fi%
  \ifdim#1<\pgf@pathminx\global\pgf@pathminx#1\fi%
  \ifdim#1>\pgf@pathmaxx\global\pgf@pathmaxx#1\fi%
  \ifdim#2<\pgf@pathminy\global\pgf@pathminy#2\fi%
  \ifdim#2>\pgf@pathmaxy\global\pgf@pathmaxy#2\fi%
}


\def\pgf@resetpathsizes{%
  \global\pgf@pathmaxx=-16000pt\relax%
  \global\pgf@pathminx=16000pt\relax%
  \global\pgf@pathmaxy=-16000pt\relax%
  \global\pgf@pathminy=16000pt\relax%
}

\def\pgf@getpathsizes#1{%
  \edef#1{{\the\pgf@pathmaxx}{\the\pgf@pathminx}{\the\pgf@pathmaxy}{\the\pgf@pathminy}}%
}
\def\pgf@setpathsizes#1{%
  \expandafter\pgf@@setpathsizes#1%
}
\def\pgf@@setpathsizes#1#2#3#4{%
  \global\pgf@pathmaxx=#1\relax%
  \global\pgf@pathminx=#2\relax%
  \global\pgf@pathmaxy=#3\relax%
  \global\pgf@pathminy=#4\relax%
}





% Append a line from the current point to #1 to the current path.
%
% #1 = end of line
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfstroke

\def\pgfpathlineto#1{%
  \pgfpointtransformed{#1}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@roundcornerifneeded%
  \pgfsyssoftpath@lineto{\the\pgf@x}{\the\pgf@y}%
  \global\pgf@path@lastx=\pgf@x%
  \global\pgf@path@lasty=\pgf@y%
}



% Close the current path.
%
% Example:
%
% % Draws two triangles
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfclosepath
% \pgfpathmoveto{\pgfxy(2,0)}
% \pgfpathlineto{\pgfxy(2,1)}
% \pgfpathlineto{\pgfxy(3,0)}
% \pgfpathclose
% \pgfstroke

\def\pgfpathclose{%
  \pgf@roundcornerifneeded%
  \pgfsyssoftpath@closepath%
}


% Append a bezier spline from the current point to #3 with control
% points #1 and #2 to the current path.
%
% #1 = first control point
% #2 = second control point
% #3 = end point
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathcurveto{\pgfxy(0,1)}{\pgfxy(1,1)}{\pgfxy(1,2)}
% \pgfstroke

\def\pgfpathcurveto#1#2#3{%
  \pgfpointtransformed{#3}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgfpointtransformed{#2}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpointtransformed{#1}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@roundcornerifneeded%
  \pgfsyssoftpath@curveto{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xb}{\the\pgf@yb}%
  \global\pgf@path@lastx=\pgf@xb%
  \global\pgf@path@lasty=\pgf@yb%
}


% Append an arc to the current point, where the current point is at
% angle #1 and the end is at angle #2. If #2 > #1, the arc is drawn
% counter-clockwise, otherwise it is clockwise.
%
% #1 = angle of first point
% #2 = angle of second point
% #3 = radius or x-radius/y-radius
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpatharc{0}{90}{2cm}
% \pgfstroke

\def\pgfpatharc#1#2#3{%
  \pgfmathsetcounter{pgf@countc}{#1}%
  \pgfmathsetcounter{pgf@countd}{#2}%
  \ifnum\c@pgf@countc>360\relax%
    \advance\c@pgf@countc by-360\relax%
  \fi%
  \ifnum\c@pgf@countc<-360\relax%
    \advance\c@pgf@countc by360\relax%
  \fi%
  \ifnum\c@pgf@countd>360\relax%
    \advance\c@pgf@countd by-360\relax%
  \fi%
  \ifnum\c@pgf@countd<-360\relax%
    \advance\c@pgf@countd by360\relax%
  \fi%
  \loop%
    \pgfutil@tempcnta=\c@pgf@countc\relax%
    \advance\pgfutil@tempcnta by-\c@pgf@countd\relax%
    \ifnum\pgfutil@tempcnta<0\relax%
      \pgfutil@tempcnta=-\pgfutil@tempcnta\relax%
    \fi%
  \ifnum\pgfutil@tempcnta>90\relax%
    \ifnum\c@pgf@countd>\c@pgf@countc\relax%
      \pgfutil@tempcnta=\c@pgf@countc\relax%
      \advance\pgfutil@tempcnta by 90\relax%
      \expandafter\pgf@arc\expandafter{\expandafter\c@pgf@countc\expandafter}\expandafter{\the\pgfutil@tempcnta}{#3}%
      \advance\c@pgf@countc by 90\relax%
    \else
      \pgfutil@tempcnta=\c@pgf@countc\relax%
      \advance\pgfutil@tempcnta by -90\relax%
      \expandafter\pgf@arc\expandafter{\expandafter\c@pgf@countc\expandafter}\expandafter{\the\pgfutil@tempcnta}{#3}%
      \advance\c@pgf@countc by -90\relax%
    \fi%
  \repeat%
  \pgf@roundcornerifneeded%
  \pgf@arc{\c@pgf@countc}{\c@pgf@countd}{#3}%
}

\def\pgf@arc#1#2#3{%
  \pgfutil@in@{and }{#3}%
  \ifpgfutil@in@%
    \pgf@@arc{#1}{#2}#3\@@%
  \else
    \pgf@@arc{#1}{#2}#3and #3\@@%
  \fi%
}

\def\pgf@@arc#1#2#3and #4\@@{%
  \pgfmathsetlength{\pgfutil@tempdima}{#3}%
  \pgfmathsetlength{\pgfutil@tempdimb}{#4}%
  \pgfutil@tempcnta=#1\relax%
  \pgfutil@tempcntb=#2\relax%
  \advance\pgfutil@tempcntb by-\pgfutil@tempcnta\relax%
  \ifnum\pgfutil@tempcntb<0\relax%
    \pgfutil@tempcntb=-\pgfutil@tempcntb\relax%
  \fi%
  \ifnum\pgfutil@tempcntb>85\relax% hackery to correct the control points
    \pgfutil@tempdima=0.0555\pgfutil@tempdima\relax%
    \pgfutil@tempdimb=0.0555\pgfutil@tempdimb\relax%
  \else%
    \ifnum\pgfutil@tempcntb>75\relax%  
      \pgfutil@tempdima=0.055\pgfutil@tempdima\relax%
      \pgfutil@tempdimb=0.055\pgfutil@tempdimb\relax%
    \else%
      \ifnum\pgfutil@tempcntb>60\relax%  
        \pgfutil@tempdima=0.0545\pgfutil@tempdima\relax%
        \pgfutil@tempdimb=0.0545\pgfutil@tempdimb\relax%
      \else%
        \pgfutil@tempdima=0.054\pgfutil@tempdima\relax%
        \pgfutil@tempdimb=0.054\pgfutil@tempdimb\relax%
      \fi%
    \fi%
  \fi
  \pgfutil@tempdima=\pgfutil@tempcntb\pgfutil@tempdima\relax%
  \divide\pgfutil@tempdima by 9\relax%
  \pgfutil@tempdimb=\pgfutil@tempcntb\pgfutil@tempdimb\relax%
  \divide\pgfutil@tempdimb by 9\relax%
  %.. controls +(\pgfutil@tempcnta+90:\pgfutil@tempdima) and +(\pgfutil@tempcntb-90:\pgfutil@tempdima) .. +(-(#1:#3)+(#2:#3))%
  % store first support vector in xa/ya:
  \pgfutil@tempcnta=#1\relax%
  \ifnum#2>#1\relax%
    \advance\pgfutil@tempcnta by 90\relax%
  \else%
    \advance\pgfutil@tempcnta by -90\relax%
  \fi%
  \pgfpointtransformed{\pgfpointpolar{\pgfutil@tempcnta}{\pgfutil@tempdima and \pgfutil@tempdimb}}%
  \advance\pgf@x by-\pgf@pt@x%
  \advance\pgf@y by-\pgf@pt@y%
  \pgf@xa=\pgf@path@lastx%
  \pgf@ya=\pgf@path@lasty%
  \advance\pgf@xa by \pgf@x%
  \advance\pgf@ya by \pgf@y%
  % store target in xb/yb:
  \pgfutil@tempcnta=#1\relax%
  \pgfpointtransformed{\pgfpointpolar{\pgfutil@tempcnta}{#3and #4}}%
  \pgf@xb=\pgf@path@lastx%
  \pgf@yb=\pgf@path@lasty%
  \advance\pgf@xb by -\pgf@x%
  \advance\pgf@yb by -\pgf@y%
  \pgfutil@tempcnta=#2\relax%
  \pgfpointtransformed{\pgfpointpolar{\pgfutil@tempcnta}{#3and #4}}%
  \advance\pgf@xb by \pgf@x%
  \advance\pgf@yb by \pgf@y%
  % store second support xc/yc:
  \pgfutil@tempcnta=#2\relax%
  \ifnum#2>#1\relax%
    \advance\pgfutil@tempcnta by -90\relax%
  \else%
    \advance\pgfutil@tempcnta by 90\relax%
  \fi%
  \pgfpointtransformed{\pgfpointpolar{\pgfutil@tempcnta}{\pgfutil@tempdima and \pgfutil@tempdimb}}%
  \advance\pgf@x by-\pgf@pt@x%
  \advance\pgf@y by-\pgf@pt@y%
  \pgf@xc=\pgf@xb\relax%
  \pgf@yc=\pgf@yb\relax%
  \advance \pgf@xc by \pgf@x\relax%
  \advance \pgf@yc by \pgf@y\relax%
  \pgfsyssoftpath@curveto{\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xc}{\the\pgf@yc}{\the\pgf@xb}{\the\pgf@yb}%
  \global\pgf@path@lastx=\pgf@xb%
  \global\pgf@path@lasty=\pgf@yb%
  \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  \pgf@protocolsizes{\pgf@xb}{\pgf@yb}%
  \pgf@protocolsizes{\pgf@xc}{\pgf@yc}%
}

% Append an arc to the current point, where the arc is on an ellipse
% given by two axis vectors.
%
% #1 = angle of first point
% #2 = angle of second point
% #3 = first axis
% #4 = second axis
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpatharcaxes{0}{90}{\pgfpointxy{2}{0}}{\pgfpointxy{0}{2}}
% \pgfstroke

\def\pgfpatharcaxes#1#2#3#4{%
  {%
    \pgftransformtriangle{\pgfpointorigin}{#3}{#4}%
    \pgfpatharc{#1}{#2}{1pt}%
  }%
}




% Append  an ellipse to the current path.
%
% #1 = center
% #2 = first axis
% #3 = second axis
%  
% Example:
%
% % Add a circle of radius 3cm around the origin
% \pgfpathellipse{\pgforigin}{\pgfxy(2,0)}{\pgfxy(0,1)}
%
% % Draw a non-filled circle of radius 1cm around the point (1,1)
% \pgfpathellipse{\pgfxy(1,1)}{\pgfxy(1,1)}{\pgfxy(-2,2)}
% \pgfstroke

\def\pgfpathellipse#1#2#3{%
  \pgfpointtransformed{#1}% store center in xc/yc
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgfpointtransformed{#2}%
  \pgf@xa=\pgf@x% store first axis in xa/ya
  \pgf@ya=\pgf@y%
  \advance\pgf@xa by-\pgf@pt@x%
  \advance\pgf@ya by-\pgf@pt@y%
  \pgfpointtransformed{#3}%
  \pgf@xb=\pgf@x% store second axis in xb/yb
  \pgf@yb=\pgf@y%
  \advance\pgf@xb by-\pgf@pt@x%
  \advance\pgf@yb by-\pgf@pt@y%
  {%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%
    \pgfsyssoftpath@moveto{\the\pgf@xa}{\the\pgf@ya}%
    \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  }%
  \pgf@x=0.555\pgf@xb% first arc
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xa%
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xb by\pgf@xc%
    \advance\pgf@yb by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xb}{\the\pgf@yb}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xb}{\pgf@yb}%
  }%
  \pgf@xa=-\pgf@xa% flip first axis
  \pgf@ya=-\pgf@ya%
  \pgf@x=0.555\pgf@xa% second arc
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xb%
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}%  
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  }%
  \pgf@xb=-\pgf@xb% flip second axis
  \pgf@yb=-\pgf@yb%
  \pgf@x=0.555\pgf@xb% third arc
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xa%
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xb by\pgf@xc%
    \advance\pgf@yb by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xb}{\the\pgf@yb}%  
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xb}{\pgf@yb}%
  }%
  \pgf@xa=-\pgf@xa% flip first axis once more
  \pgf@ya=-\pgf@ya%
  \pgf@x=0.555\pgf@xa% fourth arc
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xb%
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  }%
  \pgfsyssoftpath@closepath%
  \pgfsyssoftpath@moveto{\the\pgf@xc}{\the\pgf@yc}%
}



% Append a circle to the current path
%
% #1 = center
% #2 = radius
%  
% Example:
%
% % Append a circle of radius 3cm around the the point (1,1)
% \pgfpathcircle{\pgxy(1,1)}{3cm}

\def\pgfpathcircle#1#2{\pgfpathellipse{#1}{\pgfpoint{#2}{0pt}}{\pgfpoint{0pt}{#2}}}




% Append a rectangle to the current path
%
% #1 = lower left corner point of rectangle
% #2 = width and height vector
%  
% Example:
%
% % A rectangle with corners (2,2) and (3,3)
% \pgfpathrectangle{\pgfpointxy{2}{2}}{\pgfpointxy{1}{1}}

\def\pgfpathrectangle{%
  \let\pgfrect@next=\pgf@specialrect%
  \ifpgf@pt@identity%
    \ifpgf@arccorners%
    \else%
      \let\pgfrect@next=\pgf@normalrect%
    \fi%
  \fi%
  \pgfrect@next%
}

\def\pgf@normalrect#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpointtransformed{#1}%
  \pgfsyssoftpath@rect{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \advance\pgf@x by\pgf@xa\relax%
  \advance\pgf@y by\pgf@ya\relax%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
}

\def\pgf@specialrect#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#1}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \advance\pgf@xa by\pgf@xb%
  \advance\pgf@ya by\pgf@yb%
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathclose%
  \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
}

% Append a rectangle to the current path
%
% #1 = one corner of the rectangle
% #2 = opposite corner of the rectangle
%  
% Example:
%
% % A rectangle with corners (2,2) and (3,3)
% \pgfpathrectanglecorners{\pgfpointxy{2}{2}}{\pgfpointxy{3}{3}}

\def\pgfpathrectanglecorners#1#2{%
  \pgf@process{#2}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xc by-\pgf@x%
  \advance\pgf@yc by-\pgf@y%
  \pgfpathrectangle{#1}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
}


% Append a grid to the current path.
%
% #1 = lower left point of grid
% #2 = upper right point of grid
%  
% Options: 
%  
% stepx = x-step dimension (default 1cm)
% stepy = y-step dimension (default 1cm)
% step  = dimesion vector
%  
% Example:
%
% \pgfsetlinewidth{0.8pt}
% \pgfgrid{\pgfxy(0,0)}{\pgfxy(3,2)}
% \pgfsetlinewidth{0.4pt}
% \pgfgrid[stepx=1cm,stepy=1cm]{\pgfxy(0,0)}{\pgfxy(3,2)}

\define@key{pgfbase}{stepx}{\pgfmathsetlength{\pgf@x}{#1}\relax}
\define@key{pgfbase}{stepy}{\pgfmathsetlength{\pgf@y}{#1}\relax}
\define@key{pgfbase}{step}{\pgf@process{#1}}

\def\pgfpathgrid{\pgfutil@ifnextchar[{\pgf@pathgrid}{\pgf@pathgrid[]}}
\def\pgf@pathgrid[#1]#2#3{%
  \setkeys{pgfbase}{stepx=1cm,stepy=1cm}%
  \setkeys{pgfbase}{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgf@process{#3}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x\relax%
  \pgf@ya=\pgf@y\relax%
  {%
    % compute bounding box
    % first corner
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    % second corner
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@ya%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    % third corner
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@yb%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    % fourth corner
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  }%
  \c@pgf@counta=\pgf@y\relax%
  \c@pgf@countb=\pgf@yc\relax%
  \divide\c@pgf@counta by\c@pgf@countb\relax%
  \pgf@y=\c@pgf@counta\pgf@yc\relax%
  \ifdim\pgf@y<\pgf@ya%
    \advance\pgf@y by\pgf@yc%
  \fi%
  \loop% horizontal lines
    {%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@moveto{\the\pgf@xa}{\the\pgf@ya}%
      \pgf@xa=\pgf@xb%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@lineto{\the\pgf@xa}{\the\pgf@ya}%
    }%
    \advance\pgf@y by\pgf@yc%
  \ifdim\pgf@y<\pgf@yb%
  \repeat%
  \advance\pgf@y by-0.01pt\relax%
  \ifdim\pgf@y<\pgf@yb%
    {%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@moveto{\the\pgf@xa}{\the\pgf@ya}%
      \pgf@xa=\pgf@xb%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@lineto{\the\pgf@xa}{\the\pgf@ya}%
    }%
  \fi%
  \c@pgf@counta=\pgf@x\relax%
  \c@pgf@countb=\pgf@xc\relax%
  \divide\c@pgf@counta by\c@pgf@countb\relax%
  \pgf@x=\c@pgf@counta\pgf@xc\relax%
  \ifdim\pgf@x<\pgf@xa%
    \advance\pgf@x by\pgf@xc%
  \fi%
  \loop% vertical lines
    {%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@ya%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@moveto{\the\pgf@xc}{\the\pgf@yc}%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@yb%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@lineto{\the\pgf@xc}{\the\pgf@yc}%
    }%
    \advance\pgf@x by\pgf@xc%
  \ifdim\pgf@x<\pgf@xb%
  \repeat%
  \advance\pgf@x by-0.01pt\relax%
  \ifdim\pgf@x<\pgf@xb%
    {%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@ya%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@moveto{\the\pgf@xc}{\the\pgf@yc}%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@yb%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@lineto{\the\pgf@xc}{\the\pgf@yc}%
    }%
  \fi%
}



% Append two half-parabolas to the path
%
% #1 = bend (relative to current point)
% #2 = end point (relative to bend point)
%  
% Description:
%  
% This command appends a half-parabola that starts at the current point
% and has its bend at #1+current point. Then, a second parabola is
% appended that starts at #1+current point, where it also has its
% minimum/maximum, and ends at #1+current point+#2, which becomes the
% new current point. 
%  
% By setting #2 = (0,0) you draw only a half parabola that goes from the
% current point to the bend; by setting #1 = (0,0)
% you draw a half parabola that going to current point + #2 and has its
% bend at the current point. 
%  
% Examples:
%
% % Half-parabola going ``up and right''
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpointorigin}{\pgfpoint{2cm}{4cm}}
%
% % Half-parabola going ``down and right''
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpoint{-2cm}{4cm}}}{\pgfpointorigin}
%
% % Full parabola
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpoint{-2cm}{4cm}}{\pgfpoint{2cm}{4cm}}

\def\pgfpathparabola#1#2{%
  {%
    \pgf@process{#2}% untransformed
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempswatrue%
    \ifdim\pgf@xb=0pt\relax%
      \ifdim\pgf@yb=0pt\relax%
        \pgfutil@tempswafalse%
      \fi%
    \fi%  
    {%
      \ifpgfutil@tempswa%
        \pgf@arccornersfalse
      \else%
      \fi%
      \pgfutil@tempswatrue%
      \ifdim\pgf@xc=0pt\relax%
        \ifdim\pgf@yc=0pt\relax%
          \pgfutil@tempswafalse%
        \fi%
      \fi%
      \ifpgfutil@tempswa  
      {%
        \pgf@pt@x=\pgf@path@lastx%
        \pgf@pt@y=\pgf@path@lasty%
        \pgfpathcurveto%
          {\pgfqpoint{.1125\pgf@xc}{.225\pgf@yc}}% found by trial and error
          {\pgfqpoint{.5\pgf@xc}{\pgf@yc}}% found by trial and error
          {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
      }%
      \fi%
    }%
    \ifpgfutil@tempswa%
      \pgf@xc=\pgf@xb%
      \pgf@yc=\pgf@yb%
      {%
        \pgf@pt@x=\pgf@path@lastx%
        \pgf@pt@y=\pgf@path@lasty%
        \pgfpathcurveto%
          {\pgfqpoint{.5\pgf@xc}{0\pgf@yc}}% found by trial and error
          {\pgfqpoint{.8875\pgf@xc}{.775\pgf@yc}}% found by trial and error
          {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
      }%
    \fi%
  }%  
}  




% Append a sine curve between 0 and \pi/2 to the path.
%
% #1 = vector, describing the width and height of the curve
%  
% Description:
%  
% This command appends a sine curve in the interval 0 and \pi/2 to the
% current path. The sine curve ends at currentpoint+#1.
%  
% Examples:
%
% % One complete sine in the interval [0,\pi]
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathsine{\pgfpoint{1.57cm}{1cm}}
% \pgfpathcosine{\pgfpoint{3.141cm}{0cm}}

\def\pgfpathsine#1{%
  {%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgfpathcurveto%
      {\pgfqpoint{.31831\pgf@xc}{.5\pgf@yc}}% found by trial and error
      {\pgfqpoint{.63503\pgf@xc}{\pgf@yc}}% found by trial and error
      {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  }%  
}  

% Append a cosine curve between 0 and \pi/2 to the path.
%
% #1 = vector, describing the width and height of the curve
%  
% Examples:
%
% % One complete sine in the interval [0,\pi]
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathsine{\pgfpoint{1.57cm}{1cm}}
% \pgfpathcosine{\pgfpoint{3.141cm}{0cm}}

\def\pgfpathcosine#1{%
  {%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgfpathcurveto%
      {\pgfqpoint{.36497\pgf@xc}{0pt}}% found by trial and error
      {\pgfqpoint{.68169\pgf@xc}{.5\pgf@yc}}% found by trial and error
      {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  }%  
}  


\endinput


==> pgfcorepathprocessing.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepathprocessing.code.tex,v 1.6 2007/03/09 17:49:32 tantau Exp $



% Cleanup path
%
% #1 = a macro name that stores a path
%
% Description:
%
% This command will remove superfluous parts from a path. Movetos with
% a moveto following are removed.
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@moveto{10}{10}
% \pgfsyssoftpath@lineto{0}{0}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfprocesspathcleanup\mypath

\def\pgfprocesspathcleanup#1{%
  {%
    \let\pgf@newpath=\pgfutil@empty%
    \expandafter\pgf@cleanupprocessor#1\pgf@stop%
  }%
  \let#1=\pgf@newpath%
}

\def\pgf@cleanupprocessor#1{%
  \ifx#1\pgf@stop%
    \let\next=\pgfutil@gobble% ok, done
  \else%
    \ifx#1\pgfsyssoftpath@movetotoken%
      \let\next=\pgf@cleanupmoveto%
    \else%
      \let\next=\pgf@cleanupredo%
    \fi%
  \fi%
  \next#1%
}

\def\pgf@cleanupredo#1#2#3{%
  \pgfutil@g@addto@macro\pgf@newpath{#1{#2}{#3}}%
  \pgf@cleanupprocessor%
}

\def\pgf@cleanupmoveto#1#2#3#4{%
  \ifx#4\pgfsyssoftpath@movetotoken%
    % Ok, skip
  \else%
    \pgfutil@g@addto@macro\pgf@newpath{#1{#2}{#3}}%
  \fi%
  \pgf@cleanupprocessor#4%
}



% Extract start and end vectors of a path
%
% #1 = a macro that stores a path
%
% Description:
%
% This command will extract the first and second coordinate on the
% path as well as the last and second-last. These coordinates will be
% put in the pgfpoint-macros \pgfpointfirstonpath,
% \pgfpointsecondonpath, \pgfpointsecondlastonpath, and
% \pgfpointlastonpath. If the path is empty, these macros are set to
% \pgfpointorigin. 
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{30}{40}{40}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfprocesspathextractpoints\mypath
% 
% % \pgfpointfirstonpath is now \pgfpoint{0}{0}
% % \pgfpointsecondonpath is now \pgfpoint{10bp}{10bp}
% % \pgfpointsecondlastonpath is now \pgfpoint{30bp}{30bp}
% % \pgfpointlastonpath is now \pgfpoint{40bp}{40bp}

\def\pgfprocesspathextractpoints#1{%
  \ifx#1\pgfutil@empty%
    \let\pgfpointfirstonpath=\pgfpointorigin%
    \let\pgfpointsecondonpath=\pgfpointorigin%
    \let\pgfpointsecondlastonpath=\pgfpointorigin%
    \let\pgfpointlastonpath=\pgfpointorigin%
  \else%
    \expandafter\pgf@extractprocessorfirst#1\pgf@stop%
  \fi%
}

\def\pgf@extractprocessorfirst#1#2#3#4{%
  \def\pgfpointfirstonpath{\pgfqpoint{#2}{#3}}%
  \ifx#4\pgf@stop%
    % pretty short path...
    \let\pgfpointsecondonpath=\pgfpointfirstonpath%
    \let\pgfpointsecondlastonpath=\pgfpointfirstonpath%
    \let\pgfpointlastonpath=\pgfpointfirstonpath%
    \let\next=\pgfutil@gobble%
  \else
    \let\next=\pgf@extractprocessorsecond%
  \fi%
  \next#4%
}

\def\pgf@extractprocessorsecond#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    % Reset things...
    \let\pgf@next=\pgf@extractprocessorfirst%
  \else%
    \let\pgf@next=\pgf@@extractprocessorsecond%
  \fi%
  \pgf@next#1%
}
\def\pgf@@extractprocessorsecond#1#2#3#4{%
  \def\pgfpointsecondonpath{\pgfqpoint{#2}{#3}}%
  \let\pgfpointsecondlastonpath=\pgfpointfirstonpath%
  \let\pgfpointlastonpath=\pgfpointsecondonpath%
  \ifx#4\pgf@stop%
    % short path...
    \let\next=\pgfutil@gobble%
  \else
    \let\next=\pgf@extractprocessorother%
  \fi%
  \next#4%
}

\def\pgf@extractprocessorother#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    % Reset things...
    \let\pgf@next=\pgf@extractprocessorfirst%
  \else%
    \let\pgf@next=\pgf@@extractprocessorother%
  \fi%
  \pgf@next#1%
}
\def\pgf@@extractprocessorother#1#2#3#4{%
  \let\pgfpointsecondlastonpath=\pgfpointlastonpath%
  \def\pgfpointlastonpath{\pgfqpoint{#2}{#3}}%
  \ifx#4\pgf@stop%
    % end!
    \let\next=\pgfutil@gobble%
  \fi%
  \next#4%
}



% Check for closepath and rectangles
%
% #1 = a macro that stores a path
% #2 = command to be executed when a closepath or a rectangle is encountered
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{30}{40}{40}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfprocesscheckclosed{\mypath}{\pgf@drawarrowsfalse}

\def\pgfprocesscheckclosed#1#2{%
  {%
    \global\let\pgf@proc@todo=\relax%
    \let\pgfsyssoftpath@movetotoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@linetotoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetosupportatoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetosupportbtoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetotoken=\pgfutil@gobbletwo%
    \def\pgfsyssoftpath@rectcornertoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    \def\pgfsyssoftpath@rectsizetoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    \def\pgfsyssoftpath@closepathtoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    #1%
  }%
  \pgf@proc@todo%
}

  
% Resolve specialround
%
% #1 = a macro that stores a path
% #2 = a macro that stores the new path
%
% Description:
%
% Resolves all specialround tokens. When such a token is encountered,
% the objective is to replace the next corner by a rounded corner. 
%

\def\pgfprocessround#1#2{%
  % first, check whether #1 contains \pgfsyssoftpath@specialroundtoken.
  % if not, do quick assignment!
  \expandafter\pgf@processroundcheck\expandafter#1\expandafter#2#1\pgfsyssoftpath@specialroundtoken\pgf@stop%
}

\def\pgf@processroundcheck#1#2#3\pgfsyssoftpath@specialroundtoken#4\pgf@stop{%
  \def\pgf@test{#4}%
  \ifx\pgf@test\pgfutil@empty%
    % ok, nothing to be done!
    \let#2=#1%
  \else%
    % very well...
    \pgf@@processround#1#2%
  \fi%
}


\def\pgf@@processround#1#2{%  
  \let\pgfprocess@newpath\pgfutil@empty%
  \let\pgfprocess@moveto\pgfutil@empty%
  \let\pgfprocess@firstto\pgfutil@empty%
  \let\pgfprocess@segment\pgfutil@empty%
  \pgf@xa=0pt%
  \pgf@ya=0pt%
  \expandafter\pgfprocess@round#1\pgf@stop{0pt}{0pt}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@moveto}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@segment}%
  \let#2=\pgfprocess@newpath%
}

\def\pgfprocess@round#1#2#3{%
  \ifx#1\pgf@stop%
    \let\next=\relax%
  \else%
    \ifx#1\pgfsyssoftpath@specialroundtoken%
      \def\pgfprocess@savex{#2}%
      \def\pgfprocess@savey{#3}%
      \let\next=\pgfprocess@specialround%
      \ifdim#2=0pt%
        \ifdim#3=0pt%
          \let\next=\pgfprocess@round% skip!
        \fi%
      \fi%
    \else%
      \ifx\pgfprocess@firstto\pgfutil@empty%
        \def\pgfprocess@firstto{{#2}{#3}}%
      \fi%
      \pgf@xa=#2%
      \pgf@ya=#3%
      \ifx#1\pgfsyssoftpath@movetotoken%
        % ok, move old segment to newpath
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@moveto}%
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@segment}%
        \def\pgfprocess@moveto{#1{#2}{#3}}%
        \let\pgfprocess@firstto=\pgfutil@empty%
        \let\pgfprocess@segment=\pgfutil@empty%
      \else%
        \pgfutil@g@addto@macro\pgfprocess@segment{#1{#2}{#3}}%
      \fi%
      \let\next=\pgfprocess@round%
    \fi%
  \fi%
  \next%  
}

\def\pgfprocess@specialround#1#2#3{%
  \ifx\pgfprocess@firstto\pgfutil@empty%
    \def\pgfprocess@firstto{{#2}{#3}}%
  \fi%
  \let\next=\pgfprocess@round% default: do nothing
  \ifx#1\pgfsyssoftpath@linetotoken%
    % Ok, round a lineto
    \let\next=\pgfprocess@specialroundcope%
  \else%
    \ifx#1\pgfsyssoftpath@curvetosupportatoken%
      % Ok, round a curveto. 
      \let\next=\pgfprocess@specialroundcurveto%
    \else%
      \ifx#1\pgfsyssoftpath@closepathtoken%
        % Ok, round a closepath (this is tricky...)
        \let\next=\pgfprocess@specialroundclose%
      \fi%
    \fi%
  \fi%
  \next#1{#2}{#3}%
}%

\def\pgfprocess@specialroundcope#1#2#3#4#5#6{%
  \let\next=\pgfprocess@round% do nothing by default
  \let\pgfprocess@continueafterrounding=\pgfprocess@round%
  \ifx#4\pgfsyssoftpath@linetotoken%
    % ok, let's get kicking...
    \pgf@xc=#5%
    \pgf@yc=#6%
    \let\next=\pgfprocess@@specialround%
  \else%
    \ifx#4\pgfsyssoftpath@curvetosupportatoken%  
      \pgf@xc=#5%
      \pgf@yc=#6%
      \let\next=\pgfprocess@@specialround%
    \else%
      \ifx#4\pgfsyssoftpath@closepathtoken%  
        \pgf@xc=#5%
        \pgf@yc=#6%
        \let\next=\pgfprocess@@specialround%
      \else
        \ifx#4\pgfsyssoftpath@specialroundtoken%  
          \let\next=\pgfprocess@@findrightcoordinates%
        \fi%
      \fi%
    \fi%
  \fi%
  \next#1{#2}{#3}#4{#5}{#6}%
}

\def\pgfprocess@@findrightcoordinates#1#2#3#4#5#6#7#8#9{%
  \pgf@xc=#8%
  \pgf@yc=#9%
  \pgfprocess@@specialround#1{#2}{#3}#4{#5}{#6}#7{#8}{#9}%
}

\def\pgfprocess@@specialround#1#2#3{%
  \pgfutil@g@addto@macro\pgfprocess@segment{#1}%
  % calculate start coordinate of the curve
  \pgf@xb=#2%
  \pgf@yb=#3%
  %
  \edef\pgf@marshal%
  {\noexpand\pgfpointlineatdistance{\pgfprocess@savex}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
    {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  \pgf@process{\pgf@marshal}%
  \pgf@xa=\pgf@x% save start point of added curve
  \pgf@ya=\pgf@y%
  \edef\pgfprocess@addition{{\the\pgf@x}{\the\pgf@y}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  %
  % now add curve
  %
  \edef\pgf@marshal%
  {\noexpand\pgfpointlineatdistance{\pgfprocess@savey}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
    {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}}%
  \pgf@process{\pgf@marshal}%
  \pgf@xc=\pgf@x% save end point of added curve
  \pgf@yc=\pgf@y%
  % calculate first support:
  {%
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \advance\pgf@xa by 0.555\pgf@x%
    \advance\pgf@ya by 0.555\pgf@y%
    \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetosupportatoken{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  }%
  % calculate second support:
  {%
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xc%
    \advance\pgf@y by-\pgf@yc%
    \advance\pgf@xc by 0.555\pgf@x%
    \advance\pgf@yc by 0.555\pgf@y%
    \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetosupportbtoken{\the\pgf@xc}{\the\pgf@yc}}%
    \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  }%
  % add end:
  \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetotoken{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  %
  % continue!
  %
  \pgf@xa=#2%
  \pgf@ya=#3%
  \pgfprocess@continueafterrounding%
}

\def\pgfprocess@specialroundcurveto#1#2#3#4#5#6{%
  \pgfutil@g@addto@macro\pgfprocess@segment{#1{#2}{#3}#4{#5}{#6}}% supports
  \pgf@xa=#5%
  \pgf@ya=#6%
  \pgfprocess@specialroundcope}

\def\pgfprocess@specialroundclose{%
  \let\next=\pgfprocess@round%
  \ifx\pgfprocess@moveto\pgfutil@empty%
  \else%
    \ifx\pgfprocess@firstto\pgfutil@empty%
    \else%
      \expandafter\pgfprocess@@specialclosetarget\pgfprocess@firstto%
      \let\pgfprocess@continueafterrounding=\pgfprocess@cleanupafterclose%
      \edef\next{%
        \noexpand\pgfprocess@@specialround%
        \expandafter\expandafter\expandafter\noexpand\expandafter\pgfprocess@@specialclosemoveto\pgfprocess@moveto%
      }%
    \fi%
  \fi%  
  \next%
}

\def\pgfprocess@@specialclosetarget#1#2{%
  \pgf@xc=#1%
  \pgf@yc=#2%
}

\def\pgfprocess@@specialclosemoveto#1#2#3{%
  \pgfsyssoftpath@linetotoken{#2}{#3}%
}


\def\pgfprocess@cleanupafterclose#1#2#3{%
  \edef\pgfprocess@moveto{\noexpand\pgfsyssoftpath@movetotoken{\the\pgf@xc}{\the\pgf@yc}}%
  \edef\pgf@marshal{\noexpand\pgfprocess@round\noexpand\pgfsyssoftpath@closepathtoken{\the\pgf@xc}{\the\pgf@yc}}%
  \pgf@marshal%  
}


% Replace start and end coordinates of a path
%
% #1 = new start coordinate
% #2 = new end coordinate
%
% Description:
%
% This command will replace the first and last coordinates on a path
% by the given coordinates.
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{10}{40}{0}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfsetlinewidth{2pt}
% \pgfusepath{stroke}
% \pgfprocesspathextractpoints{\mypath}
% \pgfprocesspathreplacestartandend{\mypath}
%   {\pgfpointlineatdistance{2pt}{\pgfpointfirstonpath}{\pgfpointsecondonpath}}%
%   {\pgfpointlineatdistance{2pt}{\pgfpointlastonpath}{\pgfpointsecondlastonpath}}%
% \pgfsyssoftpath@setcurrentpath\mypath
% \pgfsetlinewidth{1pt}
% \color{red}
% \pgfusepath{stroke}

\def\pgfprocesspathreplacestartandend#1#2#3{%
  {%
    \let\pgf@newpath=\pgfutil@empty%
    \let\pgf@prepath=\pgfutil@empty%
    \ifx#1\pgfutil@empty%
    \else%
      \pgf@process{#3}%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \pgf@process{#2}%
      \expandafter\pgf@replaceprocessfirst#1\pgf@stop%
    \fi%
    \expandafter\expandafter\expandafter\def
    \expandafter\expandafter\expandafter\pgf@newpath
    \expandafter\expandafter\expandafter{\expandafter\pgf@prepath\pgf@newpath}%
    \global\let#1=\pgf@newpath%
  }%
}

\def\pgf@replaceprocessfirst#1#2#3#4{%
  \def\pgf@temppath{#1{#2}{#3}}%
  \edef\pgf@newpath{\noexpand#1{\the\pgf@x}{\the\pgf@y}}%
  \ifx#4\pgf@stop%
    \let\next=\pgfutil@gobble%
  \else%
    \let\next=\pgf@replaceprocessother%
  \fi%
  \next#4%
}

\def\pgf@replaceprocessother#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    % Arggghh! Must reset everything!
    \expandafter\expandafter\expandafter\def
    \expandafter\expandafter\expandafter\pgf@prepath
    \expandafter\expandafter\expandafter{\expandafter\pgf@prepath\pgf@temppath}%
    % Redo first.
    \let\pgf@next=\pgf@replaceprocessfirst%
  \else%
    \let\pgf@next=\pgf@@replaceprocessother%
  \fi%
  \pgf@next#1%
}
\def\pgf@@replaceprocessother#1#2#3#4{%
  \ifx#4\pgf@stop%
    \edef\pgf@newpathaddition{{\noexpand#1{\the\pgf@xa}{\the\pgf@ya}}}%
    \expandafter\pgfutil@g@addto@macro\expandafter\pgf@newpath\pgf@newpathaddition%
    \let\next=\pgfutil@gobble%
  \else%
    \pgfutil@g@addto@macro\pgf@temppath{#1{#2}{#3}}%
    \pgfutil@g@addto@macro\pgf@newpath{#1{#2}{#3}}%
    \let\next=\pgf@replaceprocessother%
  \fi%
  \next#4%
}  

\endinput


==> pgfcorepathusage.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepathusage.code.tex,v 1.8 2007/03/09 17:49:32 tantau Exp $


% Stroke/fill/clip/etc. the current path. Depending on the options,
% the current path will be stroked/filled/clipped/etc. If no options
% are given, the path is stroked. If multiple options are given, all
% of them are performed (in a sensible order).
%
% #1 = action(s) to be applied to the current path. Valid actions are: 
%      stroke -  strokes the path. If no options are given, this is the
%                default. 
%      draw -    same as stroke.
%      fill -    fills the path.
%      clip -    clip the path.
%      discard - Discards the path. Same effect as having an empty
%                options list.
%
% Example:
%
% % Draws an edge.
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfusepath{stroke}

\define@key{pgfup}{stroke}[]{\def\pgf@up@stroke{stroke}}
\define@key{pgfup}{draw}[]{\def\pgf@up@stroke{stroke}}
\define@key{pgfup}{fill}[]{\def\pgf@up@fill{fill}}
\define@key{pgfup}{clip}[]{\def\pgf@up@clip{clip}}
\define@key{pgfup}{discard}[]{}
\define@key{pgfup}{use as bounding box}[]{\def\pgf@up@bb{\pgf@relevantforpicturesizefalse}}

\def\pgfusepath#1{%
  \let\pgf@up@stroke\pgfutil@empty%
  \let\pgf@up@fill\pgfutil@empty%
  \let\pgf@up@clip\pgfutil@empty%
  \let\pgf@up@discard\pgfutil@empty%
  \let\pgf@up@bb\pgfutil@empty%
  \setkeys{pgfup}{#1}%
  \expandafter\def\expandafter\pgf@up@action\expandafter{\csname pgfsys@\pgf@up@fill\pgf@up@stroke\endcsname}%
  \ifx\pgf@up@stroke\pgfutil@empty%
    \ifx\pgf@up@fill\pgfutil@empty%
      \ifx\pgf@up@clip\pgfutil@empty%
        \let\pgf@up@action=\pgfutil@empty%
        \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
      \else%
        % only clipping  
        \let\pgf@up@action=\pgfsys@discardpath%
      \fi%
    \fi%
  \fi%  
  \pgfprocessround{\pgfsyssoftpath@currentpath}{\pgfsyssoftpath@currentpath}% change the current path
  %
  % Check whether the path is stroked. If so, add half the line width
  % to the bounding box.
  %
  \ifpgf@relevantforpicturesize%
    \ifx\pgf@up@stroke\pgfutil@empty%
    \else%
      \ifdim\pgf@picmaxx=-16000pt\relax%
      \else%
        \pgf@x=\pgf@pathminx\advance\pgf@x by-.5\pgflinewidth%
        \ifdim\pgf@x<\pgf@picminx\global\pgf@picminx\pgf@x\fi%
        \pgf@y=\pgf@pathminy\advance\pgf@y by-.5\pgflinewidth%
        \ifdim\pgf@y<\pgf@picminy\global\pgf@picminy\pgf@y\fi%
        \pgf@x=\pgf@pathmaxx\advance\pgf@x by.5\pgflinewidth%
        \ifdim\pgf@x>\pgf@picmaxx\global\pgf@picmaxx\pgf@x\fi%
        \pgf@y=\pgf@pathmaxy\advance\pgf@y by.5\pgflinewidth%
        \ifdim\pgf@y>\pgf@picmaxy\global\pgf@picmaxy\pgf@y\fi%
      \fi%
    \fi%
  \fi%
  %
  \ifx\pgf@up@clip\pgfutil@empty%
    \ifx\pgf@up@stroke\pgfutil@empty%
      \pgfsyssoftpath@invokecurrentpath%
      \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
      \pgf@up@action%
    \else%
      \pgf@check@for@arrows%
      \ifpgf@drawarrows%
        \pgf@shorten@path@as@needed%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
        \pgf@up@action%
        \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
        \pgf@add@arrows@as@needed%
      \else%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
        \pgf@up@action%
      \fi%
    \fi%
  \else%
    \pgfsyssoftpath@invokecurrentpath%
    \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
    \pgfsys@clipnext%
    \pgf@up@action%
    \pgf@relevantforpicturesizefalse%
  \fi%
  \pgf@up@bb%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgf@resetpathsizes%
  \ignorespaces%
}


% Shorten start/end of paths by a certain amount.
%
% #1 = amount by which paths should be shortened.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{10pt}{0pt}
%
% % The following has the same effect:
% \pgfsetshortenstart{1pt}
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{11pt}{0pt}

\def\pgfsetshortenstart#1{\pgfmathsetlength\pgf@shorten@start@additional{#1}}
\def\pgfsetshortenend#1{\pgfmathsetlength\pgf@shorten@end@additional{#1}}

\newif\ifpgf@drawarrows

\def\pgf@check@for@arrows{%
  \pgf@drawarrowsfalse%
  \ifx\pgf@startarrow\pgfutil@empty\else\pgf@drawarrowstrue\fi%
  \ifx\pgf@endarrow\pgfutil@empty\else\pgf@drawarrowstrue\fi%
  \ifdim\pgf@shorten@end@additional=0pt\relax\else\pgf@drawarrowstrue\fi%
  \ifdim\pgf@shorten@start@additional=0pt\relax\else\pgf@drawarrowstrue\fi%
  \ifpgf@drawarrows%
    \pgfsyssoftpath@getcurrentpath\pgf@arrowpath%
    \ifx\pgf@arrowpath\pgfutil@empty%
      \pgf@drawarrowsfalse%
    \else%
      \pgfprocesscheckclosed{\pgf@arrowpath}{\pgf@drawarrowsfalse}%
    \fi%
  \fi%
}

\newdimen\pgf@shorten@end@additional
\newdimen\pgf@shorten@start@additional

\let\pgf@shorten@end=\pgfutil@empty
\let\pgf@shorten@start=\pgfutil@empty

\def\pgf@shorten@path@as@needed{%
  \pgfprocesspathextractpoints{\pgf@arrowpath}%
  \let\pgf@arrow@next=\pgf@shorten@now%
  \ifx\pgf@shorten@start\pgfutil@empty%
    \ifx\pgf@shorten@end\pgfutil@empty%
      \ifdim\pgf@shorten@end@additional=0pt\relax%
        \ifdim\pgf@shorten@start@additional=0pt\relax%
          \let\pgf@arrow@next=\relax%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgf@arrow@next%
}

\def\pgf@shorten@now{%
  {%
    \pgf@x=0pt%
    \pgf@shorten@start%
    \advance\pgf@x by\pgf@shorten@start@additional%
    \pgf@xc=\pgf@x%
    \pgfpointlineatdistance{\pgf@xc}{\pgfpointfirstonpath}{\pgfpointsecondonpath}%
    \global\pgf@xb=\pgf@x%
    \global\pgf@yb=\pgf@y%
    \pgf@process{\pgfpointsecondonpath}%
    \global\advance\pgf@x by\pgf@xa%
    \global\advance\pgf@y by\pgf@ya%
  }%
  \edef\pgfpointfirstonpath{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \edef\pgfpointsecondonpath{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  {%
    \pgf@x=0pt%
    \pgf@shorten@end%
    \advance\pgf@x by\pgf@shorten@end@additional%
    \pgf@xc=\pgf@x%
    \pgfpointlineatdistance{\pgf@xc}{\pgfpointlastonpath}{\pgfpointsecondlastonpath}%
    \global\pgf@xb=\pgf@x%
    \global\pgf@yb=\pgf@y%
    \pgf@process{\pgfpointsecondlastonpath}%
    \global\advance\pgf@x by\pgf@xa%
    \global\advance\pgf@y by\pgf@ya%
  }%
  \edef\pgfpointlastonpath{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \edef\pgfpointsecondlastonpath{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgfprocesspathreplacestartandend{\pgf@arrowpath}{\pgfpointfirstonpath}{\pgfpointlastonpath}%
  \pgfsyssoftpath@setcurrentpath\pgf@arrowpath%
}

\def\pgf@add@arrows@as@needed{%
  \ifx\pgf@startarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondonpath}{\pgfpointfirstonpath}}
      {\pgf@startarrow}%
  \fi%
  \ifx\pgf@endarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondlastonpath}{\pgfpointlastonpath}}
      {\pgf@endarrow}%
  \fi%      
}

\let\pgf@startarrow=\pgfutil@empty
\let\pgf@endarrow=\pgfutil@empty

\endinput


==> pgfcorepoints.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepoints.code.tex,v 1.9 2007/04/19 11:57:08 tantau Exp $

\newdimen\pgf@picminx
\newdimen\pgf@picmaxx
\newdimen\pgf@picminy
\newdimen\pgf@picmaxy

\newdimen\pgf@pathminx
\newdimen\pgf@pathmaxx
\newdimen\pgf@pathminy
\newdimen\pgf@pathmaxy

\newif\ifpgf@relevantforpicturesize

\def\pgf@process#1{{#1\global\pgf@x=\pgf@x\global\pgf@y=\pgf@y}}




% Return a point
%  
% #1 = x-coordinate of the point 
% #2 = y-coordinate of the point 
%  
% x = #1
% y = #2
%
% Example:
%
% \pgfpathmoveto{\pgfpoint{2pt+3cm}{3cm}}

\def\pgfpoint#1#2{%
  \pgfmathsetlength\pgf@x{#1}%
  \pgfmathsetlength\pgf@y{#2}\ignorespaces}


% Quickly a point
%  
% #1 = x-coordinate of the point (no calculations done)
% #2 = y-coordinate of the point (no calculations done)
%  
% x = #1
% y = #2
%
% Example:
%
% \pgfpathmoveto{\pgfqpoint{2pt}{3cm}}

\def\pgfqpoint#1#2{\pgf@x=#1\pgf@y=#2}



% Return the origin.
%  
% x = 0
% y = 0
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}

\def\pgfpointorigin{\pgf@x=0pt\pgf@y=\pgf@x\ignorespaces}



% Return a transformed point
%  
% #1 = a point
%
% Description:
%
% This command applies pgf's current transformation matrix to the
% given point. Normally, this is done automatically by commands like
% lineto or moveto, but sometimes you may wish to access a transformed
% point yourself. For example, this command is useful for a low level
% coordinate system shift:
%
% Example:
%
% \begin{pgflowleveltransformshiftscope}{\pgfpointtransformed{\pgfpointorigin}}
%   \pgfbox[center,center]{Hi!}
% \end{pgflowleveltransformshiftscope}

\def\pgfpointtransformed#1{%
  \pgf@process{%
    #1%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
  }%
}


% Return the difference vector of two points.
%  
% #1 = start of vector  
% #2 = end of vector  
%  
% x = x-component of difference 
% y = y-component of difference 
%
% Example:
%
% \pgfpathmoveto{\pgfpointdiff{\pgfpointxy{1}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointdiff#1#2{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \advance\pgf@x by-\pgf@xa\relax%
  \advance\pgf@y by-\pgf@ya\relax\ignorespaces}

% Add two vectors. 
%  
% #1 = first vector  
% #2 = second vector  
%  
% x = x-component of addition
% y = y-component of addition
%
% Example:
%
% \pgfpathmoveto{\pgfpointadd{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointadd#1#2{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya}



% Multiply a vector by a factor.
%  
% #1 = factor  
% #2 = vector  
%
% Example:
%
% \pgfpointscale{2}{\pgfpointxy{0}{1}}

\def\pgfpointscale#1#2{%
  \pgf@process{#2}%
  \pgf@x=#1\pgf@x%
  \pgf@y=#1\pgf@y%
}


% The intersection of two lines
%  
% #1 = point on first line
% #2 = another point on first line
% #3 = point on second line
% #4 = another point on second line
%
% Returns the intersection of the two lines. If there is no
% intersection or if the points #1 and #2 or the points #3 and #4 are
% identical, the behaviour is not specified.
%
% Example:
%
% \pgfpointintersectionoflines{\pgfpointxy{0}{1}}{\pgfpointxy{1}{0}}{\pgfpointxy{2}{2}}{\pgfpointxy{3}{4}}

\def\pgfpointintersectionoflines#1#2#3#4{%
  {
    % 
    % Compute orthogonal vector to #1--#2
    % 
    \pgf@process{#2}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#1}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgf@ya=-\pgf@ya%
    % Normalise a bit
    \c@pgf@counta=\pgf@xa%
    \ifnum\c@pgf@counta<0\relax%
      \c@pgf@counta=-\c@pgf@counta\relax%
    \fi%
    \c@pgf@countb=\pgf@ya%
    \ifnum\c@pgf@countb<0\relax%
      \c@pgf@countb=-\c@pgf@countb\relax%
    \fi%
    \advance\c@pgf@counta by\c@pgf@countb\relax%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta>0\relax%
      \divide\pgf@xa by\c@pgf@counta\relax%
      \divide\pgf@ya by\c@pgf@counta\relax%
    \fi%
    %
    % Compute projection
    %
    \pgf@xc=\pgf@sys@tonumber{\pgf@ya}\pgf@x%
    \advance\pgf@xc by\pgf@sys@tonumber{\pgf@xa}\pgf@y%
    % 
    % The orthogonal vector is (\pgf@ya,\pgf@xa)
    % 
    % 
    % Compute orthogonal vector to #3--#4
    % 
    \pgf@process{#4}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#3}%
    \advance\pgf@xb by-\pgf@x%
    \advance\pgf@yb by-\pgf@y%
    \pgf@yb=-\pgf@yb%
    % Normalise a bit
    \c@pgf@counta=\pgf@xb%
    \ifnum\c@pgf@counta<0\relax%
      \c@pgf@counta=-\c@pgf@counta\relax%
    \fi%
    \c@pgf@countb=\pgf@yb%
    \ifnum\c@pgf@countb<0\relax%
      \c@pgf@countb=-\c@pgf@countb\relax%
    \fi%
    \advance\c@pgf@counta by\c@pgf@countb\relax%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta>0\relax%
      \divide\pgf@xb by\c@pgf@counta\relax%
      \divide\pgf@yb by\c@pgf@counta\relax%
    \fi%
    %
    % Compute projection
    %
    \pgf@yc=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
    \advance\pgf@yc by\pgf@sys@tonumber{\pgf@xb}\pgf@y%
    % 
    % The orthogonal vector is (\pgf@yb,\pgf@xb)
    % 
    % Setup transformation matrx (this is just to use the matrix
    % inversion)
    % 
    \pgfsettransform{{\pgf@sys@tonumber\pgf@ya}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@xb}{0pt}{0pt}}%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{\pgfpoint{\pgf@xc}{\pgf@yc}}}%
  }%
}


% Returns point on a line from #2 to #3 at time #1.
%  
% #1 = a time, where 0 is the start and 1 is the end
% #2 = start point
% #3 = end point 
%  
% x = x-component of #1*start + (1-#1)*end
% y = y-component of #1*start + (1-#1)*end 
%
% Example:
%
% % Middle of (1,1) and (2,3)
% \pgfpathmoveto{\pgfpointlineattime{0.5}{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointlineattime#1#2#3{%
  \pgf@process{#3}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \advance\pgf@xa by-\pgf@x\relax%
  \advance\pgf@ya by-\pgf@y\relax%
  \advance\pgf@x by #1\pgf@xa\relax%
  \advance\pgf@y by #1\pgf@ya\relax%  
  \ignorespaces}


% Move point #2 #1 many units in the direction of #3.
%  
% #1 = a distance
% #2 = start point
% #3 = end point 
%  
% x = x-component of start + #1*(normalise(end-start))
% y = y-component of start + #1*(normalise(end-start))
% xa = #1*(normalise(end-start))
% ya = #1*(normalise(end-start))
%
% Example:
%
%
% \pgfpathmoveto{\pgfpointlineatdistance{2pt}{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}
% \pgfpathlineto{\pgfpointlineatdistance{3pt}{\pgfpointxy{2}{3}}{\pgfpointxy{0}{1}}}

\def\pgfpointlineatdistance#1#2#3{%
  \pgf@process{#2}%
  \pgf@xb=\pgf@x\relax% xb/yb = start point
  \pgf@yb=\pgf@y\relax%
  \pgf@process{#3}%
  \advance\pgf@x by-\pgf@xb\relax%
  \advance\pgf@y by-\pgf@yb\relax%
  \pgf@process{\pgfpointnormalised{}}% x/y = normalised vector
  \pgfmathsetlength\pgf@xa{#1}%
  \pgf@ya=\pgf@xa\relax%
  \pgf@xa=\pgf@sys@tonumber{\pgf@x}\pgf@xa%
  \pgf@ya=\pgf@sys@tonumber{\pgf@y}\pgf@ya%
  \pgf@x=\pgf@xb\relax%
  \pgf@y=\pgf@yb\relax%
  \advance\pgf@x by\pgf@xa\relax%
  \advance\pgf@y by\pgf@ya\relax%
  \ignorespaces}


% Returns point on a curve from #2 to #5 with controls #3 and #4 at time #1.
%  
% #1 = a time
% #2 = start point
% #3 = first control point
% #4 = second control point
% #5 = end point 
%  
% x = x-component of place on the curve at time t
% y = y-component of place on the curve at time t
%
% Additionally, (\pgf@xa,\pgf@ya) and (\pgf@xb,\pgf@yb) will be on a
% tangent to the point on the curve (this can be useful for computing
% a label rotation).
%
% Example:
%
% % Middle of (1,1) and (2,3)
% \pgfpathmoveto{\pgfpointcurveattime{0.5}{\pgfpointxy{0}{1}}{\pgfpointxy{1}{1}}{\pgfpointxy{1}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointcurveattime#1#2#3#4#5{%
  \pgfmathparse{#1}%
  \let\pgf@time@s=\pgfmathresult%
  \pgf@x=\pgfmathresult pt%
  \pgf@x=-\pgf@x%
  \advance\pgf@x by 1pt%
  \edef\pgf@time@t{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@process{#5}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgf@process{#4}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#3}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  % First iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  \pgf@xb=\pgf@time@t\pgf@xb\advance\pgf@xb by\pgf@time@s\pgf@xc%
  \pgf@yb=\pgf@time@t\pgf@yb\advance\pgf@yb by\pgf@time@s\pgf@yc%
  % Second iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  % Save x/y
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  % Third iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
}






% Internal registers
\newdimen\pgf@xx
\newdimen\pgf@xy
\newdimen\pgf@yx
\newdimen\pgf@yy
\newdimen\pgf@zx
\newdimen\pgf@zy



% A polar coordinate
%
% #1 = a degree
% #2 = a radius -- either a dimension or two dimensions separated by 
%      " and ". 
%
% x = (first dimension in #2) * cos(#1)
% y = (second dimension in #2) * sin(#2)
% 
% Example:
%
% \pgfpathmoveto{\pgfpointpolar{30}{1cm}}
% \pgfpathlineto{\pgfpointpolar{30}{1cm and 2cm}}

\def\pgfpointpolar#1#2{%
  \pgfutil@in@{and }{#2}%
  \ifpgfutil@in@%
    \pgf@polar@#2\@@%
  \else%
    \pgf@polar@#2 and #2\@@%
  \fi%  
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@x=\pgfmathresult\pgf@x%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@y=\pgfmathresult\pgf@y%
}

\def\pgf@polar@#1and #2\@@{%
  \pgfmathsetlength{\pgf@y}{#2}%
  \pgfmathsetlength{\pgf@x}{#1}%  
}

% Quick version of the polar coordinate method

\def\pgfqpointpolar#1#2{%
  \pgf@x=#2%
  \pgf@y=\pgf@x%
  \pgfmathcos@{#1}%
  \pgf@x=\pgfmathresult\pgf@x%
  \pgfmathsin@{#1}%
  \pgf@y=\pgfmathresult\pgf@y\relax%
}




% A polar coordinate in the xy plane.
%
% #1 = a degree
% #2 = a radius given as a number or two radi
%
% result = (first dim in #2) * x-vector * cos(#1) +
%          (second dim in #2) * y-vector * sin(#1)
% 
% Example:
%
% \pgfpathmoveto{\pgfpointpolarxy{30}{2}}

\def\pgfpointpolarxy#1#2{%
  \pgfutil@in@{and }{#2}%
  \ifpgfutil@in@%
    \pgf@polarxy@#2\@@%
  \else%
    \pgf@polarxy@#2and #2\@@%
  \fi%  
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@xa=\pgfmathresult\pgf@xa%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@ya=\pgfmathresult\pgf@ya%
  \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@xx%
  \advance\pgf@x by \pgf@sys@tonumber{\pgf@ya}\pgf@yx%
  \pgf@y=\pgf@sys@tonumber{\pgf@xa}\pgf@xy%
  \advance\pgf@y by \pgf@sys@tonumber{\pgf@ya}\pgf@yy}

\def\pgf@polarxy@#1and #2\@@{%
  \pgfmathsetlength{\pgf@xa}{#1}%
  \pgfmathsetlength{\pgf@ya}{#2}%
}



% A cylindrical coordinate.
%
% #1 = a degree
% #2 = a radius given as a number
% #3 = a height given as a number
%
% result = #2*(x-vector * cos(#1) + y-vector * sin(#1)) + #3*z-vector
% 
% Example:
%
% \pgfpathmoveto{\pgfpointcylindrical{30}{2}{1}}

\def\pgfpointcylindrical#1#2#3{%
  \pgfpointpolarxy{#1}{#2}%
  \pgfmathparse{#3}%
  \advance\pgf@x by \pgfmathresult\pgf@zx%
  \advance\pgf@y by \pgfmathresult\pgf@zy}


% A spherical coordinate.
%
% #1 = a longitude
% #2 = a latitude
% #3 = a radius
%
% result = #3*(cos(#2)*(x-vector * cos(#1) + y-vector * sin(#1)) + sin(#2)*z-vector)
% 
% Example:
%
% \pgfpathmoveto{\pgfpointspherical{30}{30}{2}}

\def\pgfpointspherical#1#2#3{%
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@xb=\pgfmathresult\pgf@xx%
  \pgf@yb=\pgfmathresult\pgf@xy%
  \pgfmathcos@{\pgfpoint@angle}%
  \advance\pgf@xb by \pgfmathresult\pgf@yx%
  \advance\pgf@yb by \pgfmathresult\pgf@yy%
  %
  \pgfmathparse{#2}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@xc=\pgfmathresult\pgf@xb%
  \pgf@yc=\pgfmathresult\pgf@yb%
  \pgfmathsin@{\pgfpoint@angle}%
  \advance\pgf@xc by \pgfmathresult\pgf@zx%
  \advance\pgf@yc by \pgfmathresult\pgf@zy%
  \pgfmathparse{#3}%
  \pgf@x=\pgfmathresult\pgf@xc%
  \pgf@y=\pgfmathresult\pgf@yc\relax%
}


% Store the vector #1 * x-vec + #2 * y-vec
%
% #1 = a factor for the x-vector
% #2 = a factor fot the y-vector
%
% x = x-component of result vector
% y = y-component of result vector
%
% Description:
% 
% This command can be used to create a new coordinate system
% without using the rotate/translate/scale commands. This
% may be useful, if you do not want arrows and line width to
% be scaled/transformed together with the coordinate system.
% 
% Example:
%
% % Create a slanted rectangle
%
% \pgfsetxvec{\pgfpoint{1cm}{1cm}}
% \pgfsetyvec{\pgfpoint{0cm}{1cm}}
% 
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfpathlineto{\pgfpointxy{1}{0}}
% \pgfpathlineto{\pgfpointxy{1}{1}}
% \pgfpathlineto{\pgfpointxy{0}{1}}
% \pgfclosestroke

\def\pgfpointxy#1#2{%
  \pgfmathparse{#1}%
  \let\pgftemp@x=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgftemp@y=\pgfmathresult%
  \pgf@x=\pgftemp@x\pgf@xx%
  \advance\pgf@x by \pgftemp@y\pgf@yx%
  \pgf@y=\pgftemp@x\pgf@xy%
  \advance\pgf@y by \pgftemp@y\pgf@yy}


% Store the vector #1 * x-vec + #2 * y-vec + #3 * z-vec
%
% #1 = a factor for the x-vector
% #2 = a factor fot the y-vector
% #3 = a factor fot the z-vector
%
% x = x-component of result vector
% y = y-component of result vector
%
%
% Description:
% 
% This command allows you to use a 3d coordinate system.
% 
%
% Example:
%
% % Draw a cubus
% 
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{0}{0}{1}}
% \pgfline{\pgfpointxyz{0}{1}{0}}{\pgfpointxyz{0}{1}{1}}
% \pgfline{\pgfpointxyz{1}{0}{0}}{\pgfpointxyz{1}{0}{1}}
% \pgfline{\pgfpointxyz{1}{1}{0}}{\pgfpointxyz{1}{1}{1}}
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{0}{1}{0}}
% \pgfline{\pgfpointxyz{0}{0}{1}}{\pgfpointxyz{0}{1}{1}}
% \pgfline{\pgfpointxyz{1}{0}{0}}{\pgfpointxyz{1}{1}{0}}
% \pgfline{\pgfpointxyz{1}{0}{1}}{\pgfpointxyz{1}{1}{1}}
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{1}{0}{0}}
% \pgfline{\pgfpointxyz{0}{0}{1}}{\pgfpointxyz{1}{0}{1}}
% \pgfline{\pgfpointxyz{0}{1}{0}}{\pgfpointxyz{1}{1}{0}}
% \pgfline{\pgfpointxyz{0}{1}{1}}{\pgfpointxyz{1}{1}{1}}

\def\pgfpointxyz#1#2#3{%
  \pgfmathparse{#1}%
  \let\pgftemp@x=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgftemp@y=\pgfmathresult%
  \pgfmathparse{#3}%
  \let\pgftemp@z=\pgfmathresult%
  \pgf@x=\pgftemp@x\pgf@xx%
  \advance\pgf@x by \pgftemp@y\pgf@yx%
  \advance\pgf@x by \pgftemp@z\pgf@zx%
  \pgf@y=\pgftemp@x\pgf@xy%
  \advance\pgf@y by \pgftemp@y\pgf@yy%
  \advance\pgf@y by \pgftemp@z\pgf@zy}




% Set the x-vector
%
% #1 = a point the is the new x-vector
%
% Example:
%
% \pgfsetxvec{\pgfpoint{1cm}{0cm}}

\def\pgfsetxvec#1{%
  \pgf@process{#1}%
  \pgf@xx=\pgf@x%
  \pgf@xy=\pgf@y%
  \ignorespaces}


% Set the y-vector
%
% #1 = a point the is the new y-vector
%
% Example:
%
% \pgfsetyvec{\pgfpoint{0cm}{1cm}}

\def\pgfsetyvec#1{%
  \pgf@process{#1}%
  \pgf@yx=\pgf@x%
  \pgf@yy=\pgf@y%
  \ignorespaces}


% Set the z-vector
%
% #1 = a point the is the new z-vector
%
% Example:
%
% \pgfsetzvec{\pgfpoint{-0.385cm}{-0.385cm}}

\def\pgfsetzvec#1{%
  \pgf@process{#1}%
  \pgf@zx=\pgf@x%
  \pgf@zy=\pgf@y%
  \ignorespaces}



% Default values
\pgfsetxvec{\pgfpoint{1cm}{0cm}}
\pgfsetyvec{\pgfpoint{0cm}{1cm}}
\pgfsetzvec{\pgfpoint{-0.385cm}{-0.385cm}}




% Normalise a point.
%
% #1 = point with coordinates (a,b)
%
% x  = a/\sqrt(a*a+b*b)
% y  = b/\sqrt(a*a+b*b)
%
% Example:
%
% \pgfpointnormalised{\pgfpointxy{2}{1}}

\def\pgfpointnormalised#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifdim\pgf@x<0pt\relax% move into first quadrant
    \pgf@x=-\pgf@x%
  \fi%
  \ifdim\pgf@y<0pt\relax%
    \pgf@y=-\pgf@y%
  \fi%
  \ifdim\pgf@x>\pgf@y% x > y
    % make point small
    \c@pgf@counta=\pgf@x%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta=0\relax%
      \c@pgf@counta=1\relax%
    \fi%
    \divide\pgf@x by\c@pgf@counta%
    \divide\pgf@y by\c@pgf@counta%
    \divide\pgf@xa by\c@pgf@counta%
    \divide\pgf@ya by\c@pgf@counta%
    % ok.
    \pgf@x=.125\pgf@x%
    \pgf@y=.125\pgf@y%
    \c@pgf@counta=\pgf@x%
    \c@pgf@countb=\pgf@y%
    \multiply\c@pgf@countb by 100%
    \ifnum\c@pgf@counta<64\relax%
      \pgf@x=1pt\relax%
      \pgf@y=0pt\relax%
    \else%
      \divide\c@pgf@countb by \c@pgf@counta%
      \pgf@x=\csname pgf@cosfrac\the\c@pgf@countb\endcsname pt%
      \pgf@xc=8192pt%
      \divide\pgf@xc by\c@pgf@counta%
      \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@ya%
      \pgf@y=\pgf@sys@tonumber{\pgf@x}\pgf@y%
    \fi%
    \ifdim\pgf@xa<0pt%
      \pgf@x=-\pgf@x%
    \fi%
  \else% x <= y
    % make point small
    \c@pgf@counta=\pgf@y%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta=0\relax%
      \c@pgf@counta=1\relax%
    \fi%
    \divide\pgf@x by\c@pgf@counta%
    \divide\pgf@y by\c@pgf@counta%
    \divide\pgf@xa by\c@pgf@counta%
    \divide\pgf@ya by\c@pgf@counta%
    % ok.
    \pgf@x=.125\pgf@x%
    \pgf@y=.125\pgf@y%
    \c@pgf@counta=\pgf@y%
    \c@pgf@countb=\pgf@x%
    \multiply\c@pgf@countb by 100%
    \ifnum\c@pgf@counta<64\relax%
      \pgf@y=1pt\relax%
      \pgf@x=0pt\relax%
    \else%
      \divide\c@pgf@countb by \c@pgf@counta%
      \pgf@y=\csname pgf@cosfrac\the\c@pgf@countb\endcsname pt%
      \pgf@xc=8192pt%
      \divide\pgf@xc by\c@pgf@counta%
      \pgf@x=\pgf@sys@tonumber{\pgf@xc}\pgf@xa%
      \pgf@x=\pgf@sys@tonumber{\pgf@y}\pgf@x%
    \fi%
    \ifdim\pgf@ya<0pt%
      \pgf@y=-\pgf@y%
    \fi%
  \fi\ignorespaces%
}





% A point on a rectangle in a certain direction.
%
% #1 = a point pointing in some direction (length should be about 1pt,
%      but need not be exact)
% #2 = upper right corner of a rectangle centered at the origin
%
% Returns the intersection of a line starting at the origin going in
% the given direction and the rectangle's border.
%
% Example:
%
% \pgfpointborderrectangle{\pgfpointnormalised{\pgfpointxy{2}{1}}
%   {\pgfpoint{1cm}{2cm}}

\def\pgfpointborderrectangle#1#2{%
  \pgf@process{#2}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#1}%
  % Ok, let's find out about the direction:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifnum\pgf@xa<0\relax% move into first quadrant
    \pgf@x=-\pgf@x%
  \fi%
  \ifnum\pgf@ya<0\relax%
    \pgf@y=-\pgf@y%
  \fi%
  \pgf@xc=.125\pgf@x%
  \pgf@yc=.125\pgf@y%
  \c@pgf@counta=\pgf@xc%
  \c@pgf@countb=\pgf@yc%
  \ifnum\c@pgf@countb<\c@pgf@counta%
    \ifnum\c@pgf@counta<255\relax%
      \pgf@y=\pgf@yb\relax%
      \pgf@x=0pt\relax%
    \else%
      \pgf@xc=8192pt%
      \divide\pgf@xc by\c@pgf@counta% \pgf@xc = 1/\pgf@x
      \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
      \pgf@y=\pgf@sys@tonumber{\pgf@xb}\pgf@y%
      \ifnum\pgf@y<\pgf@yb%
        \pgf@x=\pgf@xb%
      \else% rats, calculate intersection on upper side
        \ifnum\c@pgf@countb<255\relax%
          \pgf@x=\pgf@xb\relax%
          \pgf@y=0pt\relax%
        \else%
          \pgf@yc=8192pt%
          \divide\pgf@yc by\c@pgf@countb% \pgf@xc = 1/\pgf@x
          \pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
          \pgf@x=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
          \pgf@y=\pgf@yb%
        \fi%
      \fi%  
    \fi%
  \else%
    \ifnum\c@pgf@countb<255\relax%
      \pgf@x=\pgf@xb\relax%
      \pgf@y=0pt\relax%
    \else%
      \pgf@yc=8192pt%
      \divide\pgf@yc by\c@pgf@countb% \pgf@xc = 1/\pgf@x
      \pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
      \pgf@x=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
      \ifnum\pgf@x<\pgf@xb%
        \pgf@y=\pgf@yb%
      \else%
        \ifnum\c@pgf@counta<255\relax%
          \pgf@y=\pgf@yb\relax%
          \pgf@x=0pt\relax%
        \else%
          \pgf@xc=8192pt%
          \divide\pgf@xc by\c@pgf@counta% \pgf@xc = 1/\pgf@x
          \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
          \pgf@y=\pgf@sys@tonumber{\pgf@xb}\pgf@y%
          \pgf@x=\pgf@xb%
        \fi%
      \fi%  
    \fi%
  \fi%  
  \ifnum\pgf@xa<0\relax\pgf@x=-\pgf@x\fi%
  \ifnum\pgf@ya<0\relax\pgf@y=-\pgf@y\fi%    
}




% An approximation to a point on an ellipse in a certain
% direction. Will be exact only if the ellipse is a circle. 
%
% #1 = a point pointing in some direction
% #2 = upper right corner of a bounding box for the ellipse
%
% Returns the intersection of a line starting at the origin going in
% the given direction and the ellipses border.
%
% Example:
%
% \pgfpointborderellipse{\pgfpointnormalised{\pgfpointxy{2}{1}}
%   {\pgfpoint{1cm}{2cm}}

\def\pgfpointborderellipse#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifdim\pgf@xa=\pgf@ya% circle. that's easy!
    \pgf@process{\pgfpointnormalised{#1}}%
    \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
    \pgf@y=\pgf@sys@tonumber{\pgf@xa}\pgf@y%
  \else%
    \ifdim\pgf@xa<\pgf@ya%
      % Ok, first, let's compute x/y:
      \c@pgf@countb=\pgf@ya%
      \divide\c@pgf@countb by65536\relax%
      \divide\pgf@x by\c@pgf@countb%
      \divide\pgf@y by\c@pgf@countb%
      \pgf@xc=\pgf@x%
      \pgf@yc=8192pt%
      \pgf@y=.125\pgf@y%
      \c@pgf@countb=\pgf@y%
      \divide\pgf@yc by\c@pgf@countb%
      \pgf@process{#1}%
      \pgf@y=\pgf@sys@tonumber{\pgf@yc}\pgf@y%
      \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
      \pgf@process{\pgfpointnormalised{}}%
      \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \else%
      % Ok, now let's compute y/x:
      \c@pgf@countb=\pgf@xa%
      \divide\c@pgf@countb by65536\relax%
      \divide\pgf@x by\c@pgf@countb%
      \divide\pgf@y by\c@pgf@countb%
      \pgf@yc=\pgf@y%
      \pgf@xc=8192pt%
      \pgf@x=.125\pgf@x%
      \c@pgf@countb=\pgf@x%
      \divide\pgf@xc by\c@pgf@countb%
      \pgf@process{#1}%
      \pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
      \pgf@x=\pgf@sys@tonumber{\pgf@xc}\pgf@x%
      \pgf@process{\pgfpointnormalised{}}%
      \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \fi%  
  \fi%
}





% Extract the x-coordinate of a point to a dimensions
%  
% #1 = a TeX dimension
% #2 = a point
%
% Example:
%
% \newdimen\mydim
% \pgfextractx{\mydim}{\pgfpoint{2cm}{4pt}}
% % \mydim is now 2cm

\def\pgfextractx#1#2{%
  \pgf@process{#2}%
  #1=\pgf@x\relax}


% Extract the y-coordinate of a point to a dimensions
%  
% #1 = a TeX dimension
% #2 = a point
%
% Example:
%
% \newdimen\mydim
% \pgfextracty{\mydim}{\pgfpoint{2cm}{4pt}}
% % \mydim is now 4pt

\def\pgfextracty#1#2{%
  \pgf@process{#2}%
  #1=\pgf@y\relax}



\def\pgf@def#1#2#3{\expandafter\def\csname pgf@#1#2\endcsname{#3}}
\pgf@def{cosfrac}{0}{1}
\pgf@def{cosfrac}{1}{0.99995}    \pgf@def{cosfrac}{2}{0.9998}
\pgf@def{cosfrac}{3}{0.99955}    \pgf@def{cosfrac}{4}{0.999201}
\pgf@def{cosfrac}{5}{0.998752}   \pgf@def{cosfrac}{6}{0.998205}
\pgf@def{cosfrac}{7}{0.997559}   \pgf@def{cosfrac}{8}{0.996815}
\pgf@def{cosfrac}{9}{0.995974}   \pgf@def{cosfrac}{10}{0.995037}
\pgf@def{cosfrac}{11}{0.994004}  \pgf@def{cosfrac}{12}{0.992877}
\pgf@def{cosfrac}{13}{0.991656}  \pgf@def{cosfrac}{14}{0.990342}
\pgf@def{cosfrac}{15}{0.988936}  \pgf@def{cosfrac}{16}{0.987441}
\pgf@def{cosfrac}{17}{0.985856}  \pgf@def{cosfrac}{18}{0.984183}
\pgf@def{cosfrac}{19}{0.982424}  \pgf@def{cosfrac}{20}{0.980581}
\pgf@def{cosfrac}{21}{0.978653}  \pgf@def{cosfrac}{22}{0.976644}
\pgf@def{cosfrac}{23}{0.974555}  \pgf@def{cosfrac}{24}{0.972387}
\pgf@def{cosfrac}{25}{0.970143}  \pgf@def{cosfrac}{26}{0.967823}
\pgf@def{cosfrac}{27}{0.965429}  \pgf@def{cosfrac}{28}{0.962964}
\pgf@def{cosfrac}{29}{0.960429}  \pgf@def{cosfrac}{30}{0.957826}
\pgf@def{cosfrac}{31}{0.955157}  \pgf@def{cosfrac}{32}{0.952424}
\pgf@def{cosfrac}{33}{0.949629}  \pgf@def{cosfrac}{34}{0.946773}
\pgf@def{cosfrac}{35}{0.943858}  \pgf@def{cosfrac}{36}{0.940887}
\pgf@def{cosfrac}{37}{0.937862}  \pgf@def{cosfrac}{38}{0.934784}
\pgf@def{cosfrac}{39}{0.931655}  \pgf@def{cosfrac}{40}{0.928477}
\pgf@def{cosfrac}{41}{0.925252}  \pgf@def{cosfrac}{42}{0.921982}
\pgf@def{cosfrac}{43}{0.918669}  \pgf@def{cosfrac}{44}{0.915315}
\pgf@def{cosfrac}{45}{0.911922}  \pgf@def{cosfrac}{46}{0.90849}
\pgf@def{cosfrac}{47}{0.905024}  \pgf@def{cosfrac}{48}{0.901523}
\pgf@def{cosfrac}{49}{0.89799}   \pgf@def{cosfrac}{50}{0.894427}
\pgf@def{cosfrac}{51}{0.890835}  \pgf@def{cosfrac}{52}{0.887217}
\pgf@def{cosfrac}{53}{0.883573}  \pgf@def{cosfrac}{54}{0.879905}
\pgf@def{cosfrac}{55}{0.876216}  \pgf@def{cosfrac}{56}{0.872506}
\pgf@def{cosfrac}{57}{0.868777}  \pgf@def{cosfrac}{58}{0.865031}
\pgf@def{cosfrac}{59}{0.861269}  \pgf@def{cosfrac}{60}{0.857493}
\pgf@def{cosfrac}{61}{0.853704}  \pgf@def{cosfrac}{62}{0.849903}
\pgf@def{cosfrac}{63}{0.846092}  \pgf@def{cosfrac}{64}{0.842271}
\pgf@def{cosfrac}{65}{0.838444}  \pgf@def{cosfrac}{66}{0.834609}
\pgf@def{cosfrac}{67}{0.83077}   \pgf@def{cosfrac}{68}{0.826927}
\pgf@def{cosfrac}{69}{0.82308}   \pgf@def{cosfrac}{70}{0.819232}
\pgf@def{cosfrac}{71}{0.815383}  \pgf@def{cosfrac}{72}{0.811534}
\pgf@def{cosfrac}{73}{0.807687}  \pgf@def{cosfrac}{74}{0.803842}
\pgf@def{cosfrac}{75}{0.8}       \pgf@def{cosfrac}{76}{0.796162}
\pgf@def{cosfrac}{77}{0.792329}  \pgf@def{cosfrac}{78}{0.788502}
\pgf@def{cosfrac}{79}{0.784682}  \pgf@def{cosfrac}{80}{0.780869}
\pgf@def{cosfrac}{81}{0.777064}  \pgf@def{cosfrac}{82}{0.773268}
\pgf@def{cosfrac}{83}{0.769481}  \pgf@def{cosfrac}{84}{0.765705}
\pgf@def{cosfrac}{85}{0.761939}  \pgf@def{cosfrac}{86}{0.758185}
\pgf@def{cosfrac}{87}{0.754443}  \pgf@def{cosfrac}{88}{0.750714}
\pgf@def{cosfrac}{89}{0.746997}  \pgf@def{cosfrac}{90}{0.743294}
\pgf@def{cosfrac}{91}{0.739605}  \pgf@def{cosfrac}{92}{0.735931}
\pgf@def{cosfrac}{93}{0.732272}  \pgf@def{cosfrac}{94}{0.728628}
\pgf@def{cosfrac}{95}{0.724999}  \pgf@def{cosfrac}{96}{0.721387}
\pgf@def{cosfrac}{97}{0.717792}  \pgf@def{cosfrac}{98}{0.714213}
\pgf@def{cosfrac}{99}{0.710651}  \pgf@def{cosfrac}{100}{0.707107}



\endinput


==> pgfcorequick.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorequick.code.tex,v 1.2 2006/10/11 15:22:25 tantau Exp $

% Quick version of basic drawing commands. Most high-level commands
% are not available if these commands are used.

% Move current point to (#1,#2).
%
% #1 = x dimension of new current point
% #2 = y dimension of new current point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqmoveto#1#2{\pgfsyssoftpath@moveto{#1}{#2}}


% Append a line to (#1,#2) to the current path.
%
% #1 = x dimension of target
% #2 = y dimension of target
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqlineto#1#2{\pgfsyssoftpath@lineto{#1}{#2}}


% Append a bezier spline to the current path.
%
% #1 = x dimension of first support point
% #2 = y dimension of first support point
% #3 = x dimension of second support point
% #4 = y dimension of second support point
% #5 = x dimension of target point
% #6 = y dimension of target point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqcurveto#1#2#3#4#5#6{\pgfsyssoftpath@curveto{#1}{#2}{#3}{#4}{#5}{#6}}




% Append a circle of the given radius around the origin.
%
% #1 = radius
% 
% Example:
%
% \pgfpathqcircle{10pt}
% is quicker than
% \pgfpathcircle{\pgforigin}{10pt}

\def\pgfpathqcircle#1{%
  {%
    \pgf@x=#1%
    \pgf@y=0.555\pgf@x%
    \pgfsyssoftpath@moveto{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{\the\pgf@x}{\the\pgf@y}{\the\pgf@y}{\the\pgf@x}{0pt}{\the\pgf@x}%
    \pgfsyssoftpath@curveto{-\the\pgf@y}{\the\pgf@x}{-\the\pgf@x}{\the\pgf@y}{-\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{-\the\pgf@x}{-\the\pgf@y}{-\the\pgf@y}{-\the\pgf@x}{0pt}{-\the\pgf@x}%
    \pgfsyssoftpath@curveto{\the\pgf@y}{-\the\pgf@x}{\the\pgf@x}{-\the\pgf@y}{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@closepath%
  }%
}



% Stroke current path. No hooks called.
% 
% Example:
%
% \pgfpathqmoveto{0cm}{0cm}
% \pgfpathqlineto{1cm}{1cm}
% \pgfpathqcurveto{2cm}{1cm}{2cm}{2cm}{3cm}{2cm}
% \pgfqstroke

\def\pgfusepathqstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@stroke%
  \pgf@resetpathsizes%
}


% Quickly fill current path.

\def\pgfusepathqfill{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fill%
  \pgf@resetpathsizes%
}


% Quickly fill and stroke current path.

\def\pgfusepathqfillstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fillstroke%
  \pgf@resetpathsizes%
}

% Quickly clip current path.

\def\pgfusepathqclip{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@clipnext%
  \pgfsys@discardpath%
  \pgf@resetpathsizes%
}


\endinput


==> pgfcorescopes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorescopes.code.tex,v 1.24 2007/06/07 07:41:10 tantau Exp $

% Globals

\newbox\pgfpic
\newbox\pgf@hbox

\newbox\pgf@layerbox@main

\newcount\pgf@picture@serial@count



% This if decides whether the position of pictures on the page is
% protocolled or not. Normally,
% this is switched off as it works only with certain drivers and it
% causes external files to be written. When switched on, the position
% of pgfpictures are protocolled and can be referenced using
% \pgfsys@getposition{XXX} where XXX is the value of \pgfpictureid
% inside the picture.
\newif\ifpgfrememberpicturepositiononpage



% Library files inclusion


% Include a library file.
%
% #1 = List of names of library file.
%  
% Description:
%
% This command includes a list of library files. For each file X in the
% list, the file pgflibraryX.code.tex is included, provided this has
% not been done earlier. 
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgflibrary{arrows}
% \usepgflibrary[patterns,snakes]

\def\usepgflibrary{\pgfutil@ifnextchar[{\use@pgflibrary}{\use@@pgflibrary}}%}
\def\use@pgflibrary[#1]{\use@@pgflibrary{#1}}
\def\use@@pgflibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname pgf@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \input pgflibrary\pgf@temp.code.tex
      \catcode`\@=\csname pgf@library@#1@atcode\endcsname
      \catcode`\|=\csname pgf@library@#1@barcode\endcsname
    \fi%
  }%
}



% Scopes


% Pgf scope environment. All changes of the graphic state are local to
% the scope.
%  
% Example:
%
% \begin{pgfscope}
%    \pgfsetlinewidth{3pt}
%    \pgfline{\pgfxy(0,0)}{\pgfxy(3,3)}
% \end{pgfscope}

\def\pgfscope{%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgfsys@beginscope%
    \pgf@resetpathsizes%
    \edef\pgfscope@linewidth{\the\pgflinewidth}%
    \begingroup}
\def\endpgfscope{%
    \endgroup%
    \global\pgflinewidth=\pgfscope@linewidth%
  \pgfsys@endscope}




% Quickly insert a box can contain normal TeX text at the origin.
% 
% #1 = box of width/height and depth 0pt
% 
% Example:
%
% \pgfqbox{\mybox}

\def\pgfqbox#1{%
  \pgfsys@hbox#1%
} 


% Insert a box that can contain normal TeX text at the origin, but
% with the current coordinate transformation matrix synced with the
% low-level transformation matrix.
% 
% #1 = box of width/height and depth 0pt
%
% In essence, this command does the same as if you first said
% \pgflowlevelsynccm and then \pgfqbox. However, pgf will use a
% ``TeX-translation'' for the translation part of the transformation
% cm. This will ensure that hyperlinks ``survive'' at least
% translations. 
% 
% Example:
%
% \pgfqboxsynced{\mybox}

\def\pgfqboxsynced#1{%
  \pgfsys@hboxsynced#1%
}


% Puts some text in a box and inserts it with the current
% transformations applied.
% 
% #1 = List of optional positioning. Possible values are ``left'', ``right'',
%      ``top'', ``bottom'' and ``base''.
% #2 = TeX text. May contain verbatims.
% 
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{0cm}}
% \pgftext{Hello World!}

\def\pgftext{\pgfutil@ifnextchar[\pgf@text{\pgf@text[]}}%
\def\pgf@text[#1]{%
  \def\pgf@text@options{#1}%
  \pgf@maketext\pgf@after@text}
\def\pgf@after@text{%
  {%
  \def\pgf@text@hshift{center}%
  \def\pgf@text@vshift{center}%
  \def\pgf@marshal{\setkeys{pgfbox}}%
  \expandafter\pgf@marshal\expandafter{\pgf@text@options}%
  \csname pgf@halign\pgf@text@hshift\endcsname%
  \csname pgf@valign\pgf@text@vshift\endcsname%
  % Protocol sizes:
  \pgf@process{\pgfpointtransformed{\pgfqpoint{0pt}{\dp\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{\wd\pgf@hbox}{\dp\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{0pt}{\ht\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{\wd\pgf@hbox}{\ht\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgfqboxsynced{\pgf@hbox}%
  }%
}

\define@key{pgfbox}{left}[]{\def\pgf@text@hshift{left}}
\define@key{pgfbox}{center}[]{}
\define@key{pgfbox}{right}[]{\def\pgf@text@hshift{right}}
\define@key{pgfbox}{top}[]{\def\pgf@text@vshift{top}}
\define@key{pgfbox}{bottom}[]{\def\pgf@text@vshift{bottom}}
\define@key{pgfbox}{base}[]{\def\pgf@text@vshift{base}}
\define@key{pgfbox}{at}{\pgftransformshift{#1}}
\define@key{pgfbox}{x}{\pgftransformxshift{#1}}
\define@key{pgfbox}{y}{\pgftransformyshift{#1}}
\define@key{pgfbox}{rotate}{\pgftransformrotate{#1}}

\def\pgf@halignleft{}% do nothing
\def\pgf@haligncenter{\pgftransformxshift{+-.5\wd\pgf@hbox}}
\def\pgf@halignright{\pgftransformxshift{+-\wd\pgf@hbox}}%
\def\pgf@valignbase{}% do nothing
\def\pgf@valignbottom{\pgftransformyshift{+\dp\pgf@hbox}}%
\def\pgf@valigncenter{\pgftransformyshift{+.5\dp\pgf@hbox}\pgftransformyshift{+-.5\ht\pgf@hbox}}%
\def\pgf@valigntop{\pgftransformyshift{+-\ht\pgf@hbox}}%


% Internal function for creating a hbox.
\def\pgf@maketext#1{%
  \def\pgf@@maketextafter{#1}%
  \setbox\pgf@hbox=\hbox\bgroup%
    \pgfinterruptpicture%
      \bgroup%
        \aftergroup\pgf@collectresetcolor%
        \let\next=%
}
\def\pgf@collectresetcolor{%
  \pgfutil@ifnextchar\reset@color%
  {\reset@color\afterassignment\pgf@collectresetcolor\let\pgf@temp=}%
  {\pgf@textdone}%
}
\def\pgf@textdone{%
    \endpgfinterruptpicture%
  \egroup%
  \pgf@@maketextafter%  
}

\long\def\pgf@makehbox#1{%
  \setbox\pgf@hbox=\hbox{{%
    \pgfinterruptpicture%
      #1%
    \endpgfinterruptpicture%
    }}}



% Picture environment
%
% Example:
%
% \begin{pgfpicture}
%   \pgfsetendarrow{\pgfarrowto}
%   \pgfpathmoveto{\pgfpointxy{-0.9}{0.2}}
%   \pgfpathlineto{\pgfpointxy{0.9}{0.4}}
%   \pgfusepath{stroke}
% \end{pgfpicture}

\newif\ifpgfpicture

\def\pgfpicture{%
  \begingroup%
    \pgfpicturetrue%
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
    \let\pgf@nodecallback=\pgfutil@gobble%
    \pgf@picmaxx=-16000pt\relax%
    \pgf@picminx=16000pt\relax%
    \pgf@picmaxy=-16000pt\relax%
    \pgf@picminy=16000pt\relax%
    \pgf@relevantforpicturesizetrue%
    \pgf@resetpathsizes%
    \pgfutil@ifnextchar\bgroup\pgf@oldpicture\pgf@picture}
\def\pgf@oldpicture#1#2#3#4{%
  \pgfmathsetlength\pgf@picminx{#1}%
  \pgfmathsetlength\pgf@picminy{#2}%
  \pgfmathsetlength\pgf@picmaxx{#3}%
  \pgfmathsetlength\pgf@picmaxy{#4}%
  \pgf@relevantforpicturesizefalse%
  \pgf@picture}

\def\pgf@picture{%
  \setbox\pgfpic\hbox to0pt\bgroup%
    \begingroup%
    \pgfsys@beginpicture%
      \pgfsys@beginscope%
        \begingroup%
        \pgfsetcolor{.}%
        \pgfsetlinewidth{0.4pt}%
        \pgftransformreset%
        \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
        \begingroup%
          \let\pgf@setlengthorig=\setlength%
          \let\pgf@addtolengthorig=\addtolength%
          \let\pgf@selectfontorig=\selectfont%
          \let\setlength=\pgf@setlength%
          \let\addtolength=\pgf@addtolength%
          \let\selectfont=\pgf@selectfont%
          \nullfont\spaceskip\z@\xspaceskip\z@%
          \setbox\pgf@layerbox@main\hbox to0pt\bgroup%
            \begingroup%
  }
\def\endpgfpicture{%
              \ifpgfrememberpicturepositiononpage%
                \hbox to0pt{\pgfsys@markposition{\pgfpictureid}}%
              \fi%    
              % ok, now let's position the box
              \ifdim\pgf@picmaxx=-16000pt\relax%
                % empty picture. make size 0.  
                \global\pgf@picmaxx=0pt\relax%
                \global\pgf@picminx=0pt\relax%
                \global\pgf@picmaxy=0pt\relax%
                \global\pgf@picminy=0pt\relax%
              \fi%
              % Shift baseline outside:
              \pgf@relevantforpicturesizefalse%
              \pgf@process{\pgf@baseline}%
              \gdef\pgf@shift@baseline{\the\pgf@y}%
            \endgroup%
            \hss%
          \egroup%
          \pgf@insertlayers%
        \endgroup%    
        \pgfsys@discardpath%
        \endgroup%
      \pgfsys@endscope%
    \pgfsys@endpicture%
    \endgroup%
    \hss
  \egroup%
  \pgfsys@typesetpicturebox\pgfpic%
  \endgroup%
}

\def\pgf@insertlayers{%
  \box\pgf@layerbox@main%
}

\def\pgf@selectfont{\pgf@selectfontorig\nullfont}

\def\pgf@setlength#1#2{% these will be used only when \nullfont is active
  \begingroup% keep font setting local
    \pgfutil@selectfont% restore font
    \pgf@setlengthorig#1{#2}% calculate dimension (possibly using calc)
    \expandafter%
  \endgroup%
  \expandafter#1\expandafter=\the#1\relax}
\def\pgf@addtolength#1#2{%
  \begingroup% keep font setting local
    \pgfutil@selectfont% restore font
    \pgf@addtolengthorig#1{#2}% calculate dimension (possibly using calc)
    \expandafter%
  \endgroup%
  \expandafter#1\expandafter=\the#1\relax}


% Sets the baseline at the y-coordinate of a given point
%
% #1 = point
%
% Sets the baseline of the picture to the y-coordinate of a given
% point. However, the point will be evaluated *at the end of the
% picture*. 
%
% Example:
%
% \pgfsetbaselinepointlater{\pgfpointanchor{mynode}{base}}

\def\pgfsetbaselinepointlater#1{\def\pgf@baseline{#1}}


% Sets the baseline at the y-coordinate of a given point, now
%
% #1 = point
%
% Sets the baseline of the picture to the y-coordinate of a given
% point.
%
% Example:
%
% \pgfsetbaselinepointnow{\pgfpoint{1cm}{2pt}}

\def\pgfsetbaselinepointnow#1{%
  \pgf@process{#1}%
  \edef\pgf@setter@baseline{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgfsetbaselinepointlater{\pgf@setter@baseline}%
}


% Sets the baseline
%
% #1 = baseline
%
% Sets the baseline of the picture. Default is the lower border, which
% is the same as \pgf@picminy
%
% Example:
%
% \pgfsetbaseline{1cm+2pt}

\def\pgfsetbaseline#1{\pgfsetbaselinepointlater{\pgfpoint{0pt}{#1}}}
\pgfsetbaseline{\pgf@picminy}




% Interrupt path
%
% Description:
%
% The environment can be used to insert some drawing commands while
% constructing a path. The drawing commands inside the environment
% will not interfere with the path being constructed ``outside.''
% However, you must ward against graphic state changes using a scope. 
%
% Example: Draw two parallel lines
%
% \pgfmoveto{\pgfpoint{0cm}{0cm}}
% \begin{pgfinterruptpath}
%   \pgfmoveto{\pgfpoint{1cm}{0cm}}
%   \pgfmoveto{\pgfpoint{1cm}{1cm}}
%   \pgfusepath{stroke}
% \end{pgfinterruptpath}
% \pgflineto{\pgfpoint{0cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfinterruptpath
{%
  \begingroup%
  % save all sorts of things...
  \edef\pgf@interrupt@savex{\the\pgf@path@lastx}%
  \edef\pgf@interrupt@savey{\the\pgf@path@lasty}%
  \pgf@getpathsizes\pgf@interrupt@pathsizes%
  \pgfsyssoftpath@getcurrentpath\pgf@interrupt@path%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \edef\pgfscope@linewidth{\the\pgflinewidth}%
  \let\pgf@interrupt@lastmoveto=\pgfsyssoftpath@lastmoveto%
  \begingroup%
}
\def\endpgfinterruptpath
{%
  \endgroup%
  \global\pgflinewidth=\pgfscope@linewidth%
  \pgfsyssoftpath@setcurrentpath\pgf@interrupt@path%
  \pgf@setpathsizes\pgf@interrupt@pathsizes%
  \global\pgf@path@lastx=\pgf@interrupt@savex%
  \global\pgf@path@lasty=\pgf@interrupt@savey%
  \global\let\pgfsyssoftpath@lastmoveto=\pgf@interrupt@lastmoveto%
  \endgroup%
}



% Interrupt bounding box
%
% Description:
%
% The environment can be used to temporarily setup a new bounding box
% computation. The bounding box will be made empty at the beginning of
% the environment and will be reset to its old value after the
% environment. 
%
% Example: 
%
% \begin{pgfinterruptboundinbox}
%   \pgfmoveto{\pgfpoint{1cm}{0cm}}
%   \pgfmoveto{\pgfpoint{1cm}{1cm}}
%   \pgfusepath{stroke}
% \end{pgfinterruptboundinbox}

\def\pgfinterruptboundingbox
{%
  \begingroup%
    \edef\pgf@interrupt@savemaxx{\the\pgf@picmaxx}%
    \edef\pgf@interrupt@saveminx{\the\pgf@picminx}%
    \edef\pgf@interrupt@savemaxy{\the\pgf@picmaxy}%
    \edef\pgf@interrupt@saveminy{\the\pgf@picminy}%
    \pgf@picmaxx=-16000pt\relax%
    \pgf@picminx=16000pt\relax%
    \pgf@picmaxy=-16000pt\relax%
    \pgf@picminy=16000pt\relax%
}
\def\endpgfinterruptboundingbox
{%
    \global\pgf@picmaxx=\pgf@interrupt@savemaxx%
    \global\pgf@picmaxy=\pgf@interrupt@savemaxy%
    \global\pgf@picminx=\pgf@interrupt@saveminx%
    \global\pgf@picminy=\pgf@interrupt@saveminy%
  \endgroup%
}





% Interrupts a picture
%
% Description:
%
% This environment interrupts a picture and temporarily returns to
% normal TeX mode. All sorts of things are saved and restored by this
% environment.
%
% WARNING: Using this environment in conjuction with low level
% transformations can *strongly* upset the typesetting. Typically, the
% contents of this environment should have size/height/depth 0pt in
% the end.
%
% WARNING: This environment should only be used inside typesetting a
% box and this box must in turn be inserted using \pgfqbox.
%
% Example: Draw two parallel lines
%
% \pgfmoveto{\pgfpoint{0cm}{0cm}}
% \setbox\mybox=\hbox{
%    \begin{pgfinterruptpicture}
%      This is normal text.
%      \begin{pgfpicture} % a subpicture
%        \pgfmoveto{\pgfpoint{1cm}{0cm}}
%        \pgfmoveto{\pgfpoint{1cm}{1cm}}
%        \pgfusepath{stroke}
%      \end{pgfpicture}
%      More text.
%    \end{pgfinterruptpicture}
%  }
% \ht\mybox=0pt
% \wd\mybox=0pt
% \dp\mybox=0pt
% \pgfqbox{\mybox}%
% \pgfpathlineto{\pgfpoint{0cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfinterruptpicture
{%
  \begingroup%
    \pgfinterruptboundingbox%
      \pgftransformreset%
      \pgfinterruptpath%
        \ifx\pgf@selectfontorig\@undefined%
        \else%
          \let\setlength\pgf@setlengthorig%
          \let\addtolength\pgf@addtolengthorig%
          \let\selectfont\pgf@selectfontorig%
        \fi%
        \pgfutil@selectfont%
        \pgfpicturefalse%
        \pgf@savelayers%
}
\def\endpgfinterruptpicture
{%
        \pgf@restorelayers%
      \endpgfinterruptpath%
    \endpgfinterruptboundingbox%
  \endgroup%
}

\let\pgf@savelayers=\relax
\let\pgf@restorelayers=\relax


\endinput


==> pgfcoreshade.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoreshade.code.tex,v 1.8 2007/03/09 17:49:32 tantau Exp $

%
% Parsing functions
%
\newdimen\pgf@max
\newcount\pgf@sys@shading@range@num
\def\pgf@parsefunc#1{%
  \edef\temp{{#1}}%
  \expandafter\pgf@convertrgbstring\temp%
  \edef\temp{{\pgf@rgbconv}}%
  \expandafter\pgf@@parsefunc\temp}
\def\pgf@@parsefunc#1{%
  \let\pgf@bounds=\pgfutil@empty%
  \let\pgf@funcs=\pgfutil@empty%
  \let\pgf@psfuncs=\pgfutil@empty%
  \let\pgf@encode=\pgfutil@empty%
  \let\pgf@sys@shading@ranges=\pgfutil@empty%
  \pgf@sys@shading@range@num=0\relax%
  \pgf@parsefirst[#1; ]%
  \pgf@parselastdom[#1; ]%
  \pgf@parsemid[#1; ]%
  \ifx\pgf@bounds\pgfutil@empty%
    \edef\pgf@pdfparseddomain{0 1}%
    \edef\pgf@pdfparsedfunction{\pgf@singlefunc\space}%
  \else%
    \edef\pgf@pdfparseddomain{\pgf@doma\space\pgf@domb}%
    \edef\pgf@pdfparsedfunction{%
      << /FunctionType 3 /Domain [\pgf@doma\space\pgf@domb] /Functions
      [\pgf@funcs\space] /Bounds [\pgf@bounds] /Encode [0 1 \pgf@encode]
      >> }%
  \fi%
  \xdef\pgf@psfuncs{\pgf@psfuncs}%
  }
\def\pgf@parsefirst[rgb(#1)=(#2,#3,#4)#5]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
  \edef\pgf@sys@shading@start@rgb{\pgf@sys@rgb}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@rgb%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@rgb}%
  \edef\pgf@firstcolor{\pgf@rgb}}
\def\pgf@parselastdom[rgb(#1)=(#2,#3,#4); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@end@rgb{\pgf@sys@rgb}%
    \pgfutil@gobble}{\pgf@parselastdom[}}
\def\pgf@parsemid[rgb(#1)=(#2,#3,#4); {\pgf@parserest[}
\def\pgf@parserest[rgb(#1)=(#2,#3,#4); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }%
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% 
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% 
    \edef\pgf@prevcolor{\pgf@rgb}%
    \pgf@parserest[}}

\def\pgf@getrgbtuplewithmixin#1#2#3{%
  \pgfutil@definecolor{pgfshadetemp}{rgb}{#1,#2,#3}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgf@getrgb@@\pgf@rgbcolor!}
\def\pgf@getrgb@@#1,#2,#3!{%
  \def\pgf@rgb{#1 #2 #3}%
  \def\pgf@sys@rgb{{#1}{#2}{#3}}%
}


\def\pgf@convertrgbstring#1{%
  \def\pgf@rgbconv{}%
  \pgf@converttorgb#1]%
  }
\def\pgf@converttorgb{%
  \pgfutil@ifnextchar]{\pgfutil@gobble}%done!
  {%
    \pgfutil@ifnextchar;{\pgf@grabsemicolor}%
    {%
      \pgfutil@ifnextchar r{\pgf@grabrgb}%
      {%
        \pgfutil@ifnextchar g{\pgf@grabgray}%
        {%
          \pgfutil@ifnextchar c{\pgf@grabcolor}%
          {\PackageError{pgfshade}{Illformed shading
              specification}{}\pgf@converttorgb}%
        }%
      }%
    }%
  }%
}
\def\pgf@grabsemicolor;{%
  \edef\pgf@rgbconv{\pgf@rgbconv; }\pgf@converttorgb}
\def\pgf@grabrgb rgb(#1)=(#2,#3,#4){%
  \edef\pgf@rgbconv{\pgf@rgbconv rgb(#1)=(#2,#3,#4)}\pgf@converttorgb}
\def\pgf@grabgray gray(#1)=(#2){%
  \edef\pgf@rgbconv{\pgf@rgbconv rgb(#1)=(#2,#2,#2)}\pgf@converttorgb}
\def\pgf@grabcolor color(#1)=(#2){%
  \pgfutil@colorlet{pgf@tempcol}{#2}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgf@convgetrgb@\expandafter{\pgf@rgbcolor}{#1}%
}
\def\pgf@convgetrgb@#1#2{%
  \edef\pgf@rgbconv{\pgf@rgbconv rgb(#2)=(#1)}\pgf@converttorgb}




% Declares a horizontal shading for later use. The shading is a
% horizontal bar that changes its color.
%
% #1 = name of the shading for later use
% #2 = height of the shading
% #3 = color specification in the following format: A list of colors
%      that the bar should have at certain points. If the bar should
%      be red at 1cm, this is specified as
%      "rgb(1cm)=(1,0,0)". Multiple specifications are separated by a
%      semicolon and a space. At least two specifications must be
%      given. The specified positions must be given in increasing
%      order. 
%
% Example:
%
% \pgfdeclarehorizontalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm long: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclarehorizontalshading{\pgfutil@ifnextchar[\pgf@declarehorizontalshading{\pgf@declarehorizontalshading[]}}%
\def\pgf@declarehorizontalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \pgfsys@horishading{#2}{#3}{#4}%
  \else%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@horishading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a vertical shading for later use. 
%
% #1 = name of the shading for later use
% #2 = height of the shading
% #3 = color specification 
%
% Example:
%
% \pgfdeclareverticalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm high: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareverticalshading{\pgfutil@ifnextchar[\pgf@declareverticalshading{\pgf@declareverticalshading[]}}%
\def\pgf@declareverticalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \pgfsys@vertshading{#2}{#3}{#4}%
  \else%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@vertshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a radial shading for later use. 
%
% #1 = name of the shading for later use
% #2 = center of inner circle
% #3 = color specification 
%
% Description:
%
% A radial shading creates a smooth color transition between two
% circles. The center of the inner circle is at the give position. Its
% radius is the start of the color specification. The
% center of the outer circle is at the center of the whole shading,
% whose radius is the end of the color specification. For example,
% suppose the color specification is "rgb(1cm)=(1,1,1); rgb(2cm)=(0,0,0)".  
% Then the shading would be 4cm times 4cm large. The inner circle would
% have diameter 1cm and the outer circle would have diameter 2cm. The
% outer circle would be centered in the middle of the shading, whereas
% the outer circle would be centered at the given position.
%
% Example:
%
% \pgfdeclareradialshading{redtogreentoblue}{\pgfpoint{2cm}{2cm}}{%
%   rgb(10pt)=(1,0,0); % red
%   rgb(2cm)=(0,1,0); % green
%   rgb(3cm)=(0,0,1)}
%
% \begin{document}
%   The following ball has diameter 3cm: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareradialshading{\pgfutil@ifnextchar[\pgf@declareradialshading{\pgf@declareradialshading[]}}%
\def\pgf@declareradialshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \pgfsys@radialshading{#2}{#3}{#4}%
  \else%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@radialshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}
  

% Inserts a box into the text that contains a previously defined
% shading. 
%
% #1 = Name of a shading
%
% Example:
%
% \pgfuseshading{redtogreentoblue}

\def\pgfuseshading#1{%
  \edef\pgf@shadingname{@pgfshading#1}%
  \pgf@tryextensions{\pgf@shadingname}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@shadingname}%
  {\PackageError{pgfshade}{Undefined shading "#1"}{}}%
  {%
    {%
      \pgfutil@globalcolorsfalse%
      \def\pgf@shade@adds{}%
      \pgfutil@ifundefined{pgf@deps\pgf@shadingname}%
      {}%
      {%
        \edef\@list{\csname pgf@deps\pgf@shadingname\endcsname}%
        \pgfutil@for\@temp:=\@list\do{%
          {%
            \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{\@temp}}%
            \pgfutil@extractcolorspec{\@temp}{\pgf@tempcolor}%
            \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
            \xdef\pgf@shade@adds{\pgf@shade@adds,\pgf@rgbcolor}%
          }%
        }%
      }%
      \expandafter\pgf@strip@shadename\pgf@shadingname!!%
      \pgfutil@ifundefined{@pgfshading\pgf@basename\pgf@shade@adds!}%
      {%
        {%
          \expandafter\def\expandafter\@temp\expandafter{\csname pgf@func\pgf@shadingname\endcsname}%
          \edef\@args{{\pgf@basename\pgf@shade@adds}}%
          \expandafter\expandafter\expandafter\def%
          \expandafter\expandafter\expandafter\@@args%
          \expandafter\expandafter\expandafter{\csname pgf@args\pgf@shadingname\endcsname}%
          \expandafter\expandafter\expandafter\@temp\expandafter\@args\@@args%
          %
        }%
      }%
      {}%
      \pgf@invokeshading{\csname @pgfshading\pgf@basename\pgf@shade@adds!\endcsname}%
    }%
  }%
}

\def\pgf@strip@shadename @pgfshading#1!!!{\def\pgf@basename{#1}}

\def\pgf@invokeshading#1{%
  \ifpgfpicture%
    \pgfsys@shadinginsidepgfpicture{#1}%
  \else%
    \pgfsys@shadingoutsidepgfpicture{#1}%  
  \fi%
}


% Create an alias name for a shading
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfaliasshading{shading!25}{shadingshaded}

\def\pgfaliasshading#1#2{%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname @pgfshading#2!\endcsname%
  \expandafter\let\csname @pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@deps@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@deps@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@func@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@func@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@args@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@args@pgfshading#1!\endcsname=\pgf@temp%
}




% Shades the current path, but does not discard it.
%
% #1 - a shading (see below)
% #2 - an angle
%
% Description:
%
% \pgfshadepath  ``tries'' to fill the
% current path with a shading. The shading's original size should
% completely cover the area between (0,0) and (100bp,100bp). The
% shading will be rotated by #2 and then rescaled so that it
% completely covers the path. Then the path will be used (locally) for
% clipping and the shading is drawn.
%
% In addition to the rotation, any transformation set by the
%\pgfsetadditionalshadetransform will also be applied.
%
% After all this, the path can still be used for the normal
% stroking/clipping operations.
%
% The shading is rotated around its middle. If no rotation occurs, the
% lower left corner of the path will lie on (25bp, 25bp), the upper
% right corner on (75bp, 75bp).
%
% Example:
%
% \pgfdeclareverticalshading{myshading}{100bp}{color(0pt)=(red); color(100bp)=(green)}
%
% \pgfpathmoveto{\pgforigin}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfpathlineto{\pgfxy(1,1)}
% \pgfshadepath{myshading}{0}
% \pgfusepath{stroke}

\def\pgfshadepath#1#2{%
  \ifdim\pgf@pathminx=16000pt%
    \PackageWarning{pgfshade}{No path specified that can be filled}%
  \else%
    \begingroup%  
      \pgfsys@beginscope%
        % Calculate center:
        \pgf@xb=.5\pgf@pathmaxx%
        \advance\pgf@xb by.5\pgf@pathminx%
        \pgf@yb=.5\pgf@pathmaxy%
        \advance\pgf@yb by.5\pgf@pathminy%
        % Calculate scaling:
        \pgf@xc=\pgf@pathmaxx%
        \advance\pgf@xc by-\pgf@pathminx%
        \pgf@yc=\pgf@pathmaxy%
        \advance\pgf@yc by-\pgf@pathminy%
        \pgf@xc=.02\pgf@xc%
        \pgf@yc=.02\pgf@yc%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsys@clipnext%
        \pgfsys@discardpath%
        % Compute new transformation matrix:
        \pgfsys@transformcm{1}{0}{0}{1}{\pgf@xb}{\pgf@yb}%
        \pgfsys@transformcm%
        {\pgf@sys@tonumber{\pgf@xc}}{0}%
        {0}{\pgf@sys@tonumber{\pgf@yc}}{0pt}{0pt}%
        \pgfmathparse{#2}%
        \let\pgfshade@angle=\pgfmathresult%
        \pgfmathsin@{\pgfshade@angle}%
        \let\pgfshade@sin=\pgfmathresult%
        \pgfmathcos@{\pgfshade@angle}%
        \let\pgfshade@cos=\pgfmathresult%
        \pgf@x=\pgfshade@sin pt%
        \pgf@xa=-\pgf@x%
        \pgfsys@transformcm{\pgfshade@cos}{\pgfshade@sin}{\pgf@sys@tonumber{\pgf@xa}}{\pgfshade@cos}{0pt}{0pt}%
        \ifx\pgf@shade@extra@transform\pgfutil@empty%
        \else%
          \pgflowlevel{\pgf@shade@extra@transform}%
        \fi%
        \pgfuseshading{#1}%
      \pgfsys@endscope%
    \endgroup%
  \fi%
}


% Additionally transform shade paths
%
% #1 = Transformation code that is used in addition to the normal
%      shading transformation.
%
% Example:
%
% \pgfsetadditionalshadetransform{\pgftransformrotate{30}}

\def\pgfsetadditionalshadetransform#1{\def\pgf@shade@extra@transform{#1}}
\let\pgf@shade@extra@transform=\pgfutil@empty





\endinput


==> pgfcoretransformations.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoretransformations.code.tex,v 1.6 2007/06/07 07:41:10 tantau Exp $


% Position transformations

\newdimen\pgf@pt@x
\newdimen\pgf@pt@y

\newdimen\pgf@pt@temp

\newif\ifpgf@pt@identity
\pgf@pt@identitytrue

\def\pgf@pt@aa{1.0} \def\pgf@pt@ab{0.0}
\def\pgf@pt@ba{0.0} \def\pgf@pt@bb{1.0}



% Store the current transformation matrix in a macro.
%
% #1 = macro name
%
% Example:
%
% \pgfgettransform\mytransform

\def\pgfgettransform#1{%
  \edef#1{{\pgf@pt@aa}{\pgf@pt@ab}{\pgf@pt@ba}{\pgf@pt@bb}{\the\pgf@pt@x}{\the\pgf@pt@y}}
}


% Restore the current transformation matrix from a macro.
%
% #1 = macro name, previously used with \pgfgettransform
%
% Example:
%
% \pgfsettransform\mytransform

\def\pgfsettransform#1{%
  \edef\pgf@temp{#1}%
  \expandafter\pgf@settransform\pgf@temp%
}
\def\pgf@settransform#1#2#3#4#5#6{%
  \def\pgf@pt@aa{#1}%
  \def\pgf@pt@ab{#2}%
  \def\pgf@pt@ba{#3}%
  \def\pgf@pt@bb{#4}%
  \pgf@pt@x=#5%
  \pgf@pt@y=#6%
  \edef\pgf@idtest{#1,#2,#3,#4}%
  \ifx\pgf@idtest\pgf@idmatrixtext%
    \pgf@pt@identitytrue%
  \else%
    \pgf@pt@identityfalse%
  \fi%
}

\def\pgf@idmatrixtext{1.0,0.0,0.0,1.0}


% Transformation command
%
% #1 = x dimension
% #2 = y dimension
%
% Description:
%
% Applies the pgfs transformation matrix to the point (#1,#2). The
% result is once more stored in the point.
%
%
% Example:
%
% \pgf@pos@transform{\pgf@x}{\pgf@y}

\def\pgf@pos@transform#1#2{%
  \ifpgf@pt@identity%
  \else%
    \pgf@pt@temp=#1%
    #1=\pgf@pt@aa#1%
    \advance#1 by\pgf@pt@ba#2%
    #2=\pgf@pt@bb#2%
    \advance#2 by\pgf@pt@ab\pgf@pt@temp%
  \fi%
  \advance#1 by\pgf@pt@x%
  \advance#2 by\pgf@pt@y%
}


% Invert the current transformation matrix
%
% Description:
%
% This command replaces the current transformation matrix by its
% inverse. The inversion is not very exact if the matrix is nearly
% singular. 
%
% Example:
%
% \pgftransforminvert

\def\pgftransforminvert{%
  % First, invert the shift. That's easy
  \pgf@pt@x=-\pgf@pt@x
  \pgf@pt@y=-\pgf@pt@y
  \ifpgf@pt@identity%
  \else%
    % Sigh. Have to calculate the inverse of the matrix.
    % Start with determinant
    % Matrix = (aa ab
    %           ba bb)
    {%
      \pgfutil@tempdima=\pgf@pt@aa pt%
      \pgfutil@tempdima=\pgf@pt@bb\pgfutil@tempdima% aa * bb
      \pgfutil@tempdimb=\pgf@pt@ba pt%
      \pgfutil@tempdimb=\pgf@pt@ab\pgfutil@tempdimb% ba * ab
      \advance\pgfutil@tempdima by -\pgfutil@tempdimb% aa*bb - ba*ab
      % Invert
      \pgfutil@tempdima=.125\pgfutil@tempdima%
      \c@pgf@counta=\pgfutil@tempdima\relax% 8192*determinant
      \pgfutil@tempdima=8192pt%
      \divide\pgfutil@tempdima by\c@pgf@counta%
      \pgf@x=\pgf@pt@bb\pgfutil@tempdima% bb/(det A)
      \xdef\pgf@new@pt@aa{\pgf@sys@tonumber{\pgf@x}}%
      \pgf@x=\pgf@pt@aa\pgfutil@tempdima% aa/(det A)
      \xdef\pgf@new@pt@bb{\pgf@sys@tonumber{\pgf@x}}%
      \pgfutil@tempdima=-\pgfutil@tempdima%
      \pgf@x=\pgf@pt@ba\pgfutil@tempdima% -ba/(det A)
      \xdef\pgf@new@pt@ba{\pgf@sys@tonumber{\pgf@x}}%
      \pgf@x=\pgf@pt@ab\pgfutil@tempdima% -ab/(det A)
      \xdef\pgf@new@pt@ab{\pgf@sys@tonumber{\pgf@x}}%
    }%
    \expandafter\def\expandafter\pgf@pt@aa\expandafter{\pgf@new@pt@aa}%
    \expandafter\def\expandafter\pgf@pt@ab\expandafter{\pgf@new@pt@ab}%
    \expandafter\def\expandafter\pgf@pt@ba\expandafter{\pgf@new@pt@ba}%
    \expandafter\def\expandafter\pgf@pt@bb\expandafter{\pgf@new@pt@bb}%
    \pgf@pt@temp=\pgf@pt@x%
    \pgf@pt@x=\pgf@pt@aa\pgf@pt@x%
    \advance\pgf@pt@x by\pgf@pt@ba\pgf@pt@y%
    \pgf@pt@y=\pgf@pt@bb\pgf@pt@y%
    \advance\pgf@pt@y by\pgf@pt@ab\pgf@pt@temp%
  \fi%
}




% PGF-Level concatenation of the transformation matrix with a given
% matrix. 
%
% #1 - #5 = a concatenation matrix (see pdf spec). Entry #5 is a
%           translation point.
%
% Description:
%
% All coordinates given to subsequent path construction commands will
% be transformed additionally by the given transformation matrix. If
% the command is followed by a 6th argument, the transformation is
% only applied to this argument.
%
%
% Example:
%
% \pgftransformcm{1}{0}{0}{1}{\pgfpoint{100pt}{0pt}} % 100pt to the right.
%
% \pgftransformcm{2}{0}{0}{2}{\pgfpointorigin} % double in in size
% \pgfpathmoveto{\pgfpoint{0cm}{0cm}}
% \pgfpathlineto{\pgflineto{1cm}{1cm}} % actually 2cm/2cm

\def\pgftransformcm#1#2#3#4#5{%
  \edef\pgf@marshal{\noexpand\pgf@transformcm{#1}{#2}{#3}{#4}}%
  \pgf@marshal{#5}%
}
\def\pgf@transformcm#1#2#3#4#5{%
  {%
    \pgf@process{#5}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    %
    \pgf@x=#1pt%
    \pgf@y=#2pt%
    %
    \pgf@xa=\pgf@pt@aa\pgf@x%
    \advance\pgf@xa by \pgf@pt@ba\pgf@y%
    %
    \pgf@ya=\pgf@pt@ab\pgf@x%
    \advance\pgf@ya by \pgf@pt@bb\pgf@y%
    %
    \pgf@x=#3pt%
    \pgf@y=#4pt%
    %
    \pgf@xb=\pgf@pt@aa\pgf@x%
    \advance\pgf@xb by \pgf@pt@ba\pgf@y%
    %
    \pgf@yb=\pgf@pt@ab\pgf@x%
    \advance\pgf@yb by \pgf@pt@bb\pgf@y%
    %
    \pgf@x=\pgf@pt@aa\pgf@xc%
    \advance\pgf@x by\pgf@pt@ba\pgf@yc%
    \advance\pgf@x by\pgf@pt@x%
    %
    \pgf@y=\pgf@pt@ab\pgf@xc%
    \advance\pgf@y by\pgf@pt@bb\pgf@yc%
    \advance\pgf@y by\pgf@pt@y%
    %
    \global\pgf@x=\pgf@x%
    \global\pgf@y=\pgf@y%
    \xdef\pgf@tempaa{\pgf@sys@tonumber{\pgf@xa}}%
    \xdef\pgf@tempab{\pgf@sys@tonumber{\pgf@ya}}%
    \xdef\pgf@tempba{\pgf@sys@tonumber{\pgf@xb}}%
    \xdef\pgf@tempbb{\pgf@sys@tonumber{\pgf@yb}}%
  }%
  \pgf@pt@x=\pgf@x%
  \pgf@pt@y=\pgf@y%
  \let\pgf@pt@aa=\pgf@tempaa%
  \let\pgf@pt@ba=\pgf@tempba%
  \let\pgf@pt@ab=\pgf@tempab%
  \let\pgf@pt@bb=\pgf@tempbb%
  \def\pgf@trans@idtest{#1,#2,#3,#4}%
  \ifx\pgf@trans@idtest\pgf@trans@idtext%
  \else%
    \pgf@pt@identityfalse%
  \fi%
}
\def\pgf@trans@idtext{1.0,0,0,1.0}



% Transformation into a given triangle. The three corners of the
% triangle are called "origin", "x" and "y" are given. After this
% transformation has been applied, the canvas origin is at "origin",
% the vector (1pt,0pt) lies at "x" and the vector (0pt,1pt) lies at
% "y". 
%
% #1 = origin
% #2 = x
% #3 = y
%
% Example:
%
% \pgftransformtriangle{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}{\pgfpoint{-1cm}{1cm}}

\def\pgftransformtriangle#1#2#3{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#3}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  \advance\pgf@xb by-\pgf@x%
  \advance\pgf@yb by-\pgf@y%
  \pgftransformcm%
  {\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
  {\pgf@sys@tonumber\pgf@xb}{\pgf@sys@tonumber\pgf@yb}%
  {\pgfpoint{\pgf@x}{\pgf@y}}%
}



% Undo all transformations
%
% Example:
%
% \pgftansformreset

\def\pgftransformreset{%
  \pgf@pt@x=0pt%
  \pgf@pt@y=0pt%
  \def\pgf@pt@aa{1.0}%
  \def\pgf@pt@ba{0.0}%
  \def\pgf@pt@ab{0.0}%
  \def\pgf@pt@bb{1.0}%
  \pgf@pt@identitytrue%
}


% Undo all slanting/rotation, but not translations
%
% Example:
%
% \pgftansformreset

\def\pgftransformresetnontranslations{%
  \def\pgf@pt@aa{1.0}%
  \def\pgf@pt@ba{0.0}%
  \def\pgf@pt@ab{0.0}%
  \def\pgf@pt@bb{1.0}%
  \pgf@pt@identitytrue%
}




% Shifting command and environment
%
% #1 = vector by which all subsequent points should be moved.
%
% Example:
%
% \pgftansformshift{\pgfpoint{1cm}{1cm}}

\def\pgftransformshift#1{\pgftransformcm{1.0}{0}{0}{1.0}{#1}}
\def\pgftransformxshift#1{\pgftransformcm{1.0}{0}{0}{1.0}{\pgfpoint{#1}{0pt}}}
\def\pgftransformyshift#1{\pgftransformcm{1.0}{0}{0}{1.0}{\pgfpoint{0pt}{#1}}}




% Scaling commands
%
% #1 = scaling for all subsequent points.
%
% Example:
%
% \pgftransformscale{2}
% \pgftransformxscale{2}
% \pgftransformyscale{2}

\def\pgftransformscale#1{\pgftransformcm{#1}{0}{0}{#1}{\pgfpointorigin}}
\def\pgftransformxscale#1{\pgftransformcm{#1}{0}{0}{1.0}{\pgfpointorigin}}
\def\pgftransformyscale#1{\pgftransformcm{1.0}{0}{0}{#1}{\pgfpointorigin}}



% Slanting commands
%
% #1 = slanting in x-direction. 1 means 45 degrees.
%
% Example:
%
% \pgftransformxslant{2}
% \pgftransformyslant{2}

\def\pgftransformxslant#1{\pgftransformcm{1.0}{0}{#1}{1.0}{\pgfpointorigin}}
\def\pgftransformyslant#1{\pgftransformcm{1.0}{#1}{0}{1.0}{\pgfpointorigin}}



% Rotation commands
%
% #1 = degrees for the rotation
%
% Example:
%
% \pgftransformrotate{30}

\def\pgftransformrotate#1{%
  \pgfmathparse{#1}%
  \let\pgftransform@angle=\pgfmathresult%
  \pgfmathsin@{\pgftransform@angle}%
  \let\pgftransform@sin=\pgfmathresult%
  \pgfmathcos@{\pgftransform@angle}%
  \let\pgftransform@cos=\pgfmathresult%
  \pgf@x=\pgftransform@sin pt%
  \pgf@xa=-\pgf@x%
  \pgftransformcm{\pgftransform@cos}{\pgftransform@sin}{\pgf@sys@tonumber{\pgf@xa}}{\pgftransform@cos}{\pgfpointorigin}%
}



% The following if's have the following effect:
%
% \ifpgfslopedattime decides whether the coordinate system of an
% xxxattime transformation command should be rotated such that text
% drawn on the line should be tangent to the line
%
% \ifpgfallowupsidedowattime decides whether the transformation should
% be done in such a way that the text is always ``upright,'' that is,
% text drawn in this coordiante system is never upside-down. 
%
% \ifpgfresetnontranslationattime decides whether the coordinate
% system of an xxxattime transformation command should be reset
% (concerning the non-translations) before a possible rotation is
% applied. This is useful, for example, if the main coordinate system
% is scaled by, say, a factor of 2 and you do not want that to apply
% to the text, but you do want the rotation to applyu.

\newif\ifpgfslopedattime
\newif\ifpgfallowupsidedownattime
\newif\ifpgfresetnontranslationattime


% Transform to the coordinate system of a point on a line
%
% #1 = a time fraction of line where to put the label, where 0 means start,
%      1 means end, and for example 0.5 means the middle.
% #2 = start of line
% #3 = end of line
%
% Example:
%
% {
%   \pgftransformlineattime{.5}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftext{Hi!}
% }
%
% {
%   \pgftransformlineattime{.75}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftransformresetnontranslations
%   \pgftext{Hi!}
% }
%
\def\pgftransformlineattime#1#2#3{%
  \pgftransformshift{\pgfpointlineattime{#1}{#2}{#3}}%
  \ifpgfresetnontranslationattime%
    \pgftransformresetnontranslations%
  \fi%
  \ifpgfslopedattime%
    \pgf@process{#2}%
    \pgf@xa=\pgf@x% xb/yb = start point
    \pgf@ya=\pgf@y%
    \pgf@process{#3}%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \ifpgfallowupsidedownattime%
    \else%
      \ifdim\pgf@x<0pt%   
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      \fi%
    \fi%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
    {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
  \fi%
}




% Transform to the coordinate system of a point on a curve
%
% #1 = a time fraction of line where to put the label, where 0 means start,
%      1 means end, and for example 0.5 means the middle.
% #2 = start of line
% #3 = first control
% #4 = second control
% #5 = end of line
%
% Example:
%
% {
%   \pgftransformlabel{.5}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftext{Hi!}
% }
%
% {
%   \pgftransformlabel{.75}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftransformresetnontranslations
%   \pgftext{Hi!}
% }
%
\def\pgftransformcurveattime#1#2#3#4#5{%
  \pgfpointcurveattime{#1}{#2}{#3}{#4}{#5}%
  \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \ifpgfresetnontranslationattime%
    \pgftransformresetnontranslations%
  \fi%
  \ifpgfslopedattime%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
    \advance\pgf@x by-\pgf@xb%
    \advance\pgf@y by-\pgf@yb%
    \ifpgfallowupsidedownattime%
    \else%
      \ifdim\pgf@x<0pt%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      \fi%
    \fi%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
    {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
  \fi%
}





% Transform to the coordinate system of an arrow at the end of the
% line going from point #1 to point #2 with the correct rotation.
%
% #1 = a start point an (invisible) line
% #2 = an end point an (invisible) line
%
% Example:
%
% \pgftransformarrow{\pgfpointorigin}{\pgfpoint{1cm}{0cm}}

\def\pgftransformarrow#1#2{%
  \pgftransformshift{#2}%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  \pgf@x=\pgf@xa%
  \pgf@y=\pgf@ya%
  \pgfpointnormalised{}%
  \pgf@ya=-\pgf@y%
  \pgftransformcm%
  {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
  {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfqpoint{0pt}{0pt}}%
}



% Low-level transformations

% Causes the current high-level transformation command to be applied
% to the low-level.
%
% Description:
%
% All subsequent drawing will be transformed additionally by the
% current high-level transformation. Thus, the high-level
% transformation becomes the low-level transformation. The high-level
% transformation is reset at this point.

\def\pgflowlevelsynccm{%
  \pgfsys@transformcm%
  {\pgf@pt@aa}{\pgf@pt@ab}%
  {\pgf@pt@ba}{\pgf@pt@bb}%
  {\pgf@pt@x}{\pgf@pt@y}%
  \pgftransformreset%
  \pgf@relevantforpicturesizefalse%
}  



% Causes a transformation command to be applied to the ``lowlevel''
% transformation matrix. 
%
% #1 - a high-level transformation command
%
% Description:
%
% All subsequent drawing will be transformed additionally by the given
% transformation matrix. Note that PGF will no longer be able to
% ``keep track'' of the coordinates. Also, transformations are applied
% to *everything*, including line thickness and line endings. Most
% often, this is not desirable.
%
% Example:
%
% \pgflowlevel{\pgftransformcm{1}{0}{0}{1}{\pgfpoint{100pt}{0pt}}} % 100bp to the right.
%
% \begin{pgflowlevelscope}{\pgftransformcm{2}{0}{0}{2}{\pgfpointorigin}} % double in in size
%  \pgfmoveto{\pgfpoint{0cm}{0cm}}
%  \pgflineto{\pgflineto{1cm}{1cm}} % actually 2cm/2cm
% \end{pgflowlevelscope}

\def\pgflowlevel#1{%
  {%
    \pgftransformreset%
    #1%
    \pgflowlevelsynccm%
  }%
  \pgf@relevantforpicturesizefalse%
}

\def\pgflowlevelscope#1{\pgfscope\pgflowlevel{#1}}
\def\endpgflowlevelscope{\endpgfscope}

\long\def\pgflowlevelobj#1#2{\pgfscope{\pgflowlevel{#1}#2}\endpgfscope}




\endinput


==> pgffor.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/utilities/pgffor.code.tex,v 1.5 2006/10/16 22:32:59 tantau Exp $

\newdimen\pgffor@iter
\newdimen\pgffor@skip
\newif\ifpgffor@continue

\let\pgffor@beginhook=\pgfutil@empty
\let\pgffor@endhook=\pgfutil@empty
\let\pgffor@afterhook=\pgfutil@empty

\def\pgffor@emptyvalues{, \pgffor@stop,}%

\def\foreach#1in#2{%
  \def\pgffor@var{#1}%
  \def\pgffor@values{#2, \pgffor@stop,}%
  \ifx\pgffor@values\pgffor@emptyvalues
    \def\pgffor@values{\pgffor@stop,}%
  \fi%
  \let\pgffor@body\pgfutil@empty%
  \global\pgffor@continuetrue%
  \pgffor@collectbody}

\def\pgffor@collectbody{%
  \pgfutil@ifnextchar\foreach{\pgffor@collectforeach}{%
    \pgfutil@ifnextchar\bgroup{\pgffor@collectargument}{\pgffor@collectsemicolon}}%
}

\def\pgffor@collectforeach\foreach#1in#2{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body\foreach#1in{#2}}%
  \pgffor@collectbody%
}

\long\def\pgffor@collectargument#1{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body{#1}}%
  \pgffor@iterate%
}


\def\pgffor@collectsemicolon{%
  \let\pgffor@next=\pgffor@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\pgffor@next=\pgffor@collectactivesemicolon%
  \fi%
  \pgffor@next%
}

\def\pgffor@collectnormalsemicolon#1;{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
  \pgffor@iterate%
}

{
  \catcode`\;=\active
  
  \gdef\pgffor@collectactivesemicolon#1;{%
    \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
    \pgffor@iterate%
  }
}

\def\pgffor@iterate{%
  \let\pgffor@last\pgfutil@empty%
  \let\pgffor@prevlast\pgfutil@empty%
  \expandafter\pgffor@scan\pgffor@values}

\def\pgffor@stop{\pgffor@stop}%
\def\pgffor@dots{...}%

\def\pgffor@scan{\pgfutil@ifnextchar({\pgffor@scanround}{\pgffor@scanone}}
\def\pgffor@scanround(#1)#2,{\def\pgffor@value{(#1)}\pgffor@scanned}
\def\pgffor@scanone#1,{\def\pgffor@value{#1}\pgffor@scanned}

\def\pgffor@scanned{%
  \ifx\pgffor@value\pgffor@stop%
    \let\pgffor@next=\pgffor@after% done!
  \else%
    \ifx\pgffor@value\pgffor@dots%
      \let\pgffor@next=\pgffor@handledots%
    \else%
      \let\pgffor@next=\pgffor@handlevalue%
    \fi%
    \ifpgffor@continue%
    \else%
      \let\pgffor@next=\pgffor@scan% done!
    \fi%
  \fi%
  \pgffor@next}

\def\pgffor@after{%
  \global\pgffor@continuetrue%
  \pgffor@afterhook}

\def\pgffor@handlevalue{%
  \let\pgffor@prevlast\pgffor@last%
  \let\pgffor@last\pgffor@value%
  \pgffor@invokebody%
  \pgffor@scan%
}

\def\pgffor@invokebody{%
  \begingroup%
    \expandafter\in@\expandafter/\expandafter{\pgffor@var}%
    \ifin@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@value//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
      \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@value}%
    \fi%
    \expandafter\pgffor@beginhook\pgffor@body\pgffor@endhook%
  \endgroup%
}


\def\pgffor@multiassign#1/#2/\relax{%
  \def\pgffor@currentvar{#1}%
  \def\pgffor@rest{#2}%
  \ifx\pgffor@currentvar\pgffor@stop%
    \let\pgffor@next=\relax%
  \else%
    \let\pgffor@next=\pgffor@multiassignrest%
  \fi%
  \pgffor@next%
}

\def\pgffor@multiassignrest{\expandafter\pgffor@multiassignfinal\pgffor@valuerest}
\def\pgffor@multiassignfinal#1/#2/\relax{%
  \def\pgffor@test{#2}%
  \ifx\pgffor@test\pgfutil@empty%
    \def\pgffor@valuerest{#1//\relax}% repeat
  \else%
    \def\pgffor@valuerest{#2/\relax}%
  \fi%
  \expandafter\def\pgffor@currentvar{#1}%
  \expandafter\pgffor@multiassign\pgffor@rest/\relax%
}
  



\def\pgffor@handledots{%
  \ifx\pgffor@last\pgfutil@empty%
    \PackageError{pgffor}{``...'' not allowed without prior value}{}%
  \fi%
  \pgffor@dotsscanend%
}
\def\pgffor@dotsscanend#1,{%
  \def\pgffor@dotsend{#1}%
  % calculate skip%
  \ifx\pgffor@prevlast\pgfutil@empty%
    \ifdim\pgffor@dotsend pt>\pgffor@last pt%
      \pgffor@skip=1pt%
    \else%
      \pgffor@skip=-1pt%
    \fi%
  \else%
    \pgffor@skip=\pgffor@last pt%
    \pgffor@iter=\pgffor@prevlast pt%
    \advance\pgffor@skip by-\pgffor@iter%
  \fi%
  \pgffor@iter=\pgffor@last pt%
  % do loop
  \pgffor@loop%
}

\def\pgffor@loop{%
  \advance\pgffor@iter by\pgffor@skip%
  \let\pgffor@next=\pgffor@doloop%
  \ifdim\pgffor@skip<0pt%
    \ifdim\pgffor@iter<\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \else%
    \ifdim\pgffor@iter>\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \fi%
  \ifpgffor@continue%
  \else%
    \let\pgffor@next=\pgffor@endloop% done!
  \fi%
  \pgffor@next%
}

\def\pgffor@endloop{%
  \pgffor@scan%
}

{\catcode`\p=12\catcode`\t=12\gdef\Pgffor@geT#1pt{#1}}

\def\pgffor@doloop{%
  \begingroup%
    \edef\pgffor@temp{\expandafter\Pgffor@geT\the\pgffor@iter}%
    \edef\pgffor@incheck{{.0/}{\pgffor@temp/}}%
    \expandafter\in@\pgffor@incheck%
    \ifin@%
      \expandafter\pgffor@strip\pgffor@temp%
    \fi%
    \expandafter\in@\expandafter/\expandafter{\pgffor@var}%
    \ifin@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@temp//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
      \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@temp}%
    \fi%
    \expandafter\pgffor@beginhook\pgffor@body\pgffor@endhook%
  \endgroup%
  \pgffor@loop%  
}

\def\pgffor@strip#1.0{\def\pgffor@temp{#1}}


\def\breakforeach{\global\pgffor@continuefalse}
  
\endinput


==> pgflibraryplothandlers.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryplothandlers.code.tex,v 1.9 2007/03/09 17:49:32 tantau Exp $

\newif\ifpgf@plot@started


% This handler converts each plot stream command into a curveto
% command, except for the first, which is converted to the previously
% specified action.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfsetlinetofirstplotpoint
% \pgfplothandlercurveto
% \pgfplotxyfile{mytable}

\def\pgfplothandlercurveto{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@initial%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgf@plot@curveto@handler@finish%
    \global\pgf@plot@startedfalse%
  }%
}

\def\pgf@plot@curveto@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@plot@first@action{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@curveto@first{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plot@curveto@first@support=\pgf@plot@curveto@first%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@second%
}

\def\pgf@plot@curveto@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@second{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@third%
  \global\pgf@plot@startedtrue%
}

\def\pgf@plot@curveto@handler@third#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@curveto@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@curveto@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@curveto@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@curveto@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@curveto@first=\pgf@plot@curveto@second%
  \global\let\pgf@plot@curveto@second=\pgf@plot@curveto@current%
  \xdef\pgf@plot@curveto@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}

\def\pgf@plot@curveto@handler@finish{%
  \ifpgf@plot@started%
    \pgfpathcurveto{\pgf@plot@curveto@first@support}{\pgf@plot@curveto@second}{\pgf@plot@curveto@second}%
  \fi%
}


% This commands sets the tension for smoothing of plots.
%
% #1 = tension of curves. A value of 1 will yield a circle when the
%      control points are at quarters of a circle. A smaller value
%      will result in a tighter curve. Default is 0.5. 
%
% Example:
%
% \pgfsetplottension{0.2}

\def\pgfsetplottension#1{%
  \pgf@x=#1pt\relax%
  \pgf@x=0.2775\pgf@x\relax%
  \edef\pgf@plottension{\pgf@sys@tonumber\pgf@x}}
\pgfsetplottension{0.5}


% This handler converts the plot stream command into a curveto
% command that is closed using a closepath.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfplothandlerclosedcurve
% \pgfplotxyfile{mytable}

\def\pgfplothandlerclosedcurve{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@initial%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgf@plot@closedcurve@handler@finish%
  }%
}

\def\pgf@plot@closedcurve@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@closedcurve@initial{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@second%
  \global\pgf@plot@startedfalse%
}

\def\pgf@plot@closedcurve@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@after@initial{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  {\pgfpathmoveto{}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@third%
}

\def\pgf@plot@closedcurve@handler@third#1{%
  \global\pgf@plot@startedtrue%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@initial}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@after@initial}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@after@initial%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@after@initial@presupport{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@fourth%
}

\def\pgf@plot@closedcurve@handler@fourth#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@second%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}

\def\pgf@plot@closedcurve@handler@finish{%
  \ifpgf@plot@started
    %
    % first, draw line from 2nd last to last:
    %
    \pgf@process{\pgf@plot@closedcurve@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@first}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@second}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
    {\pgf@marshal}%
    \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    %
    % second, draw line from last point to start:
    %
    \pgf@process{\pgf@plot@closedcurve@after@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@second}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@initial}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@initial}}%
    {\pgf@marshal}%
    %
    % third, draw line from first to second point:
    %
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgf@plot@closedcurve@after@initial@presupport}{\noexpand\pgf@plot@closedcurve@after@initial}}%
    {\pgf@marshal}%
    \pgfpathclose%
  \fi%
}





% This handler converts each point in a stream into a line from the
% $y$-axis to the given points coordinate, resulting in a
% ``comb.'' 
%
% Example:
%
% \pgfplothandlerxcomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerxcomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@xcomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@xcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}


% This handler converts each point in a stream into a line from the
% $x$-axis straight up to the given points coordinate, resulting in a
% ``comb.'' 
%
% Example:
%
% \pgfplothandlerycomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerycomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@ycomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@ycomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}






% This handler converts each point in a stream into a line from the
% origin to the point's coordinate, resulting in a ``star''.
%
% Example:
%
% \pgfplothandlerpolarcomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerpolarcomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@polarcomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@polarcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfpointorigin}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}




% This handler draws a given mark at each point. 
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
%
% Example:
%
% \pgfplothandlermark{\pgfuseplotmark{*}}
% \pgfplotxyfile{mytable}

\def\pgfplothandlermark#1{%
  \pgf@plothandlermark{%
    \ifnum\pgf@plot@mark@count<\pgf@plot@mark@repeat\relax%
    \else%
      \global\pgf@plot@mark@count=0\relax%
      #1%
    \fi%
    }%
}

\newcount\pgf@plot@mark@count
\def\pgf@plot@mark@phase{0}

\def\pgf@plothandlermark#1{%
  \def\pgf@plot@mark{#1}%
  \def\pgf@plotstreamstart{%
    \global\pgf@plot@mark@count=\pgf@plot@mark@repeat\relax%
    \global\advance\pgf@plot@mark@count by-\pgf@plot@mark@phase\relax%
    \global\let\pgf@plotstreampoint=\pgf@plot@mark@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@mark@handler#1{%
  \global\advance\pgf@plot@mark@count by1\relax%
  {\pgftransformshift{#1}\pgf@plot@mark}%
}


% Set the repeat count for marks. For example, if 3 is given as a
% value, only every third point will get a mark.
%
% #1 = repeat count
%
% Example:
%
% \pgfsetplotmarkrepeat{2}

\def\pgfsetplotmarkrepeat#1{\def\pgf@plot@mark@repeat{#1}}
\pgfsetplotmarkrepeat{1}


% Set the phase for marks. For example, if 3 is the repeat and 3 is 
% the phase, already the first point will be marked. 
%
% #1 = the index of the first point that should be marked.
%
% Example:
%
% \pgfsetplotmarkphase{3}

\def\pgfsetplotmarkphase#1{\def\pgf@plot@mark@phase{#1}}
\pgfsetplotmarkphase{1}



% This handler draws a given mark at those points whose number is
% given in the (pgffor-like) list.
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
% #2 = list of positions like "1,2,4,...,9,10"
%
% Example:
%
% \pgfplothandlermarklisted{\pgfuseplotmark{*}}{1,2,4,...,9}
% \pgfplotxyfile{mytable}

\def\pgfplothandlermarklisted#1#2{%
  \let\pgf@plot@mark@list=\pgfutil@empty%
  \edef\pgf@marshal{\noexpand\foreach\noexpand\pgf@temp in{#2}}
  \pgf@marshal{\xdef\pgf@plot@mark@list{\pgf@plot@mark@list(\pgf@temp)}}%
  \pgf@plothandlermark{%
    \edef\pgf@marshal{\noexpand\pgfutil@in@{(\the\pgf@plot@mark@count)}{\pgf@plot@mark@list}}%
    \pgf@marshal%
    \ifpgfutil@in@#1\fi}%
}


% Define a new plot mark for use with \pgfplotmark.
%
% #1 = a plot mark mnemonic
% #2 = code for drawing the mark
%
% Example:
%
% \pgfdeclareplotmark{*}{\pgfpathcircle{\pgfpointorigin}{2pt}\pgfusepathqfill}

\def\pgfdeclareplotmark#1#2{\expandafter\def\csname pgf@plot@mark@#1\endcsname{#2}}


% Set the size of plot marks. For circles, this will be the radius,
% for other shapes it should be about half the width/height.
%
% Example:
%
% \pgfsetplotmarksize{1pt}

\def\pgfsetplotmarksize#1{\pgfmathsetlength\pgfplotmarksize{#1}}

\newdimen\pgfplotmarksize
\pgfplotmarksize=2pt


% Insert a plot mark's code at the origin.
%
% #1 = plot mark mnemonic
%
% Example:
%
% \pgfuseplotmark{*}

\def\pgfuseplotmark#1{\csname pgf@plot@mark@#1\endcsname}


% A stroke-filled circle mark

\pgfdeclareplotmark{*}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfusepathqfillstroke
}


% A plus-sign like mark

\pgfdeclareplotmark{+}
{%
  \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfusepathqstroke
}


% An x-shaped mark

\pgfdeclareplotmark{x}
{%
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfusepathqstroke
}

% See pgflibraryplotmarks for more plot marks






\endinput


==> pgflibrarysnakes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarysnakes.code.tex,v 1.15 2007/03/09 17:49:32 tantau Exp $


\newdimen\pgfsnakesegmentamplitude
\newdimen\pgfsnakesegmentlength
\def\pgfsnakesegmentangle{45}
\def\pgfsnakesegmentobjectlength{\pgfsnakesegmentamplitude}
\def\pgfsnakesegmentaspect{0.5}

\pgfsnakesegmentlength=10pt
\pgfsnakesegmentamplitude=2.5pt



% snake snake
%
% This snake produces a hopefully optically pleasing squiggly snake. 
%
% Parameters: \pgfsnakesegmentamplitude, \pgfsnakesegmentlength

\pgfdeclaresnake{snake}{initial}
{
  \state{initial}[switch if less than=+.625\pgfsnakesegmentlength to final,
                  width=+.3125\pgfsnakesegmentlength,
                  next state=down]
  { 
    \pgfpathcurveto
    {\pgfqpoint{.125\pgfsnakesegmentlength}{0pt}}
    {\pgfqpoint{.1875\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    {\pgfqpoint{.3125\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
  }
  \state{down}[switch if less than=+.8125\pgfsnakesegmentlength to end down,
               width=+.5\pgfsnakesegmentlength,
               next state=up]
  {
    \pgfpathcosine{\pgfqpoint{.25\pgfsnakesegmentlength}{-1\pgfsnakesegmentamplitude}}
    \pgfpathsine{\pgfqpoint{.25\pgfsnakesegmentlength}{-1\pgfsnakesegmentamplitude}}
  }               
  \state{up}[switch if less than=+.8125\pgfsnakesegmentlength to end up,
             width=+.5\pgfsnakesegmentlength,
             next state=down]
  {
    \pgfpathcosine{\pgfqpoint{.25\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    \pgfpathsine{\pgfqpoint{.25\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
  }               
  \state{end down}[width=+.3125\pgfsnakesegmentlength,
                   next state=final]
  {
    \pgfpathcurveto
    {\pgfqpoint{.125\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    {\pgfqpoint{.1875\pgfsnakesegmentlength}{0pt}}
    {\pgfqpoint{.3125\pgfsnakesegmentlength}{0pt}}
  }  
  \state{end up}[width=+.3125\pgfsnakesegmentlength,
                 next state=final]
  {
    \pgfpathcurveto
    {\pgfqpoint{.125\pgfsnakesegmentlength}{-\pgfsnakesegmentamplitude}}
    {\pgfqpoint{.1875\pgfsnakesegmentlength}{0pt}}
    {\pgfqpoint{.3125\pgfsnakesegmentlength}{0pt}}
  }  
  \state{final}
  { \pgfpathlineto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}} }
}




% zigzag snake
%
% Parameters: \pgfsnakesegmentamplitude, \pgfsnakesegmentlength

\pgfdeclaresnake{zigzag}{up}
{
  \state{up}[width=+.5\pgfsnakesegmentlength,%
             next state=down]
  {
    \pgfpathlineto{\pgfqpoint{.25\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{.5\pgfsnakesegmentlength}{0pt}}
  }
  \state{down}[width=+.5\pgfsnakesegmentlength,%
               next state=up]
  {
    \pgfpathlineto{\pgfqpoint{.25\pgfsnakesegmentlength}{-\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{.5\pgfsnakesegmentlength}{0pt}}
  }
  \state{final}
  { \pgfpathlineto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}} }
}



% saw snake
%
% Parameters: \pgfsnakesegmentamplitude, \pgfsnakesegmentlength

\pgfdeclaresnake{saw}{initial}
{
  \state{initial}[width=+\pgfsnakesegmentlength]
  {
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentlength}{0pt}}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}


% coil snake
%
% Parameters: \pgfsnakesegmentamplitude, \pgfsnakesegmentlength,

\pgfdeclaresnake{coil}{coil}
{
  \state{coil}[switch if less than=%
    1.5\pgfsnakesegmentlength+%
    \pgfsnakesegmentaspect\pgfsnakesegmentamplitude+%
    \pgfsnakesegmentaspect\pgfsnakesegmentamplitude to last,
               width=+\pgfsnakesegmentlength]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{2    }{-0.555}{7}}
    {\pgfpoint@oncoil{1.555}{-1    }{8}}
    {\pgfpoint@oncoil{1    }{-1    }{9}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{0.445}{-1    }{10}}
    {\pgfpoint@oncoil{0    }{-0.555}{11}}
    {\pgfpoint@oncoil{0    }{ 0    }{12}}
  }
  \state{last}[width=.5\pgfsnakesegmentlength+%
    \pgfsnakesegmentaspect\pgfsnakesegmentamplitude+%
    \pgfsnakesegmentaspect\pgfsnakesegmentamplitude,next state=final]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}

\def\pgfpoint@oncoil#1#2#3{%
  \pgf@x=#1\pgfsnakesegmentamplitude%
  \pgf@x=\pgfsnakesegmentaspect\pgf@x%
  \pgf@y=#2\pgfsnakesegmentamplitude%
  \pgf@xa=0.083333333333\pgfsnakesegmentlength%
  \advance\pgf@x by#3\pgf@xa%
}


% bumps snake
%
% Parameters: \pgfsnakesegmentamplitude, \pgfsnakesegmentlength

\pgfdeclaresnake{bumps}{initial}
{
  \state{initial}[width=+.5\pgfsnakesegmentlength]
  {
    \pgfpathcurveto
    {\pgfqpoint{0pt}{.555\pgfsnakesegmentamplitude}}
    {\pgfqpoint{0.11125\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    {\pgfqpoint{.25\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    \pgfpathcurveto
    {\pgfqpoint{.38875\pgfsnakesegmentlength}{\pgfsnakesegmentamplitude}}
    {\pgfqpoint{.5\pgfsnakesegmentlength}{.5\pgfsnakesegmentamplitude}}
    {\pgfqpoint{.5\pgfsnakesegmentlength}{0\pgfsnakesegmentamplitude}}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}



% expanding waves snake
%
% Parameters: \pgfsnakesegmentangle, \pgfsnakesegmentlength

\pgfdeclaresnake{expanding waves}{initial}
{
  \state{initial}[width=+\pgfsnakesegmentlength,next state=wave]
  {}

  \state{wave}[switch if less than=+\pgfsnakesegmentlength to last,
               width=+\pgfsnakesegmentlength]
  {
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfsnakecompleteddistance}{0pt}}%
      {\pgfpointpolar{\pgfsnakesegmentangle}{+\pgfsnakecompleteddistance}}}%
    \pgfpatharc{\pgfsnakesegmentangle}{-\pgfsnakesegmentangle}{+\pgfsnakecompleteddistance}%
  }
  \state{last}[width=+0pt,next state=final]
  {
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfsnakecompleteddistance}{0pt}}%
      {\pgfpointpolar{\pgfsnakesegmentangle}{+\pgfsnakecompleteddistance}}}%
    \pgfpatharc{\pgfsnakesegmentangle}{-\pgfsnakesegmentangle}{+\pgfsnakecompleteddistance}%
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}



% waves snake
%
% Parameters: \pgfsnakesegmentangle, \pgfsnakesegmentlength

\pgfdeclaresnake{waves}{wave}
{
  \state{wave}[width=\pgfsnakesegmentlength]
  {
    \pgftransformxshift{+\pgfsnakesegmentlength}
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfsnakesegmentobjectlength}{0pt}}%
      {\pgfpointpolar{\pgfsnakesegmentangle}{+\pgfsnakesegmentobjectlength}}}%
    \pgfpatharc{\pgfsnakesegmentangle}{-\pgfsnakesegmentangle}{+\pgfsnakesegmentobjectlength}%
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}


% triangle snakes
%
% Parameters: \pgfsnakesegmentlength, \pgfsnakeobjectsize, \pgfsnakesegmentamplitude

\pgfdeclaresnake{triangles}{triangle}
{
  \state{triangle}[switch if less than=+\pgfsnakesegmentlength to last,
                   width=+\pgfsnakesegmentlength]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentobjectlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfsnakesegmentamplitude}}
    \pgfpathclose
  }
  \state{last}[width=+\pgfsnakesegmentobjectlength,next state=final]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentobjectlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfsnakesegmentamplitude}}
    \pgfpathclose
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}



% crosses snakes
%
% Parameters: \pgfsnakesegmentlength, \pgfsnakeobjectsize, \pgfsnakesegmentamplitude

\pgfdeclaresnake{crosses}{crosses}
{
  \state{crosses}[switch if less than=+\pgfsnakesegmentlength to last,
                   width=+\pgfsnakesegmentlength]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentobjectlength}{-\pgfsnakesegmentamplitude}}
    \pgfpathmoveto{\pgfqpoint{0pt}{-\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentobjectlength}{\pgfsnakesegmentamplitude}}
  }
  \state{last}[width=\pgfsnakesegmentobjectlength,next state=final]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentobjectlength}{-1\pgfsnakesegmentamplitude}}
    \pgfpathmoveto{\pgfqpoint{0pt}{-\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfsnakesegmentobjectlength}{\pgfsnakesegmentamplitude}}
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}



% ticks snakes
%
% Parameters: \pgfsnakesegmentlength, \pgfsnakesegmentamplitude

\pgfdeclaresnake{ticks}{ticks}
{
  \state{ticks}[width=+\pgfsnakesegmentlength]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfsnakesegmentamplitude}}
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfsnakesegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfsnakesegmentamplitude}}
    \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}


% border snake
%
% Parameters: \pgfsnakesegmentlength, \pgfsnakesegmentamplitude, \pgfsnakesegmentangle

\pgfdeclaresnake{border}{tick}
{
  \state{tick}[switch if less than=+\pgfsnakesegmentlength to last,
               width=+\pgfsnakesegmentlength]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpointpolar{\pgfsnakesegmentangle}{+\pgfsnakesegmentamplitude}}
  }
  \state{last}[width=+\pgfsnakesegmentamplitude,next state=final]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpointpolar{\pgfsnakesegmentangle}{+\pgfsnakesegmentamplitude}}
  }  
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
}




% brace snakes
%
% Parameters: \pgfsnakesegmentamplitude

\pgfdeclaresnake{brace}{brace}
{
  \state{brace}[width=+\pgfsnakeremainingdistance,next state=final]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathcurveto
    {\pgfqpoint{.15\pgfsnakesegmentamplitude}{.3\pgfsnakesegmentamplitude}}
    {\pgfqpoint{.5\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
    {\pgfqpoint{\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
    {
      \pgftransformxshift{+\pgfsnakesegmentaspect\pgfsnakeremainingdistance}
      \pgfpathlineto{\pgfqpoint{-\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{-.5\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
      {\pgfqpoint{-.15\pgfsnakesegmentamplitude}{.7\pgfsnakesegmentamplitude}}
      {\pgfqpoint{0\pgfsnakesegmentamplitude}{1\pgfsnakesegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{.15\pgfsnakesegmentamplitude}{.7\pgfsnakesegmentamplitude}}
      {\pgfqpoint{.5\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
      {\pgfqpoint{\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
    }
    {
      \pgftransformxshift{+\pgfsnakeremainingdistance}
      \pgfpathlineto{\pgfqpoint{-\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{-.5\pgfsnakesegmentamplitude}{.5\pgfsnakesegmentamplitude}}
      {\pgfqpoint{-.15\pgfsnakesegmentamplitude}{.3\pgfsnakesegmentamplitude}}
      {\pgfqpoint{0pt}{0pt}}
    }
  }
  \state{final}
  {}
}



% bent snake
%
% A snake that looks like someone bent the line a bit.
%
% Parameters: \pgfsnakesegmentamplitude, \pgfsnakesegmentaspect

\pgfdeclaresnake{bent}{bent}
{
  \state{bent}[width=+\pgfsnakeremainingdistance,next state=final]
  {
    \pgfpathcurveto
    {\pgfqpoint{\pgfsnakesegmentaspect\pgfsnakeremainingdistance}{\pgfsnakesegmentamplitude}}
    {\pgfpointadd{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
       {\pgfqpoint{-\pgfsnakesegmentaspect\pgfsnakeremainingdistance}{\pgfsnakesegmentamplitude}}}
    {\pgfqpoint{\pgfsnakeremainingdistance}{0pt}}
  }
  \state{final}
  {}
}



\endinput


==> pgflibrarytikzmatrix.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzmatrix.code.tex,v 1.5 2007/01/08 10:42:19 tantau Exp $


% A matrix of nodes contains a node in each cell.

\tikzstyle{matrix of nodes}=[%
   matrix,%
   cells={anchor=base},%
   nodes={%
     execute at begin node=,%
     execute at end node=,
     name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn%
   },
   execute at begin cell=\tikz@lib@matrix@start@cell,%
   execute at end cell=\tikz@lib@matrix@end@cell,%
   execute at empty cell=\tikz@lib@matrix@empty@cell
]

\def\tikz@lib@matrix@empty@cell{\iftikz@lib@matrix@empty\node{};\fi}

\newif\iftikz@lib@matrix@plain

\def\tikz@lib@matrix@start@cell{%
  \pgfutil@ifnextchar|{\tikz@lib@matrix@with@options}{\tikz@lib@matrix@normal@start@cell}}

\def\tikz@lib@matrix@with@options|#1|{\tikz@lib@matrix@plainfalse\node#1\bgroup}


\def\tikz@lib@matrix@normal@start@cell{\pgfutil@ifnextchar\let{\tikz@lib@matrix@check}{\tikz@lib@matrix@plainfalse\node\bgroup}}%

\def\tikz@lib@matrix@check#1{% evil hackery to find out about start of path
  \pgfutil@ifnextchar\tikz@signal@path{\tikz@lib@matrix@plaintrue\let}{\tikz@lib@matrix@plainfalse\node\bgroup\let}%
}
  
\def\tikz@lib@matrix@end@cell{%
  \iftikz@lib@matrix@plain%
  \else%
    \expandafter\egroup\expandafter;%
  \fi%    
}

% Fill empty nodes in a matrix of nodes

\newif\iftikz@lib@matrix@empty

\tikzoption{nodes in empty cells}[true]{\csname tikz@lib@matrix@empty#1\endcsname}


% Same as a matrix of nodes, but switch on math mode in each cell
\tikzstyle{matrix of math nodes}=[%
  matrix of nodes,
  nodes={%
   execute at begin node=$,%
   execute at end node=$%
  }%
]



% Provide a delimiter

\tikzoption{left delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south east}%
    {south west}%
    {every delimiter,every left delimiter}%
    {south}%
    {north}%
    {#1}%
    {.}%
    {\pgf@y}}}

\tikzoption{right delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south west}%
    {south east}%
    {every delimiter,every right delimiter}%
    {south}%
    {north}%
    {.}%
    {#1}%
    {\pgf@y}}}

\tikzoption{above delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south east}%
    {north west}%
    {every delimiter,every above delimiter,rotate=-90}%
    {west}%
    {east}%
    {#1}%
    {.}%
    {\pgf@x}}}

\tikzoption{below delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south west}%
    {south west}%
    {every delimiter,every below delimiter,rotate=-90}%
    {west}%
    {east}%
    {.}%
    {#1}%
    {\pgf@x}}}

\def\tikz@delimiter#1#2#3#4#5#6#7#8{%
  \bgroup
    \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name}%
    node[outer sep=0pt,inner sep=0pt,draw=none,fill=none,anchor=#1,at=(\tikz@last@fig@name.#2),#3]
    {%
      {\nullfont\pgf@process{\pgfpointdiff{\pgfpointanchor{\tikz@last@fig@name}{#4}}{\pgfpointanchor{\tikz@last@fig@name}{#5}}}}%
      $\left#6\vcenter{\hrule height .5#8 depth .5#8 width0pt}\right#7$%
    }
    \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}%
  \egroup%
}

\tikzstyle{every delimiter}=[]
\tikzstyle{every left delimiter}=[]
\tikzstyle{every right delimiter}=[]
\tikzstyle{every above delimiter}=[]
\tikzstyle{every below delimiter}=[]

\endinput


==> pgflibrarytikzsnakes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikzsnakes.code.tex,v 1.2 2006/10/11 15:22:26 tantau Exp $

\usepgflibrary{snakes}

\endinput


==> pgflibrarytikztopaths.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarytikztopaths.code.tex,v 1.7 2007/06/07 07:41:11 tantau Exp $


% Straight to

\tikzstyle{line to}=                 [to path={-- (\tikztotarget) \tikztonodes}]


% Curved to

\tikzstyle{every curve to}=          []
\tikzstyle{curve to}=                [to path=\tikz@to@curve@path]

\tikzoption{bend angle}{\def\tikz@to@bend{#1}}

\tikzoption{bend left}[]{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \def\tikz@to@bend{#1}%
  \fi%
  \let\tikz@to@out=\tikz@to@bend%
  \c@pgf@counta=180\relax%
  \advance\c@pgf@counta by-\tikz@to@out\relax%
  \edef\tikz@to@in{\the\c@pgf@counta}%
  \tikz@to@switch@on%
  \tikz@to@relativetrue%
}

\tikzoption{bend right}[]{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \def\tikz@to@bend{#1}%
  \fi%
  % Now, negate
  \c@pgf@counta=\tikz@to@bend\relax%
  \c@pgf@counta=-\c@pgf@counta\relax%
  \edef\tikz@to@out{\the\c@pgf@counta}%
  \c@pgf@counta=180\relax%
  \advance\c@pgf@counta by-\tikz@to@out\relax%
  \edef\tikz@to@in{\the\c@pgf@counta}%
  \tikz@to@switch@on%
  \tikz@to@relativetrue%
}

\tikzoption{relative}[true]{\csname tikz@to@relative#1\endcsname}
\newif\iftikz@to@relative
\tikz@to@relativefalse

\tikzoption{in}{\def\tikz@to@in{#1}\tikz@to@switch@on}
\tikzoption{out}{\def\tikz@to@out{#1}\tikz@to@switch@on}

\tikzoption{in looseness}{\tikz@to@set@in@looseness{#1}}
\tikzoption{out looseness}{\tikz@to@set@out@looseness{#1}}
\tikzoption{looseness}{\tikz@to@set@in@looseness{#1}\tikz@to@set@out@looseness{#1}}

\tikzoption{in control}{\tikz@to@set@in@control{#1}}
\tikzoption{out control}{\tikz@to@set@out@control{#1}}
\tikzoption{controls}{\tikz@to@parse@controls#1\pgf@stop}

\tikzoption{in min distance}{\tikz@to@set@distances{#1}{}{}{}}
\tikzoption{in max distance}{\tikz@to@set@distances{}{#1}{}{}}
\tikzoption{in distance}{\tikz@to@set@distances{#1}{#1}{}{}}
\tikzoption{out min distance}{\tikz@to@set@distances{}{}{#1}{}}
\tikzoption{out max distance}{\tikz@to@set@distances{}{}{}{#1}}
\tikzoption{out distance}{\tikz@to@set@distances{}{}{#1}{#1}}
\tikzoption{min distance}{\tikz@to@set@distances{#1}{}{#1}{}}
\tikzoption{max distance}{\tikz@to@set@distances{}{#1}{}{#1}}
\tikzoption{distance}{\tikz@to@set@distances{#1}{#1}{#1}{#1}}

\def\tikz@to@set@distances#1#2#3#4{%
  \tikz@to@setifnotempy{#1}{\tikz@to@in@min}{\let\tikz@to@end@compute=\tikz@to@end@compute@looseness}%
  \tikz@to@setifnotempy{#2}{\tikz@to@in@max}{\let\tikz@to@end@compute=\tikz@to@end@compute@looseness}%
  \tikz@to@setifnotempy{#3}{\tikz@to@out@min}{\let\tikz@to@start@compute=\tikz@to@start@compute@looseness}%
  \tikz@to@setifnotempy{#4}{\tikz@to@out@max}{\let\tikz@to@start@compute=\tikz@to@start@compute@looseness}%
  \tikz@to@switch@on%
}

\def\tikz@to@setifnotempy#1#2#3{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty\else\def#2{#1}#3\fi%
}


\def\tikz@to@set@in@looseness#1{%
  \def\tikz@to@in@looseness{#1}%
  \let\tikz@to@end@compute=\tikz@to@end@compute@looseness%
  \tikz@to@switch@on%
}
\def\tikz@to@set@out@looseness#1{%
  \def\tikz@to@out@looseness{#1}%
  \let\tikz@to@start@compute=\tikz@to@start@compute@looseness%
  \tikz@to@switch@on%
}

\def\tikz@to@parse@controls#1and#2\pgf@stop{\tikz@to@set@in@control{#2}\tikz@to@set@out@control{#1}}

\def\tikz@to@set@in@control#1{%
  \def\tikz@to@in@control{#1}%
  \let\tikz@to@end@compute=\tikz@to@end@compute@control%
  \tikz@to@switch@on%
}
\def\tikz@to@set@out@control#1{%
  \def\tikz@to@out@control{#1}%
  \let\tikz@to@start@compute=\tikz@to@start@compute@control%
  \tikz@to@switch@on%
}


\def\tikz@to@bend{30}

\def\tikz@to@out{45}
\def\tikz@to@in{135}

\def\tikz@to@out@looseness{1}
\def\tikz@to@in@looseness{1}

\def\tikz@to@in@min{0pt}
\def\tikz@to@in@max{10000pt}
\def\tikz@to@out@min{0pt}
\def\tikz@to@out@max{10000pt}

\def\tikz@to@switch@on{\let\tikz@to@path=\tikz@to@curve@path}

\def\tikz@to@curve@path{%
  [every curve to]
  \pgfextra{\iftikz@to@relative\tikz@to@compute@relative\else\tikz@to@compute\fi}
  \tikz@computed@path
  \tikztonodes%
}

\def\tikz@to@modify#1#2{%
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {}%
  {\edef#1{#1.#2}}
}%

\def\tikz@to@compute{%
  \let\tikz@tofrom=\tikztostart%
  \let\tikz@toto=\tikztotarget%
  \tikz@to@modify\tikz@tofrom\tikz@to@out%
  \tikz@to@modify\tikz@toto\tikz@to@in%
  \ifx\tikz@to@start@compute\tikz@to@start@compute@looseness%
    \tikz@to@compute@distance%
  \else%
    \ifx\tikz@from@start@compute\tikz@to@start@compute@looseness%  
      \tikz@to@compute@distance%
    \fi%
  \fi%
  \tikz@to@start@compute%
  \tikz@to@end@compute%
  \edef\tikz@computed@path{.. controls \tikz@computed@start and \tikz@computed@end .. (\tikz@toto)}
}

\def\tikz@to@compute@distance{\tikz@scan@one@point\tikz@@to@compute@distance(\tikz@tofrom)}
\def\tikz@@to@compute@distance#1{%
  \def\tikz@first@point{#1}%
  \tikz@scan@one@point\tikz@@@to@compute@distance(\tikz@toto)}
\def\tikz@@@to@compute@distance#1{%
  \def\tikz@second@point{#1}%
  \tikz@to@compute@distance@main%
}
\def\tikz@to@compute@distance@main{%
  \pgf@process{\pgfpointdiff{\tikz@first@point}{\tikz@second@point}}%
  \ifdim\pgf@x<0pt\pgf@xa=-\pgf@x\else\pgf@xa=\pgf@x\fi%
  \ifdim\pgf@y<0pt\pgf@ya=-\pgf@y\else\pgf@ya=\pgf@y\fi%
  % 
  % Calculate length of second to first vector:
  % 
  \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
  \ifdim\pgf@x>\pgf@y%
    \c@pgf@counta=\pgf@x%
    \ifnum\c@pgf@counta=0\relax%
    \else%
      \divide\c@pgf@counta by 255\relax%
      \pgf@xa=16\pgf@xa\relax%
      \divide\pgf@xa by\c@pgf@counta%
      \pgf@xa=16\pgf@xa\relax%
    \fi%
  \else%
    \c@pgf@counta=\pgf@y%
    \ifnum\c@pgf@counta=0\relax%
    \else%
      \divide\c@pgf@counta by 255\relax%
      \pgf@ya=16\pgf@ya\relax%
      \divide\pgf@ya by\c@pgf@counta%
      \pgf@xa=16\pgf@ya\relax%
    \fi%
  \fi%
  \pgf@x=0.3915\pgf@xa%
  \pgf@xa=\tikz@to@out@looseness\pgf@x%
  \pgf@xb=\tikz@to@in@looseness\pgf@x%
  % Adjust as necessary
  \pgfmathsetlength{\pgf@ya}{\tikz@to@out@min}
  \ifdim\pgf@xa<\pgf@ya%
    \pgf@xa=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@out@max}
  \ifdim\pgf@xa>\pgf@ya%
    \pgf@xa=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@in@min}
  \ifdim\pgf@xb<\pgf@ya%
    \pgf@xb=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@in@max}
  \ifdim\pgf@xb>\pgf@ya%
    \pgf@xb=\pgf@ya%
  \fi%
}

\def\tikz@to@start@compute@looseness{%
  \edef\tikz@computed@start{([shift=(\tikz@to@out:\the\pgf@xa)]\tikz@tofrom)}%
}
\def\tikz@to@end@compute@looseness{%
  \edef\tikz@computed@end{([shift=(\tikz@to@in:\the\pgf@xb)]\tikz@toto)}%
}
\def\tikz@to@start@compute@control{%
  \let\tikz@computed@start=\tikz@to@out@control%
}
\def\tikz@to@end@compute@control{%
  \let\tikz@computed@end=\tikz@to@in@control%
}

\let\tikz@to@start@compute=\tikz@to@start@compute@looseness%
\let\tikz@to@end@compute=\tikz@to@end@compute@looseness%




% Relative curves

\def\tikz@to@compute@relative{%
  \tikz@scan@one@point\tikz@@to@compute@relative(\tikztostart)%
}
\def\tikz@@to@compute@relative#1{%
  \def\tikz@tofrom{#1}%
  \tikz@scan@one@point\tikz@@@to@compute@relative(\tikztotarget)%
}
\def\tikz@@@to@compute@relative#1{%
  \def\tikz@toto{#1}%
  \begingroup
    % 
    % Adjust start and target so that they lie on the border in the
    % rotated coordinate system.
    %  
    \pgfutil@ifundefined{pgf@sh@ns@\tikztostart}
    {%
      \let\tikz@first@point=\tikz@tofrom%
      \let\tikz@tostart@tikz=\pgfutil@empty
    }%
    {%
      % Start computation of new start.
      {%
        \tikz@tofrom%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        {%
          \pgftransformreset%
          \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgftransformrotate{\tikz@to@out}%
          \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
          \pgf@process{\pgfpointtransformed{\tikz@toto}}%
        }%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgfpointshapeborder{\tikztostart}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
        \xdef\tikz@tofrom@smuggle{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      }%
      \let\tikz@first@point=\tikz@tofrom@smuggle%
      \tikz@first@point%
      \edef\tikz@tostart@tikz{(\the\pgf@x,\the\pgf@y)}%
    }%
    \pgfutil@ifundefined{pgf@sh@ns@\tikztotarget}
    {%
      \let\tikz@second@point=\tikz@toto%
    }%
    {%
      % Start computation of new target.
      {%
        \tikz@toto%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        {%
          \pgftransformreset%
          \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgftransformrotate{180}%
          \pgftransformrotate{\tikz@to@in}%
          \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
          \pgf@process{\pgfpointtransformed{\tikz@tofrom}}%
        }%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgfpointshapeborder{\tikztotarget}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
        \xdef\tikz@toto@smuggle{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      }%
      \let\tikz@second@point=\tikz@toto@smuggle%
    }%
    \tikz@second@point%
    \edef\tikz@totarget@tikz{(\the\pgf@x,\the\pgf@y)}%
    %
    % Compute distances
    %
    \tikz@to@compute@distance@main%
    \edef\tikz@to@first@distance{\the\pgf@xa}%
    \edef\tikz@to@second@distance{\the\pgf@xb}%
    %
    % Next step: Establish a transformed coordinate system so that the (modified)
    % start is at the origin and the (modified) target is at (1,0)
    %
    \pgftransformreset%
    \pgf@process{\tikz@first@point}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@second@point}%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgfpointnormalised{}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@xb=-\pgf@x%
    \pgf@yb=-\pgf@y%
    %
    % Now compute the control points.
    %
    {%
      \pgftransformshift{\tikz@first@point}%
      \pgftransformcm{\pgf@sys@tonumber\pgf@xc}{\pgf@sys@tonumber\pgf@yc}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xc}%
                      {\pgfpointorigin}%
      \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@to@out}{\tikz@to@first@distance}}}%
      \xdef\tikz@computed@start{(\the\pgf@x,\the\pgf@y)}%
    }
    {%
      \pgftransformshift{\tikz@second@point}%
      \pgftransformcm{\pgf@sys@tonumber\pgf@xc}{\pgf@sys@tonumber\pgf@yc}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xc}%
                      {\pgfpointorigin}%
      \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@to@in}{\tikz@to@second@distance}}}%
      \xdef\tikz@computed@end{(\the\pgf@x,\the\pgf@y)}%
    }
    \xdef\tikz@computed@path{
      \tikz@tostart@tikz
      .. controls \tikz@computed@start and \tikz@computed@end ..
      \tikz@totarget@tikz}%
  \endgroup
}



% Loops

\tikzstyle{loop}=                    [to path={
  \pgfextra{\let\tikztotarget=\tikztostart}
  [looseness=8,min distance=5mm,every loop]
  \tikz@to@curve@path
  }]

\tikzstyle{every loop}=              [->,shorten >=1pt]

\tikzstyle{loop right}=              [right,out=15,in=-15,loop]
\tikzstyle{loop above}=              [above,out=105,in=75,loop]
\tikzstyle{loop left}=               [left,out=195,in=165,loop]
\tikzstyle{loop below}=              [below,out=285,in=255,loop]





\endinput


==> pgfmath.code.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\input pgfmathcalc.code.tex


==> pgfmathbase.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file provides basic macros for converting between bases.
%
% Version 0.0 08/03/2007

% \pgfmathbasetodec
%
% Convert a representation of an integer from 
% the spcified base to base 10.
%
% #1 - a macro to store the result.
% #2 - the representation of a number (i.e. not a register)
% #3 - the current base.
%
% e.g.
%
% \pgfmathbasetodec\mynumber{10111}{2}
%
% \mynumber <- 23
%
\def\pgfmathbasetodec#1#2#3{%
	\pgfmath@checknumber{#2}%
	\pgfmath@checkbase{#3}%
	\def\pgfmath@base{#3}%
	\def\pgfmath@macro{#1}%
	\c@pgfmath@counta1\relax%
	\def\pgfmath@reversed{}%
	\expandafter\pgfmathbasetodec@#2\pgfmathbasetodec}
	
\def\pgfmathbasetodec@#1{%
	\ifx\pgfmathbasetodec#1%
		\c@pgfmath@countb0%
		\divide\c@pgfmath@counta by\pgfmath@base\relax%
		\expandafter\pgfmathbasetodec@@%
	\else%
		\edef\pgfmath@reversed{\pgfmath@reversed#1}%
		\expandafter\multiply\expandafter\c@pgfmath@counta\pgfmath@base\relax%
		\expandafter\pgfmathbasetodec@%
	\fi}

\def\pgfmathbasetodec@@{\expandafter\pgfmathbasetodec@@@\pgfmath@reversed\pgfmathbasetodec}
	
\def\pgfmathbasetodec@@@#1{%
	\ifx\pgfmathbasetodec#1\relax%
		\expandafter\edef\pgfmath@macro{\the\c@pgfmath@countb}%
		\let\pgfmath@next\pgfmathbasetodec@@@@%
	\else%
		\chardef\pgfmath@charnum`#1\relax%
		\c@pgfmath@countc\pgfmath@charnum%
		\ifnum\c@pgfmath@countc>96\relax%
			\advance\c@pgfmath@countc-87\relax%
		\else
			\ifnum\c@pgfmath@countc>64\relax%
				\advance\c@pgfmath@countc-55\relax%
			\else
				\advance\c@pgfmath@countc-48\relax%
		\fi\fi%
		\ifnum\c@pgfmath@countc<\pgfmath@base\relax%
			\multiply\c@pgfmath@countc\c@pgfmath@counta\relax%
			\advance\c@pgfmath@countb\c@pgfmath@countc%
			\divide\c@pgfmath@counta by\pgfmath@base\relax%
			\let\pgfmath@next\pgfmathbasetodec@@@%
		\else
			\pgfmath@error{Digit `#1' invalid for base \pgfmath@base}%
			\let\pgfmath@next\relax%
		\fi%	
	\fi%
	\pgfmath@next}
\def\pgfmathbasetodec@@@@{%
	\expandafter\pgfmath@ensurenumberlength\expandafter{\pgfmath@macro}%
}

% \pgfmathdectobase
%
% Convert a representation of an integer from 
% base 10 to the spcified base. Letters for bases
% greater than 10 are in lowercase.
%
% #1 - a macro to store the result.
% #2 - a number in base 10 (in a macro, not a register)
% #3 - the required base.
%
% e.g.
%
% \pgfmathdectobase\mynumber{127}{16}
%
% \mynumber <- 7f
%
\def\pgfmathdectobase#1#2#3{%
	\pgfmath@checknumber{#2}%
	\pgfmath@checkbase{#3}%
	\c@pgfmath@counta#2\relax%
	\def#1{}%
	\pgfmathloop
		\ifnum\c@pgfmath@counta>0\relax%
			\c@pgfmath@countb\c@pgfmath@counta%
			\divide\c@pgfmath@countb#3\relax%
			\multiply\c@pgfmath@countb-#3\relax%
			\advance\c@pgfmath@countb\c@pgfmath@counta%
			\edef#1{\csname pgfmath@lowercase digit@\the\c@pgfmath@countb\endcsname#1}%
			\divide\c@pgfmath@counta#3\relax%
	\repeatpgfmathloop%
	\pgfmath@ensurenumberlength{#1}}

% \pgfmathdectoBase
%
% Convert a representation of an integer from 
% base 10 to the spcified base. Letters for bases
% greater than 10 are in uppercase.
%
% #1 - a macro to store the result.
% #2 - a number in base 10 (in a macro, not a register)
% #3 - the required base.
%
% e.g.
%
% \pgfmathdectoBase\mynumber{127}{16}
%
% \mynumber <- 7F
%	
\def\pgfmathdectoBase#1#2#3{%
	\pgfmath@checkbase{#3}%
	\pgfmath@checknumber{#2}%
	\c@pgfmath@counta#2\relax%
	\def#1{}%
	\pgfmathloop
		\ifnum\c@pgfmath@counta>0\relax%
			\c@pgfmath@countb\c@pgfmath@counta%
			\divide\c@pgfmath@countb#3\relax%
			\multiply\c@pgfmath@countb-#3\relax%
			\advance\c@pgfmath@countb\c@pgfmath@counta%
			\edef#1{\csname pgfmath@uppercase digit@\the\c@pgfmath@countb\endcsname#1}%
			\divide\c@pgfmath@counta#3\relax%
	\repeatpgfmathloop%
	\pgfmath@ensurenumberlength{#1}}

\def\pgfmath@createdigits{%
	\def\pgfmath@digitstyle{lowercase digit}%
	\c@pgfmath@counta0\relax%
	\pgfmath@createdigits@0123456789abcdefghijklmnopqrstuvwxyz\pgfmath@createdigits%
	\def\pgfmath@digitstyle{uppercase digit}%
	\c@pgfmath@counta0\relax%
	\pgfmath@createdigits@0123456789ABCDEFGHIJKLMNOPQRSTUVWXYZ\pgfmath@createdigits}

\def\pgfmath@createdigits@#1{%
	\ifx\pgfmath@createdigits#1\relax%
	\else%
		\expandafter\pgfmath@def\expandafter{\pgfmath@digitstyle}{\the\c@pgfmath@counta}{#1}%
		\advance\c@pgfmath@counta1\relax%
		\expandafter\pgfmath@createdigits@%
	\fi}
\pgfmath@createdigits

% \pgfmathbasetobase
%
% Convert a representation of an integer from 
% between the specified bases. Letters for target
% bases greater than 10 are in lppercase.
%
% #1 - a macro to store the result.
% #2 - a number (in a macro, not a register)
% #3 - the source base.
% #4 - the target base.
%
% e.g.
%
% \pgfmathbasetobase\mynumber{4321}{5}{9}
%
% \mynumber <- 721
%	
\def\pgfmathbasetobase#1#2#3#4{%
	\pgfmathbasetodec{\pgfmath@temp}{#2}{#3}%
	\pgfmathdectobase{#1}{\pgfmath@temp}{#4}
}

% \pgfmathbasetobase
%
% Convert a representation of an integer from 
% between the specified bases. Letters for target
% bases greater than 10 are in lppercase.
%
% #1 - a macro to store the result.
% #2 - a number (in a macro, not a register)
% #3 - the source base.
% #4 - the target base.
%
% e.g.
%
% \pgfmathbasetobase\mynumber{1234}{5}{12}
%
% \mynumber <- 142
%	
\def\pgfmathbasetoBase#1#2#3#4{%
	\pgfmathbasetodec{\pgfmath@temp}{#2}{#3}%
	\pgfmathdectoBase{#1}{\pgfmath@temp}{#4}
}

\def\pgfmath@checkbase#1{%
	\ifnum#1<2\relax%
		\pgfmath@error{Cannot process numbers in base `#1'.}%
	\else%
		\ifnum#1>36\relax%
			\pgfmath@error{Cannot process numbers in base `#1'.}%
	\fi\fi}
	
\def\pgfmath@checknumber#1{%
	\expandafter\pgfmath@checknumber@#1\pgfmath@}
\def\pgfmath@checknumber@#1#2\pgfmath@{%
	\ifx#1-%
		\pgfmath@error{Cannot process negative numbers.}%
	\fi}


% \pgfmath@ensurenumberlength
%
% Internal macro for making a representation of a number have
% a specific length, byt prefixing zeros to the number.
%
% #1 - a macro contatining a representation of an integer.
% #2 - the number of digits to ensure.
%
% e.g.
%
% \foo <- 7FF
%
% \pgfmathsetnumberlength{8}%
% \pgfmath@ensurenumberlength\foo
%
% \foo <- 000007FF
%
\def\pgfmath@ensurenumberlength#1{%
	\def\pgfmath@tempa{#1}%
	\expandafter\c@pgfmath@counta\pgfmath@basenumberlength\relax%
	\expandafter\pgfmath@ensurenumberlength@#1\pgfmath@ensurenumberlength}
\def\pgfmath@ensurenumberlength@#1{%
	\ifx\pgfmath@ensurenumberlength#1\relax%
		\expandafter\pgfmath@ensurenumberlength@@%
	\else%
		\advance\c@pgfmath@counta-1\relax%
		\expandafter\pgfmath@ensurenumberlength@
	\fi}

\def\pgfmath@ensurenumberlength@@{%
	\edef\pgfmath@tempb{\pgfmath@tempa}%
	\pgfmath@ensurenumberlength@@@}
\def\pgfmath@ensurenumberlength@@@{%
	\ifnum\c@pgfmath@counta>0\relax%
		\advance\c@pgfmath@counta-1\relax%
		\edef\pgfmath@tempb{0\pgfmath@tempb}%
		\expandafter\pgfmath@ensurenumberlength@@@%
	\fi%
	\expandafter\edef\pgfmath@tempa{\pgfmath@tempb}}
	
\def\pgfmathsetbasenumberlength#1{\def\pgfmath@basenumberlength{#1}}
\pgfmathsetbasenumberlength{1}%

==> pgfmathcalc.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file loads all the parsing, functions and operator stuff
%
% Version 0.0 08/03/2007

\input pgfmathutil.code.tex
\input pgfmathparser.code.tex
\input pgfmathoperations.code.tex
\input pgfmathbase.code.tex


% \pgfmathsetlength, \pgfmathaddtolength
%
% #1 = dimension register
% #2 = expression
%
% Description:
%
% These functions work similar to \setlength and \addtolength. Only,
% they allow #2 to contain an expression, which is evaluated before
% assignment. Furthermore, the font is setup before the assignment is
% done, so that dimensions like 1em are evaluated correctly.
%
% If #2 starts with "+", then a simple assignment is done (but the
% font is still setup). This is orders of magnitude faster than a
% parsed assignment.

\def\pgfmathsetlength#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
 {%
 	 % Ok, quick version:
 	 \begingroup%
 	 	\pgfutil@selectfont%
    	\pgfmath@x#2\unskip%
    	\pgfmath@returnone\pgfmath@x%
    \endgroup%
    #1\pgfmathresult pt\relax%
  }%
  {%
   \pgfmathparse{#2}#1\pgfmathresult pt\relax%
}%
}
\def\pgfmathaddtolength#1#2{%
	 \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
  	\begingroup%
  		\pgfutil@selectfont%
  		\pgfmath@x#1\relax%
  		\advance\pgfmath@x#2\unskip%
  		\pgfmath@returnone\pgfmath@x%
    \endgroup%
    #1\pgfmathresult pt\relax%
  }%
  {\pgfmathparse{#2}\advance#1\pgfmathresult pt\relax}%
}

% Not really needed and does not work in plain TeX:
%\def\pgfmathnewcounter#1{%
%	\expandafter\let\expandafter\pgfmath@register\csname c@#1\endcsname%
%	\expandafter\ifx\pgfmath@register\relax%
%    	\expandafter\newcount\csname c@#1\endcsname%
%    	\csname c@#1\endcsname0\relax%
%		\expandafter\def\csname the#1\endcsname{\expandafter\the\csname c@#1\endcsname}%
%	\else% Do nothing.
%   \fi}%
   
% \pgfmathsetcounter, \pgfmathaddtocounter
%
% Results of parsing are truncated.
%
\def\pgfmathsetcounter#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \csname c@#1\endcsname=#2\relax%
  }%
  {%
    \pgfmath@ifundefined{c@#1}{\pgfmath@error{No counter named '#1' is known}{}}{%
      \pgfmathparse{#2}%
      \afterassignment\pgfmath@gobbletilpgfmath@%
      \csname c@#1\endcsname\pgfmathresult\relax\pgfmath@%
    }%
  }%
}

\def\pgfmathaddtocounter#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \advance\csname c@#1\endcsname by#2\relax%
  }%
  {%
    \pgfmath@ifundefined{c@#1}{\pgfmath@error{No counter named '#1' is known}{}}{%
      \edef\pgfmath@addtocountertemp{\expandafter\the\csname c@#1\endcsname}%
      \pgfmathparse{#2}%
      \afterassignment\pgfmath@gobbletilpgfmath@%
      \csname c@#1\endcsname\pgfmathresult\relax\pgfmath@%
      \expandafter\advance\csname c@#1\endcsname\pgfmath@addtocountertemp%
    }%
  }%
}

% \pgfmathsetcount, \pgfmathaddtocount
%
% Results of parsing are truncated.
%
\def\pgfmathsetcount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    #1#2\relax%
  }%
  {%
    \pgfmathparse{#2}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1\pgfmathresult\relax\pgfmath@%
  }%
}

\def\pgfmathaddtocount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \advance#1 by#2\relax%
  }%
  {%
    \edef\pgfmath@addtocounttemp{\the#1}%
    \pgfmathparse{#2}%
     \afterassignment\pgfmath@gobbletilpgfmath@%
     #1\pgfmathresult\relax\pgfmath@%
     \advance#1\pgfmath@addtocounttemp%
  }%
}

\def\pgfmathsetmacro#1#2{%
	\expandafter\pgfmath@onquick#2\pgfmath@%
  {%
  		\begingroup%
    		\afterassignment\pgfmath@gobbletilpgfmath@%
    		\pgfmath@x#2pt\relax\pgfmath@%
    		\edef#1{\pgfmath@tonumber{\pgfmath@x}}%
    		\pgfmath@smuggleone{#1}
    	\endgroup%
  }%
  {%
    \pgfmathparse{#2}%
    \edef#1{\pgfmathresult}%
  }%
}

\def\pgfmathtruncatemacro#1#2{%
	\expandafter\pgfmath@onquick#2\pgfmath@%
  {%
  		\begingroup%
    		\afterassignment\pgfmath@gobbletilpgfmath@%
    		\c@pgfmath@counta#2\relax\pgfmath@%
    		\edef#1{\the\c@pgfmath@counta}%
    		\pgfmath@smuggleone{#1}
    	\endgroup%
  }%
  {%
    \pgfmathparse{#2}%
    \edef#1{\pgfmathresult}%
  }%
}

% Check whether a given parameter starts with quick.
%
% The command should be followed by nonempty text, ending with
% \pgfmath@ as a stop-token. Then should follow
%
% #1 = code to execute if text starts with +
% #2 = code to execute if text does not
%
% Example:
%
% \pgfmath@onquick+0pt\pgfmath@{is quick}{is slow}

\def\pgfmath@onquick{%
  \afterassignment\pgfmath@afterquick%
  \let\pgfmath@next=%
}

\def\pgfmath@afterquick#1\pgfmath@{%
  \ifx\pgfmath@next+%
    \expandafter\pgfmath@firstoftwo%
  \else%
    \expandafter\pgfmath@secondoftwo%
  \fi%
}

==> pgfmathoperations.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the mathematical functions and operators.
%
% Version 0.0 08/03/2007

% This file defines the mathematical functions and operators.
%
% Adding/redefining extra operators/functions:
%
% Each operator/function XXX has two forms:
%
%
% \pgfmathXXX#1...   a public version which evaluates any
%                    arguments passed to it and passes the
%                    results on to...
%
% \pgfmathXXX@#1...  a non-public version which performs 
%                    required calculation on arguments which
%                    must have already been evaluated (i.e.
%                    *without* dimensions).
% 
% If a function XXX is to be included in the parser, it is 
% recommended, for consistency, that where possible, the 
% pgfmathparser file should define the macro \pgfmath@parseXXX.
% The parser should (ideally) then call \pgfmathXXX@.
%
% It is recommend that the pgfmath versions of the pgf dimension
% and count registers be used, i.e., \pgfmath@x for \pgfmath@x, 
% \c@pgfmath@counta for c@pgfmath@counta, and so on. These are currently
% \let to their pgf equivalents, but it may be necessary to change 
% this.
%
% It is also recommened that all calculations (where necessary)
% take place within a TeX group. \pgfmath@returnone#1 makes and
% expanded version of #1 global and stores this in \pgfmathresult 
% after the group is ended.
%

\input pgfmathtrig.code.tex% Load the trig. stuff.
\input pgfmathrnd.code.tex%  Load the random stuff.


% \pgfmathadd
%
% Add #1 and #2.
%
\def\pgfmathadd#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@adda{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@addb{\pgfmathresult}%
	\pgfmathadd@{\pgfmath@adda}{\pgfmath@addb}}
\def\pgfmathadd@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\advance\pgfmath@x by\pgfmath@y%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathsubtract
%
% Subtract #2 from #1.
%
\def\pgfmathsubtract#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@subtracta{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@subtractb{\pgfmathresult}%
	\pgfmathsubtract@{\pgfmath@subtracta}{\pgfmath@subtractb}}

\def\pgfmathsubtract@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\advance\pgfmath@x by-\pgfmath@y%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathmultiply
%
% Multiply #1 by #2.
%
\def\pgfmathmultiply#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@multiplya{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@multiplyb{\pgfmathresult}%
	\pgfmathmultiply@{\pgfmath@multiplya}{\pgfmath@multiplyb}}
\def\pgfmathmultiply@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@x#2\pgfmath@x%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathdivide
%
% Divide #1 by #2.
%
\def\pgfmathdivide#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@dividea{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@divideb{\pgfmathresult}%
	\pgfmathdivide@{\pgfmath@dividea}{\pgfmath@divideb}}
\def\pgfmathdivide@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		% If #2 is an integer use TeX arithmatic.
		\expandafter\pgfmath@xa#2pt\relax%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@xa\relax%
		\ifdim\pgfmath@xa=0pt\relax%
			\ifnum\c@pgfmath@counta=0\relax%
			\pgfmath@error{Division by zero.}{}%
		\fi%
			\divide\pgfmath@x\c@pgfmath@counta%
		\else%
			\pgfmathreciprocal@{#2}%
			\pgfmath@x=\pgfmathresult\pgfmath@x%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathgreaterthan
%
% 1.0 if #1 > #2. Otherwise 0.0
%
\def\pgfmathgreaterthan#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@greaterthana{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@greaterthanb{\pgfmathresult}%
	\pgfmathgreaterthan@{\pgfmath@greaterthana}{\pgfmath@greaterthanb}}
\def\pgfmathgreaterthan@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\advance\pgfmath@x-\pgfmath@y%
		\ifdim\pgfmath@x>0pt\relax%
			\pgfmath@x1pt\relax%
		\else%
			\pgfmath@x0pt\relax%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathlessthan
%
% 1.0 if #1< #2. Otherwise 0.0
%
\def\pgfmathlessthan#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@lessthana{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@lessthanb{\pgfmathresult}%
	\pgfmathlessthan@{\pgfmath@lessthana}{\pgfmath@lessthanb}}
\def\pgfmathlessthan@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\advance\pgfmath@x-\pgfmath@y\relax%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x1pt\relax%
		\else%
			\pgfmath@x0pt\relax%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathequalto
%
% 1.0 if #1 = #2. Otherwise 0.0
%
\def\pgfmathequalto#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@equaltoa{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@equaltob{\pgfmathresult}%
	\pgfmathadd@{\pgfmath@equaltoa}{\pgfmath@equaltob}}
\def\pgfmathequalto@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\advance\pgfmath@x-\pgfmath@y%
		\ifdim\pgfmath@x=0pt\relax%
			\pgfmath@x1pt\relax%
		\else%
			\pgfmath@x0pt\relax%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathreciprocal
%
% 1 / #1
%
\def\pgfmathreciprocal#1{%
	\pgfmathparse{#1}%
	\pgfmathreciprocal@{\pgfmathresult}}
\def\pgfmathreciprocal@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x=0pt\relax%
			\pgfmath@error{Division by zero.}{}%
		\fi%
		\edef\pgfmath@reciprocaltemp{\pgfmath@tonumber{\pgfmath@x}}%
		\expandafter\pgfmathreciprocal@@\pgfmath@reciprocaltemp00000\pgfmath@}
\def\pgfmathreciprocal@@#1.#2#3#4#5#6#7\pgfmath@{%
		\c@pgfmath@counta#2#3#4#5#6\relax%
		% If the number is an integer, use TeX arithmatic.
		\ifnum\c@pgfmath@counta=0\relax%
			\pgfmath@x1pt\relax%
			\divide\pgfmath@x#1\relax%
		\else%
			\c@pgfmath@counta#1#2#3#4#5#6\relax%
			\c@pgfmath@countb1000000000\relax%
			\divide\c@pgfmath@countb\c@pgfmath@counta%
			\c@pgfmath@counta\c@pgfmath@countb%
			\divide\c@pgfmath@counta10000\relax%
			\pgfmath@x\c@pgfmath@counta pt\relax%
			\multiply\c@pgfmath@counta-10000\relax%
			\advance\c@pgfmath@countb\c@pgfmath@counta%
			\pgfmath@y\c@pgfmath@countb pt\relax%
			\pgfmath@y.1\pgfmath@y% Yes! This way is more accurate. Go figure...
			\pgfmath@y.1\pgfmath@y%	
			\pgfmath@y.1\pgfmath@y%	
			\pgfmath@y.1\pgfmath@y%			
			\advance\pgfmath@x\pgfmath@y%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup
}

	
% \pgfmathabs
%
% Calculate |#1|
%
\def\pgfmathabs#1{%
	\pgfmathparse{#1}%
	\pgfmathabsolute@{\pgfmathresult}}
\def\pgfmathabs@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x=-\pgfmath@x%
		\fi%
	\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathmod
%
% Calculate #1 mod #2.
%
\def\pgfmathmod#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@moda{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@modb{\pgfmathresult}%
	\pgfmathmod@{\pgfmath@mod@a}{\pgfmath@modb}%
}
\def\pgfmathmod@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@xa\pgfmath@x%
		\expandafter\pgfmath@xb#2pt\relax%
		\c@pgfmath@counta=\pgfmath@xa%
		\c@pgfmath@countb=\pgfmath@xb%
		\divide\c@pgfmath@counta\c@pgfmath@countb%
		\multiply\pgfmath@xb\c@pgfmath@counta%
		\advance\pgfmath@x-\pgfmath@xb%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathsqrt
%
% Square-root of #1.
%
%
\def\pgfmathsqrt#1{%
	\pgfmathparse{#1}%
	\pgfmathsqrt{\pgfmathresult}}
\def\pgfmathsqrt@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x>9999pt\relax%
			\def\pgfmath@zeros{0}%
			\def\pgfmath@targetiterations{3}%
		\else%
			\ifdim\pgfmath@x>999pt\relax%
				\def\pgfmath@zeros{}%
				\def\pgfmath@targetiterations{2}%
			\else%
				\ifdim\pgfmath@x>99pt\relax%
					\def\pgfmath@zeros{0}%
					\def\pgfmath@targetiterations{2}%
				\else%
					\ifdim\pgfmath@x>9pt\relax%
						\def\pgfmath@zeros{}%
						\def\pgfmath@targetiterations{1}%
					\else%
						\ifdim\pgfmath@x<0pt\relax%
							\pgfmath@error{Cannot calculate the square-root of the negative number `#1'}{}%
						\else%
							\def\pgfmath@zeros{0}%
							\def\pgfmath@targetiterations{1}%
		\fi\fi\fi\fi\fi%
		\edef\pgfmath@temp{\pgfmath@zeros\pgfmath@tonumber{\pgfmath@x}}%
		\expandafter\pgfmath@sqrt@\pgfmath@temp\pgfmath@%
}
\def\pgfmath@sqrt@#1.#2\pgfmath@{\pgfmath@@sqrt@#1#2\pgfmath@empty\pgfmath@empty\pgfmath@}

\def\pgfmath@@sqrt@#1#2{%
		\c@pgfmath@countb#1#2\relax%
		\ifnum\c@pgfmath@countb>35\relax%
			\ifnum\c@pgfmath@countb>63\relax%
				\ifnum\c@pgfmath@countb>80\relax%
					\c@pgfmath@counta9\relax%
				\else%
					\c@pgfmath@counta8\relax%
				\fi%
			\else%
				\ifnum\c@pgfmath@countb>48\relax%
					\c@pgfmath@counta7\relax%
				\else%
					\c@pgfmath@counta6\relax%
				\fi%
			\fi%
		\else%
			\ifnum\c@pgfmath@countb>15\relax%
				\ifnum\c@pgfmath@countb>24\relax%
					\c@pgfmath@counta5\relax%
				\else%
					\c@pgfmath@counta4\relax%
				\fi%
			\else%
				\ifnum\c@pgfmath@countb>3\relax%
					\ifnum\c@pgfmath@countb>8\relax%
						\c@pgfmath@counta3\relax%
					\else%
						\c@pgfmath@counta2\relax%
					\fi%
				\else%
					\ifnum\c@pgfmath@countb>0\relax%
						\c@pgfmath@counta1\relax%
					\else%
						\c@pgfmath@counta0\relax%
					\fi%
				\fi%
			\fi%
		\fi%
		\edef\pgfmath@root{\the\c@pgfmath@counta}%
		\edef\pgfmath@rootspecial{\the\c@pgfmath@counta}%
		\multiply\c@pgfmath@counta-\c@pgfmath@counta\relax%
		\advance\c@pgfmath@counta#1#2\relax%
		\edef\pgfmath@remainder{\the\c@pgfmath@counta}%
		\pgfmath@@@sqrt@%
}

\def\pgfmath@@@sqrt@#1#2{%
		\ifx\pgfmath@empty#1%
			\edef\pgfmath@remainder{\pgfmath@remainder00}%
			\def\pgfmath@tokens{\pgfmath@empty\pgfmath@empty}%
		\else%
			\ifx\pgfmath@empty#2%
				\edef\pgfmath@remainder{\pgfmath@remainder#10}%
				\def\pgfmath@tokens{\pgfmath@empty\pgfmath@empty}%
			\else%
				\edef\pgfmath@remainder{\pgfmath@remainder#1#2}%
				\def\pgfmath@tokens{}%
		\fi\fi%
		\c@pgfmath@counta\pgfmath@rootspecial\relax%
		\multiply\c@pgfmath@counta20\relax%
		\c@pgfmath@countb\c@pgfmath@counta%
		\multiply\c@pgfmath@countb6\relax%
		\advance\c@pgfmath@countb36\relax%
		\c@pgfmath@countc\c@pgfmath@counta\relax%
		\multiply\c@pgfmath@countc2\relax%
		\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax% 
			\advance\c@pgfmath@countb-\c@pgfmath@countc%
			\advance\c@pgfmath@countb-20\relax%
			\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
				\advance\c@pgfmath@countb-\c@pgfmath@countc%
				\advance\c@pgfmath@countb-12\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\advance\c@pgfmath@countb-\c@pgfmath@counta%
					\advance\c@pgfmath@countb-3\relax%
					\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
						\def\pgfmath@digit{0}%
					\else%
						\def\pgfmath@digit{1}%
					\fi%
				\else%
					\advance\c@pgfmath@countb\c@pgfmath@counta%
					\advance\c@pgfmath@countb5\relax%
					\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
						\def\pgfmath@digit{2}%
					\else%
						\def\pgfmath@digit{3}%
					\fi%
				\fi%
			\else%
				\advance\c@pgfmath@countb\c@pgfmath@counta%
				\advance\c@pgfmath@countb9\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\def\pgfmath@digit{4}%
				\else%
					\def\pgfmath@digit{5}%
				\fi%
			\fi%
		\else%
			\advance\c@pgfmath@countb\c@pgfmath@countc%
			\advance\c@pgfmath@countb28\relax%
			\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
				\advance\c@pgfmath@countb-\c@pgfmath@counta%
				\advance\c@pgfmath@countb-15\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\def\pgfmath@digit{6}%
				\else%
					\def\pgfmath@digit{7}%
				\fi%
			\else%
				\advance\c@pgfmath@countb\c@pgfmath@counta%
				\advance\c@pgfmath@countb17\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\def\pgfmath@digit{8}%
				\else%
					\def\pgfmath@digit{9}%
				\fi%
			\fi%
		\fi%
		\edef\pgfmath@rootspecial{\pgfmath@rootspecial\pgfmath@digit}%
		\advance\c@pgfmath@counta\pgfmath@digit\relax%
		\multiply\c@pgfmath@counta-\pgfmath@digit\relax%
		\advance\c@pgfmath@counta\pgfmath@remainder\relax%
		\edef\pgfmath@remainder{\the\c@pgfmath@counta}%
		\c@pgfmath@counta\pgfmath@targetiterations\relax%
		\advance\c@pgfmath@counta-1\relax%
		\edef\pgfmath@targetiterations{\the\c@pgfmath@counta}%
		\ifnum\c@pgfmath@counta=0\relax%
			\edef\pgfmath@root{\pgfmath@root.\pgfmath@digit}%
		\else%
			\edef\pgfmath@root{\pgfmath@root\pgfmath@digit}%
		\fi%
		\ifnum\c@pgfmath@counta=-4\relax%
			\let\pgfmath@next\pgfmath@sqrt@end%
		\else%
			\let\pgfmath@next\pgfmath@@@sqrt@%
		\fi%
		\expandafter\pgfmath@next\pgfmath@tokens%
}

\def\pgfmath@sqrt@end#1\pgfmath@{%
		\edef\pgfmathresult{\pgfmath@root}%
		\pgfmath@smuggleone\pgfmathresult%
	\endgroup}

% \pgfmathpow
%
% Calculates #1 ^ #2
%
% #2 is expected to be an integer.
%
\def\pgfmathpow#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@powera{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@powerb{\pgfmathresult}%
	\pgfmathpow@{\pgfmath@powera}{\pgfmath@powerb}}
\def\pgfmathpow@#1#2{%
	\begingroup%
		\expandafter\pgfmath@xa#1pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta#2\relax\pgfmath@
		% If #2 is negative, take the reciprocal of #1
		% and the absolute value of #2, and carry on.
		%
		\ifnum\c@pgfmath@counta<0\relax%
			\c@pgfmath@counta-\c@pgfmath@counta%
			\pgfmathreciprocal@{#1}%
			\pgfmath@xa\pgfmathresult pt\relax%
		\fi%
		\pgfmath@x=1pt\relax%
		\pgfmathloop%
			\ifnum\c@pgfmath@counta>0\relax%
				\ifodd\c@pgfmath@counta%
					\pgfmath@x\pgfmath@tonumber{\pgfmath@x}\pgfmath@xa%
				\fi
				\ifnum\c@pgfmath@counta>1\relax%
					\pgfmath@xa=\pgfmath@tonumber{\pgfmath@xa}\pgfmath@xa%
				\fi%
				\divide\c@pgfmath@counta by 2\relax%
		\repeatpgfmathloop%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}	


% \pgfmathround
% 
% Half-up rounding.
%
\def\pgfmathround#1{%
	\pgfmathparse{#1}%
	\pgfmathround@{\pgfmathresult}}
\def\pgfmathround@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		\pgfmath@xb\pgfmath@x%
		\ifdim\pgfmath@xb<0pt\relax%
			\ifdim\pgfmath@xa<0.5pt\relax%
			\else%
				\advance\c@pgfmath@counta-1\relax%
			\fi%
		\else%
			\ifdim\pgfmath@xa<0.5pt\relax%
			\else%
				\advance\c@pgfmath@counta1\relax%
			\fi%
		\fi%
		\pgfmath@returnone\c@pgfmath@counta%
	\endgroup%
}%

% \pgfmathfloor
% 
% Floor function.
%
\def\pgfmathfloor#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathfloor@\expandafter{\pgfmathresult}}
\def\pgfmathfloor@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\pgfmath@x\c@pgfmath@counta pt\relax%
		\pgfmath@returnone\pgfmath@x%
	\endgroup
}%

% \pgfmathceil
% 
% Ceiling function.
%
\def\pgfmathceil#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathceil@\expandafter{\pgfmathresult}}
\def\pgfmathceil@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\pgfmath@y\pgfmath@x%
		\advance\pgfmath@y-\c@pgfmath@counta pt\relax%
		\pgfmath@x\c@pgfmath@counta pt\relax%
		\ifdim\pgfmath@y>0pt\relax%
			\advance\pgfmath@x1pt\relax%
		\fi%
	\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathexp
%
% A Maclaurens expansion for e^#1.
% 0 <= #1 < ln(16384).
%
\def\pgfmathexp#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathexp@\expandafter{\pgfmathresult}}
\def\pgfmathexp@#1{%
	\begingroup%
		\pgfmath@x1pt\relax%
		\pgfmath@xa1pt\relax%
		\pgfmath@xb\pgfmath@x%
		\pgfmathloop%
			\pgfmath@xc\pgfmathcounter pt\relax%
			\c@pgfmath@counta\pgfmath@xc%
			\divide\c@pgfmath@counta65536\relax%
			\pgfmath@xc1pt\relax%
			\divide\pgfmath@xc\c@pgfmath@counta%
			\pgfmath@xa\pgfmath@tonumber{\pgfmath@xc}\pgfmath@xa%
			\expandafter\pgfmath@xa#1\pgfmath@xa%
			\advance\pgfmath@x\pgfmath@xa%
			\ifdim\pgfmath@x=\pgfmath@xb%
			\else%
				\pgfmath@xb\pgfmath@x%
		\repeatpgfmathloop%
	\pgfmath@returnone\pgfmath@x%
	\endgroup%
}



% \pgfmathvectorlength
%
% Calcluate the Eulidean length of a 2D vector.
%
% This based on polynomial approximation co-efficents
% contributed by Rouben Rostamian.
%
% #1 - the x component of the vector.
% #2 - the y component of the vector.
%
% P(x) = c0 + x^2 * (c1 + x^2 * (c2 + x^2 * ( c3 + c4 * x^2)))
\def\pgfmath@cE{-0.01019}
\def\pgfmath@cD{0.04453}
\def\pgfmath@cC{-0.11951}
\def\pgfmath@cB{0.49936}
\def\pgfmath@cA{1.00001}

\def\pgfmathveclen#1#2{%
	\pgfmathparse{#1}\edef\pgfmath@vecx{\pgfmathresult}%
	\pgfmathparse{#2}\edef\pgfmath@vecy{\pgfmathresult}%
	\pgfmathveclen@{\pgfmath@vecx}{\pgfmath@vecy}%
}
\def\pgfmathveclen@#1#2{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\pgfmath@xa\pgfmath@x%
		\ifdim\pgfmath@xa=0pt\relax%
			\pgfmath@xa\pgfmath@y%
		\fi%
		\ifdim\pgfmath@xa=0pt\relax%
		\else%
			\ifdim\pgfmath@x<0pt\relax\pgfmath@x-\pgfmath@x\fi%
			\ifdim\pgfmath@y<0pt\relax\pgfmath@y-\pgfmath@y\fi%
			\ifdim\pgfmath@x>\pgfmath@y%
				\pgfmath@xa\pgfmath@x%
				\pgfmath@x\pgfmath@y%
				\pgfmath@y\pgfmath@xa%
			\fi%
			% We use a scaling factor to reduce errors.
			\ifdim\pgfmath@y>10000pt\relax%
				\c@pgfmath@counta1500\relax%
			\else%
				\ifdim\pgfmath@y>1000pt\relax%
					\c@pgfmath@counta150\relax%
				\else%
					\ifdim\pgfmath@y>100pt\relax%
						\c@pgfmath@counta50\relax%
					\else%
						\c@pgfmath@counta1\relax%
					\fi%
				\fi%
			\fi%
			\divide\pgfmath@x by\c@pgfmath@counta\relax%
			\divide\pgfmath@y by\c@pgfmath@counta\relax%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgfmath@y}}%
			\pgfmath@x=\pgfmathresult\pgfmath@x%
			\pgfmath@xa=\pgfmath@tonumber{\pgfmath@x}\pgfmath@x%
			\edef\pgfmath@xsq{\pgfmath@tonumber{\pgfmath@xa}}%
			\pgfmath@x=\pgfmath@cE\pgfmath@xa%
			\advance\pgfmath@x by\pgfmath@cD pt\relax%
			\pgfmath@x=\pgfmath@xsq\pgfmath@x%
			\advance\pgfmath@x by\pgfmath@cC pt\relax%
			\pgfmath@x=\pgfmath@xsq\pgfmath@x%
			\advance\pgfmath@x by\pgfmath@cB pt\relax%
			\pgfmath@x=\pgfmath@xsq\pgfmath@x%
			\advance\pgfmath@x by\pgfmath@cA pt\relax%
			\ifdim\pgfmath@y<0pt\relax%
				\pgfmath@y=-\pgfmath@y%
			\fi%
			\pgfmath@x=\pgfmath@tonumber{\pgfmath@y}\pgfmath@x%
			% Invert the scaling factor.
			\multiply\pgfmath@x by\c@pgfmath@counta\relax%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathmax
%
% Return the maximum of #1 or #2
%
\def\pgfmathmax#1#2{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\pgfmathparse@{#2}\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmax@{\pgfmath@firstoperand}{\pgfmath@secondoperand}}
\def\pgfmathmax@#1#2{%
	\begingroup
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\ifdim\pgfmath@x>\pgfmath@y%
			\pgfmath@returnone\pgfmath@x%
		\else%
			\pgfmath@returnone\pgfmath@y%
		\fi%
	\endgroup}

% \pgfmathmax
%
% Return the minimim of #1 or #2
%
\def\pgfmathmin#1#2{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\pgfmathparse@{#2}\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmin@{\pgfmath@firstoperand}{\pgfmath@secondoperand}}
\def\pgfmathmin@#1#2{%
	\begingroup
		\expandafter\pgfmath@x#1pt\relax%
		\expandafter\pgfmath@y#2pt\relax%
		\ifdim\pgfmath@x<\pgfmath@y%
			\pgfmath@returnone\pgfmath@x%
		\else%
			\pgfmath@returnone\pgfmath@y%
		\fi%
	\endgroup%
}

% \pgfmathscientific
%
% Return the value of #1e#2
%
% e.g. \pgfmathscientific{1.23456789123}{4}
%
% defines \pgfmathresult as 12345.67891
%
% NB This arguments *are not parsed*, as the long mantissa would be lost.
%
\def\pgfmathscientific#1#2{%
	\begingroup%
		\edef\pgfmath@sci@exponent{#2}%
		\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
			\edef\pgfmath@sci@sign{-}%
			\edef\pgfmath@temp{\pgfmath@gobbleone#1}%
		\else%
			\edef\pgfmath@sci@sign{+}%
			\edef\pgfmath@temp{#1}%
		\fi%
		\expandafter\pgfmath@scientific@@\pgfmath@temp00000000000\pgfmath@}

\def\pgfmath@scientific@@#1.#2#3#4#5#6{%
		\edef\pgfmath@sci@int{#1}%
		\edef\pgfmath@sci@mantissaA{#2#3#4#5#6}%
		\pgfmath@scientific@@@}
	
\def\pgfmath@scientific@@@#1#2#3#4#5#6\pgfmath@{%
		\edef\pgfmath@sci@mantissaB{#1#2#3#4#5}%
		\c@pgfmath@counta\pgfmath@sci@exponent\relax%
		\c@pgfmath@countb\c@pgfmath@counta%
		\ifnum\c@pgfmath@counta<0\relax%
			\c@pgfmath@counta-\c@pgfmath@counta%
		\fi%
		\pgfmathpow@{10}{\the\c@pgfmath@counta}%
		\afterassignment\pgfmath@gobbletilpgfmath@
		\c@pgfmath@countc\pgfmathresult\relax\pgfmath@
		\edef\pgfmath@sci@factor{\the\c@pgfmath@countc}%
		\ifnum\c@pgfmath@countb<0\relax%
			% xE-y: easy...
			\pgfmath@x\pgfmath@sci@int.\pgfmath@sci@mantissaA pt\relax%
			\divide\pgfmath@x\pgfmath@sci@factor\relax%
		\else%
			% xE+y: 
			% Must do this way so as not lose digits in a long mantissa. Sigh...
			\c@pgfmath@counta\pgfmath@sci@int%
			\c@pgfmath@countb\pgfmath@sci@mantissaA%
			\multiply\c@pgfmath@counta\pgfmath@sci@factor\relax%
			\multiply\c@pgfmath@countb\pgfmath@sci@factor\relax%
			\c@pgfmath@countc\c@pgfmath@countb%
			\divide\c@pgfmath@countb100000\relax%
			\advance\c@pgfmath@counta\c@pgfmath@countb%
			\multiply\c@pgfmath@countb100000\relax%
			\advance\c@pgfmath@countc-\c@pgfmath@countb%
			\c@pgfmath@countb\pgfmath@sci@mantissaB\relax%
			\multiply\c@pgfmath@countb\pgfmath@sci@factor\relax%
			\divide\c@pgfmath@countb100000\relax%
			\advance\c@pgfmath@countc\c@pgfmath@countb%
			\advance\c@pgfmath@countc100000\relax%
			\edef\pgfmath@sci@result{\pgfmath@sci@sign\the\c@pgfmath@counta.\expandafter\pgfmath@gobbleone\the\c@pgfmath@countc pt}%
			\pgfmath@x\pgfmath@sci@result\relax%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup}

==> pgfmathparser.code.tex <==
% This file parses/evaluates a decimal expression.
%
% (c) 2007 Mark Wibrow
%
% but subject to the LaTeX Project Public License, 
% (http://www.latex-project.org/lppl.txt)
%
% and the GNU Public License,
% (http://www.gnu.org/licenses/gpl.txt)

% \pgfmathparse, \pgfmathqparse
%
% Evaluates a decimal expression.
%
% #1 - the expression.
%
% returns
%
% x = the result as a dimension.
%
% E.g.
% \pgfmathparse{3pt*2cm+1.5}
% \pgfmathqparse{3pt*2cm+1.5pt}
%
% Every number in \pgfmathqparse *must*
% specify a unit.
%
\newif\ifpgfmath@quickparse

\def\pgfmathparse{%
	\pgfmath@quickparsefalse%
	\pgfmathparse@}

\def\pgfmathqparse{%
	\pgfmath@quickparsetrue%
	\pgfmathparse@}
		
\def\pgfmathparse@#1{%
	\begingroup%
    % Reinstall correct font, so that dimensions like 1em are correct
	 \pgfutil@selectfont%
		\edef\pgfmath@temp{#1}%
		\pgfmath@resetparsingparameters%
		\global\pgfmathunitsdeclaredfalse%
		\ifpgfmath@quickparse%
			\let\pgfmath@parseoperand\pgfmath@quickparseoperand%
		\else%
			\let\pgfmath@parseoperand\pgfmath@parseoperand%
		\fi%
		\let\pgfmath@parsepostgroup\pgfmath@parseoperator%
		\expandafter\pgfmath@parse@\pgfmath@temp @@@@@@@@@@@\pgfmath@empty}


% \pgfmath@resetparsingparameters
%
% Reset the stack at the begining of the parse/group.
%
\def\pgfmath@resetparsingparameters{%
	\pgfmath@stack{\pgfmath@empty\pgfmath@empty\pgfmath@empty\pgfmath@empty}%
	\def\pgfmath@stacknextoperator{\pgfmath@empty}% Will not work with \let
}
% \pgfmath@parse@
%
% Start parsing. Expect one of
% 1) the end of the parse
% 2) the start of a group
% 3) a (possible) operand.
%
\def\pgfmath@parse@#1{%
	\def\pgfmath@token{}%
	\ifx#1@%
		\let\pgfmath@parsenext\pgfmath@endparse%
	\else%
		\ifx#1(%
			\let\pgfmath@parsenext\pgfmath@startparsegroup%
		\else%
			\edef\pgfmath@token{#1}%
			\let\pgfmath@parsenext\pgfmath@parseoperand%
	\fi\fi%
	\pgfmath@parsenext%
}

% If no TeX units are declared *at any point* in the parse
% the result is scaled by \pgfmathresultunitscale.
\newif\ifpgfmathunitsdeclared
\def\pgfmathsetresultunitscale#1{\def\pgfmathresultunitscale{#1}}
\def\pgfmathresultunitscale{1}

% \pgfmath@endparse
%
% Everything stops here.
%
\def\pgfmath@endparse#1\pgfmath@empty{%
	\pgfmath@processalloperations%
	\pgfmath@stackpop{\pgfmathresult}%
		\begingroup%
			\ifpgfmathunitsdeclared%
				\pgfmath@x1pt\relax%
			\else%
				\afterassignment\pgfmath@gobbletilpgfmath@%
				\pgfmath@x\pgfmathresultunitscale pt\relax\pgfmath@%
			\fi%
			\expandafter\pgfmath@x\pgfmathresult\pgfmath@x%
			\pgfmath@returnone\pgfmath@x%
		\endgroup%
		\pgfmath@smuggleone{\pgfmathresult}%
	\endgroup%
}

% \pgfmath@startparsegroup
%
% When opening ( is scanned start a new group.
%
\def\pgfmath@startparsegroup{%
	\begingroup%
		\let\pgfmath@parsepostgroup\pgfmath@parseoperator%
		\pgfmath@resetparsingparameters%
		\pgfmath@parse@}

% \pgfmath@endparsegroup
%
% When closing ) is scanned, processes all waiting
% operations (within the group) and close the group.
%
\def\pgfmath@endparsegroup{%
		\pgfmath@processalloperations%
		\pgfmath@stackpop{\pgfmathresult}%
		\expandafter\pgfmath@x\pgfmathresult pt\relax%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
	\pgfmath@parsepostgroup%
}

% \pgfmath@parseoperator
%
% An operator is expected here. 
% Or the end of the parse or parse group.
% 
\def\pgfmath@parseoperator#1{%
	\def\pgfmath@token{}%
	% Push the operand in \pgfmathresult on to the stack. 
	\expandafter\pgfmath@stackpushoperand\expandafter{\pgfmathresult}%
	\ifx#1@%
		\let\pgfmath@parsenext\pgfmath@endparse%
	\else%
		\ifx#1+%
			\let\pgfmath@parsenext\pgfmath@parseadd%
		\else%
			\ifx#1-%
				\let\pgfmath@parsenext\pgfmath@parsesubtract%
			\else%
				\ifx#1*%
					\let\pgfmath@parsenext\pgfmath@parsemultiply%
				\else%
					\ifx#1/%
						\let\pgfmath@parsenext\pgfmath@parsedivide%
					\else
						\ifx#1)%
							\let\pgfmath@parsenext\pgfmath@endparsegroup%
						\else%
							\ifx#1r%
								\let\pgfmath@parsenext\pgfmath@parseradians%
							\else%
								\ifx#1>%
									\let\pgfmath@parsenext\pgfmath@parsegreaterthan%
								\else%
									\ifx#1<%
										\let\pgfmath@parsenext\pgfmath@parselessthan%
									\else%
										\if#1=%
											\let\pgfmath@parsenext\pgfmath@parseequalto%
										\else%
											\if#1^%
												\let\pgfmath@parsenext\pgfmath@parsepower%
											\else%
												\pgfmath@error{Unknown operator `#1'}%
												\let\pgfmath@parsenext\relax%
	\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi%
	\pgfmath@parsenext%
}

% Use a \toks register as a stack.
\newtoks\pgfmath@stack

% \pgfmath@stackpushoperator
% 
% Push an operator (actually its macro e.g., \pgfmathadd@)
% on to the stack. And keep track of it using the macro
% \pgfmath@stacknextoperator.
%
\def\pgfmath@stackpushoperator#1{%
	\edef\pgfmath@temp{\noexpand#1\the\pgfmath@stack}%
	\expandafter\pgfmath@stack\expandafter{\pgfmath@temp}%
	\def\pgfmath@stacknextoperator{#1}}% <- Must \def. Cannot \let.

% \pgfmath@stackpushoperand
%
% Push an operand (i.e. a number) on the stack. It is
% put within a TeX group to make popping a lot simpler.
%
\def\pgfmath@stackpushoperand#1{%
	\edef\pgfmath@temp{{#1}\the\pgfmath@stack}%
	\expandafter\pgfmath@stack\expandafter{\pgfmath@temp}%
}

% \pgfmath@stackpeek
%
% Peek (i.e. without removal) at the top of the stack.
%
\def\pgfmath@stackpeek{\expandafter\pgfmath@stackpeek@\the\pgfmath@stack\pgfmath@}
\def\pgfmath@stackpeek@#1#2\pgfmath@{#1}%

% \pgfmath@stackpop
%
% Pop (i.e. remove) the top of the stack into #1.
%
\def\pgfmath@stackpop#1{\expandafter\pgfmath@stackpop@\expandafter#1\the\pgfmath@stack\pgfmath@}
\def\pgfmath@stackpop@#1#2#3\pgfmath@{\edef#1{#2}\pgfmath@stack{#3}}%

% \pgfmath@stackpopoperation
%
% Remove and perform an operation from the stack.
%
\def\pgfmath@stackpopoperation{%
	\expandafter\pgfmath@stackpopoperation@\the\pgfmath@stack\pgfmath@%
}
\def\pgfmath@stackpopoperation@#1#2#3#4#5\pgfmath@{%
	\ifx\pgfmath@empty#1\relax%
			\pgfmath@stack{\pgfmath@empty\pgfmath@empty\pgfmath@empty\pgfmath@empty}%
	\else%
		\ifx\pgfmath@empty#2\relax%
			\pgfmath@stack{{#1}\pgfmath@empty\pgfmath@empty\pgfmath@empty\pgfmath@empty}%
		\else%
			#2{#3}{#1}%
			\pgfmath@stack{#4#5}%
			\expandafter\pgfmath@stackpushoperand\expandafter{\pgfmathresult}%
	\fi\fi%
	\def\pgfmath@stacknextoperator{#4}}

% \pgfmath@processalloperations
%
% Process all operation in the stack. The 
% overall result is at the top of the stack.
%
\def\pgfmath@processalloperations{%
	\expandafter\pgfutil@in@\pgfmath@stacknextoperator{\pgfmath@empty}%
	\ifpgfutil@in@%
		\let\pgfmath@processnext\relax%		
	\else%
		\pgfmath@stackpopoperation%
		\let\pgfmath@processnext\pgfmath@processalloperations%
	\fi%
	\pgfmath@processnext}

% \pgfmath@processoperationsuntil
%
% Process operations in the stack, until the specified
% operation/s is/are encountered. The overall result is 
% at the top of the stack.
%
\def\pgfmath@processoperationsuntil#1{%
	\expandafter\pgfutil@in@\pgfmath@stacknextoperator{#1\pgfmath@empty}%
	\ifpgfutil@in@%
		\let\pgfmath@processnext\pgfmath@processoperationsuntil@end%		
	\else%
		\pgfmath@stackpopoperation%
		\let\pgfmath@processnext\pgfmath@processoperationsuntil%
	\fi%
	\pgfmath@processnext{#1}}
\def\pgfmath@processoperationsuntil@end#1{}


% OK. Now the operators are parsed.
% These correspond to the + - / * ^ < > = mod and r operators 
%
\def\pgfmath@parseadd{%	
	% If no operator has been assigned (i.e. + is the first operator scanned),
	% do nothing, except add addition to the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Empty the process stack up to any inequalities.
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathadd@}%
	\pgfmath@parse@}
	
\def\pgfmath@parsesubtract{%	
	% If no operator has been assigned (i.e. - is the first operator scanned),
	% do nothing, except add subtract to the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Empty the process stack up to any inequalities.
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathsubtract@}%
	\pgfmath@parse@}
	

\def\pgfmath@parsemultiply{%
	% If no operator has been assigned (i.e. * is the first operator scanned),
	% do nothing, except push multiply onto the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Process all operations up to inequalites or addition/subtraction
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@%
			\pgfmathadd@\pgfmathsubtract@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathmultiply@}%
	\pgfmath@parse@}
	
\def\pgfmath@parsedivide{%
	% If no operator has been assigned (i.e. / is the first operator scanned),
	% do nothing, except push divide onto the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Process all operations up to inequalites or addition/subtraction
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@%
			\pgfmathadd@\pgfmathsubtract@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathdivide@}%
	\pgfmath@parse@}

\def\pgfmath@parsegreaterthan{%
	% On scanning an equality/inequality operator everything up to
	% (but not including) the operator is evaluated... 
	\pgfmath@processalloperations%
	% ...and the operation pushed onto the stack.
	\pgfmath@stackpushoperator{\pgfmathgreaterthan@}%
	\pgfmath@parse@}

\def\pgfmath@parselessthan{%
	\pgfmath@processalloperations%
	\pgfmath@stackpushoperator{\pgfmathlessthan@}%
	\pgfmath@parse@}

\def\pgfmath@parseequalto={%
	\pgfmath@processalloperations%
	\pgfmath@stackpushoperator{\pgfmathequalto@}%
	\pgfmath@parse@}

\def\pgfmath@parsepower{%
	% Easy, just push power onto the stack.
	\pgfmath@stackpushoperator{\pgfmathpow@}%
	\pgfmath@parse@}

\def\pgfmath@parseradians{%
	% Actually this is a post-fix function...
	\ifx\pgfmath@primaryoperation\pgfmath@empty%
	\else%
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@%
			\pgfmathadd@\pgfmathsubtract@}%
	\fi%	
	\pgfmath@stackpop{\pgfmath@temp}%
	\pgfmathdeg@{\pgfmath@temp}%
	% ...so processing returns to \pgfmath@parseoperator
	\pgfmath@parseoperator}
	
\newcount\c@pgfmath@parsecounta
\newcount\c@pgfmath@parsecountb
\newcount\c@pgfmath@parsecountc
\newdimen\pgfmath@parsex

% \pgfmath@quickparseoperand
%
% An operand can *only* be a dimension.
%
\def\pgfmath@quickparseoperand{%
	\afterassignment\pgfmath@quickparseoperand@%
	\pgfmath@parsex\pgfmath@token}
\def\pgfmath@quickparseoperand@{%
	\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}
	\pgfmath@parseoperator%
}
	
% \pgfmath@parseoperand
%
% An operand can be an ASCII number (with or without dimensions, with
% or without a decimal point), a TeX register (count, dimen or skip,
% which may have expanded with \the), or a function e.g. sin(X).
%
% It is assumed that after \edef-ing, the only unexpanded tokens are registers. 
%
\def\pgfmath@parseoperand{%
	\def\pgfmath@sign{}%
	\expandafter\pgfmath@parseoperandsign\pgfmath@token}
\def\pgfmath@parseoperandsign#1{%
	\pgfmath@in@#1{-+}% 
	\ifpgfmath@in@
		% I suppose there are (silly) people who might complain if
		% they can't say 2---5, or 3+-----7. Just for them...
		\edef\pgfmath@sign{\pgfmath@sign#1}%
		\expandafter\pgfmath@parseoperandsign%
	\else%
		\expandafter\pgfmath@parsenumberorfunction\expandafter#1%
	\fi%
}


\newif\ifpgfmath@dimen@

\def\pgfmath@ifregisterdimen@#1\pgfmath@{%
	\pgfmath@in@{p}{#1}%
	\ifpgfmath@in@%
		\pgfmath@dimen@true%
	\else%
		\pgfmath@dimen@false%
	\fi} 	
		

\def\pgfmath@parsenumberorfunction#1{%
  \let\pgfmath@parsenext\pgfmath@parsenumberorfunction@simple%
  \ifx#1\wd\let\pgfmath@parsenext\pgfmath@boxdimen\fi%
  \ifx#1\ht\let\pgfmath@parsenext\pgfmath@boxdimen\fi%
  \ifx#1\dp\let\pgfmath@parsenext\pgfmath@boxdimen\fi%
  \pgfmath@parsenext#1%
}

\def\pgfmath@boxdimen#1#2{%
  \pgfmath@parsex=#1#2%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
  \global\pgfmathunitsdeclaredtrue% a dimension has units 
  \pgfmath@parseoperator%
}

\def\pgfmath@parsenumberorfunction@simple#1{%	
	\expandafter\ifcat#1\relax%
		% So, a TeX register.
		\afterassignment\pgfmath@ifregisterdimen@%
		\pgfmath@parsex\pgfmath@sign#1pt\relax\pgfmath@%
		\ifpgfmath@dimen@% 
			% A dimension! So stop scanning operand here.
			\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
         \global\pgfmathunitsdeclaredtrue% a dimension has units
			\def\pgfmath@temp{}%
			\let\pgfmath@parsenext\pgfmath@parseoperator%
		\else%
			% A count! Expand it, but carry on as usual as it might
			% be immediately followed by a dimension.
			\ifdim\pgfmath@parsex<0pt\relax%
				\edef\pgfmath@sign{\pgfmath@sign-}%
				\pgfmath@parsex-\pgfmath@parsex%
			\fi%
			\edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@parsex}}%
			\let\pgfmath@parsenext\pgfmath@parsenumberorfunction@%
		\fi%
	\else%
		% Could be a number or a function...?
		\edef\pgfmath@temp{#1}%
		\let\pgfmath@parsenext\pgfmath@parsenumberorfunction@%
	\fi%
	\expandafter\pgfmath@parsenext\pgfmath@temp%
}%

\def\pgfmath@parsenumberorfunction@#1{%
	\pgfmath@in@{#1}{.0123456789}%
	\ifpgfmath@in@%
		\let\pgfmath@parsenext\pgfmath@parsenumber%
	\else%
		\let\pgfmath@parsenext\pgfmath@parsefunction%
	\fi%
	\pgfmath@parsenext#1%
}%

\def\pgfmath@parsenumber{% 
	% Consider the number 3.14159
	% 3 is parsed by assignment to a, then '.' is absorbed and 14159
	% parsed by assignement to b (actually b=114159, see below). 
	\c@pgfmath@parsecountc0\relax%
	\afterassignment\pgfmath@parsedecimalpoint%
	\c@pgfmath@parsecounta0}

\def\pgfmath@parsedecimalpoint#1{%
	\ifx#1.% Is there a decimal point? If not, see if there are any units.
		\let\pgfmath@parsenext\pgfmath@parsemantissa%
	\else%
		\c@pgfmath@parsecountb10\relax% The first digit of b is gobbled (see below). 
		\let\pgfmath@parsenext\pgfmath@parseunits%
	\fi%
	\pgfmath@parsenext#1}



% We would like to assign the following number (which is the mantisse)
% to a number. However, for a very long mantisse as in 3.141592653589793238462643
% this will fail since the number becomes too large.
%
% Because of this, we have to do some ``magic'': We scan 9 tokens and
% then do an assignment with a guard after 9 tokens so that the
% assigment cannot fail.
%
\def\pgfmath@parsemantissa.#1#2#3#4#5#6#7#8#9{%
  \afterassignment\pgfmath@checkforguard%    
  % Consider the number: 2.005
  % 2 is assigned to a, but b will be assigned 5, which is *not right*. 
  % So using 1 here hereresults in  b=1005. The first digit is then  
  % gobbled later, when expanded with \the.
  \c@pgfmath@parsecountb1#1#2#3#4#5#6#7#8#9\relax}%

\def\pgfmath@checkforguard{%
  \pgfutil@ifnextchar\relax%
  {%
    % Ok, this is a looong mantisse. Start gobbling all following
    % numbers
    \pgfmath@gobblemantisse%
  }%
  {%
    \pgfmath@removeguard%
  }%
}

\def\pgfmath@gobblemantisse\relax#1#2#3#4#5#6#7#8#9{%
  \afterassignment\pgfmath@checkforguard%
  \c@pgfmath@parsecountc0#1#2#3#4#5#6#7#8#9\relax% these digits are ignored
}

\def\pgfmath@removeguard#1\relax{\pgfmath@parseunits#1}



 
\def\pgfmath@parseunits#1{%
  % Here the extra first digit in b is gobbled. 
  \edef\pgfmath@resulttemp{%
    \pgfmath@sign\the\c@pgfmath@parsecounta.\expandafter\pgfmath@gobbleone\the\c@pgfmath@parsecountb}%
  % Check whether #1 is a \dp, \wd, or \ht
  \let\pgfmath@parsenext=\pgfmath@parseunits@simple%
  \ifx#1\wd\let\pgfmath@parsenext=\pgfmath@parseunits@boxdimen\fi%
  \ifx#1\ht\let\pgfmath@parsenext=\pgfmath@parseunits@boxdimen\fi%
  \ifx#1\dp\let\pgfmath@parsenext=\pgfmath@parseunits@boxdimen\fi%
  \pgfmath@parsenext#1%
}

\def\pgfmath@parseunits@boxdimen#1#2{%
  \pgfmath@parsex=#1#2%
  \pgfmath@parsex\pgfmath@resulttemp\pgfmath@parsex%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
  \global\pgfmathunitsdeclaredtrue% a dimension has units 
  \pgfmath@parseoperator%
}

\def\pgfmath@parseunits@simple#1{%
	% Now check if #1 is actually a register.
	\ifcat#1\relax%
		\afterassignment\pgfmath@ifregisterdimen@%
		\pgfmath@parsex#1pt\relax\pgfmath@%
		\pgfmath@parsex\pgfmath@resulttemp\pgfmath@parsex%
		\ifpgfmath@dimen@% If it's a dimen stop scanning operand here.
                        \global\pgfmathunitsdeclaredtrue% a dimension has units
			\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
			\let\pgfmath@parsenext\pgfmath@parseoperator%
		\else
			\edef\pgfmath@resulttemp{\pgfmath@tonumber{\pgfmath@parsex}}%
			\let\pgfmath@parsenext\pgfmath@parseunits@%
		\fi%
		\expandafter\pgfmath@parsenext%
	\else%
		\expandafter\pgfmath@parseunits@\expandafter#1%
	\fi}

\def\pgfmath@parseunits@#1#2{%
	% Check if #1 is an operator, or the character `@' indicating the end of the parse.
	\pgfmath@in@#1{@+-*/^r<>=()}%
	\ifpgfmath@in@%
		\edef\pgfmath@tokens{#1#2}%
		\edef\pgfmathresult{\pgfmath@resulttemp}%
		\let\pgfmath@parsenext\pgfmath@parseoperator%
	\else%
		\pgfmath@in@#1{Ee}% e+0X
		\ifpgfmath@in@%
			% Oh no! It might be and em or an ex...
			\pgfmath@in@#2{mx}%
			\ifpgfmath@in@%
				\global\pgfmathunitsdeclaredtrue%
				\pgfmath@parsex\pgfmath@resulttemp#1#2\relax%
				\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
				\edef\pgfmath@tokens{}%
				\let\pgfmath@parsenext\pgfmath@parseoperator%
			\else%
				\edef\pgfmath@tokens{#2}%
				\let\pgfmath@parsenext\pgfmath@parsescientific%
			\fi%
		\else
			% Anything else *should* be a TeX unit.
			\global\pgfmathunitsdeclaredtrue%
			\pgfmath@parsex\pgfmath@resulttemp#1#2\relax%
			\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
			\edef\pgfmath@tokens{}%
			\let\pgfmath@parsenext\pgfmath@parseoperator%
	\fi\fi%
	\expandafter\pgfmath@parsenext\pgfmath@tokens%
}

% Parse 'Scientific' notation in the form xEyy
%
\def\pgfmath@parsescientific{%
	\afterassignment\pgfmath@parsescientific@%
	\c@pgfmath@parsecounta}

\def\pgfmath@parsescientific@{%
	\edef\pgfmath@parsesci@temp{\pgfmath@resulttemp\the\c@pgfmath@parsecountc}%
	\expandafter\pgfmathscientific\expandafter{\pgfmath@parsesci@temp}%
		{\the\c@pgfmath@parsecounta}%
	\edef\pgfmath@resulttemp{\pgfmathresult}%
	\pgfmath@parseunits@}

	
% OK. Now the fun stuff. We parse functions here. Note that 
% *no* calulations are done in the following macros. All the
% mathematics is done in pgfmathoperations.code and friends. 
%
% Functions dealt with here are:
%
% round(X)         'half-up' rounding.
% floor(X)         floor function.
% ciel(X)          ceiling function.
% abs(X)           absolute function.
%
% exp(X)           e^X (0 <= X <~= 9.7).
%
% sin(X)           sine function.
% cos(X)           cosine function.
% tan(X)           tan function.
% asin(X)          arcsine of X (in radians)    -1 <= X <= 1
% acos(X)          arccosine of X (in radians)  -1 <= X <= 1
% atan(X)          arctangent of X (in radians) -1 <= X <= 1
% veclen(X,Y)      the length Z where Z^2 = X^2 + Y^2
% mod(X,Y)         X modulo Y
% max(X,Y)         the maximum of X or Y
% min(X,Y)         the minimum of X or Y
%
% NB veclen, mod, max, and min *cannot* be nested.
%
% deg(X)           converts X to degrees (X in radians)
% rad(X)           converts X to radians (X in degrees)
%
% rnd              generate pseudo-random number X (0 <= X <= 1).
% rand             generate pseudo-random number X (1 <= X <= -1).
% sqrt(X)          square root.
% 
% pi               the constant PI.

\def\pgfmath@parsefunction{%
	\def\pgfmath@parsedfunctionname{}%
	\futurelet\pgfmath@parsetoken\pgfmath@parsefunction@@}
\def\pgfmath@parsefunction@@#1{%
	\pgfmath@in@#1{()@+-*/^<>=}% A function name ends with one of these...
	\ifpgfmath@in@%
		\let\pgfmath@parsefunctionnext\pgfmath@parsefunction@end%
	\else%
		\ifx\pgfmath@parsetoken\pgfutil@sptoken% ...or a space.
			\let\pgfmath@parsefunctionnext\pgfmath@parsefunction@end%
		\else%
			\let\pgfmath@parsefunctionnext\pgfmath@parsefunction@continue%
	\fi\fi%
	\pgfmath@parsefunctionnext#1}

\def\pgfmath@parsefunction@end#1{%
	\expandafter\ifx\csname pgfmath@parsefunction@\pgfmath@parsedfunctionname\endcsname\relax%
		\pgfmath@reportunknownfunction%
		\let\pgfmath@parsefunctionnext\relax%
	\else%
		\let\pgfmath@parsefunctionnext\pgfmath@executeparsefunction@%
	\fi%
	\pgfmath@parsefunctionnext#1}

\def\pgfmath@parsefunction@continue#1{%
	\edef\pgfmath@parsedfunctionname{\pgfmath@parsedfunctionname#1}%
	\futurelet\pgfmath@parsetoken\pgfmath@parsefunction@@}
	
\def\pgfmath@executeparsefunction@{\csname pgfmath@parsefunction@\pgfmath@parsedfunctionname\endcsname}
		
		
\def\pgfmath@reportunknownfunction{%
	\pgfmath@error{Unknown function `\pgfmath@parsedfunctionname'}{}%
}

% \pgfmath@postfunction
% 
% In scanning a function e.g. sin(40), we subvert the normal parsing 
% group mechanism by messing around with \pgfmath@parsepostgroup, so 
% that after scanning ), the parser doesn't scan for an operator, but 
% returns to the macros scanning the function. 
% Here the mechanism is restored, and the value of the function is 
% stored along with the approprate sign, which was saved earlier.
%
\def\pgfmath@postfunction{%
	\let\pgfmath@parsepostgroup\pgfmath@parseoperator%
	\edef\pgfmathresult{\pgfmath@sign\pgfmathresult}%
	\pgfmath@parseoperator}
	

% \pgfmath@parsefunction@abs
%
\def\pgfmath@parsefunction@abs{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@abs@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@abs@{%	
	\expandafter\pgfmathabs@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@sqrt
%
\def\pgfmath@parsefunction@sqrt{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@sqrt@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@sqrt@{%	
	\expandafter\pgfmathsqrt@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@round
%
\def\pgfmath@parsefunction@round{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@round@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@round@{%	
	\expandafter\pgfmathround@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@floor
%
\def\pgfmath@parsefunction@floor{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@floor@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@floor@{%	
	\expandafter\pgfmathfloor@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@ceil
%
\def\pgfmath@parsefunction@ceil{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@ceil@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@ceil@{%	
	\expandafter\pgfmathceil@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@sin
%
\def\pgfmath@parsefunction@sin{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@sin@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@sin@{%	
	\expandafter\pgfmathsin@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@cos
%
\def\pgfmath@parsefunction@cos{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@cos@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@cos@{%	
	\expandafter\pgfmathcos@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@asin
%
\def\pgfmath@parsefunction@asin{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@asin@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@asin@{%	
	\expandafter\pgfmathasin@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@acos
%
\def\pgfmath@parsefunction@acos{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@acos@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@acos@{%	
	\expandafter\pgfmathacos@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction}

% \pgfmath@parsefunction@atan
%
\def\pgfmath@parsefunction@atan{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@atan@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@atan@{%	
	\expandafter\pgfmathatan@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@tan
%
\def\pgfmath@parsefunction@tan{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@tan@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@tan@{%	
	\expandafter\pgfmathtan@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@rad
%
\def\pgfmath@parsefunction@rad{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@rad@%
	\pgfmath@parse@}
\def\pgfmath@parsefunction@rad@{%
	\expandafter\pgfmathrad@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction}%
	
% \pgfmath@parsefunction@rad
%
\def\pgfmath@parsefunction@deg{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@deg@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@deg@{%
	\expandafter\pgfmathdeg@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction}%
	
% \pgfmath@parsefunction@rnd
%
\def\pgfmath@parsefunction@rnd{%
	\expandafter\pgfmathrnd%
	\expandafter\pgfmath@postfunction}
			
% \pgfmath@parsefunction@rand
%
\def\pgfmath@parsefunction@rand{%
	\expandafter\pgfmathrand%
	\expandafter\pgfmath@postfunction}%
			
% \pgfmath@parsefunction@exp
%
\def\pgfmath@parsefunction@exp{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@exp@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@exp@{%	
	\expandafter\pgfmathexp@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@pi
%
\def\pgfmath@parsefunction@pi{%
	\pgfmathpi%
	\pgfmath@postfunction%
}


% \pgfmath@parsefunction@veclen
%
\def\pgfmath@parsefunction@veclen{%
	\expandafter\pgfmath@parsefunction@veclen@}
\def\pgfmath@parsefunction@veclen@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@veclen@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@veclen@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathveclen@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}

% \pgfmath@parsefunction@mod 
%
\def\pgfmath@parsefunction@mod{%
	\expandafter\pgfmath@parsefunction@mod@}
\def\pgfmath@parsefunction@mod@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@mod@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@mod@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmod@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}

% \pgfmath@parsefunction@max
%
\def\pgfmath@parsefunction@max{%
	\expandafter\pgfmath@parsefunction@max@}
\def\pgfmath@parsefunction@max@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@max@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@max@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmax@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}	

% \pgfmath@parsefunction@min 
%
\def\pgfmath@parsefunction@min{%
	\expandafter\pgfmath@parsefunction@min@}
\def\pgfmath@parsefunction@min@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@min@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@min@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmin@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}
	
% \pgfmath@parsefunction@pow 
%
\def\pgfmath@parsefunction@pow{%
	\expandafter\pgfmath@parsefunction@pow@}
\def\pgfmath@parsefunction@pow@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@pow@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@pow@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathpow@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}

==> pgfmathrnd.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the pesudorandom numbers.
%
% Version 0.0 08/03/2007

% Pseudo-random number generation.
%
% See:
% \book@{pressetal1992,
%    author    = {William H. Press and Brian P. Flannery and Saul A. 
%                 Teukolsky and William T. Vetterling}, 
%    title     = {Numerical Recipies in C},
%    edition   = {Second},
%    publisher = {Cambridge University Press}
% }
%
% See also, the documentation for the lcg package by Erich Janka:
% (http://www.ctan.org/tex-archive/macros/latex/contrib/lcg/lcg.pdf)
%
\def\pgfmath@rnd@m{2147483647}% LaTeX Maximum.

\begingroup
\c@pgfmath@counta=\time%
\multiply\c@pgfmath@counta by\year%
\xdef\pgfmath@rnd@z{\the\c@pgfmath@counta}% The seed. 
\endgroup

% \pgfmathsetseed
%
% Explictly set the seed for the generator
%   
% #1 -> the new seed.
%

\def\pgfmathsetseed#1{\pgfmathparse{#1}\expandafter\pgfmath@setseed\pgfmathresult\relax}%
\def\pgfmath@setseed#1.#2\relax{\def\pgfmath@rnd@z{#1}}%  

% Alternative paramaters - see Press et al (1992) p278-279, 
% for discussion.
%
% a=16807 q=127773 r=2836
% a=48271 q=4488   r=3399
%
\def\pgfmath@rnd@a{69621}
\def\pgfmath@rnd@r{23902}
\def\pgfmath@rnd@q{30845}

% \pgfmathgeneratepseudorandomnumber
% 
% A linear congruency generator for generating
% pseudo-random numbers. Generates numbers in
% the range 1 - 2^31-1.
%
\def\pgfmathgeneratepseudorandomnumber{%
	\begingroup%
		\c@pgfmath@counta=\pgfmath@rnd@z%
		\c@pgfmath@countb=\pgfmath@rnd@z%
		\c@pgfmath@countc=\pgfmath@rnd@q%
		\divide\c@pgfmath@counta by\c@pgfmath@countc%
		\multiply\c@pgfmath@counta by-\c@pgfmath@countc%
		\advance\c@pgfmath@counta by\c@pgfmath@countb
		\c@pgfmath@countc=\pgfmath@rnd@a%
		\multiply\c@pgfmath@counta by\c@pgfmath@countc%
		\c@pgfmath@countc=\pgfmath@rnd@q%
		\divide\c@pgfmath@countb by\c@pgfmath@countc%
		\c@pgfmath@countc=\pgfmath@rnd@r%
		\multiply\c@pgfmath@countb by\c@pgfmath@countc%
		\advance\c@pgfmath@counta by-\c@pgfmath@countb%
		\ifnum\c@pgfmath@counta<0\relax%
			\c@pgfmath@countb=\pgfmath@rnd@m%
			\advance\c@pgfmath@counta by\c@pgfmath@countb%
		\fi%
		\xdef\pgfmath@rnd@z{\the\c@pgfmath@counta}%
	\endgroup%
	\edef\pgfmathresult{\pgfmath@rnd@z}%
}

% \pgfmathrnd
%
% Generates a pseudo-random number between 0 and 1.
%
\def\pgfmathrnd{%
	\begingroup%
		\pgfmathgeneratepseudorandomnumber%
		\c@pgfmath@counta\pgfmathresult%
		\c@pgfmath@countb\c@pgfmath@counta%
		\divide\c@pgfmath@countb100001\relax% To get one.
		\multiply\c@pgfmath@countb-100001\relax%
		\advance\c@pgfmath@countb\c@pgfmath@counta%
		\advance\c@pgfmath@countb1000000\relax%
		\expandafter\pgfmathrnd@\the\c@pgfmath@countb\pgfmath@%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

\def\pgfmathrnd@#1#2#3\pgfmath@{%
	\edef\pgfmath@temp{#2.#3}%
	\pgfmath@x=\pgfmath@temp pt\relax%
}%

% \pgfmathrand
%
% Generates a pseudo-random number between -1 and 1.
%
\def\pgfmathrand{%
	\begingroup%
		\pgfmathgeneratepseudorandomnumber%
		\c@pgfmath@counta\pgfmathresult%
		\c@pgfmath@countb\c@pgfmath@counta%
		\divide\c@pgfmath@countb200001\relax%
		\multiply\c@pgfmath@countb-200001\relax%
		\advance\c@pgfmath@countb\c@pgfmath@counta%
		\advance\c@pgfmath@countb-100000\relax%
		\ifnum\c@pgfmath@countb<0\relax%
			\advance\c@pgfmath@countb-1000000\relax%
		\else%
			\advance\c@pgfmath@countb1000000\relax%
		\fi%
		\expandafter\pgfmathrand@\the\c@pgfmath@countb\pgfmath@%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

\def\pgfmathrand@#1#2#3#4\pgfmath@{%
	\ifx#1-%
		\edef\pgfmath@temp{-#3.#4}%
	\else%
		\edef\pgfmath@temp{#2.#3#4}%
	\fi%
	\pgfmath@x=\pgfmath@temp pt\relax%
}%

% \pgfmathrandominteger
%
% Return a 'randomly' selected integer in the range #2 - #3 (inclusive).
%
% #1 - a macro to store the integer (not a count register).
% #2 - the lower limit of the range.
% #3 - the upper limit of the range.
%
\def\pgfmathrandominteger#1#2#3{%
	\begingroup%
		\pgfmathgeneratepseudorandomnumber%
		\c@pgfmath@counta#2\relax%
		\c@pgfmath@countb#3\relax%
		\c@pgfmath@countc\c@pgfmath@countb%
		% OK. Maybe #2 > #3.
		\ifnum\c@pgfmath@counta>\c@pgfmath@countb\relax%
			\c@pgfmath@countc\c@pgfmath@countb%
			\c@pgfmath@countb\c@pgfmath@counta%
			\c@pgfmath@counta\c@pgfmath@countc%
		\fi%
		\advance\c@pgfmath@countc1\relax%
		\advance\c@pgfmath@countc-\c@pgfmath@counta%
		\c@pgfmath@counta\pgfmathresult\relax%
		\c@pgfmath@countb\c@pgfmath@counta%
		\divide\c@pgfmath@countb\c@pgfmath@countc%
		\multiply\c@pgfmath@countb-\c@pgfmath@countc%
		\advance\c@pgfmath@counta\c@pgfmath@countb%
		\advance\c@pgfmath@counta#2\relax%
		\edef\pgfmathresult{\the\c@pgfmath@counta}%
		\pgfmath@smuggleone{\pgfmathresult}%
	\endgroup%
	\edef#1{\pgfmathresult}%
}

% \pgfmathdeclarerandomlist
%
% Create a list to be used with \pgfmathrandomelement.
%
% #1 - the name of the list
% #2 - a list of comma separated elements.
%
\def\pgfmathdeclarerandomlist#1#2{%
	\def\pgfmath@randomlistname{#1}%
	\begingroup%
		\c@pgfmath@counta=1\relax%
		% {} is a possible random element so (locally) 
		% redefine \pgfmath@empty.
		\def\pgfmath@empty{pgfmath@empty}% 
		\expandafter\pgfmath@scanrandomlist#2{pgfmath@empty}}
\def\pgfmath@scanrandomlist#1{%
	\def\pgfmath@scanneditem{#1}%
	\ifx\pgfmath@scanneditem\pgfmath@empty%
		\advance\c@pgfmath@counta-1\relax%
		\expandafter\xdef\csname pgfmath@randomlist@\pgfmath@randomlistname\endcsname{\the\c@pgfmath@counta}%
		\endgroup%	
	\else%
		\expandafter\gdef\csname pgfmath@randomlist@\pgfmath@randomlistname @\the\c@pgfmath@counta\endcsname{#1}%
		\advance\c@pgfmath@counta1\relax%
		\expandafter\pgfmath@scanrandomlist%
	\fi}

% \pgfmathrandomitem
%
% Return a 'randomly' selected element from a list.
%
% #1 - a macro to store the item.
% #2 - the name of the list.
%
\def\pgfmathrandomitem#1#2{%
	\pgfmath@ifundefined{pgfmath@randomlist@#2}{\pgfmath@error{Unknown random list `#2'}}{%
		\edef\pgfmath@randomlistlength{\csname pgfmath@randomlist@#2\endcsname}%
		\pgfmathrandominteger{\pgfmath@randomtemp}{1}{\pgfmath@randomlistlength}%
		\def#1{\csname pgfmath@randomlist@#2@\pgfmath@randomtemp\endcsname}}}

==> pgfmathtrig.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the trigonometric functions/operations.
%
% Much of this file is based on ideas and code (particularly 
% \pgfcoremath.code.tex) due to Till Tantau
%
% Version 0.0 08/03/2007

% \pgfmathpi
%
\def\pgfmathpi{\edef\pgfmathresult{\pgfmath@pi}}
\def\pgfmath@pi{3.14159}

% \pgfmathradians
% 
% Convert #1 from radians to degrees (accurate to 1 deg).
%
\def\pgfmathradians#1{%
	\pgfmathparse{#1}%
	\pgfmathradians@{\pgfmathresult}}
\def\pgfmathradians@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@x57.29577\pgfmath@x\relax% 57.29577 = 360/(2*pi)
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathdeg
% 
% Convert #1 from radians to degrees.
%
\def\pgfmathdeg#1{%
	\pgfmathparse{#1}%
	\pgfmathdeg@{\pgfmathresult}}
\def\pgfmathdeg@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@x57.29577\pgfmath@x\relax% 57.29577 = 360/(2*pi)
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathrad
% 
% Convert #1 from degrees to radians.
%
\def\pgfmathrad#1{%
	\pgfmathparse{#1}%
	\pgfmathrad@{\pgfmathresult}}
\def\pgfmathrad@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@x3.14159\pgfmath@x% 
		\divide\pgfmath@x180\relax%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathsin
% 
% Calculate the sine of #1 (in degrees).
%
\def\pgfmathsin#1{%
	\pgfmathparse{#1}%
	\pgfmathsin@{\pgfmathresult}}
\def\pgfmathsin@#1{%
	% Let #1 = a.b
	% Then sin(#1) \approx (1-b)*cos(a) + b*cos(a+1)
	%
	\begingroup%
		\pgfmath@x#1pt\relax%
		\advance\pgfmath@x-90pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@
		\divide\c@pgfmath@counta360\relax%
		\multiply\c@pgfmath@counta-360\relax%
		\advance\pgfmath@x\c@pgfmath@counta pt\relax%
		\ifdim\pgfmath@x<0pt\relax\pgfmath@x-\pgfmath@x\fi%
		\ifdim\pgfmath@x<180pt\relax%
		\else
			\pgfmath@x-\pgfmath@x%
			\advance\pgfmath@x360pt\relax%
		\fi%
		% Now 0 <= x < 179. So split x into integer and decimal...
		%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		%
		% ...if #1 is an integer, don't do anything fancy.
		\ifdim\pgfmath@xa=0pt%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname pt\relax%
		\else%
			\pgfmath@x-\pgfmath@xa%
			\advance\pgfmath@x1pt\relax%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@x%
			\advance\c@pgfmath@counta1\relax%
			\expandafter\advance\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@xa%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup
}

% \pgfmathcos
% 
% Calculate the cosine of #1 (in degrees).
%
\def\pgfmathcos#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathcos@\expandafter{\pgfmathresult}}
\def\pgfmathcos@#1{%
	% Let x = a.b
	% Then cos(x) \approx (1-b)*cos(a) + b*cos(a+1)
	%
	\begingroup%
		\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@% 
		\divide\c@pgfmath@counta360\relax%
		\multiply\c@pgfmath@counta-360\relax%
		\advance\pgfmath@x\c@pgfmath@counta pt\relax%
		\ifdim\pgfmath@x<0pt\relax\pgfmath@x-\pgfmath@x\fi%
		\ifdim\pgfmath@x<180pt\relax%
		\else%
			\pgfmath@x-\pgfmath@x%
			\advance\pgfmath@x360pt\relax%
		\fi%
		% Now 0 <= x < 179. So split x into integer and decimal...
		%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		%
		% ...if #1 is an integer, don't do anything fancy.
		\ifdim\pgfmath@xa=0pt%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname pt%
		\else%
			\pgfmath@x-\pgfmath@xa%
			\advance\pgfmath@x1pt\relax%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@x%
			\advance\c@pgfmath@counta1\relax%
			\ifnum\c@pgfmath@counta=181\relax\c@pgfmath@counta179\relax\fi%
			\expandafter\advance\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@xa%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}


% \pgfmathsincos
% 
% Calculate the sin and cosine of #1 (in degrees).
%
\def\pgfmathsincos#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathcos@\expandafter{\pgfmathresult}}
\def\pgfmathsincos@#1{%
	\pgfmathsin@{#1}\edef\pgfmathresulty{\pgfmathresult}%
	\pgfmathcos@{#1}\edef\pgfmathresultx{\pgfmathresult}%
}
% \pgfmathtan
% 
% Calculate the cotangent of #1 (in degrees).
%
\def\pgfmathtan#1{%
	\pgfmathparse{#1}%
	\pgfmathtan@{\pgfmathresult}}
\def\pgfmathtan@#1{%
	\begingroup%
		\pgfmathcos@{#1}%
		\expandafter\pgfmathreciprocal@\expandafter{\pgfmathresult}%
		\edef\pgfmath@tantemp{\pgfmathresult}%
		\pgfmathsin@{#1}%
		\pgfmath@x\pgfmathresult pt\relax%
		\pgfmath@x\pgfmath@tantemp\pgfmath@x%
		% Adjust to 4 decimal places. This gets rid of some annoyingly tiny errors.
		\afterassignment\pgfmath@x%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		\ifdim\pgfmath@x<.0001pt\relax%
			\pgfmath@x0pt\relax%
		\fi%
		\advance\pgfmath@x\c@pgfmath@counta pt%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}


% \pgfmathasin
%
% The asin of #1
%
\def\pgfmathasin#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathasin@\expandafter{\pgfmathresult}}
\def\pgfmathasin@#1{%
	\begingroup%
		\pgfmath@x#1pt\relax%
		\pgfmath@xa\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@x1000\pgfmath@x%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\expandafter\pgfmath@x\csname pgfmath@asin@\the\c@pgfmath@counta\endcsname pt\relax%
		\ifdim\pgfmath@xa<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathacos
%
% The acos of #1
%	
\def\pgfmathacos#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathacos@\expandafter{\pgfmathresult}}
\def\pgfmathacos@#1{%
	\begingroup%
		\pgfmath@x#1pt\relax%
		\pgfmath@xa\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@x1000\pgfmath@x%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\expandafter\pgfmath@x\csname pgfmath@acos@\the\c@pgfmath@counta\endcsname pt\relax%
		\ifdim\pgfmath@xa<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathasin
%
% The atan of #1
%
\def\pgfmathatan#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathatan@\expandafter{\pgfmathresult}}
\def\pgfmathatan@#1{%
	\begingroup%
		\pgfmath@x#1pt\relax%
		\pgfmath@xa\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@xb\pgfmath@x%
		\ifdim\pgfmath@x>1pt\relax%
			\edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
			\pgfmathreciprocal@{\pgfmath@temp}%
			\pgfmath@x\pgfmathresult pt\relax%
		\fi%
		\pgfmath@x1000\pgfmath@x%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\ifdim\pgfmath@xb>1pt\relax%
			\expandafter\pgfmath@x\expandafter-\csname pgfmath@atan@\the\c@pgfmath@counta\endcsname pt\relax%
			\advance\pgfmath@x90pt%
		\else%
			\expandafter\pgfmath@x\csname pgfmath@atan@\the\c@pgfmath@counta\endcsname pt\relax%
		\fi%
		\ifdim\pgfmath@xa<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

	
\def\pgfmath@def#1#2#3{\expandafter\def\csname pgfmath@#1@#2\endcsname{#3}}
\pgfmath@def{cos}{0}{1.00000}		\pgfmath@def{cos}{1}{0.99985}
\pgfmath@def{cos}{2}{0.99939}		\pgfmath@def{cos}{3}{0.99863}
\pgfmath@def{cos}{4}{0.99756}		\pgfmath@def{cos}{5}{0.99619}
\pgfmath@def{cos}{6}{0.99452}		\pgfmath@def{cos}{7}{0.99255}
\pgfmath@def{cos}{8}{0.99027}		\pgfmath@def{cos}{9}{0.98769}
\pgfmath@def{cos}{10}{0.98481}		\pgfmath@def{cos}{11}{0.98163}
\pgfmath@def{cos}{12}{0.97815}		\pgfmath@def{cos}{13}{0.97437}
\pgfmath@def{cos}{14}{0.97030}		\pgfmath@def{cos}{15}{0.96593}
\pgfmath@def{cos}{16}{0.96126}		\pgfmath@def{cos}{17}{0.95630}
\pgfmath@def{cos}{18}{0.95106}		\pgfmath@def{cos}{19}{0.94552}
\pgfmath@def{cos}{20}{0.93969}		\pgfmath@def{cos}{21}{0.93358}
\pgfmath@def{cos}{22}{0.92718}		\pgfmath@def{cos}{23}{0.92050}
\pgfmath@def{cos}{24}{0.91355}		\pgfmath@def{cos}{25}{0.90631}
\pgfmath@def{cos}{26}{0.89879}		\pgfmath@def{cos}{27}{0.89101}
\pgfmath@def{cos}{28}{0.88295}		\pgfmath@def{cos}{29}{0.87462}
\pgfmath@def{cos}{30}{0.86603}		\pgfmath@def{cos}{31}{0.85717}
\pgfmath@def{cos}{32}{0.84805}		\pgfmath@def{cos}{33}{0.83867}
\pgfmath@def{cos}{34}{0.82904}		\pgfmath@def{cos}{35}{0.81915}
\pgfmath@def{cos}{36}{0.80902}		\pgfmath@def{cos}{37}{0.79864}
\pgfmath@def{cos}{38}{0.78801}		\pgfmath@def{cos}{39}{0.77715}
\pgfmath@def{cos}{40}{0.76604}		\pgfmath@def{cos}{41}{0.75471}
\pgfmath@def{cos}{42}{0.74314}		\pgfmath@def{cos}{43}{0.73135}
\pgfmath@def{cos}{44}{0.71934}		\pgfmath@def{cos}{45}{0.70711}
\pgfmath@def{cos}{46}{0.69466}		\pgfmath@def{cos}{47}{0.68200}
\pgfmath@def{cos}{48}{0.66913}		\pgfmath@def{cos}{49}{0.65606}
\pgfmath@def{cos}{50}{0.64279}		\pgfmath@def{cos}{51}{0.62932}
\pgfmath@def{cos}{52}{0.61566}		\pgfmath@def{cos}{53}{0.60182}
\pgfmath@def{cos}{54}{0.58779}		\pgfmath@def{cos}{55}{0.57358}
\pgfmath@def{cos}{56}{0.55919}		\pgfmath@def{cos}{57}{0.54464}
\pgfmath@def{cos}{58}{0.52992}		\pgfmath@def{cos}{59}{0.51504}
\pgfmath@def{cos}{60}{0.50000}		\pgfmath@def{cos}{61}{0.48481}
\pgfmath@def{cos}{62}{0.46947}		\pgfmath@def{cos}{63}{0.45399}
\pgfmath@def{cos}{64}{0.43837}		\pgfmath@def{cos}{65}{0.42262}
\pgfmath@def{cos}{66}{0.40674}		\pgfmath@def{cos}{67}{0.39073}
\pgfmath@def{cos}{68}{0.37461}		\pgfmath@def{cos}{69}{0.35837}
\pgfmath@def{cos}{70}{0.34202}		\pgfmath@def{cos}{71}{0.32557}
\pgfmath@def{cos}{72}{0.30902}		\pgfmath@def{cos}{73}{0.29237}
\pgfmath@def{cos}{74}{0.27564}		\pgfmath@def{cos}{75}{0.25882}
\pgfmath@def{cos}{76}{0.24192}		\pgfmath@def{cos}{77}{0.22495}
\pgfmath@def{cos}{78}{0.20791}		\pgfmath@def{cos}{79}{0.19081}
\pgfmath@def{cos}{80}{0.17365}		\pgfmath@def{cos}{81}{0.15643}
\pgfmath@def{cos}{82}{0.13917}		\pgfmath@def{cos}{83}{0.12187}
\pgfmath@def{cos}{84}{0.10453}		\pgfmath@def{cos}{85}{0.08716}
\pgfmath@def{cos}{86}{0.06976}		\pgfmath@def{cos}{87}{0.05234}
\pgfmath@def{cos}{88}{0.03490}		\pgfmath@def{cos}{89}{0.01745}
\pgfmath@def{cos}{90}{0.00000}		\pgfmath@def{cos}{91}{-0.01745}
\pgfmath@def{cos}{92}{-0.03490}		\pgfmath@def{cos}{93}{-0.05234}
\pgfmath@def{cos}{94}{-0.06976}		\pgfmath@def{cos}{95}{-0.08716}
\pgfmath@def{cos}{96}{-0.10453}		\pgfmath@def{cos}{97}{-0.12187}
\pgfmath@def{cos}{98}{-0.13917}		\pgfmath@def{cos}{99}{-0.15643}
\pgfmath@def{cos}{100}{-0.17365}		\pgfmath@def{cos}{101}{-0.19081}
\pgfmath@def{cos}{102}{-0.20791}		\pgfmath@def{cos}{103}{-0.22495}
\pgfmath@def{cos}{104}{-0.24192}		\pgfmath@def{cos}{105}{-0.25882}
\pgfmath@def{cos}{106}{-0.27564}		\pgfmath@def{cos}{107}{-0.29237}
\pgfmath@def{cos}{108}{-0.30902}		\pgfmath@def{cos}{109}{-0.32557}
\pgfmath@def{cos}{110}{-0.34202}		\pgfmath@def{cos}{111}{-0.35837}
\pgfmath@def{cos}{112}{-0.37461}		\pgfmath@def{cos}{113}{-0.39073}
\pgfmath@def{cos}{114}{-0.40674}		\pgfmath@def{cos}{115}{-0.42262}
\pgfmath@def{cos}{116}{-0.43837}		\pgfmath@def{cos}{117}{-0.45399}
\pgfmath@def{cos}{118}{-0.46947}		\pgfmath@def{cos}{119}{-0.48481}
\pgfmath@def{cos}{120}{-0.50000}		\pgfmath@def{cos}{121}{-0.51504}
\pgfmath@def{cos}{122}{-0.52992}		\pgfmath@def{cos}{123}{-0.54464}
\pgfmath@def{cos}{124}{-0.55919}		\pgfmath@def{cos}{125}{-0.57358}
\pgfmath@def{cos}{126}{-0.58779}		\pgfmath@def{cos}{127}{-0.60182}
\pgfmath@def{cos}{128}{-0.61566}		\pgfmath@def{cos}{129}{-0.62932}
\pgfmath@def{cos}{130}{-0.64279}		\pgfmath@def{cos}{131}{-0.65606}
\pgfmath@def{cos}{132}{-0.66913}		\pgfmath@def{cos}{133}{-0.68200}
\pgfmath@def{cos}{134}{-0.69466}		\pgfmath@def{cos}{135}{-0.70711}
\pgfmath@def{cos}{136}{-0.71934}		\pgfmath@def{cos}{137}{-0.73135}
\pgfmath@def{cos}{138}{-0.74314}		\pgfmath@def{cos}{139}{-0.75471}
\pgfmath@def{cos}{140}{-0.76604}		\pgfmath@def{cos}{141}{-0.77715}
\pgfmath@def{cos}{142}{-0.78801}		\pgfmath@def{cos}{143}{-0.79864}
\pgfmath@def{cos}{144}{-0.80902}		\pgfmath@def{cos}{145}{-0.81915}
\pgfmath@def{cos}{146}{-0.82904}		\pgfmath@def{cos}{147}{-0.83867}
\pgfmath@def{cos}{148}{-0.84805}		\pgfmath@def{cos}{149}{-0.85717}
\pgfmath@def{cos}{150}{-0.86603}		\pgfmath@def{cos}{151}{-0.87462}
\pgfmath@def{cos}{152}{-0.88295}		\pgfmath@def{cos}{153}{-0.89101}
\pgfmath@def{cos}{154}{-0.89879}		\pgfmath@def{cos}{155}{-0.90631}
\pgfmath@def{cos}{156}{-0.91355}		\pgfmath@def{cos}{157}{-0.92050}
\pgfmath@def{cos}{158}{-0.92718}		\pgfmath@def{cos}{159}{-0.93358}
\pgfmath@def{cos}{160}{-0.93969}		\pgfmath@def{cos}{161}{-0.94552}
\pgfmath@def{cos}{162}{-0.95106}		\pgfmath@def{cos}{163}{-0.95630}
\pgfmath@def{cos}{164}{-0.96126}		\pgfmath@def{cos}{165}{-0.96593}
\pgfmath@def{cos}{166}{-0.97030}		\pgfmath@def{cos}{167}{-0.97437}
\pgfmath@def{cos}{168}{-0.97815}		\pgfmath@def{cos}{169}{-0.98163}
\pgfmath@def{cos}{170}{-0.98481}		\pgfmath@def{cos}{171}{-0.98769}
\pgfmath@def{cos}{172}{-0.99027}		\pgfmath@def{cos}{173}{-0.99255}
\pgfmath@def{cos}{174}{-0.99452}		\pgfmath@def{cos}{175}{-0.99619}
\pgfmath@def{cos}{176}{-0.99756}		\pgfmath@def{cos}{177}{-0.99863}
\pgfmath@def{cos}{178}{-0.99939}		\pgfmath@def{cos}{179}{-0.99985}
\pgfmath@def{cos}{180}{-1.00000}	   \pgfmath@def{cos}{181}{-0.99985}

\pgfmath@def{cosfrac}{0}{1.00000}		\pgfmath@def{cosfrac}{1}{0.99995}
\pgfmath@def{cosfrac}{2}{0.99980}		\pgfmath@def{cosfrac}{3}{0.99955}
\pgfmath@def{cosfrac}{4}{0.99920}		\pgfmath@def{cosfrac}{5}{0.99875}
\pgfmath@def{cosfrac}{6}{0.99820}		\pgfmath@def{cosfrac}{7}{0.99755}
\pgfmath@def{cosfrac}{8}{0.99681}		\pgfmath@def{cosfrac}{9}{0.99597}
\pgfmath@def{cosfrac}{10}{0.99503}		\pgfmath@def{cosfrac}{11}{0.99400}
\pgfmath@def{cosfrac}{12}{0.99287}		\pgfmath@def{cosfrac}{13}{0.99165}
\pgfmath@def{cosfrac}{14}{0.99034}		\pgfmath@def{cosfrac}{15}{0.98893}
\pgfmath@def{cosfrac}{16}{0.98744}		\pgfmath@def{cosfrac}{17}{0.98585}
\pgfmath@def{cosfrac}{18}{0.98418}		\pgfmath@def{cosfrac}{19}{0.98242}
\pgfmath@def{cosfrac}{20}{0.98058}		\pgfmath@def{cosfrac}{21}{0.97865}
\pgfmath@def{cosfrac}{22}{0.97664}		\pgfmath@def{cosfrac}{23}{0.97455}
\pgfmath@def{cosfrac}{24}{0.97238}		\pgfmath@def{cosfrac}{25}{0.97014}
\pgfmath@def{cosfrac}{26}{0.96782}		\pgfmath@def{cosfrac}{27}{0.96542}
\pgfmath@def{cosfrac}{28}{0.96296}		\pgfmath@def{cosfrac}{29}{0.96042}
\pgfmath@def{cosfrac}{30}{0.95782}		\pgfmath@def{cosfrac}{31}{0.95515}
\pgfmath@def{cosfrac}{32}{0.95242}		\pgfmath@def{cosfrac}{33}{0.94962}
\pgfmath@def{cosfrac}{34}{0.94677}		\pgfmath@def{cosfrac}{35}{0.94385}
\pgfmath@def{cosfrac}{36}{0.94088}		\pgfmath@def{cosfrac}{37}{0.93786}
\pgfmath@def{cosfrac}{38}{0.93478}		\pgfmath@def{cosfrac}{39}{0.93165}
\pgfmath@def{cosfrac}{40}{0.92847}		\pgfmath@def{cosfrac}{41}{0.92525}
\pgfmath@def{cosfrac}{42}{0.92198}		\pgfmath@def{cosfrac}{43}{0.91866}
\pgfmath@def{cosfrac}{44}{0.91531}		\pgfmath@def{cosfrac}{45}{0.91192}
\pgfmath@def{cosfrac}{46}{0.90849}		\pgfmath@def{cosfrac}{47}{0.90502}
\pgfmath@def{cosfrac}{48}{0.90152}		\pgfmath@def{cosfrac}{49}{0.89799}
\pgfmath@def{cosfrac}{50}{0.89442}		\pgfmath@def{cosfrac}{51}{0.89083}
\pgfmath@def{cosfrac}{52}{0.88721}		\pgfmath@def{cosfrac}{53}{0.88357}
\pgfmath@def{cosfrac}{54}{0.87990}		\pgfmath@def{cosfrac}{55}{0.87621}
\pgfmath@def{cosfrac}{56}{0.87250}		\pgfmath@def{cosfrac}{57}{0.86877}
\pgfmath@def{cosfrac}{58}{0.86503}		\pgfmath@def{cosfrac}{59}{0.86126}
\pgfmath@def{cosfrac}{60}{0.85749}		\pgfmath@def{cosfrac}{61}{0.85370}
\pgfmath@def{cosfrac}{62}{0.84990}		\pgfmath@def{cosfrac}{63}{0.84609}
\pgfmath@def{cosfrac}{64}{0.84227}		\pgfmath@def{cosfrac}{65}{0.83844}
\pgfmath@def{cosfrac}{66}{0.83460}		\pgfmath@def{cosfrac}{67}{0.83077}
\pgfmath@def{cosfrac}{68}{0.82692}		\pgfmath@def{cosfrac}{69}{0.82308}
\pgfmath@def{cosfrac}{70}{0.81923}		\pgfmath@def{cosfrac}{71}{0.81538}
\pgfmath@def{cosfrac}{72}{0.81153}		\pgfmath@def{cosfrac}{73}{0.80768}
\pgfmath@def{cosfrac}{74}{0.80384}		\pgfmath@def{cosfrac}{75}{0.80000}
\pgfmath@def{cosfrac}{76}{0.79616}		\pgfmath@def{cosfrac}{77}{0.79232}
\pgfmath@def{cosfrac}{78}{0.78850}		\pgfmath@def{cosfrac}{79}{0.78468}
\pgfmath@def{cosfrac}{80}{0.78086}		\pgfmath@def{cosfrac}{81}{0.77706}
\pgfmath@def{cosfrac}{82}{0.77326}		\pgfmath@def{cosfrac}{83}{0.76948}
\pgfmath@def{cosfrac}{84}{0.76570}		\pgfmath@def{cosfrac}{85}{0.76193}
\pgfmath@def{cosfrac}{86}{0.75818}		\pgfmath@def{cosfrac}{87}{0.75444}
\pgfmath@def{cosfrac}{88}{0.75071}		\pgfmath@def{cosfrac}{89}{0.74699}
\pgfmath@def{cosfrac}{90}{0.74329}		\pgfmath@def{cosfrac}{91}{0.73960}
\pgfmath@def{cosfrac}{92}{0.73593}		\pgfmath@def{cosfrac}{93}{0.73227}
\pgfmath@def{cosfrac}{94}{0.72862}		\pgfmath@def{cosfrac}{95}{0.72499}
\pgfmath@def{cosfrac}{96}{0.72138}		\pgfmath@def{cosfrac}{97}{0.71779}
\pgfmath@def{cosfrac}{98}{0.71421}		\pgfmath@def{cosfrac}{99}{0.71065}
\pgfmath@def{cosfrac}{100}{0.70710}	

% Oh No! Some really loooooong tables.
\pgfmath@def{atan}{0}{0.00000}		\pgfmath@def{atan}{1}{0.05729}
\pgfmath@def{atan}{2}{0.11459}		\pgfmath@def{atan}{3}{0.17188}
\pgfmath@def{atan}{4}{0.22918}		\pgfmath@def{atan}{5}{0.28647}
\pgfmath@def{atan}{6}{0.34377}		\pgfmath@def{atan}{7}{0.40106}
\pgfmath@def{atan}{8}{0.45835}		\pgfmath@def{atan}{9}{0.51564}
\pgfmath@def{atan}{10}{0.57293}		\pgfmath@def{atan}{11}{0.63022}
\pgfmath@def{atan}{12}{0.68751}		\pgfmath@def{atan}{13}{0.74480}
\pgfmath@def{atan}{14}{0.80208}		\pgfmath@def{atan}{15}{0.85937}
\pgfmath@def{atan}{16}{0.91665}		\pgfmath@def{atan}{17}{0.97393}
\pgfmath@def{atan}{18}{1.03121}		\pgfmath@def{atan}{19}{1.08848}
\pgfmath@def{atan}{20}{1.14576}		\pgfmath@def{atan}{21}{1.20303}
\pgfmath@def{atan}{22}{1.26030}		\pgfmath@def{atan}{23}{1.31757}
\pgfmath@def{atan}{24}{1.37483}		\pgfmath@def{atan}{25}{1.43209}
\pgfmath@def{atan}{26}{1.48935}		\pgfmath@def{atan}{27}{1.54661}
\pgfmath@def{atan}{28}{1.60386}		\pgfmath@def{atan}{29}{1.66111}
\pgfmath@def{atan}{30}{1.71835}		\pgfmath@def{atan}{31}{1.77560}
\pgfmath@def{atan}{32}{1.83284}		\pgfmath@def{atan}{33}{1.89007}
\pgfmath@def{atan}{34}{1.94730}		\pgfmath@def{atan}{35}{2.00453}
\pgfmath@def{atan}{36}{2.06175}		\pgfmath@def{atan}{37}{2.11897}
\pgfmath@def{atan}{38}{2.17619}		\pgfmath@def{atan}{39}{2.23340}
\pgfmath@def{atan}{40}{2.29061}		\pgfmath@def{atan}{41}{2.34781}
\pgfmath@def{atan}{42}{2.40500}		\pgfmath@def{atan}{43}{2.46220}
\pgfmath@def{atan}{44}{2.51938}		\pgfmath@def{atan}{45}{2.57657}
\pgfmath@def{atan}{46}{2.63374}		\pgfmath@def{atan}{47}{2.69092}
\pgfmath@def{atan}{48}{2.74808}		\pgfmath@def{atan}{49}{2.80524}
\pgfmath@def{atan}{50}{2.86240}		\pgfmath@def{atan}{51}{2.91955}
\pgfmath@def{atan}{52}{2.97669}		\pgfmath@def{atan}{53}{3.03383}
\pgfmath@def{atan}{54}{3.09097}		\pgfmath@def{atan}{55}{3.14809}
\pgfmath@def{atan}{56}{3.20521}		\pgfmath@def{atan}{57}{3.26232}
\pgfmath@def{atan}{58}{3.31943}		\pgfmath@def{atan}{59}{3.37653}
\pgfmath@def{atan}{60}{3.43363}		\pgfmath@def{atan}{61}{3.49071}
\pgfmath@def{atan}{62}{3.54779}		\pgfmath@def{atan}{63}{3.60487}
\pgfmath@def{atan}{64}{3.66193}		\pgfmath@def{atan}{65}{3.71899}
\pgfmath@def{atan}{66}{3.77604}		\pgfmath@def{atan}{67}{3.83308}
\pgfmath@def{atan}{68}{3.89012}		\pgfmath@def{atan}{69}{3.94715}
\pgfmath@def{atan}{70}{4.00417}		\pgfmath@def{atan}{71}{4.06118}
\pgfmath@def{atan}{72}{4.11819}		\pgfmath@def{atan}{73}{4.17518}
\pgfmath@def{atan}{74}{4.23217}		\pgfmath@def{atan}{75}{4.28915}
\pgfmath@def{atan}{76}{4.34612}		\pgfmath@def{atan}{77}{4.40308}
\pgfmath@def{atan}{78}{4.46004}		\pgfmath@def{atan}{79}{4.51698}
\pgfmath@def{atan}{80}{4.57392}		\pgfmath@def{atan}{81}{4.63084}
\pgfmath@def{atan}{82}{4.68776}		\pgfmath@def{atan}{83}{4.74467}
\pgfmath@def{atan}{84}{4.80157}		\pgfmath@def{atan}{85}{4.85846}
\pgfmath@def{atan}{86}{4.91534}		\pgfmath@def{atan}{87}{4.97221}
\pgfmath@def{atan}{88}{5.02907}		\pgfmath@def{atan}{89}{5.08592}
\pgfmath@def{atan}{90}{5.14276}		\pgfmath@def{atan}{91}{5.19959}
\pgfmath@def{atan}{92}{5.25641}		\pgfmath@def{atan}{93}{5.31322}
\pgfmath@def{atan}{94}{5.37002}		\pgfmath@def{atan}{95}{5.42681}
\pgfmath@def{atan}{96}{5.48359}		\pgfmath@def{atan}{97}{5.54035}
\pgfmath@def{atan}{98}{5.59711}		\pgfmath@def{atan}{99}{5.65385}
\pgfmath@def{atan}{100}{5.71059}		\pgfmath@def{atan}{101}{5.76731}
\pgfmath@def{atan}{102}{5.82402}		\pgfmath@def{atan}{103}{5.88072}
\pgfmath@def{atan}{104}{5.93741}		\pgfmath@def{atan}{105}{5.99409}
\pgfmath@def{atan}{106}{6.05075}		\pgfmath@def{atan}{107}{6.10741}
\pgfmath@def{atan}{108}{6.16405}		\pgfmath@def{atan}{109}{6.22068}
\pgfmath@def{atan}{110}{6.27729}		\pgfmath@def{atan}{111}{6.33390}
\pgfmath@def{atan}{112}{6.39049}		\pgfmath@def{atan}{113}{6.44707}
\pgfmath@def{atan}{114}{6.50364}		\pgfmath@def{atan}{115}{6.56019}
\pgfmath@def{atan}{116}{6.61673}		\pgfmath@def{atan}{117}{6.67326}
\pgfmath@def{atan}{118}{6.72978}		\pgfmath@def{atan}{119}{6.78628}
\pgfmath@def{atan}{120}{6.84277}		\pgfmath@def{atan}{121}{6.89924}
\pgfmath@def{atan}{122}{6.95571}		\pgfmath@def{atan}{123}{7.01216}
\pgfmath@def{atan}{124}{7.06859}		\pgfmath@def{atan}{125}{7.12501}
\pgfmath@def{atan}{126}{7.18142}		\pgfmath@def{atan}{127}{7.23781}
\pgfmath@def{atan}{128}{7.29419}		\pgfmath@def{atan}{129}{7.35056}
\pgfmath@def{atan}{130}{7.40691}		\pgfmath@def{atan}{131}{7.46324}
\pgfmath@def{atan}{132}{7.51957}		\pgfmath@def{atan}{133}{7.57587}
\pgfmath@def{atan}{134}{7.63217}		\pgfmath@def{atan}{135}{7.68844}
\pgfmath@def{atan}{136}{7.74471}		\pgfmath@def{atan}{137}{7.80095}
\pgfmath@def{atan}{138}{7.85719}		\pgfmath@def{atan}{139}{7.91340}
\pgfmath@def{atan}{140}{7.96961}		\pgfmath@def{atan}{141}{8.02579}
\pgfmath@def{atan}{142}{8.08196}		\pgfmath@def{atan}{143}{8.13812}
\pgfmath@def{atan}{144}{8.19426}		\pgfmath@def{atan}{145}{8.25038}
\pgfmath@def{atan}{146}{8.30649}		\pgfmath@def{atan}{147}{8.36258}
\pgfmath@def{atan}{148}{8.41866}		\pgfmath@def{atan}{149}{8.47472}
\pgfmath@def{atan}{150}{8.53076}		\pgfmath@def{atan}{151}{8.58679}
\pgfmath@def{atan}{152}{8.64280}		\pgfmath@def{atan}{153}{8.69879}
\pgfmath@def{atan}{154}{8.75477}		\pgfmath@def{atan}{155}{8.81073}
\pgfmath@def{atan}{156}{8.86667}		\pgfmath@def{atan}{157}{8.92260}
\pgfmath@def{atan}{158}{8.97851}		\pgfmath@def{atan}{159}{9.03440}
\pgfmath@def{atan}{160}{9.09027}		\pgfmath@def{atan}{161}{9.14613}
\pgfmath@def{atan}{162}{9.20197}		\pgfmath@def{atan}{163}{9.25779}
\pgfmath@def{atan}{164}{9.31359}		\pgfmath@def{atan}{165}{9.36938}
\pgfmath@def{atan}{166}{9.42515}		\pgfmath@def{atan}{167}{9.48090}
\pgfmath@def{atan}{168}{9.53663}		\pgfmath@def{atan}{169}{9.59235}
\pgfmath@def{atan}{170}{9.64804}		\pgfmath@def{atan}{171}{9.70372}
\pgfmath@def{atan}{172}{9.75938}		\pgfmath@def{atan}{173}{9.81502}
\pgfmath@def{atan}{174}{9.87064}		\pgfmath@def{atan}{175}{9.92624}
\pgfmath@def{atan}{176}{9.98182}		\pgfmath@def{atan}{177}{10.03739}
\pgfmath@def{atan}{178}{10.09294}		\pgfmath@def{atan}{179}{10.14846}
\pgfmath@def{atan}{180}{10.20397}		\pgfmath@def{atan}{181}{10.25946}
\pgfmath@def{atan}{182}{10.31493}		\pgfmath@def{atan}{183}{10.37037}
\pgfmath@def{atan}{184}{10.42580}		\pgfmath@def{atan}{185}{10.48121}
\pgfmath@def{atan}{186}{10.53660}		\pgfmath@def{atan}{187}{10.59197}
\pgfmath@def{atan}{188}{10.64732}		\pgfmath@def{atan}{189}{10.70265}
\pgfmath@def{atan}{190}{10.75796}		\pgfmath@def{atan}{191}{10.81325}
\pgfmath@def{atan}{192}{10.86852}		\pgfmath@def{atan}{193}{10.92377}
\pgfmath@def{atan}{194}{10.97900}		\pgfmath@def{atan}{195}{11.03420}
\pgfmath@def{atan}{196}{11.08939}		\pgfmath@def{atan}{197}{11.14456}
\pgfmath@def{atan}{198}{11.19970}		\pgfmath@def{atan}{199}{11.25483}
\pgfmath@def{atan}{200}{11.30993}		\pgfmath@def{atan}{201}{11.36501}
\pgfmath@def{atan}{202}{11.42007}		\pgfmath@def{atan}{203}{11.47511}
\pgfmath@def{atan}{204}{11.53013}		\pgfmath@def{atan}{205}{11.58512}
\pgfmath@def{atan}{206}{11.64010}		\pgfmath@def{atan}{207}{11.69505}
\pgfmath@def{atan}{208}{11.74998}		\pgfmath@def{atan}{209}{11.80489}
\pgfmath@def{atan}{210}{11.85977}		\pgfmath@def{atan}{211}{11.91464}
\pgfmath@def{atan}{212}{11.96948}		\pgfmath@def{atan}{213}{12.02430}
\pgfmath@def{atan}{214}{12.07910}		\pgfmath@def{atan}{215}{12.13388}
\pgfmath@def{atan}{216}{12.18863}		\pgfmath@def{atan}{217}{12.24336}
\pgfmath@def{atan}{218}{12.29807}		\pgfmath@def{atan}{219}{12.35275}
\pgfmath@def{atan}{220}{12.40741}		\pgfmath@def{atan}{221}{12.46205}
\pgfmath@def{atan}{222}{12.51667}		\pgfmath@def{atan}{223}{12.57126}
\pgfmath@def{atan}{224}{12.62583}		\pgfmath@def{atan}{225}{12.68038}
\pgfmath@def{atan}{226}{12.73490}		\pgfmath@def{atan}{227}{12.78940}
\pgfmath@def{atan}{228}{12.84388}		\pgfmath@def{atan}{229}{12.89833}
\pgfmath@def{atan}{230}{12.95276}		\pgfmath@def{atan}{231}{13.00717}
\pgfmath@def{atan}{232}{13.06155}		\pgfmath@def{atan}{233}{13.11590}
\pgfmath@def{atan}{234}{13.17024}		\pgfmath@def{atan}{235}{13.22455}
\pgfmath@def{atan}{236}{13.27883}		\pgfmath@def{atan}{237}{13.33309}
\pgfmath@def{atan}{238}{13.38733}		\pgfmath@def{atan}{239}{13.44154}
\pgfmath@def{atan}{240}{13.49573}		\pgfmath@def{atan}{241}{13.54989}
\pgfmath@def{atan}{242}{13.60403}		\pgfmath@def{atan}{243}{13.65814}
\pgfmath@def{atan}{244}{13.71223}		\pgfmath@def{atan}{245}{13.76630}
\pgfmath@def{atan}{246}{13.82034}		\pgfmath@def{atan}{247}{13.87435}
\pgfmath@def{atan}{248}{13.92834}		\pgfmath@def{atan}{249}{13.98230}
\pgfmath@def{atan}{250}{14.03624}		\pgfmath@def{atan}{251}{14.09015}
\pgfmath@def{atan}{252}{14.14404}		\pgfmath@def{atan}{253}{14.19790}
\pgfmath@def{atan}{254}{14.25174}		\pgfmath@def{atan}{255}{14.30555}
\pgfmath@def{atan}{256}{14.35933}		\pgfmath@def{atan}{257}{14.41309}
\pgfmath@def{atan}{258}{14.46682}		\pgfmath@def{atan}{259}{14.52053}
\pgfmath@def{atan}{260}{14.57421}		\pgfmath@def{atan}{261}{14.62787}
\pgfmath@def{atan}{262}{14.68149}		\pgfmath@def{atan}{263}{14.73510}
\pgfmath@def{atan}{264}{14.78867}		\pgfmath@def{atan}{265}{14.84222}
\pgfmath@def{atan}{266}{14.89575}		\pgfmath@def{atan}{267}{14.94924}
\pgfmath@def{atan}{268}{15.00271}		\pgfmath@def{atan}{269}{15.05615}
\pgfmath@def{atan}{270}{15.10957}		\pgfmath@def{atan}{271}{15.16296}
\pgfmath@def{atan}{272}{15.21632}		\pgfmath@def{atan}{273}{15.26966}
\pgfmath@def{atan}{274}{15.32297}		\pgfmath@def{atan}{275}{15.37625}
\pgfmath@def{atan}{276}{15.42950}		\pgfmath@def{atan}{277}{15.48273}
\pgfmath@def{atan}{278}{15.53593}		\pgfmath@def{atan}{279}{15.58910}
\pgfmath@def{atan}{280}{15.64224}		\pgfmath@def{atan}{281}{15.69536}
\pgfmath@def{atan}{282}{15.74845}		\pgfmath@def{atan}{283}{15.80151}
\pgfmath@def{atan}{284}{15.85454}		\pgfmath@def{atan}{285}{15.90755}
\pgfmath@def{atan}{286}{15.96052}		\pgfmath@def{atan}{287}{16.01347}
\pgfmath@def{atan}{288}{16.06640}		\pgfmath@def{atan}{289}{16.11929}
\pgfmath@def{atan}{290}{16.17215}		\pgfmath@def{atan}{291}{16.22499}
\pgfmath@def{atan}{292}{16.27780}		\pgfmath@def{atan}{293}{16.33058}
\pgfmath@def{atan}{294}{16.38333}		\pgfmath@def{atan}{295}{16.43605}
\pgfmath@def{atan}{296}{16.48875}		\pgfmath@def{atan}{297}{16.54142}
\pgfmath@def{atan}{298}{16.59405}		\pgfmath@def{atan}{299}{16.64666}
\pgfmath@def{atan}{300}{16.69924}		\pgfmath@def{atan}{301}{16.75179}
\pgfmath@def{atan}{302}{16.80431}		\pgfmath@def{atan}{303}{16.85680}
\pgfmath@def{atan}{304}{16.90927}		\pgfmath@def{atan}{305}{16.96170}
\pgfmath@def{atan}{306}{17.01411}		\pgfmath@def{atan}{307}{17.06648}
\pgfmath@def{atan}{308}{17.11883}		\pgfmath@def{atan}{309}{17.17114}
\pgfmath@def{atan}{310}{17.22343}		\pgfmath@def{atan}{311}{17.27569}
\pgfmath@def{atan}{312}{17.32792}		\pgfmath@def{atan}{313}{17.38012}
\pgfmath@def{atan}{314}{17.43228}		\pgfmath@def{atan}{315}{17.48442}
\pgfmath@def{atan}{316}{17.53653}		\pgfmath@def{atan}{317}{17.58861}
\pgfmath@def{atan}{318}{17.64066}		\pgfmath@def{atan}{319}{17.69268}
\pgfmath@def{atan}{320}{17.74467}		\pgfmath@def{atan}{321}{17.79663}
\pgfmath@def{atan}{322}{17.84855}		\pgfmath@def{atan}{323}{17.90045}
\pgfmath@def{atan}{324}{17.95232}		\pgfmath@def{atan}{325}{18.00416}
\pgfmath@def{atan}{326}{18.05596}		\pgfmath@def{atan}{327}{18.10774}
\pgfmath@def{atan}{328}{18.15949}		\pgfmath@def{atan}{329}{18.21120}
\pgfmath@def{atan}{330}{18.26289}		\pgfmath@def{atan}{331}{18.31454}
\pgfmath@def{atan}{332}{18.36616}		\pgfmath@def{atan}{333}{18.41775}
\pgfmath@def{atan}{334}{18.46931}		\pgfmath@def{atan}{335}{18.52084}
\pgfmath@def{atan}{336}{18.57234}		\pgfmath@def{atan}{337}{18.62381}
\pgfmath@def{atan}{338}{18.67525}		\pgfmath@def{atan}{339}{18.72665}
\pgfmath@def{atan}{340}{18.77803}		\pgfmath@def{atan}{341}{18.82937}
\pgfmath@def{atan}{342}{18.88068}		\pgfmath@def{atan}{343}{18.93196}
\pgfmath@def{atan}{344}{18.98321}		\pgfmath@def{atan}{345}{19.03443}
\pgfmath@def{atan}{346}{19.08562}		\pgfmath@def{atan}{347}{19.13677}
\pgfmath@def{atan}{348}{19.18789}		\pgfmath@def{atan}{349}{19.23898}
\pgfmath@def{atan}{350}{19.29004}		\pgfmath@def{atan}{351}{19.34107}
\pgfmath@def{atan}{352}{19.39206}		\pgfmath@def{atan}{353}{19.44303}
\pgfmath@def{atan}{354}{19.49396}		\pgfmath@def{atan}{355}{19.54486}
\pgfmath@def{atan}{356}{19.59572}		\pgfmath@def{atan}{357}{19.64656}
\pgfmath@def{atan}{358}{19.69736}		\pgfmath@def{atan}{359}{19.74813}
\pgfmath@def{atan}{360}{19.79887}		\pgfmath@def{atan}{361}{19.84958}
\pgfmath@def{atan}{362}{19.90025}		\pgfmath@def{atan}{363}{19.95089}
\pgfmath@def{atan}{364}{20.00150}		\pgfmath@def{atan}{365}{20.05208}
\pgfmath@def{atan}{366}{20.10262}		\pgfmath@def{atan}{367}{20.15313}
\pgfmath@def{atan}{368}{20.20361}		\pgfmath@def{atan}{369}{20.25406}
\pgfmath@def{atan}{370}{20.30447}		\pgfmath@def{atan}{371}{20.35485}
\pgfmath@def{atan}{372}{20.40520}		\pgfmath@def{atan}{373}{20.45551}
\pgfmath@def{atan}{374}{20.50579}		\pgfmath@def{atan}{375}{20.55604}
\pgfmath@def{atan}{376}{20.60626}		\pgfmath@def{atan}{377}{20.65644}
\pgfmath@def{atan}{378}{20.70659}		\pgfmath@def{atan}{379}{20.75670}
\pgfmath@def{atan}{380}{20.80679}		\pgfmath@def{atan}{381}{20.85684}
\pgfmath@def{atan}{382}{20.90685}		\pgfmath@def{atan}{383}{20.95684}
\pgfmath@def{atan}{384}{21.00678}		\pgfmath@def{atan}{385}{21.05670}
\pgfmath@def{atan}{386}{21.10658}		\pgfmath@def{atan}{387}{21.15643}
\pgfmath@def{atan}{388}{21.20625}		\pgfmath@def{atan}{389}{21.25603}
\pgfmath@def{atan}{390}{21.30578}		\pgfmath@def{atan}{391}{21.35549}
\pgfmath@def{atan}{392}{21.40517}		\pgfmath@def{atan}{393}{21.45482}
\pgfmath@def{atan}{394}{21.50444}		\pgfmath@def{atan}{395}{21.55402}
\pgfmath@def{atan}{396}{21.60356}		\pgfmath@def{atan}{397}{21.65307}
\pgfmath@def{atan}{398}{21.70255}		\pgfmath@def{atan}{399}{21.75200}
\pgfmath@def{atan}{400}{21.80140}		\pgfmath@def{atan}{401}{21.85078}
\pgfmath@def{atan}{402}{21.90012}		\pgfmath@def{atan}{403}{21.94943}
\pgfmath@def{atan}{404}{21.99870}		\pgfmath@def{atan}{405}{22.04794}
\pgfmath@def{atan}{406}{22.09715}		\pgfmath@def{atan}{407}{22.14632}
\pgfmath@def{atan}{408}{22.19546}		\pgfmath@def{atan}{409}{22.24456}
\pgfmath@def{atan}{410}{22.29362}		\pgfmath@def{atan}{411}{22.34266}
\pgfmath@def{atan}{412}{22.39166}		\pgfmath@def{atan}{413}{22.44062}
\pgfmath@def{atan}{414}{22.48955}		\pgfmath@def{atan}{415}{22.53845}
\pgfmath@def{atan}{416}{22.58731}		\pgfmath@def{atan}{417}{22.63613}
\pgfmath@def{atan}{418}{22.68492}		\pgfmath@def{atan}{419}{22.73368}
\pgfmath@def{atan}{420}{22.78240}		\pgfmath@def{atan}{421}{22.83109}
\pgfmath@def{atan}{422}{22.87974}		\pgfmath@def{atan}{423}{22.92836}
\pgfmath@def{atan}{424}{22.97694}		\pgfmath@def{atan}{425}{23.02549}
\pgfmath@def{atan}{426}{23.07400}		\pgfmath@def{atan}{427}{23.12248}
\pgfmath@def{atan}{428}{23.17092}		\pgfmath@def{atan}{429}{23.21933}
\pgfmath@def{atan}{430}{23.26770}		\pgfmath@def{atan}{431}{23.31604}
\pgfmath@def{atan}{432}{23.36434}		\pgfmath@def{atan}{433}{23.41261}
\pgfmath@def{atan}{434}{23.46084}		\pgfmath@def{atan}{435}{23.50904}
\pgfmath@def{atan}{436}{23.55720}		\pgfmath@def{atan}{437}{23.60532}
\pgfmath@def{atan}{438}{23.65341}		\pgfmath@def{atan}{439}{23.70147}
\pgfmath@def{atan}{440}{23.74949}		\pgfmath@def{atan}{441}{23.79747}
\pgfmath@def{atan}{442}{23.84542}		\pgfmath@def{atan}{443}{23.89334}
\pgfmath@def{atan}{444}{23.94122}		\pgfmath@def{atan}{445}{23.98906}
\pgfmath@def{atan}{446}{24.03687}		\pgfmath@def{atan}{447}{24.08464}
\pgfmath@def{atan}{448}{24.13238}		\pgfmath@def{atan}{449}{24.18008}
\pgfmath@def{atan}{450}{24.22774}		\pgfmath@def{atan}{451}{24.27537}
\pgfmath@def{atan}{452}{24.32296}		\pgfmath@def{atan}{453}{24.37052}
\pgfmath@def{atan}{454}{24.41804}		\pgfmath@def{atan}{455}{24.46553}
\pgfmath@def{atan}{456}{24.51298}		\pgfmath@def{atan}{457}{24.56040}
\pgfmath@def{atan}{458}{24.60778}		\pgfmath@def{atan}{459}{24.65512}
\pgfmath@def{atan}{460}{24.70243}		\pgfmath@def{atan}{461}{24.74970}
\pgfmath@def{atan}{462}{24.79693}		\pgfmath@def{atan}{463}{24.84413}
\pgfmath@def{atan}{464}{24.89130}		\pgfmath@def{atan}{465}{24.93842}
\pgfmath@def{atan}{466}{24.98551}		\pgfmath@def{atan}{467}{25.03257}
\pgfmath@def{atan}{468}{25.07959}		\pgfmath@def{atan}{469}{25.12657}
\pgfmath@def{atan}{470}{25.17352}		\pgfmath@def{atan}{471}{25.22043}
\pgfmath@def{atan}{472}{25.26731}		\pgfmath@def{atan}{473}{25.31414}
\pgfmath@def{atan}{474}{25.36095}		\pgfmath@def{atan}{475}{25.40771}
\pgfmath@def{atan}{476}{25.45444}		\pgfmath@def{atan}{477}{25.50114}
\pgfmath@def{atan}{478}{25.54780}		\pgfmath@def{atan}{479}{25.59442}
\pgfmath@def{atan}{480}{25.64100}		\pgfmath@def{atan}{481}{25.68755}
\pgfmath@def{atan}{482}{25.73406}		\pgfmath@def{atan}{483}{25.78054}
\pgfmath@def{atan}{484}{25.82698}		\pgfmath@def{atan}{485}{25.87338}
\pgfmath@def{atan}{486}{25.91975}		\pgfmath@def{atan}{487}{25.96608}
\pgfmath@def{atan}{488}{26.01237}		\pgfmath@def{atan}{489}{26.05863}
\pgfmath@def{atan}{490}{26.10485}		\pgfmath@def{atan}{491}{26.15103}
\pgfmath@def{atan}{492}{26.19718}		\pgfmath@def{atan}{493}{26.24329}
\pgfmath@def{atan}{494}{26.28937}		\pgfmath@def{atan}{495}{26.33541}
\pgfmath@def{atan}{496}{26.38141}		\pgfmath@def{atan}{497}{26.42737}
\pgfmath@def{atan}{498}{26.47330}		\pgfmath@def{atan}{499}{26.51919}
\pgfmath@def{atan}{500}{26.56505}		\pgfmath@def{atan}{501}{26.61086}
\pgfmath@def{atan}{502}{26.65665}		\pgfmath@def{atan}{503}{26.70239}
\pgfmath@def{atan}{504}{26.74810}		\pgfmath@def{atan}{505}{26.79377}
\pgfmath@def{atan}{506}{26.83941}		\pgfmath@def{atan}{507}{26.88500}
\pgfmath@def{atan}{508}{26.93057}		\pgfmath@def{atan}{509}{26.97609}
\pgfmath@def{atan}{510}{27.02158}		\pgfmath@def{atan}{511}{27.06703}
\pgfmath@def{atan}{512}{27.11244}		\pgfmath@def{atan}{513}{27.15782}
\pgfmath@def{atan}{514}{27.20316}		\pgfmath@def{atan}{515}{27.24846}
\pgfmath@def{atan}{516}{27.29373}		\pgfmath@def{atan}{517}{27.33896}
\pgfmath@def{atan}{518}{27.38415}		\pgfmath@def{atan}{519}{27.42931}
\pgfmath@def{atan}{520}{27.47443}		\pgfmath@def{atan}{521}{27.51951}
\pgfmath@def{atan}{522}{27.56455}		\pgfmath@def{atan}{523}{27.60956}
\pgfmath@def{atan}{524}{27.65453}		\pgfmath@def{atan}{525}{27.69947}
\pgfmath@def{atan}{526}{27.74437}		\pgfmath@def{atan}{527}{27.78923}
\pgfmath@def{atan}{528}{27.83405}		\pgfmath@def{atan}{529}{27.87884}
\pgfmath@def{atan}{530}{27.92359}		\pgfmath@def{atan}{531}{27.96830}
\pgfmath@def{atan}{532}{28.01297}		\pgfmath@def{atan}{533}{28.05761}
\pgfmath@def{atan}{534}{28.10221}		\pgfmath@def{atan}{535}{28.14678}
\pgfmath@def{atan}{536}{28.19130}		\pgfmath@def{atan}{537}{28.23579}
\pgfmath@def{atan}{538}{28.28025}		\pgfmath@def{atan}{539}{28.32466}
\pgfmath@def{atan}{540}{28.36904}		\pgfmath@def{atan}{541}{28.41338}
\pgfmath@def{atan}{542}{28.45769}		\pgfmath@def{atan}{543}{28.50196}
\pgfmath@def{atan}{544}{28.54619}		\pgfmath@def{atan}{545}{28.59038}
\pgfmath@def{atan}{546}{28.63454}		\pgfmath@def{atan}{547}{28.67865}
\pgfmath@def{atan}{548}{28.72274}		\pgfmath@def{atan}{549}{28.76678}
\pgfmath@def{atan}{550}{28.81079}		\pgfmath@def{atan}{551}{28.85476}
\pgfmath@def{atan}{552}{28.89869}		\pgfmath@def{atan}{553}{28.94259}
\pgfmath@def{atan}{554}{28.98645}		\pgfmath@def{atan}{555}{29.03027}
\pgfmath@def{atan}{556}{29.07405}		\pgfmath@def{atan}{557}{29.11780}
\pgfmath@def{atan}{558}{29.16151}		\pgfmath@def{atan}{559}{29.20519}
\pgfmath@def{atan}{560}{29.24882}		\pgfmath@def{atan}{561}{29.29242}
\pgfmath@def{atan}{562}{29.33598}		\pgfmath@def{atan}{563}{29.37951}
\pgfmath@def{atan}{564}{29.42299}		\pgfmath@def{atan}{565}{29.46644}
\pgfmath@def{atan}{566}{29.50986}		\pgfmath@def{atan}{567}{29.55323}
\pgfmath@def{atan}{568}{29.59657}		\pgfmath@def{atan}{569}{29.63987}
\pgfmath@def{atan}{570}{29.68314}		\pgfmath@def{atan}{571}{29.72636}
\pgfmath@def{atan}{572}{29.76955}		\pgfmath@def{atan}{573}{29.81270}
\pgfmath@def{atan}{574}{29.85582}		\pgfmath@def{atan}{575}{29.89890}
\pgfmath@def{atan}{576}{29.94194}		\pgfmath@def{atan}{577}{29.98494}
\pgfmath@def{atan}{578}{30.02791}		\pgfmath@def{atan}{579}{30.07084}
\pgfmath@def{atan}{580}{30.11373}		\pgfmath@def{atan}{581}{30.15658}
\pgfmath@def{atan}{582}{30.19940}		\pgfmath@def{atan}{583}{30.24218}
\pgfmath@def{atan}{584}{30.28492}		\pgfmath@def{atan}{585}{30.32763}
\pgfmath@def{atan}{586}{30.37030}		\pgfmath@def{atan}{587}{30.41293}
\pgfmath@def{atan}{588}{30.45552}		\pgfmath@def{atan}{589}{30.49808}
\pgfmath@def{atan}{590}{30.54060}		\pgfmath@def{atan}{591}{30.58308}
\pgfmath@def{atan}{592}{30.62553}		\pgfmath@def{atan}{593}{30.66794}
\pgfmath@def{atan}{594}{30.71031}		\pgfmath@def{atan}{595}{30.75264}
\pgfmath@def{atan}{596}{30.79494}		\pgfmath@def{atan}{597}{30.83720}
\pgfmath@def{atan}{598}{30.87942}		\pgfmath@def{atan}{599}{30.92160}
\pgfmath@def{atan}{600}{30.96375}		\pgfmath@def{atan}{601}{31.00586}
\pgfmath@def{atan}{602}{31.04794}		\pgfmath@def{atan}{603}{31.08997}
\pgfmath@def{atan}{604}{31.13197}		\pgfmath@def{atan}{605}{31.17393}
\pgfmath@def{atan}{606}{31.21586}		\pgfmath@def{atan}{607}{31.25775}
\pgfmath@def{atan}{608}{31.29960}		\pgfmath@def{atan}{609}{31.34141}
\pgfmath@def{atan}{610}{31.38319}		\pgfmath@def{atan}{611}{31.42493}
\pgfmath@def{atan}{612}{31.46663}		\pgfmath@def{atan}{613}{31.50829}
\pgfmath@def{atan}{614}{31.54992}		\pgfmath@def{atan}{615}{31.59151}
\pgfmath@def{atan}{616}{31.63306}		\pgfmath@def{atan}{617}{31.67458}
\pgfmath@def{atan}{618}{31.71606}		\pgfmath@def{atan}{619}{31.75750}
\pgfmath@def{atan}{620}{31.79891}		\pgfmath@def{atan}{621}{31.84028}
\pgfmath@def{atan}{622}{31.88161}		\pgfmath@def{atan}{623}{31.92290}
\pgfmath@def{atan}{624}{31.96416}		\pgfmath@def{atan}{625}{32.00538}
\pgfmath@def{atan}{626}{32.04656}		\pgfmath@def{atan}{627}{32.08771}
\pgfmath@def{atan}{628}{32.12882}		\pgfmath@def{atan}{629}{32.16989}
\pgfmath@def{atan}{630}{32.21092}		\pgfmath@def{atan}{631}{32.25192}
\pgfmath@def{atan}{632}{32.29288}		\pgfmath@def{atan}{633}{32.33381}
\pgfmath@def{atan}{634}{32.37469}		\pgfmath@def{atan}{635}{32.41554}
\pgfmath@def{atan}{636}{32.45636}		\pgfmath@def{atan}{637}{32.49713}
\pgfmath@def{atan}{638}{32.53787}		\pgfmath@def{atan}{639}{32.57857}
\pgfmath@def{atan}{640}{32.61924}		\pgfmath@def{atan}{641}{32.65987}
\pgfmath@def{atan}{642}{32.70046}		\pgfmath@def{atan}{643}{32.74101}
\pgfmath@def{atan}{644}{32.78153}		\pgfmath@def{atan}{645}{32.82201}
\pgfmath@def{atan}{646}{32.86246}		\pgfmath@def{atan}{647}{32.90286}
\pgfmath@def{atan}{648}{32.94323}		\pgfmath@def{atan}{649}{32.98357}
\pgfmath@def{atan}{650}{33.02386}		\pgfmath@def{atan}{651}{33.06412}
\pgfmath@def{atan}{652}{33.10435}		\pgfmath@def{atan}{653}{33.14453}
\pgfmath@def{atan}{654}{33.18468}		\pgfmath@def{atan}{655}{33.22479}
\pgfmath@def{atan}{656}{33.26487}		\pgfmath@def{atan}{657}{33.30491}
\pgfmath@def{atan}{658}{33.34491}		\pgfmath@def{atan}{659}{33.38488}
\pgfmath@def{atan}{660}{33.42481}		\pgfmath@def{atan}{661}{33.46470}
\pgfmath@def{atan}{662}{33.50455}		\pgfmath@def{atan}{663}{33.54437}
\pgfmath@def{atan}{664}{33.58416}		\pgfmath@def{atan}{665}{33.62390}
\pgfmath@def{atan}{666}{33.66361}		\pgfmath@def{atan}{667}{33.70328}
\pgfmath@def{atan}{668}{33.74292}		\pgfmath@def{atan}{669}{33.78252}
\pgfmath@def{atan}{670}{33.82208}		\pgfmath@def{atan}{671}{33.86161}
\pgfmath@def{atan}{672}{33.90110}		\pgfmath@def{atan}{673}{33.94055}
\pgfmath@def{atan}{674}{33.97997}		\pgfmath@def{atan}{675}{34.01935}
\pgfmath@def{atan}{676}{34.05869}		\pgfmath@def{atan}{677}{34.09800}
\pgfmath@def{atan}{678}{34.13727}		\pgfmath@def{atan}{679}{34.17650}
\pgfmath@def{atan}{680}{34.21570}		\pgfmath@def{atan}{681}{34.25486}
\pgfmath@def{atan}{682}{34.29398}		\pgfmath@def{atan}{683}{34.33307}
\pgfmath@def{atan}{684}{34.37212}		\pgfmath@def{atan}{685}{34.41114}
\pgfmath@def{atan}{686}{34.45012}		\pgfmath@def{atan}{687}{34.48906}
\pgfmath@def{atan}{688}{34.52797}		\pgfmath@def{atan}{689}{34.56684}
\pgfmath@def{atan}{690}{34.60567}		\pgfmath@def{atan}{691}{34.64447}
\pgfmath@def{atan}{692}{34.68323}		\pgfmath@def{atan}{693}{34.72195}
\pgfmath@def{atan}{694}{34.76064}		\pgfmath@def{atan}{695}{34.79930}
\pgfmath@def{atan}{696}{34.83791}		\pgfmath@def{atan}{697}{34.87649}
\pgfmath@def{atan}{698}{34.91504}		\pgfmath@def{atan}{699}{34.95354}
\pgfmath@def{atan}{700}{34.99202}		\pgfmath@def{atan}{701}{35.03045}
\pgfmath@def{atan}{702}{35.06885}		\pgfmath@def{atan}{703}{35.10721}
\pgfmath@def{atan}{704}{35.14554}		\pgfmath@def{atan}{705}{35.18383}
\pgfmath@def{atan}{706}{35.22209}		\pgfmath@def{atan}{707}{35.26031}
\pgfmath@def{atan}{708}{35.29849}		\pgfmath@def{atan}{709}{35.33664}
\pgfmath@def{atan}{710}{35.37475}		\pgfmath@def{atan}{711}{35.41282}
\pgfmath@def{atan}{712}{35.45086}		\pgfmath@def{atan}{713}{35.48886}
\pgfmath@def{atan}{714}{35.52683}		\pgfmath@def{atan}{715}{35.56476}
\pgfmath@def{atan}{716}{35.60266}		\pgfmath@def{atan}{717}{35.64052}
\pgfmath@def{atan}{718}{35.67834}		\pgfmath@def{atan}{719}{35.71613}
\pgfmath@def{atan}{720}{35.75388}		\pgfmath@def{atan}{721}{35.79160}
\pgfmath@def{atan}{722}{35.82928}		\pgfmath@def{atan}{723}{35.86692}
\pgfmath@def{atan}{724}{35.90453}		\pgfmath@def{atan}{725}{35.94211}
\pgfmath@def{atan}{726}{35.97965}		\pgfmath@def{atan}{727}{36.01715}
\pgfmath@def{atan}{728}{36.05461}		\pgfmath@def{atan}{729}{36.09204}
\pgfmath@def{atan}{730}{36.12944}		\pgfmath@def{atan}{731}{36.16680}
\pgfmath@def{atan}{732}{36.20412}		\pgfmath@def{atan}{733}{36.24141}
\pgfmath@def{atan}{734}{36.27866}		\pgfmath@def{atan}{735}{36.31588}
\pgfmath@def{atan}{736}{36.35306}		\pgfmath@def{atan}{737}{36.39021}
\pgfmath@def{atan}{738}{36.42732}		\pgfmath@def{atan}{739}{36.46440}
\pgfmath@def{atan}{740}{36.50144}		\pgfmath@def{atan}{741}{36.53844}
\pgfmath@def{atan}{742}{36.57541}		\pgfmath@def{atan}{743}{36.61234}
\pgfmath@def{atan}{744}{36.64924}		\pgfmath@def{atan}{745}{36.68611}
\pgfmath@def{atan}{746}{36.72293}		\pgfmath@def{atan}{747}{36.75973}
\pgfmath@def{atan}{748}{36.79648}		\pgfmath@def{atan}{749}{36.83321}
\pgfmath@def{atan}{750}{36.86989}		\pgfmath@def{atan}{751}{36.90654}
\pgfmath@def{atan}{752}{36.94316}		\pgfmath@def{atan}{753}{36.97974}
\pgfmath@def{atan}{754}{37.01629}		\pgfmath@def{atan}{755}{37.05280}
\pgfmath@def{atan}{756}{37.08928}		\pgfmath@def{atan}{757}{37.12572}
\pgfmath@def{atan}{758}{37.16212}		\pgfmath@def{atan}{759}{37.19849}
\pgfmath@def{atan}{760}{37.23483}		\pgfmath@def{atan}{761}{37.27113}
\pgfmath@def{atan}{762}{37.30740}		\pgfmath@def{atan}{763}{37.34363}
\pgfmath@def{atan}{764}{37.37982}		\pgfmath@def{atan}{765}{37.41598}
\pgfmath@def{atan}{766}{37.45211}		\pgfmath@def{atan}{767}{37.48820}
\pgfmath@def{atan}{768}{37.52426}		\pgfmath@def{atan}{769}{37.56028}
\pgfmath@def{atan}{770}{37.59627}		\pgfmath@def{atan}{771}{37.63222}
\pgfmath@def{atan}{772}{37.66814}		\pgfmath@def{atan}{773}{37.70402}
\pgfmath@def{atan}{774}{37.73987}		\pgfmath@def{atan}{775}{37.77568}
\pgfmath@def{atan}{776}{37.81146}		\pgfmath@def{atan}{777}{37.84720}
\pgfmath@def{atan}{778}{37.88291}		\pgfmath@def{atan}{779}{37.91859}
\pgfmath@def{atan}{780}{37.95423}		\pgfmath@def{atan}{781}{37.98983}
\pgfmath@def{atan}{782}{38.02540}		\pgfmath@def{atan}{783}{38.06094}
\pgfmath@def{atan}{784}{38.09644}		\pgfmath@def{atan}{785}{38.13191}
\pgfmath@def{atan}{786}{38.16734}		\pgfmath@def{atan}{787}{38.20274}
\pgfmath@def{atan}{788}{38.23811}		\pgfmath@def{atan}{789}{38.27344}
\pgfmath@def{atan}{790}{38.30873}		\pgfmath@def{atan}{791}{38.34399}
\pgfmath@def{atan}{792}{38.37922}		\pgfmath@def{atan}{793}{38.41441}
\pgfmath@def{atan}{794}{38.44957}		\pgfmath@def{atan}{795}{38.48469}
\pgfmath@def{atan}{796}{38.51979}		\pgfmath@def{atan}{797}{38.55484}
\pgfmath@def{atan}{798}{38.58986}		\pgfmath@def{atan}{799}{38.62485}
\pgfmath@def{atan}{800}{38.65980}		\pgfmath@def{atan}{801}{38.69472}
\pgfmath@def{atan}{802}{38.72961}		\pgfmath@def{atan}{803}{38.76446}
\pgfmath@def{atan}{804}{38.79928}		\pgfmath@def{atan}{805}{38.83406}
\pgfmath@def{atan}{806}{38.86881}		\pgfmath@def{atan}{807}{38.90353}
\pgfmath@def{atan}{808}{38.93821}		\pgfmath@def{atan}{809}{38.97285}
\pgfmath@def{atan}{810}{39.00747}		\pgfmath@def{atan}{811}{39.04205}
\pgfmath@def{atan}{812}{39.07659}		\pgfmath@def{atan}{813}{39.11111}
\pgfmath@def{atan}{814}{39.14558}		\pgfmath@def{atan}{815}{39.18003}
\pgfmath@def{atan}{816}{39.21444}		\pgfmath@def{atan}{817}{39.24882}
\pgfmath@def{atan}{818}{39.28316}		\pgfmath@def{atan}{819}{39.31747}
\pgfmath@def{atan}{820}{39.35175}		\pgfmath@def{atan}{821}{39.38599}
\pgfmath@def{atan}{822}{39.42020}		\pgfmath@def{atan}{823}{39.45438}
\pgfmath@def{atan}{824}{39.48852}		\pgfmath@def{atan}{825}{39.52263}
\pgfmath@def{atan}{826}{39.55670}		\pgfmath@def{atan}{827}{39.59074}
\pgfmath@def{atan}{828}{39.62475}		\pgfmath@def{atan}{829}{39.65873}
\pgfmath@def{atan}{830}{39.69267}		\pgfmath@def{atan}{831}{39.72658}
\pgfmath@def{atan}{832}{39.76045}		\pgfmath@def{atan}{833}{39.79429}
\pgfmath@def{atan}{834}{39.82810}		\pgfmath@def{atan}{835}{39.86188}
\pgfmath@def{atan}{836}{39.89562}		\pgfmath@def{atan}{837}{39.92933}
\pgfmath@def{atan}{838}{39.96300}		\pgfmath@def{atan}{839}{39.99665}
\pgfmath@def{atan}{840}{40.03025}		\pgfmath@def{atan}{841}{40.06383}
\pgfmath@def{atan}{842}{40.09737}		\pgfmath@def{atan}{843}{40.13088}
\pgfmath@def{atan}{844}{40.16436}		\pgfmath@def{atan}{845}{40.19781}
\pgfmath@def{atan}{846}{40.23122}		\pgfmath@def{atan}{847}{40.26459}
\pgfmath@def{atan}{848}{40.29794}		\pgfmath@def{atan}{849}{40.33125}
\pgfmath@def{atan}{850}{40.36453}		\pgfmath@def{atan}{851}{40.39778}
\pgfmath@def{atan}{852}{40.43099}		\pgfmath@def{atan}{853}{40.46417}
\pgfmath@def{atan}{854}{40.49732}		\pgfmath@def{atan}{855}{40.53044}
\pgfmath@def{atan}{856}{40.56352}		\pgfmath@def{atan}{857}{40.59657}
\pgfmath@def{atan}{858}{40.62959}		\pgfmath@def{atan}{859}{40.66257}
\pgfmath@def{atan}{860}{40.69553}		\pgfmath@def{atan}{861}{40.72845}
\pgfmath@def{atan}{862}{40.76133}		\pgfmath@def{atan}{863}{40.79419}
\pgfmath@def{atan}{864}{40.82701}		\pgfmath@def{atan}{865}{40.85980}
\pgfmath@def{atan}{866}{40.89256}		\pgfmath@def{atan}{867}{40.92528}
\pgfmath@def{atan}{868}{40.95798}		\pgfmath@def{atan}{869}{40.99064}
\pgfmath@def{atan}{870}{41.02326}		\pgfmath@def{atan}{871}{41.05586}
\pgfmath@def{atan}{872}{41.08842}		\pgfmath@def{atan}{873}{41.12095}
\pgfmath@def{atan}{874}{41.15345}		\pgfmath@def{atan}{875}{41.18592}
\pgfmath@def{atan}{876}{41.21836}		\pgfmath@def{atan}{877}{41.25076}
\pgfmath@def{atan}{878}{41.28313}		\pgfmath@def{atan}{879}{41.31547}
\pgfmath@def{atan}{880}{41.34777}		\pgfmath@def{atan}{881}{41.38005}
\pgfmath@def{atan}{882}{41.41229}		\pgfmath@def{atan}{883}{41.44450}
\pgfmath@def{atan}{884}{41.47668}		\pgfmath@def{atan}{885}{41.50882}
\pgfmath@def{atan}{886}{41.54094}		\pgfmath@def{atan}{887}{41.57302}
\pgfmath@def{atan}{888}{41.60507}		\pgfmath@def{atan}{889}{41.63709}
\pgfmath@def{atan}{890}{41.66908}		\pgfmath@def{atan}{891}{41.70103}
\pgfmath@def{atan}{892}{41.73296}		\pgfmath@def{atan}{893}{41.76485}
\pgfmath@def{atan}{894}{41.79671}		\pgfmath@def{atan}{895}{41.82854}
\pgfmath@def{atan}{896}{41.86034}		\pgfmath@def{atan}{897}{41.89210}
\pgfmath@def{atan}{898}{41.92383}		\pgfmath@def{atan}{899}{41.95554}
\pgfmath@def{atan}{900}{41.98721}		\pgfmath@def{atan}{901}{42.01885}
\pgfmath@def{atan}{902}{42.05046}		\pgfmath@def{atan}{903}{42.08203}
\pgfmath@def{atan}{904}{42.11358}		\pgfmath@def{atan}{905}{42.14509}
\pgfmath@def{atan}{906}{42.17657}		\pgfmath@def{atan}{907}{42.20802}
\pgfmath@def{atan}{908}{42.23944}		\pgfmath@def{atan}{909}{42.27083}
\pgfmath@def{atan}{910}{42.30219}		\pgfmath@def{atan}{911}{42.33352}
\pgfmath@def{atan}{912}{42.36481}		\pgfmath@def{atan}{913}{42.39607}
\pgfmath@def{atan}{914}{42.42731}		\pgfmath@def{atan}{915}{42.45851}
\pgfmath@def{atan}{916}{42.48968}		\pgfmath@def{atan}{917}{42.52082}
\pgfmath@def{atan}{918}{42.55193}		\pgfmath@def{atan}{919}{42.58300}
\pgfmath@def{atan}{920}{42.61405}		\pgfmath@def{atan}{921}{42.64507}
\pgfmath@def{atan}{922}{42.67605}		\pgfmath@def{atan}{923}{42.70701}
\pgfmath@def{atan}{924}{42.73793}		\pgfmath@def{atan}{925}{42.76882}
\pgfmath@def{atan}{926}{42.79968}		\pgfmath@def{atan}{927}{42.83051}
\pgfmath@def{atan}{928}{42.86131}		\pgfmath@def{atan}{929}{42.89208}
\pgfmath@def{atan}{930}{42.92282}		\pgfmath@def{atan}{931}{42.95353}
\pgfmath@def{atan}{932}{42.98421}		\pgfmath@def{atan}{933}{43.01485}
\pgfmath@def{atan}{934}{43.04547}		\pgfmath@def{atan}{935}{43.07605}
\pgfmath@def{atan}{936}{43.10661}		\pgfmath@def{atan}{937}{43.13713}
\pgfmath@def{atan}{938}{43.16763}		\pgfmath@def{atan}{939}{43.19809}
\pgfmath@def{atan}{940}{43.22853}		\pgfmath@def{atan}{941}{43.25893}
\pgfmath@def{atan}{942}{43.28930}		\pgfmath@def{atan}{943}{43.31964}
\pgfmath@def{atan}{944}{43.34996}		\pgfmath@def{atan}{945}{43.38024}
\pgfmath@def{atan}{946}{43.41049}		\pgfmath@def{atan}{947}{43.44071}
\pgfmath@def{atan}{948}{43.47090}		\pgfmath@def{atan}{949}{43.50106}
\pgfmath@def{atan}{950}{43.53119}		\pgfmath@def{atan}{951}{43.56130}
\pgfmath@def{atan}{952}{43.59137}		\pgfmath@def{atan}{953}{43.62141}
\pgfmath@def{atan}{954}{43.65142}		\pgfmath@def{atan}{955}{43.68140}
\pgfmath@def{atan}{956}{43.71135}		\pgfmath@def{atan}{957}{43.74127}
\pgfmath@def{atan}{958}{43.77116}		\pgfmath@def{atan}{959}{43.80102}
\pgfmath@def{atan}{960}{43.83086}		\pgfmath@def{atan}{961}{43.86066}
\pgfmath@def{atan}{962}{43.89043}		\pgfmath@def{atan}{963}{43.92017}
\pgfmath@def{atan}{964}{43.94988}		\pgfmath@def{atan}{965}{43.97957}
\pgfmath@def{atan}{966}{44.00922}		\pgfmath@def{atan}{967}{44.03884}
\pgfmath@def{atan}{968}{44.06844}		\pgfmath@def{atan}{969}{44.09800}
\pgfmath@def{atan}{970}{44.12754}		\pgfmath@def{atan}{971}{44.15704}
\pgfmath@def{atan}{972}{44.18652}		\pgfmath@def{atan}{973}{44.21597}
\pgfmath@def{atan}{974}{44.24538}		\pgfmath@def{atan}{975}{44.27477}
\pgfmath@def{atan}{976}{44.30413}		\pgfmath@def{atan}{977}{44.33346}
\pgfmath@def{atan}{978}{44.36276}		\pgfmath@def{atan}{979}{44.39203}
\pgfmath@def{atan}{980}{44.42127}		\pgfmath@def{atan}{981}{44.45048}
\pgfmath@def{atan}{982}{44.47966}		\pgfmath@def{atan}{983}{44.50882}
\pgfmath@def{atan}{984}{44.53794}		\pgfmath@def{atan}{985}{44.56704}
\pgfmath@def{atan}{986}{44.59610}		\pgfmath@def{atan}{987}{44.62514}
\pgfmath@def{atan}{988}{44.65415}		\pgfmath@def{atan}{989}{44.68313}
\pgfmath@def{atan}{990}{44.71208}		\pgfmath@def{atan}{991}{44.74100}
\pgfmath@def{atan}{992}{44.76989}		\pgfmath@def{atan}{993}{44.79876}
\pgfmath@def{atan}{994}{44.82759}		\pgfmath@def{atan}{995}{44.85640}
\pgfmath@def{atan}{996}{44.88517}		\pgfmath@def{atan}{997}{44.91392}
\pgfmath@def{atan}{998}{44.94264}		\pgfmath@def{atan}{999}{44.97133}
\pgfmath@def{atan}{1000}{45.00000}		

\pgfmath@def{asin}{0}{0.00000}		\pgfmath@def{asin}{1}{0.05729}
\pgfmath@def{asin}{2}{0.11459}		\pgfmath@def{asin}{3}{0.17188}
\pgfmath@def{asin}{4}{0.22918}		\pgfmath@def{asin}{5}{0.28648}
\pgfmath@def{asin}{6}{0.34377}		\pgfmath@def{asin}{7}{0.40107}
\pgfmath@def{asin}{8}{0.45837}		\pgfmath@def{asin}{9}{0.51566}
\pgfmath@def{asin}{10}{0.57296}		\pgfmath@def{asin}{11}{0.63026}
\pgfmath@def{asin}{12}{0.68756}		\pgfmath@def{asin}{13}{0.74486}
\pgfmath@def{asin}{14}{0.80216}		\pgfmath@def{asin}{15}{0.85946}
\pgfmath@def{asin}{16}{0.91677}		\pgfmath@def{asin}{17}{0.97407}
\pgfmath@def{asin}{18}{1.03138}		\pgfmath@def{asin}{19}{1.08868}
\pgfmath@def{asin}{20}{1.14599}		\pgfmath@def{asin}{21}{1.20330}
\pgfmath@def{asin}{22}{1.26060}		\pgfmath@def{asin}{23}{1.31791}
\pgfmath@def{asin}{24}{1.37523}		\pgfmath@def{asin}{25}{1.43254}
\pgfmath@def{asin}{26}{1.48985}		\pgfmath@def{asin}{27}{1.54717}
\pgfmath@def{asin}{28}{1.60449}		\pgfmath@def{asin}{29}{1.66181}
\pgfmath@def{asin}{30}{1.71913}		\pgfmath@def{asin}{31}{1.77645}
\pgfmath@def{asin}{32}{1.83377}		\pgfmath@def{asin}{33}{1.89110}
\pgfmath@def{asin}{34}{1.94843}		\pgfmath@def{asin}{35}{2.00576}
\pgfmath@def{asin}{36}{2.06309}		\pgfmath@def{asin}{37}{2.12042}
\pgfmath@def{asin}{38}{2.17776}		\pgfmath@def{asin}{39}{2.23510}
\pgfmath@def{asin}{40}{2.29244}		\pgfmath@def{asin}{41}{2.34978}
\pgfmath@def{asin}{42}{2.40713}		\pgfmath@def{asin}{43}{2.46447}
\pgfmath@def{asin}{44}{2.52182}		\pgfmath@def{asin}{45}{2.57918}
\pgfmath@def{asin}{46}{2.63653}		\pgfmath@def{asin}{47}{2.69389}
\pgfmath@def{asin}{48}{2.75125}		\pgfmath@def{asin}{49}{2.80861}
\pgfmath@def{asin}{50}{2.86598}		\pgfmath@def{asin}{51}{2.92335}
\pgfmath@def{asin}{52}{2.98072}		\pgfmath@def{asin}{53}{3.03810}
\pgfmath@def{asin}{54}{3.09547}		\pgfmath@def{asin}{55}{3.15285}
\pgfmath@def{asin}{56}{3.21024}		\pgfmath@def{asin}{57}{3.26763}
\pgfmath@def{asin}{58}{3.32502}		\pgfmath@def{asin}{59}{3.38241}
\pgfmath@def{asin}{60}{3.43981}		\pgfmath@def{asin}{61}{3.49721}
\pgfmath@def{asin}{62}{3.55461}		\pgfmath@def{asin}{63}{3.61202}
\pgfmath@def{asin}{64}{3.66943}		\pgfmath@def{asin}{65}{3.72685}
\pgfmath@def{asin}{66}{3.78427}		\pgfmath@def{asin}{67}{3.84169}
\pgfmath@def{asin}{68}{3.89912}		\pgfmath@def{asin}{69}{3.95655}
\pgfmath@def{asin}{70}{4.01398}		\pgfmath@def{asin}{71}{4.07142}
\pgfmath@def{asin}{72}{4.12886}		\pgfmath@def{asin}{73}{4.18631}
\pgfmath@def{asin}{74}{4.24376}		\pgfmath@def{asin}{75}{4.30122}
\pgfmath@def{asin}{76}{4.35868}		\pgfmath@def{asin}{77}{4.41614}
\pgfmath@def{asin}{78}{4.47361}		\pgfmath@def{asin}{79}{4.53108}
\pgfmath@def{asin}{80}{4.58856}		\pgfmath@def{asin}{81}{4.64604}
\pgfmath@def{asin}{82}{4.70353}		\pgfmath@def{asin}{83}{4.76102}
\pgfmath@def{asin}{84}{4.81852}		\pgfmath@def{asin}{85}{4.87602}
\pgfmath@def{asin}{86}{4.93353}		\pgfmath@def{asin}{87}{4.99104}
\pgfmath@def{asin}{88}{5.04855}		\pgfmath@def{asin}{89}{5.10608}
\pgfmath@def{asin}{90}{5.16360}		\pgfmath@def{asin}{91}{5.22113}
\pgfmath@def{asin}{92}{5.27867}		\pgfmath@def{asin}{93}{5.33621}
\pgfmath@def{asin}{94}{5.39376}		\pgfmath@def{asin}{95}{5.45132}
\pgfmath@def{asin}{96}{5.50887}		\pgfmath@def{asin}{97}{5.56644}
\pgfmath@def{asin}{98}{5.62401}		\pgfmath@def{asin}{99}{5.68158}
\pgfmath@def{asin}{100}{5.73917}		\pgfmath@def{asin}{101}{5.79675}
\pgfmath@def{asin}{102}{5.85435}		\pgfmath@def{asin}{103}{5.91195}
\pgfmath@def{asin}{104}{5.96955}		\pgfmath@def{asin}{105}{6.02716}
\pgfmath@def{asin}{106}{6.08478}		\pgfmath@def{asin}{107}{6.14240}
\pgfmath@def{asin}{108}{6.20003}		\pgfmath@def{asin}{109}{6.25767}
\pgfmath@def{asin}{110}{6.31531}		\pgfmath@def{asin}{111}{6.37296}
\pgfmath@def{asin}{112}{6.43062}		\pgfmath@def{asin}{113}{6.48828}
\pgfmath@def{asin}{114}{6.54595}		\pgfmath@def{asin}{115}{6.60362}
\pgfmath@def{asin}{116}{6.66130}		\pgfmath@def{asin}{117}{6.71899}
\pgfmath@def{asin}{118}{6.77669}		\pgfmath@def{asin}{119}{6.83439}
\pgfmath@def{asin}{120}{6.89210}		\pgfmath@def{asin}{121}{6.94981}
\pgfmath@def{asin}{122}{7.00754}		\pgfmath@def{asin}{123}{7.06527}
\pgfmath@def{asin}{124}{7.12301}		\pgfmath@def{asin}{125}{7.18075}
\pgfmath@def{asin}{126}{7.23850}		\pgfmath@def{asin}{127}{7.29626}
\pgfmath@def{asin}{128}{7.35403}		\pgfmath@def{asin}{129}{7.41181}
\pgfmath@def{asin}{130}{7.46959}		\pgfmath@def{asin}{131}{7.52738}
\pgfmath@def{asin}{132}{7.58518}		\pgfmath@def{asin}{133}{7.64298}
\pgfmath@def{asin}{134}{7.70079}		\pgfmath@def{asin}{135}{7.75862}
\pgfmath@def{asin}{136}{7.81644}		\pgfmath@def{asin}{137}{7.87428}
\pgfmath@def{asin}{138}{7.93213}		\pgfmath@def{asin}{139}{7.98998}
\pgfmath@def{asin}{140}{8.04784}		\pgfmath@def{asin}{141}{8.10571}
\pgfmath@def{asin}{142}{8.16359}		\pgfmath@def{asin}{143}{8.22148}
\pgfmath@def{asin}{144}{8.27937}		\pgfmath@def{asin}{145}{8.33727}
\pgfmath@def{asin}{146}{8.39519}		\pgfmath@def{asin}{147}{8.45311}
\pgfmath@def{asin}{148}{8.51104}		\pgfmath@def{asin}{149}{8.56898}
\pgfmath@def{asin}{150}{8.62692}		\pgfmath@def{asin}{151}{8.68488}
\pgfmath@def{asin}{152}{8.74284}		\pgfmath@def{asin}{153}{8.80082}
\pgfmath@def{asin}{154}{8.85880}		\pgfmath@def{asin}{155}{8.91679}
\pgfmath@def{asin}{156}{8.97479}		\pgfmath@def{asin}{157}{9.03280}
\pgfmath@def{asin}{158}{9.09082}		\pgfmath@def{asin}{159}{9.14885}
\pgfmath@def{asin}{160}{9.20689}		\pgfmath@def{asin}{161}{9.26494}
\pgfmath@def{asin}{162}{9.32300}		\pgfmath@def{asin}{163}{9.38107}
\pgfmath@def{asin}{164}{9.43914}		\pgfmath@def{asin}{165}{9.49723}
\pgfmath@def{asin}{166}{9.55533}		\pgfmath@def{asin}{167}{9.61343}
\pgfmath@def{asin}{168}{9.67155}		\pgfmath@def{asin}{169}{9.72968}
\pgfmath@def{asin}{170}{9.78781}		\pgfmath@def{asin}{171}{9.84596}
\pgfmath@def{asin}{172}{9.90412}		\pgfmath@def{asin}{173}{9.96229}
\pgfmath@def{asin}{174}{10.02047}		\pgfmath@def{asin}{175}{10.07865}
\pgfmath@def{asin}{176}{10.13685}		\pgfmath@def{asin}{177}{10.19506}
\pgfmath@def{asin}{178}{10.25328}		\pgfmath@def{asin}{179}{10.31151}
\pgfmath@def{asin}{180}{10.36976}		\pgfmath@def{asin}{181}{10.42801}
\pgfmath@def{asin}{182}{10.48627}		\pgfmath@def{asin}{183}{10.54455}
\pgfmath@def{asin}{184}{10.60283}		\pgfmath@def{asin}{185}{10.66113}
\pgfmath@def{asin}{186}{10.71944}		\pgfmath@def{asin}{187}{10.77775}
\pgfmath@def{asin}{188}{10.83608}		\pgfmath@def{asin}{189}{10.89443}
\pgfmath@def{asin}{190}{10.95278}		\pgfmath@def{asin}{191}{11.01114}
\pgfmath@def{asin}{192}{11.06952}		\pgfmath@def{asin}{193}{11.12791}
\pgfmath@def{asin}{194}{11.18631}		\pgfmath@def{asin}{195}{11.24472}
\pgfmath@def{asin}{196}{11.30314}		\pgfmath@def{asin}{197}{11.36158}
\pgfmath@def{asin}{198}{11.42002}		\pgfmath@def{asin}{199}{11.47848}
\pgfmath@def{asin}{200}{11.53695}		\pgfmath@def{asin}{201}{11.59544}
\pgfmath@def{asin}{202}{11.65393}		\pgfmath@def{asin}{203}{11.71244}
\pgfmath@def{asin}{204}{11.77096}		\pgfmath@def{asin}{205}{11.82949}
\pgfmath@def{asin}{206}{11.88804}		\pgfmath@def{asin}{207}{11.94660}
\pgfmath@def{asin}{208}{12.00517}		\pgfmath@def{asin}{209}{12.06375}
\pgfmath@def{asin}{210}{12.12235}		\pgfmath@def{asin}{211}{12.18096}
\pgfmath@def{asin}{212}{12.23958}		\pgfmath@def{asin}{213}{12.29821}
\pgfmath@def{asin}{214}{12.35686}		\pgfmath@def{asin}{215}{12.41552}
\pgfmath@def{asin}{216}{12.47420}		\pgfmath@def{asin}{217}{12.53288}
\pgfmath@def{asin}{218}{12.59159}		\pgfmath@def{asin}{219}{12.65030}
\pgfmath@def{asin}{220}{12.70903}		\pgfmath@def{asin}{221}{12.76777}
\pgfmath@def{asin}{222}{12.82653}		\pgfmath@def{asin}{223}{12.88529}
\pgfmath@def{asin}{224}{12.94408}		\pgfmath@def{asin}{225}{13.00287}
\pgfmath@def{asin}{226}{13.06168}		\pgfmath@def{asin}{227}{13.12051}
\pgfmath@def{asin}{228}{13.17935}		\pgfmath@def{asin}{229}{13.23820}
\pgfmath@def{asin}{230}{13.29707}		\pgfmath@def{asin}{231}{13.35595}
\pgfmath@def{asin}{232}{13.41484}		\pgfmath@def{asin}{233}{13.47375}
\pgfmath@def{asin}{234}{13.53268}		\pgfmath@def{asin}{235}{13.59162}
\pgfmath@def{asin}{236}{13.65057}		\pgfmath@def{asin}{237}{13.70954}
\pgfmath@def{asin}{238}{13.76852}		\pgfmath@def{asin}{239}{13.82752}
\pgfmath@def{asin}{240}{13.88654}		\pgfmath@def{asin}{241}{13.94556}
\pgfmath@def{asin}{242}{14.00461}		\pgfmath@def{asin}{243}{14.06367}
\pgfmath@def{asin}{244}{14.12274}		\pgfmath@def{asin}{245}{14.18183}
\pgfmath@def{asin}{246}{14.24093}		\pgfmath@def{asin}{247}{14.30005}
\pgfmath@def{asin}{248}{14.35919}		\pgfmath@def{asin}{249}{14.41834}
\pgfmath@def{asin}{250}{14.47751}		\pgfmath@def{asin}{251}{14.53669}
\pgfmath@def{asin}{252}{14.59589}		\pgfmath@def{asin}{253}{14.65510}
\pgfmath@def{asin}{254}{14.71433}		\pgfmath@def{asin}{255}{14.77358}
\pgfmath@def{asin}{256}{14.83284}		\pgfmath@def{asin}{257}{14.89212}
\pgfmath@def{asin}{258}{14.95142}		\pgfmath@def{asin}{259}{15.01073}
\pgfmath@def{asin}{260}{15.07006}		\pgfmath@def{asin}{261}{15.12940}
\pgfmath@def{asin}{262}{15.18876}		\pgfmath@def{asin}{263}{15.24814}
\pgfmath@def{asin}{264}{15.30754}		\pgfmath@def{asin}{265}{15.36695}
\pgfmath@def{asin}{266}{15.42638}		\pgfmath@def{asin}{267}{15.48582}
\pgfmath@def{asin}{268}{15.54529}		\pgfmath@def{asin}{269}{15.60477}
\pgfmath@def{asin}{270}{15.66426}		\pgfmath@def{asin}{271}{15.72378}
\pgfmath@def{asin}{272}{15.78331}		\pgfmath@def{asin}{273}{15.84286}
\pgfmath@def{asin}{274}{15.90243}		\pgfmath@def{asin}{275}{15.96201}
\pgfmath@def{asin}{276}{16.02161}		\pgfmath@def{asin}{277}{16.08123}
\pgfmath@def{asin}{278}{16.14087}		\pgfmath@def{asin}{279}{16.20053}
\pgfmath@def{asin}{280}{16.26020}		\pgfmath@def{asin}{281}{16.31989}
\pgfmath@def{asin}{282}{16.37960}		\pgfmath@def{asin}{283}{16.43933}
\pgfmath@def{asin}{284}{16.49908}		\pgfmath@def{asin}{285}{16.55884}
\pgfmath@def{asin}{286}{16.61863}		\pgfmath@def{asin}{287}{16.67843}
\pgfmath@def{asin}{288}{16.73825}		\pgfmath@def{asin}{289}{16.79809}
\pgfmath@def{asin}{290}{16.85795}		\pgfmath@def{asin}{291}{16.91783}
\pgfmath@def{asin}{292}{16.97773}		\pgfmath@def{asin}{293}{17.03764}
\pgfmath@def{asin}{294}{17.09758}		\pgfmath@def{asin}{295}{17.15753}
\pgfmath@def{asin}{296}{17.21751}		\pgfmath@def{asin}{297}{17.27750}
\pgfmath@def{asin}{298}{17.33751}		\pgfmath@def{asin}{299}{17.39755}
\pgfmath@def{asin}{300}{17.45760}		\pgfmath@def{asin}{301}{17.51767}
\pgfmath@def{asin}{302}{17.57776}		\pgfmath@def{asin}{303}{17.63788}
\pgfmath@def{asin}{304}{17.69801}		\pgfmath@def{asin}{305}{17.75816}
\pgfmath@def{asin}{306}{17.81833}		\pgfmath@def{asin}{307}{17.87852}
\pgfmath@def{asin}{308}{17.93874}		\pgfmath@def{asin}{309}{17.99897}
\pgfmath@def{asin}{310}{18.05923}		\pgfmath@def{asin}{311}{18.11950}
\pgfmath@def{asin}{312}{18.17980}		\pgfmath@def{asin}{313}{18.24011}
\pgfmath@def{asin}{314}{18.30045}		\pgfmath@def{asin}{315}{18.36081}
\pgfmath@def{asin}{316}{18.42119}		\pgfmath@def{asin}{317}{18.48159}
\pgfmath@def{asin}{318}{18.54201}		\pgfmath@def{asin}{319}{18.60246}
\pgfmath@def{asin}{320}{18.66292}		\pgfmath@def{asin}{321}{18.72341}
\pgfmath@def{asin}{322}{18.78392}		\pgfmath@def{asin}{323}{18.84445}
\pgfmath@def{asin}{324}{18.90500}		\pgfmath@def{asin}{325}{18.96557}
\pgfmath@def{asin}{326}{19.02617}		\pgfmath@def{asin}{327}{19.08678}
\pgfmath@def{asin}{328}{19.14742}		\pgfmath@def{asin}{329}{19.20809}
\pgfmath@def{asin}{330}{19.26877}		\pgfmath@def{asin}{331}{19.32948}
\pgfmath@def{asin}{332}{19.39021}		\pgfmath@def{asin}{333}{19.45096}
\pgfmath@def{asin}{334}{19.51174}		\pgfmath@def{asin}{335}{19.57253}
\pgfmath@def{asin}{336}{19.63335}		\pgfmath@def{asin}{337}{19.69420}
\pgfmath@def{asin}{338}{19.75507}		\pgfmath@def{asin}{339}{19.81596}
\pgfmath@def{asin}{340}{19.87687}		\pgfmath@def{asin}{341}{19.93781}
\pgfmath@def{asin}{342}{19.99877}		\pgfmath@def{asin}{343}{20.05975}
\pgfmath@def{asin}{344}{20.12076}		\pgfmath@def{asin}{345}{20.18179}
\pgfmath@def{asin}{346}{20.24285}		\pgfmath@def{asin}{347}{20.30393}
\pgfmath@def{asin}{348}{20.36503}		\pgfmath@def{asin}{349}{20.42616}
\pgfmath@def{asin}{350}{20.48731}		\pgfmath@def{asin}{351}{20.54849}
\pgfmath@def{asin}{352}{20.60969}		\pgfmath@def{asin}{353}{20.67091}
\pgfmath@def{asin}{354}{20.73216}		\pgfmath@def{asin}{355}{20.79344}
\pgfmath@def{asin}{356}{20.85474}		\pgfmath@def{asin}{357}{20.91607}
\pgfmath@def{asin}{358}{20.97742}		\pgfmath@def{asin}{359}{21.03879}
\pgfmath@def{asin}{360}{21.10019}		\pgfmath@def{asin}{361}{21.16162}
\pgfmath@def{asin}{362}{21.22307}		\pgfmath@def{asin}{363}{21.28455}
\pgfmath@def{asin}{364}{21.34605}		\pgfmath@def{asin}{365}{21.40758}
\pgfmath@def{asin}{366}{21.46913}		\pgfmath@def{asin}{367}{21.53071}
\pgfmath@def{asin}{368}{21.59232}		\pgfmath@def{asin}{369}{21.65395}
\pgfmath@def{asin}{370}{21.71561}		\pgfmath@def{asin}{371}{21.77730}
\pgfmath@def{asin}{372}{21.83901}		\pgfmath@def{asin}{373}{21.90075}
\pgfmath@def{asin}{374}{21.96252}		\pgfmath@def{asin}{375}{22.02431}
\pgfmath@def{asin}{376}{22.08613}		\pgfmath@def{asin}{377}{22.14797}
\pgfmath@def{asin}{378}{22.20985}		\pgfmath@def{asin}{379}{22.27175}
\pgfmath@def{asin}{380}{22.33368}		\pgfmath@def{asin}{381}{22.39563}
\pgfmath@def{asin}{382}{22.45762}		\pgfmath@def{asin}{383}{22.51963}
\pgfmath@def{asin}{384}{22.58167}		\pgfmath@def{asin}{385}{22.64374}
\pgfmath@def{asin}{386}{22.70583}		\pgfmath@def{asin}{387}{22.76795}
\pgfmath@def{asin}{388}{22.83011}		\pgfmath@def{asin}{389}{22.89229}
\pgfmath@def{asin}{390}{22.95449}		\pgfmath@def{asin}{391}{23.01673}
\pgfmath@def{asin}{392}{23.07900}		\pgfmath@def{asin}{393}{23.14129}
\pgfmath@def{asin}{394}{23.20362}		\pgfmath@def{asin}{395}{23.26597}
\pgfmath@def{asin}{396}{23.32835}		\pgfmath@def{asin}{397}{23.39076}
\pgfmath@def{asin}{398}{23.45320}		\pgfmath@def{asin}{399}{23.51567}
\pgfmath@def{asin}{400}{23.57817}		\pgfmath@def{asin}{401}{23.64070}
\pgfmath@def{asin}{402}{23.70326}		\pgfmath@def{asin}{403}{23.76585}
\pgfmath@def{asin}{404}{23.82847}		\pgfmath@def{asin}{405}{23.89112}
\pgfmath@def{asin}{406}{23.95380}		\pgfmath@def{asin}{407}{24.01651}
\pgfmath@def{asin}{408}{24.07926}		\pgfmath@def{asin}{409}{24.14203}
\pgfmath@def{asin}{410}{24.20483}		\pgfmath@def{asin}{411}{24.26766}
\pgfmath@def{asin}{412}{24.33053}		\pgfmath@def{asin}{413}{24.39343}
\pgfmath@def{asin}{414}{24.45635}		\pgfmath@def{asin}{415}{24.51931}
\pgfmath@def{asin}{416}{24.58230}		\pgfmath@def{asin}{417}{24.64532}
\pgfmath@def{asin}{418}{24.70838}		\pgfmath@def{asin}{419}{24.77146}
\pgfmath@def{asin}{420}{24.83458}		\pgfmath@def{asin}{421}{24.89773}
\pgfmath@def{asin}{422}{24.96092}		\pgfmath@def{asin}{423}{25.02413}
\pgfmath@def{asin}{424}{25.08738}		\pgfmath@def{asin}{425}{25.15066}
\pgfmath@def{asin}{426}{25.21397}		\pgfmath@def{asin}{427}{25.27732}
\pgfmath@def{asin}{428}{25.34070}		\pgfmath@def{asin}{429}{25.40411}
\pgfmath@def{asin}{430}{25.46756}		\pgfmath@def{asin}{431}{25.53103}
\pgfmath@def{asin}{432}{25.59455}		\pgfmath@def{asin}{433}{25.65809}
\pgfmath@def{asin}{434}{25.72167}		\pgfmath@def{asin}{435}{25.78529}
\pgfmath@def{asin}{436}{25.84894}		\pgfmath@def{asin}{437}{25.91262}
\pgfmath@def{asin}{438}{25.97634}		\pgfmath@def{asin}{439}{26.04009}
\pgfmath@def{asin}{440}{26.10388}		\pgfmath@def{asin}{441}{26.16770}
\pgfmath@def{asin}{442}{26.23155}		\pgfmath@def{asin}{443}{26.29545}
\pgfmath@def{asin}{444}{26.35937}		\pgfmath@def{asin}{445}{26.42333}
\pgfmath@def{asin}{446}{26.48733}		\pgfmath@def{asin}{447}{26.55136}
\pgfmath@def{asin}{448}{26.61543}		\pgfmath@def{asin}{449}{26.67954}
\pgfmath@def{asin}{450}{26.74368}		\pgfmath@def{asin}{451}{26.80786}
\pgfmath@def{asin}{452}{26.87207}		\pgfmath@def{asin}{453}{26.93632}
\pgfmath@def{asin}{454}{27.00061}		\pgfmath@def{asin}{455}{27.06493}
\pgfmath@def{asin}{456}{27.12929}		\pgfmath@def{asin}{457}{27.19369}
\pgfmath@def{asin}{458}{27.25812}		\pgfmath@def{asin}{459}{27.32259}
\pgfmath@def{asin}{460}{27.38710}		\pgfmath@def{asin}{461}{27.45165}
\pgfmath@def{asin}{462}{27.51623}		\pgfmath@def{asin}{463}{27.58086}
\pgfmath@def{asin}{464}{27.64552}		\pgfmath@def{asin}{465}{27.71022}
\pgfmath@def{asin}{466}{27.77496}		\pgfmath@def{asin}{467}{27.83973}
\pgfmath@def{asin}{468}{27.90455}		\pgfmath@def{asin}{469}{27.96940}
\pgfmath@def{asin}{470}{28.03429}		\pgfmath@def{asin}{471}{28.09922}
\pgfmath@def{asin}{472}{28.16419}		\pgfmath@def{asin}{473}{28.22921}
\pgfmath@def{asin}{474}{28.29426}		\pgfmath@def{asin}{475}{28.35935}
\pgfmath@def{asin}{476}{28.42448}		\pgfmath@def{asin}{477}{28.48965}
\pgfmath@def{asin}{478}{28.55486}		\pgfmath@def{asin}{479}{28.62011}
\pgfmath@def{asin}{480}{28.68540}		\pgfmath@def{asin}{481}{28.75073}
\pgfmath@def{asin}{482}{28.81610}		\pgfmath@def{asin}{483}{28.88152}
\pgfmath@def{asin}{484}{28.94697}		\pgfmath@def{asin}{485}{29.01247}
\pgfmath@def{asin}{486}{29.07801}		\pgfmath@def{asin}{487}{29.14359}
\pgfmath@def{asin}{488}{29.20921}		\pgfmath@def{asin}{489}{29.27487}
\pgfmath@def{asin}{490}{29.34058}		\pgfmath@def{asin}{491}{29.40633}
\pgfmath@def{asin}{492}{29.47212}		\pgfmath@def{asin}{493}{29.53795}
\pgfmath@def{asin}{494}{29.60383}		\pgfmath@def{asin}{495}{29.66975}
\pgfmath@def{asin}{496}{29.73571}		\pgfmath@def{asin}{497}{29.80171}
\pgfmath@def{asin}{498}{29.86776}		\pgfmath@def{asin}{499}{29.93386}
\pgfmath@def{asin}{500}{30.00000}		\pgfmath@def{asin}{501}{30.06618}
\pgfmath@def{asin}{502}{30.13240}		\pgfmath@def{asin}{503}{30.19867}
\pgfmath@def{asin}{504}{30.26499}		\pgfmath@def{asin}{505}{30.33135}
\pgfmath@def{asin}{506}{30.39775}		\pgfmath@def{asin}{507}{30.46420}
\pgfmath@def{asin}{508}{30.53070}		\pgfmath@def{asin}{509}{30.59724}
\pgfmath@def{asin}{510}{30.66383}		\pgfmath@def{asin}{511}{30.73046}
\pgfmath@def{asin}{512}{30.79714}		\pgfmath@def{asin}{513}{30.86386}
\pgfmath@def{asin}{514}{30.93063}		\pgfmath@def{asin}{515}{30.99745}
\pgfmath@def{asin}{516}{31.06432}		\pgfmath@def{asin}{517}{31.13123}
\pgfmath@def{asin}{518}{31.19819}		\pgfmath@def{asin}{519}{31.26519}
\pgfmath@def{asin}{520}{31.33225}		\pgfmath@def{asin}{521}{31.39935}
\pgfmath@def{asin}{522}{31.46650}		\pgfmath@def{asin}{523}{31.53370}
\pgfmath@def{asin}{524}{31.60094}		\pgfmath@def{asin}{525}{31.66824}
\pgfmath@def{asin}{526}{31.73558}		\pgfmath@def{asin}{527}{31.80298}
\pgfmath@def{asin}{528}{31.87042}		\pgfmath@def{asin}{529}{31.93791}
\pgfmath@def{asin}{530}{32.00545}		\pgfmath@def{asin}{531}{32.07304}
\pgfmath@def{asin}{532}{32.14068}		\pgfmath@def{asin}{533}{32.20837}
\pgfmath@def{asin}{534}{32.27611}		\pgfmath@def{asin}{535}{32.34391}
\pgfmath@def{asin}{536}{32.41175}		\pgfmath@def{asin}{537}{32.47964}
\pgfmath@def{asin}{538}{32.54759}		\pgfmath@def{asin}{539}{32.61559}
\pgfmath@def{asin}{540}{32.68363}		\pgfmath@def{asin}{541}{32.75173}
\pgfmath@def{asin}{542}{32.81989}		\pgfmath@def{asin}{543}{32.88809}
\pgfmath@def{asin}{544}{32.95635}		\pgfmath@def{asin}{545}{33.02466}
\pgfmath@def{asin}{546}{33.09302}		\pgfmath@def{asin}{547}{33.16144}
\pgfmath@def{asin}{548}{33.22991}		\pgfmath@def{asin}{549}{33.29843}
\pgfmath@def{asin}{550}{33.36701}		\pgfmath@def{asin}{551}{33.43564}
\pgfmath@def{asin}{552}{33.50433}		\pgfmath@def{asin}{553}{33.57307}
\pgfmath@def{asin}{554}{33.64186}		\pgfmath@def{asin}{555}{33.71071}
\pgfmath@def{asin}{556}{33.77962}		\pgfmath@def{asin}{557}{33.84858}
\pgfmath@def{asin}{558}{33.91759}		\pgfmath@def{asin}{559}{33.98666}
\pgfmath@def{asin}{560}{34.05579}		\pgfmath@def{asin}{561}{34.12498}
\pgfmath@def{asin}{562}{34.19422}		\pgfmath@def{asin}{563}{34.26352}
\pgfmath@def{asin}{564}{34.33287}		\pgfmath@def{asin}{565}{34.40229}
\pgfmath@def{asin}{566}{34.47176}		\pgfmath@def{asin}{567}{34.54129}
\pgfmath@def{asin}{568}{34.61087}		\pgfmath@def{asin}{569}{34.68052}
\pgfmath@def{asin}{570}{34.75022}		\pgfmath@def{asin}{571}{34.81998}
\pgfmath@def{asin}{572}{34.88981}		\pgfmath@def{asin}{573}{34.95969}
\pgfmath@def{asin}{574}{35.02963}		\pgfmath@def{asin}{575}{35.09963}
\pgfmath@def{asin}{576}{35.16969}		\pgfmath@def{asin}{577}{35.23981}
\pgfmath@def{asin}{578}{35.30999}		\pgfmath@def{asin}{579}{35.38023}
\pgfmath@def{asin}{580}{35.45054}		\pgfmath@def{asin}{581}{35.52090}
\pgfmath@def{asin}{582}{35.59133}		\pgfmath@def{asin}{583}{35.66182}
\pgfmath@def{asin}{584}{35.73237}		\pgfmath@def{asin}{585}{35.80299}
\pgfmath@def{asin}{586}{35.87366}		\pgfmath@def{asin}{587}{35.94440}
\pgfmath@def{asin}{588}{36.01521}		\pgfmath@def{asin}{589}{36.08607}
\pgfmath@def{asin}{590}{36.15700}		\pgfmath@def{asin}{591}{36.22800}
\pgfmath@def{asin}{592}{36.29906}		\pgfmath@def{asin}{593}{36.37018}
\pgfmath@def{asin}{594}{36.44137}		\pgfmath@def{asin}{595}{36.51263}
\pgfmath@def{asin}{596}{36.58395}		\pgfmath@def{asin}{597}{36.65533}
\pgfmath@def{asin}{598}{36.72679}		\pgfmath@def{asin}{599}{36.79831}
\pgfmath@def{asin}{600}{36.86989}		\pgfmath@def{asin}{601}{36.94155}
\pgfmath@def{asin}{602}{37.01327}		\pgfmath@def{asin}{603}{37.08506}
\pgfmath@def{asin}{604}{37.15691}		\pgfmath@def{asin}{605}{37.22884}
\pgfmath@def{asin}{606}{37.30083}		\pgfmath@def{asin}{607}{37.37289}
\pgfmath@def{asin}{608}{37.44503}		\pgfmath@def{asin}{609}{37.51723}
\pgfmath@def{asin}{610}{37.58950}		\pgfmath@def{asin}{611}{37.66184}
\pgfmath@def{asin}{612}{37.73425}		\pgfmath@def{asin}{613}{37.80674}
\pgfmath@def{asin}{614}{37.87929}		\pgfmath@def{asin}{615}{37.95192}
\pgfmath@def{asin}{616}{38.02461}		\pgfmath@def{asin}{617}{38.09738}
\pgfmath@def{asin}{618}{38.17023}		\pgfmath@def{asin}{619}{38.24314}
\pgfmath@def{asin}{620}{38.31613}		\pgfmath@def{asin}{621}{38.38919}
\pgfmath@def{asin}{622}{38.46233}		\pgfmath@def{asin}{623}{38.53554}
\pgfmath@def{asin}{624}{38.60882}		\pgfmath@def{asin}{625}{38.68218}
\pgfmath@def{asin}{626}{38.75562}		\pgfmath@def{asin}{627}{38.82913}
\pgfmath@def{asin}{628}{38.90272}		\pgfmath@def{asin}{629}{38.97638}
\pgfmath@def{asin}{630}{39.05012}		\pgfmath@def{asin}{631}{39.12393}
\pgfmath@def{asin}{632}{39.19783}		\pgfmath@def{asin}{633}{39.27180}
\pgfmath@def{asin}{634}{39.34585}		\pgfmath@def{asin}{635}{39.41998}
\pgfmath@def{asin}{636}{39.49419}		\pgfmath@def{asin}{637}{39.56847}
\pgfmath@def{asin}{638}{39.64284}		\pgfmath@def{asin}{639}{39.71729}
\pgfmath@def{asin}{640}{39.79181}		\pgfmath@def{asin}{641}{39.86642}
\pgfmath@def{asin}{642}{39.94111}		\pgfmath@def{asin}{643}{40.01588}
\pgfmath@def{asin}{644}{40.09074}		\pgfmath@def{asin}{645}{40.16567}
\pgfmath@def{asin}{646}{40.24069}		\pgfmath@def{asin}{647}{40.31579}
\pgfmath@def{asin}{648}{40.39098}		\pgfmath@def{asin}{649}{40.46624}
\pgfmath@def{asin}{650}{40.54160}		\pgfmath@def{asin}{651}{40.61704}
\pgfmath@def{asin}{652}{40.69256}		\pgfmath@def{asin}{653}{40.76817}
\pgfmath@def{asin}{654}{40.84386}		\pgfmath@def{asin}{655}{40.91965}
\pgfmath@def{asin}{656}{40.99551}		\pgfmath@def{asin}{657}{41.07147}
\pgfmath@def{asin}{658}{41.14751}		\pgfmath@def{asin}{659}{41.22365}
\pgfmath@def{asin}{660}{41.29987}		\pgfmath@def{asin}{661}{41.37618}
\pgfmath@def{asin}{662}{41.45258}		\pgfmath@def{asin}{663}{41.52907}
\pgfmath@def{asin}{664}{41.60565}		\pgfmath@def{asin}{665}{41.68232}
\pgfmath@def{asin}{666}{41.75908}		\pgfmath@def{asin}{667}{41.83594}
\pgfmath@def{asin}{668}{41.91289}		\pgfmath@def{asin}{669}{41.98993}
\pgfmath@def{asin}{670}{42.06706}		\pgfmath@def{asin}{671}{42.14429}
\pgfmath@def{asin}{672}{42.22161}		\pgfmath@def{asin}{673}{42.29903}
\pgfmath@def{asin}{674}{42.37654}		\pgfmath@def{asin}{675}{42.45415}
\pgfmath@def{asin}{676}{42.53185}		\pgfmath@def{asin}{677}{42.60965}
\pgfmath@def{asin}{678}{42.68755}		\pgfmath@def{asin}{679}{42.76554}
\pgfmath@def{asin}{680}{42.84364}		\pgfmath@def{asin}{681}{42.92183}
\pgfmath@def{asin}{682}{43.00012}		\pgfmath@def{asin}{683}{43.07852}
\pgfmath@def{asin}{684}{43.15701}		\pgfmath@def{asin}{685}{43.23560}
\pgfmath@def{asin}{686}{43.31430}		\pgfmath@def{asin}{687}{43.39310}
\pgfmath@def{asin}{688}{43.47199}		\pgfmath@def{asin}{689}{43.55100}
\pgfmath@def{asin}{690}{43.63010}		\pgfmath@def{asin}{691}{43.70932}
\pgfmath@def{asin}{692}{43.78863}		\pgfmath@def{asin}{693}{43.86805}
\pgfmath@def{asin}{694}{43.94758}		\pgfmath@def{asin}{695}{44.02721}
\pgfmath@def{asin}{696}{44.10695}		\pgfmath@def{asin}{697}{44.18680}
\pgfmath@def{asin}{698}{44.26676}		\pgfmath@def{asin}{699}{44.34682}
\pgfmath@def{asin}{700}{44.42700}		\pgfmath@def{asin}{701}{44.50728}
\pgfmath@def{asin}{702}{44.58768}		\pgfmath@def{asin}{703}{44.66819}
\pgfmath@def{asin}{704}{44.74881}		\pgfmath@def{asin}{705}{44.82954}
\pgfmath@def{asin}{706}{44.91038}		\pgfmath@def{asin}{707}{44.99134}
\pgfmath@def{asin}{708}{45.07242}		\pgfmath@def{asin}{709}{45.15361}
\pgfmath@def{asin}{710}{45.23491}		\pgfmath@def{asin}{711}{45.31633}
\pgfmath@def{asin}{712}{45.39787}		\pgfmath@def{asin}{713}{45.47953}
\pgfmath@def{asin}{714}{45.56130}		\pgfmath@def{asin}{715}{45.64319}
\pgfmath@def{asin}{716}{45.72521}		\pgfmath@def{asin}{717}{45.80734}
\pgfmath@def{asin}{718}{45.88960}		\pgfmath@def{asin}{719}{45.97198}
\pgfmath@def{asin}{720}{46.05448}		\pgfmath@def{asin}{721}{46.13710}
\pgfmath@def{asin}{722}{46.21985}		\pgfmath@def{asin}{723}{46.30272}
\pgfmath@def{asin}{724}{46.38572}		\pgfmath@def{asin}{725}{46.46884}
\pgfmath@def{asin}{726}{46.55210}		\pgfmath@def{asin}{727}{46.63548}
\pgfmath@def{asin}{728}{46.71898}		\pgfmath@def{asin}{729}{46.80262}
\pgfmath@def{asin}{730}{46.88639}		\pgfmath@def{asin}{731}{46.97029}
\pgfmath@def{asin}{732}{47.05432}		\pgfmath@def{asin}{733}{47.13848}
\pgfmath@def{asin}{734}{47.22278}		\pgfmath@def{asin}{735}{47.30721}
\pgfmath@def{asin}{736}{47.39178}		\pgfmath@def{asin}{737}{47.47648}
\pgfmath@def{asin}{738}{47.56132}		\pgfmath@def{asin}{739}{47.64630}
\pgfmath@def{asin}{740}{47.73141}		\pgfmath@def{asin}{741}{47.81667}
\pgfmath@def{asin}{742}{47.90206}		\pgfmath@def{asin}{743}{47.98760}
\pgfmath@def{asin}{744}{48.07327}		\pgfmath@def{asin}{745}{48.15909}
\pgfmath@def{asin}{746}{48.24506}		\pgfmath@def{asin}{747}{48.33117}
\pgfmath@def{asin}{748}{48.41742}		\pgfmath@def{asin}{749}{48.50382}
\pgfmath@def{asin}{750}{48.59037}		\pgfmath@def{asin}{751}{48.67707}
\pgfmath@def{asin}{752}{48.76392}		\pgfmath@def{asin}{753}{48.85092}
\pgfmath@def{asin}{754}{48.93806}		\pgfmath@def{asin}{755}{49.02537}
\pgfmath@def{asin}{756}{49.11282}		\pgfmath@def{asin}{757}{49.20043}
\pgfmath@def{asin}{758}{49.28819}		\pgfmath@def{asin}{759}{49.37611}
\pgfmath@def{asin}{760}{49.46419}		\pgfmath@def{asin}{761}{49.55243}
\pgfmath@def{asin}{762}{49.64083}		\pgfmath@def{asin}{763}{49.72939}
\pgfmath@def{asin}{764}{49.81810}		\pgfmath@def{asin}{765}{49.90699}
\pgfmath@def{asin}{766}{49.99603}		\pgfmath@def{asin}{767}{50.08525}
\pgfmath@def{asin}{768}{50.17462}		\pgfmath@def{asin}{769}{50.26417}
\pgfmath@def{asin}{770}{50.35388}		\pgfmath@def{asin}{771}{50.44377}
\pgfmath@def{asin}{772}{50.53382}		\pgfmath@def{asin}{773}{50.62405}
\pgfmath@def{asin}{774}{50.71445}		\pgfmath@def{asin}{775}{50.80503}
\pgfmath@def{asin}{776}{50.89578}		\pgfmath@def{asin}{777}{50.98671}
\pgfmath@def{asin}{778}{51.07782}		\pgfmath@def{asin}{779}{51.16910}
\pgfmath@def{asin}{780}{51.26057}		\pgfmath@def{asin}{781}{51.35222}
\pgfmath@def{asin}{782}{51.44406}		\pgfmath@def{asin}{783}{51.53607}
\pgfmath@def{asin}{784}{51.62828}		\pgfmath@def{asin}{785}{51.72067}
\pgfmath@def{asin}{786}{51.81326}		\pgfmath@def{asin}{787}{51.90603}
\pgfmath@def{asin}{788}{51.99899}		\pgfmath@def{asin}{789}{52.09215}
\pgfmath@def{asin}{790}{52.18551}		\pgfmath@def{asin}{791}{52.27906}
\pgfmath@def{asin}{792}{52.37280}		\pgfmath@def{asin}{793}{52.46675}
\pgfmath@def{asin}{794}{52.56090}		\pgfmath@def{asin}{795}{52.65525}
\pgfmath@def{asin}{796}{52.74981}		\pgfmath@def{asin}{797}{52.84457}
\pgfmath@def{asin}{798}{52.93953}		\pgfmath@def{asin}{799}{53.03471}
\pgfmath@def{asin}{800}{53.13010}		\pgfmath@def{asin}{801}{53.22570}
\pgfmath@def{asin}{802}{53.32151}		\pgfmath@def{asin}{803}{53.41754}
\pgfmath@def{asin}{804}{53.51379}		\pgfmath@def{asin}{805}{53.61025}
\pgfmath@def{asin}{806}{53.70694}		\pgfmath@def{asin}{807}{53.80385}
\pgfmath@def{asin}{808}{53.90098}		\pgfmath@def{asin}{809}{53.99834}
\pgfmath@def{asin}{810}{54.09593}		\pgfmath@def{asin}{811}{54.19374}
\pgfmath@def{asin}{812}{54.29180}		\pgfmath@def{asin}{813}{54.39008}
\pgfmath@def{asin}{814}{54.48860}		\pgfmath@def{asin}{815}{54.58736}
\pgfmath@def{asin}{816}{54.68636}		\pgfmath@def{asin}{817}{54.78560}
\pgfmath@def{asin}{818}{54.88508}		\pgfmath@def{asin}{819}{54.98481}
\pgfmath@def{asin}{820}{55.08479}		\pgfmath@def{asin}{821}{55.18502}
\pgfmath@def{asin}{822}{55.28550}		\pgfmath@def{asin}{823}{55.38624}
\pgfmath@def{asin}{824}{55.48723}		\pgfmath@def{asin}{825}{55.58849}
\pgfmath@def{asin}{826}{55.69000}		\pgfmath@def{asin}{827}{55.79178}
\pgfmath@def{asin}{828}{55.89383}		\pgfmath@def{asin}{829}{55.99615}
\pgfmath@def{asin}{830}{56.09873}		\pgfmath@def{asin}{831}{56.20160}
\pgfmath@def{asin}{832}{56.30473}		\pgfmath@def{asin}{833}{56.40815}
\pgfmath@def{asin}{834}{56.51185}		\pgfmath@def{asin}{835}{56.61583}
\pgfmath@def{asin}{836}{56.72010}		\pgfmath@def{asin}{837}{56.82467}
\pgfmath@def{asin}{838}{56.92952}		\pgfmath@def{asin}{839}{57.03467}
\pgfmath@def{asin}{840}{57.14012}		\pgfmath@def{asin}{841}{57.24586}
\pgfmath@def{asin}{842}{57.35192}		\pgfmath@def{asin}{843}{57.45828}
\pgfmath@def{asin}{844}{57.56495}		\pgfmath@def{asin}{845}{57.67193}
\pgfmath@def{asin}{846}{57.77923}		\pgfmath@def{asin}{847}{57.88685}
\pgfmath@def{asin}{848}{57.99480}		\pgfmath@def{asin}{849}{58.10307}
\pgfmath@def{asin}{850}{58.21166}		\pgfmath@def{asin}{851}{58.32060}
\pgfmath@def{asin}{852}{58.42987}		\pgfmath@def{asin}{853}{58.53948}
\pgfmath@def{asin}{854}{58.64943}		\pgfmath@def{asin}{855}{58.75973}
\pgfmath@def{asin}{856}{58.87038}		\pgfmath@def{asin}{857}{58.98139}
\pgfmath@def{asin}{858}{59.09275}		\pgfmath@def{asin}{859}{59.20448}
\pgfmath@def{asin}{860}{59.31658}		\pgfmath@def{asin}{861}{59.42904}
\pgfmath@def{asin}{862}{59.54189}		\pgfmath@def{asin}{863}{59.65511}
\pgfmath@def{asin}{864}{59.76871}		\pgfmath@def{asin}{865}{59.88270}
\pgfmath@def{asin}{866}{59.99708}		\pgfmath@def{asin}{867}{60.11187}
\pgfmath@def{asin}{868}{60.22705}		\pgfmath@def{asin}{869}{60.34264}
\pgfmath@def{asin}{870}{60.45863}		\pgfmath@def{asin}{871}{60.57505}
\pgfmath@def{asin}{872}{60.69189}		\pgfmath@def{asin}{873}{60.80915}
\pgfmath@def{asin}{874}{60.92684}		\pgfmath@def{asin}{875}{61.04497}
\pgfmath@def{asin}{876}{61.16354}		\pgfmath@def{asin}{877}{61.28256}
\pgfmath@def{asin}{878}{61.40203}		\pgfmath@def{asin}{879}{61.52196}
\pgfmath@def{asin}{880}{61.64236}		\pgfmath@def{asin}{881}{61.76322}
\pgfmath@def{asin}{882}{61.88457}		\pgfmath@def{asin}{883}{62.00639}
\pgfmath@def{asin}{884}{62.12871}		\pgfmath@def{asin}{885}{62.25152}
\pgfmath@def{asin}{886}{62.37483}		\pgfmath@def{asin}{887}{62.49865}
\pgfmath@def{asin}{888}{62.62299}		\pgfmath@def{asin}{889}{62.74785}
\pgfmath@def{asin}{890}{62.87324}		\pgfmath@def{asin}{891}{62.99917}
\pgfmath@def{asin}{892}{63.12565}		\pgfmath@def{asin}{893}{63.25268}
\pgfmath@def{asin}{894}{63.38027}		\pgfmath@def{asin}{895}{63.50843}
\pgfmath@def{asin}{896}{63.63716}		\pgfmath@def{asin}{897}{63.76649}
\pgfmath@def{asin}{898}{63.89640}		\pgfmath@def{asin}{899}{64.02693}
\pgfmath@def{asin}{900}{64.15806}		\pgfmath@def{asin}{901}{64.28982}
\pgfmath@def{asin}{902}{64.42221}		\pgfmath@def{asin}{903}{64.55524}
\pgfmath@def{asin}{904}{64.68893}		\pgfmath@def{asin}{905}{64.82328}
\pgfmath@def{asin}{906}{64.95830}		\pgfmath@def{asin}{907}{65.09401}
\pgfmath@def{asin}{908}{65.23041}		\pgfmath@def{asin}{909}{65.36752}
\pgfmath@def{asin}{910}{65.50535}		\pgfmath@def{asin}{911}{65.64391}
\pgfmath@def{asin}{912}{65.78321}		\pgfmath@def{asin}{913}{65.92327}
\pgfmath@def{asin}{914}{66.06411}		\pgfmath@def{asin}{915}{66.20572}
\pgfmath@def{asin}{916}{66.34814}		\pgfmath@def{asin}{917}{66.49136}
\pgfmath@def{asin}{918}{66.63542}		\pgfmath@def{asin}{919}{66.78032}
\pgfmath@def{asin}{920}{66.92608}		\pgfmath@def{asin}{921}{67.07271}
\pgfmath@def{asin}{922}{67.22024}		\pgfmath@def{asin}{923}{67.36867}
\pgfmath@def{asin}{924}{67.51804}		\pgfmath@def{asin}{925}{67.66835}
\pgfmath@def{asin}{926}{67.81963}		\pgfmath@def{asin}{927}{67.97189}
\pgfmath@def{asin}{928}{68.12516}		\pgfmath@def{asin}{929}{68.27946}
\pgfmath@def{asin}{930}{68.43481}		\pgfmath@def{asin}{931}{68.59123}
\pgfmath@def{asin}{932}{68.74875}		\pgfmath@def{asin}{933}{68.90739}
\pgfmath@def{asin}{934}{69.06718}		\pgfmath@def{asin}{935}{69.22814}
\pgfmath@def{asin}{936}{69.39030}		\pgfmath@def{asin}{937}{69.55369}
\pgfmath@def{asin}{938}{69.71835}		\pgfmath@def{asin}{939}{69.88429}
\pgfmath@def{asin}{940}{70.05155}		\pgfmath@def{asin}{941}{70.22017}
\pgfmath@def{asin}{942}{70.39018}		\pgfmath@def{asin}{943}{70.56162}
\pgfmath@def{asin}{944}{70.73453}		\pgfmath@def{asin}{945}{70.90894}
\pgfmath@def{asin}{946}{71.08490}		\pgfmath@def{asin}{947}{71.26245}
\pgfmath@def{asin}{948}{71.44164}		\pgfmath@def{asin}{949}{71.62251}
\pgfmath@def{asin}{950}{71.80512}		\pgfmath@def{asin}{951}{71.98952}
\pgfmath@def{asin}{952}{72.17576}		\pgfmath@def{asin}{953}{72.36390}
\pgfmath@def{asin}{954}{72.55401}		\pgfmath@def{asin}{955}{72.74614}
\pgfmath@def{asin}{956}{72.94037}		\pgfmath@def{asin}{957}{73.13678}
\pgfmath@def{asin}{958}{73.33542}		\pgfmath@def{asin}{959}{73.53640}
\pgfmath@def{asin}{960}{73.73979}		\pgfmath@def{asin}{961}{73.94569}
\pgfmath@def{asin}{962}{74.15419}		\pgfmath@def{asin}{963}{74.36540}
\pgfmath@def{asin}{964}{74.57942}		\pgfmath@def{asin}{965}{74.79639}
\pgfmath@def{asin}{966}{75.01642}		\pgfmath@def{asin}{967}{75.23966}
\pgfmath@def{asin}{968}{75.46625}		\pgfmath@def{asin}{969}{75.69635}
\pgfmath@def{asin}{970}{75.93013}		\pgfmath@def{asin}{971}{76.16778}
\pgfmath@def{asin}{972}{76.40950}		\pgfmath@def{asin}{973}{76.65552}
\pgfmath@def{asin}{974}{76.90607}		\pgfmath@def{asin}{975}{77.16143}
\pgfmath@def{asin}{976}{77.42188}		\pgfmath@def{asin}{977}{77.68774}
\pgfmath@def{asin}{978}{77.95939}		\pgfmath@def{asin}{979}{78.23721}
\pgfmath@def{asin}{980}{78.52165}		\pgfmath@def{asin}{981}{78.81323}
\pgfmath@def{asin}{982}{79.11251}		\pgfmath@def{asin}{983}{79.42015}
\pgfmath@def{asin}{984}{79.73690}		\pgfmath@def{asin}{985}{80.06363}
\pgfmath@def{asin}{986}{80.40136}		\pgfmath@def{asin}{987}{80.75129}
\pgfmath@def{asin}{988}{81.11487}		\pgfmath@def{asin}{989}{81.49385}
\pgfmath@def{asin}{990}{81.89038}		\pgfmath@def{asin}{991}{82.30718}
\pgfmath@def{asin}{992}{82.74775}		\pgfmath@def{asin}{993}{83.21671}
\pgfmath@def{asin}{994}{83.72041}		\pgfmath@def{asin}{995}{84.26803}
\pgfmath@def{asin}{996}{84.87360}		\pgfmath@def{asin}{997}{85.56077}
\pgfmath@def{asin}{998}{86.37569}		\pgfmath@def{asin}{999}{87.43744}
\pgfmath@def{asin}{1000}{90.00000}	
	
\pgfmath@def{acos}{0}{90.00000}		\pgfmath@def{acos}{1}{89.94270}
\pgfmath@def{acos}{2}{89.88540}		\pgfmath@def{acos}{3}{89.82811}
\pgfmath@def{acos}{4}{89.77081}		\pgfmath@def{acos}{5}{89.71352}
\pgfmath@def{acos}{6}{89.65622}		\pgfmath@def{acos}{7}{89.59892}
\pgfmath@def{acos}{8}{89.54162}		\pgfmath@def{acos}{9}{89.48433}
\pgfmath@def{acos}{10}{89.42703}		\pgfmath@def{acos}{11}{89.36973}
\pgfmath@def{acos}{12}{89.31243}		\pgfmath@def{acos}{13}{89.25513}
\pgfmath@def{acos}{14}{89.19783}		\pgfmath@def{acos}{15}{89.14053}
\pgfmath@def{acos}{16}{89.08322}		\pgfmath@def{acos}{17}{89.02592}
\pgfmath@def{acos}{18}{88.96862}		\pgfmath@def{acos}{19}{88.91131}
\pgfmath@def{acos}{20}{88.85400}		\pgfmath@def{acos}{21}{88.79670}
\pgfmath@def{acos}{22}{88.73939}		\pgfmath@def{acos}{23}{88.68208}
\pgfmath@def{acos}{24}{88.62476}		\pgfmath@def{acos}{25}{88.56745}
\pgfmath@def{acos}{26}{88.51014}		\pgfmath@def{acos}{27}{88.45282}
\pgfmath@def{acos}{28}{88.39550}		\pgfmath@def{acos}{29}{88.33818}
\pgfmath@def{acos}{30}{88.28086}		\pgfmath@def{acos}{31}{88.22354}
\pgfmath@def{acos}{32}{88.16622}		\pgfmath@def{acos}{33}{88.10889}
\pgfmath@def{acos}{34}{88.05156}		\pgfmath@def{acos}{35}{87.99423}
\pgfmath@def{acos}{36}{87.93690}		\pgfmath@def{acos}{37}{87.87957}
\pgfmath@def{acos}{38}{87.82223}		\pgfmath@def{acos}{39}{87.76489}
\pgfmath@def{acos}{40}{87.70755}		\pgfmath@def{acos}{41}{87.65021}
\pgfmath@def{acos}{42}{87.59286}		\pgfmath@def{acos}{43}{87.53552}
\pgfmath@def{acos}{44}{87.47817}		\pgfmath@def{acos}{45}{87.42081}
\pgfmath@def{acos}{46}{87.36346}		\pgfmath@def{acos}{47}{87.30610}
\pgfmath@def{acos}{48}{87.24874}		\pgfmath@def{acos}{49}{87.19138}
\pgfmath@def{acos}{50}{87.13401}		\pgfmath@def{acos}{51}{87.07664}
\pgfmath@def{acos}{52}{87.01927}		\pgfmath@def{acos}{53}{86.96190}
\pgfmath@def{acos}{54}{86.90452}		\pgfmath@def{acos}{55}{86.84714}
\pgfmath@def{acos}{56}{86.78975}		\pgfmath@def{acos}{57}{86.73237}
\pgfmath@def{acos}{58}{86.67497}		\pgfmath@def{acos}{59}{86.61758}
\pgfmath@def{acos}{60}{86.56018}		\pgfmath@def{acos}{61}{86.50278}
\pgfmath@def{acos}{62}{86.44538}		\pgfmath@def{acos}{63}{86.38797}
\pgfmath@def{acos}{64}{86.33056}		\pgfmath@def{acos}{65}{86.27314}
\pgfmath@def{acos}{66}{86.21572}		\pgfmath@def{acos}{67}{86.15830}
\pgfmath@def{acos}{68}{86.10087}		\pgfmath@def{acos}{69}{86.04344}
\pgfmath@def{acos}{70}{85.98601}		\pgfmath@def{acos}{71}{85.92857}
\pgfmath@def{acos}{72}{85.87113}		\pgfmath@def{acos}{73}{85.81368}
\pgfmath@def{acos}{74}{85.75623}		\pgfmath@def{acos}{75}{85.69877}
\pgfmath@def{acos}{76}{85.64131}		\pgfmath@def{acos}{77}{85.58385}
\pgfmath@def{acos}{78}{85.52638}		\pgfmath@def{acos}{79}{85.46891}
\pgfmath@def{acos}{80}{85.41143}		\pgfmath@def{acos}{81}{85.35395}
\pgfmath@def{acos}{82}{85.29646}		\pgfmath@def{acos}{83}{85.23897}
\pgfmath@def{acos}{84}{85.18147}		\pgfmath@def{acos}{85}{85.12397}
\pgfmath@def{acos}{86}{85.06646}		\pgfmath@def{acos}{87}{85.00895}
\pgfmath@def{acos}{88}{84.95144}		\pgfmath@def{acos}{89}{84.89392}
\pgfmath@def{acos}{90}{84.83639}		\pgfmath@def{acos}{91}{84.77886}
\pgfmath@def{acos}{92}{84.72132}		\pgfmath@def{acos}{93}{84.66378}
\pgfmath@def{acos}{94}{84.60623}		\pgfmath@def{acos}{95}{84.54868}
\pgfmath@def{acos}{96}{84.49112}		\pgfmath@def{acos}{97}{84.43355}
\pgfmath@def{acos}{98}{84.37598}		\pgfmath@def{acos}{99}{84.31841}
\pgfmath@def{acos}{100}{84.26083}		\pgfmath@def{acos}{101}{84.20324}
\pgfmath@def{acos}{102}{84.14564}		\pgfmath@def{acos}{103}{84.08805}
\pgfmath@def{acos}{104}{84.03044}		\pgfmath@def{acos}{105}{83.97283}
\pgfmath@def{acos}{106}{83.91521}		\pgfmath@def{acos}{107}{83.85759}
\pgfmath@def{acos}{108}{83.79996}		\pgfmath@def{acos}{109}{83.74232}
\pgfmath@def{acos}{110}{83.68468}		\pgfmath@def{acos}{111}{83.62703}
\pgfmath@def{acos}{112}{83.56938}		\pgfmath@def{acos}{113}{83.51171}
\pgfmath@def{acos}{114}{83.45405}		\pgfmath@def{acos}{115}{83.39637}
\pgfmath@def{acos}{116}{83.33869}		\pgfmath@def{acos}{117}{83.28100}
\pgfmath@def{acos}{118}{83.22330}		\pgfmath@def{acos}{119}{83.16560}
\pgfmath@def{acos}{120}{83.10789}		\pgfmath@def{acos}{121}{83.05018}
\pgfmath@def{acos}{122}{82.99245}		\pgfmath@def{acos}{123}{82.93472}
\pgfmath@def{acos}{124}{82.87698}		\pgfmath@def{acos}{125}{82.81924}
\pgfmath@def{acos}{126}{82.76149}		\pgfmath@def{acos}{127}{82.70373}
\pgfmath@def{acos}{128}{82.64596}		\pgfmath@def{acos}{129}{82.58819}
\pgfmath@def{acos}{130}{82.53040}		\pgfmath@def{acos}{131}{82.47261}
\pgfmath@def{acos}{132}{82.41482}		\pgfmath@def{acos}{133}{82.35701}
\pgfmath@def{acos}{134}{82.29920}		\pgfmath@def{acos}{135}{82.24138}
\pgfmath@def{acos}{136}{82.18355}		\pgfmath@def{acos}{137}{82.12571}
\pgfmath@def{acos}{138}{82.06786}		\pgfmath@def{acos}{139}{82.01001}
\pgfmath@def{acos}{140}{81.95215}		\pgfmath@def{acos}{141}{81.89428}
\pgfmath@def{acos}{142}{81.83640}		\pgfmath@def{acos}{143}{81.77851}
\pgfmath@def{acos}{144}{81.72062}		\pgfmath@def{acos}{145}{81.66272}
\pgfmath@def{acos}{146}{81.60480}		\pgfmath@def{acos}{147}{81.54688}
\pgfmath@def{acos}{148}{81.48895}		\pgfmath@def{acos}{149}{81.43102}
\pgfmath@def{acos}{150}{81.37307}		\pgfmath@def{acos}{151}{81.31511}
\pgfmath@def{acos}{152}{81.25715}		\pgfmath@def{acos}{153}{81.19917}
\pgfmath@def{acos}{154}{81.14119}		\pgfmath@def{acos}{155}{81.08320}
\pgfmath@def{acos}{156}{81.02520}		\pgfmath@def{acos}{157}{80.96719}
\pgfmath@def{acos}{158}{80.90917}		\pgfmath@def{acos}{159}{80.85114}
\pgfmath@def{acos}{160}{80.79310}		\pgfmath@def{acos}{161}{80.73505}
\pgfmath@def{acos}{162}{80.67699}		\pgfmath@def{acos}{163}{80.61893}
\pgfmath@def{acos}{164}{80.56085}		\pgfmath@def{acos}{165}{80.50276}
\pgfmath@def{acos}{166}{80.44466}		\pgfmath@def{acos}{167}{80.38656}
\pgfmath@def{acos}{168}{80.32844}		\pgfmath@def{acos}{169}{80.27031}
\pgfmath@def{acos}{170}{80.21218}		\pgfmath@def{acos}{171}{80.15403}
\pgfmath@def{acos}{172}{80.09587}		\pgfmath@def{acos}{173}{80.03770}
\pgfmath@def{acos}{174}{79.97953}		\pgfmath@def{acos}{175}{79.92134}
\pgfmath@def{acos}{176}{79.86314}		\pgfmath@def{acos}{177}{79.80493}
\pgfmath@def{acos}{178}{79.74671}		\pgfmath@def{acos}{179}{79.68848}
\pgfmath@def{acos}{180}{79.63024}		\pgfmath@def{acos}{181}{79.57198}
\pgfmath@def{acos}{182}{79.51372}		\pgfmath@def{acos}{183}{79.45545}
\pgfmath@def{acos}{184}{79.39716}		\pgfmath@def{acos}{185}{79.33886}
\pgfmath@def{acos}{186}{79.28056}		\pgfmath@def{acos}{187}{79.22224}
\pgfmath@def{acos}{188}{79.16391}		\pgfmath@def{acos}{189}{79.10556}
\pgfmath@def{acos}{190}{79.04721}		\pgfmath@def{acos}{191}{78.98885}
\pgfmath@def{acos}{192}{78.93047}		\pgfmath@def{acos}{193}{78.87208}
\pgfmath@def{acos}{194}{78.81368}		\pgfmath@def{acos}{195}{78.75527}
\pgfmath@def{acos}{196}{78.69685}		\pgfmath@def{acos}{197}{78.63841}
\pgfmath@def{acos}{198}{78.57997}		\pgfmath@def{acos}{199}{78.52151}
\pgfmath@def{acos}{200}{78.46304}		\pgfmath@def{acos}{201}{78.40455}
\pgfmath@def{acos}{202}{78.34606}		\pgfmath@def{acos}{203}{78.28755}
\pgfmath@def{acos}{204}{78.22903}		\pgfmath@def{acos}{205}{78.17050}
\pgfmath@def{acos}{206}{78.11195}		\pgfmath@def{acos}{207}{78.05339}
\pgfmath@def{acos}{208}{77.99482}		\pgfmath@def{acos}{209}{77.93624}
\pgfmath@def{acos}{210}{77.87764}		\pgfmath@def{acos}{211}{77.81903}
\pgfmath@def{acos}{212}{77.76041}		\pgfmath@def{acos}{213}{77.70178}
\pgfmath@def{acos}{214}{77.64313}		\pgfmath@def{acos}{215}{77.58447}
\pgfmath@def{acos}{216}{77.52579}		\pgfmath@def{acos}{217}{77.46711}
\pgfmath@def{acos}{218}{77.40841}		\pgfmath@def{acos}{219}{77.34969}
\pgfmath@def{acos}{220}{77.29096}		\pgfmath@def{acos}{221}{77.23222}
\pgfmath@def{acos}{222}{77.17347}		\pgfmath@def{acos}{223}{77.11470}
\pgfmath@def{acos}{224}{77.05591}		\pgfmath@def{acos}{225}{76.99712}
\pgfmath@def{acos}{226}{76.93831}		\pgfmath@def{acos}{227}{76.87948}
\pgfmath@def{acos}{228}{76.82064}		\pgfmath@def{acos}{229}{76.76179}
\pgfmath@def{acos}{230}{76.70292}		\pgfmath@def{acos}{231}{76.64404}
\pgfmath@def{acos}{232}{76.58515}		\pgfmath@def{acos}{233}{76.52624}
\pgfmath@def{acos}{234}{76.46731}		\pgfmath@def{acos}{235}{76.40837}
\pgfmath@def{acos}{236}{76.34942}		\pgfmath@def{acos}{237}{76.29045}
\pgfmath@def{acos}{238}{76.23147}		\pgfmath@def{acos}{239}{76.17247}
\pgfmath@def{acos}{240}{76.11346}		\pgfmath@def{acos}{241}{76.05443}
\pgfmath@def{acos}{242}{75.99538}		\pgfmath@def{acos}{243}{75.93632}
\pgfmath@def{acos}{244}{75.87725}		\pgfmath@def{acos}{245}{75.81816}
\pgfmath@def{acos}{246}{75.75906}		\pgfmath@def{acos}{247}{75.69994}
\pgfmath@def{acos}{248}{75.64080}		\pgfmath@def{acos}{249}{75.58165}
\pgfmath@def{acos}{250}{75.52248}		\pgfmath@def{acos}{251}{75.46330}
\pgfmath@def{acos}{252}{75.40410}		\pgfmath@def{acos}{253}{75.34489}
\pgfmath@def{acos}{254}{75.28566}		\pgfmath@def{acos}{255}{75.22641}
\pgfmath@def{acos}{256}{75.16715}		\pgfmath@def{acos}{257}{75.10787}
\pgfmath@def{acos}{258}{75.04857}		\pgfmath@def{acos}{259}{74.98926}
\pgfmath@def{acos}{260}{74.92993}		\pgfmath@def{acos}{261}{74.87059}
\pgfmath@def{acos}{262}{74.81123}		\pgfmath@def{acos}{263}{74.75185}
\pgfmath@def{acos}{264}{74.69245}		\pgfmath@def{acos}{265}{74.63304}
\pgfmath@def{acos}{266}{74.57361}		\pgfmath@def{acos}{267}{74.51417}
\pgfmath@def{acos}{268}{74.45471}		\pgfmath@def{acos}{269}{74.39523}
\pgfmath@def{acos}{270}{74.33573}		\pgfmath@def{acos}{271}{74.27621}
\pgfmath@def{acos}{272}{74.21668}		\pgfmath@def{acos}{273}{74.15713}
\pgfmath@def{acos}{274}{74.09757}		\pgfmath@def{acos}{275}{74.03798}
\pgfmath@def{acos}{276}{73.97838}		\pgfmath@def{acos}{277}{73.91876}
\pgfmath@def{acos}{278}{73.85912}		\pgfmath@def{acos}{279}{73.79946}
\pgfmath@def{acos}{280}{73.73979}		\pgfmath@def{acos}{281}{73.68010}
\pgfmath@def{acos}{282}{73.62039}		\pgfmath@def{acos}{283}{73.56066}
\pgfmath@def{acos}{284}{73.50091}		\pgfmath@def{acos}{285}{73.44115}
\pgfmath@def{acos}{286}{73.38136}		\pgfmath@def{acos}{287}{73.32156}
\pgfmath@def{acos}{288}{73.26174}		\pgfmath@def{acos}{289}{73.20190}
\pgfmath@def{acos}{290}{73.14204}		\pgfmath@def{acos}{291}{73.08216}
\pgfmath@def{acos}{292}{73.02226}		\pgfmath@def{acos}{293}{72.96235}
\pgfmath@def{acos}{294}{72.90241}		\pgfmath@def{acos}{295}{72.84246}
\pgfmath@def{acos}{296}{72.78248}		\pgfmath@def{acos}{297}{72.72249}
\pgfmath@def{acos}{298}{72.66248}		\pgfmath@def{acos}{299}{72.60244}
\pgfmath@def{acos}{300}{72.54239}		\pgfmath@def{acos}{301}{72.48232}
\pgfmath@def{acos}{302}{72.42223}		\pgfmath@def{acos}{303}{72.36212}
\pgfmath@def{acos}{304}{72.30198}		\pgfmath@def{acos}{305}{72.24183}
\pgfmath@def{acos}{306}{72.18166}		\pgfmath@def{acos}{307}{72.12147}
\pgfmath@def{acos}{308}{72.06125}		\pgfmath@def{acos}{309}{72.00102}
\pgfmath@def{acos}{310}{71.94077}		\pgfmath@def{acos}{311}{71.88049}
\pgfmath@def{acos}{312}{71.82019}		\pgfmath@def{acos}{313}{71.75988}
\pgfmath@def{acos}{314}{71.69954}		\pgfmath@def{acos}{315}{71.63918}
\pgfmath@def{acos}{316}{71.57880}		\pgfmath@def{acos}{317}{71.51840}
\pgfmath@def{acos}{318}{71.45798}		\pgfmath@def{acos}{319}{71.39754}
\pgfmath@def{acos}{320}{71.33707}		\pgfmath@def{acos}{321}{71.27658}
\pgfmath@def{acos}{322}{71.21608}		\pgfmath@def{acos}{323}{71.15555}
\pgfmath@def{acos}{324}{71.09499}		\pgfmath@def{acos}{325}{71.03442}
\pgfmath@def{acos}{326}{70.97382}		\pgfmath@def{acos}{327}{70.91321}
\pgfmath@def{acos}{328}{70.85257}		\pgfmath@def{acos}{329}{70.79190}
\pgfmath@def{acos}{330}{70.73122}		\pgfmath@def{acos}{331}{70.67051}
\pgfmath@def{acos}{332}{70.60978}		\pgfmath@def{acos}{333}{70.54903}
\pgfmath@def{acos}{334}{70.48826}		\pgfmath@def{acos}{335}{70.42746}
\pgfmath@def{acos}{336}{70.36664}		\pgfmath@def{acos}{337}{70.30579}
\pgfmath@def{acos}{338}{70.24493}		\pgfmath@def{acos}{339}{70.18404}
\pgfmath@def{acos}{340}{70.12312}		\pgfmath@def{acos}{341}{70.06218}
\pgfmath@def{acos}{342}{70.00122}		\pgfmath@def{acos}{343}{69.94024}
\pgfmath@def{acos}{344}{69.87923}		\pgfmath@def{acos}{345}{69.81820}
\pgfmath@def{acos}{346}{69.75714}		\pgfmath@def{acos}{347}{69.69606}
\pgfmath@def{acos}{348}{69.63496}		\pgfmath@def{acos}{349}{69.57383}
\pgfmath@def{acos}{350}{69.51268}		\pgfmath@def{acos}{351}{69.45150}
\pgfmath@def{acos}{352}{69.39030}		\pgfmath@def{acos}{353}{69.32908}
\pgfmath@def{acos}{354}{69.26783}		\pgfmath@def{acos}{355}{69.20655}
\pgfmath@def{acos}{356}{69.14525}		\pgfmath@def{acos}{357}{69.08393}
\pgfmath@def{acos}{358}{69.02258}		\pgfmath@def{acos}{359}{68.96120}
\pgfmath@def{acos}{360}{68.89980}		\pgfmath@def{acos}{361}{68.83837}
\pgfmath@def{acos}{362}{68.77692}		\pgfmath@def{acos}{363}{68.71544}
\pgfmath@def{acos}{364}{68.65394}		\pgfmath@def{acos}{365}{68.59241}
\pgfmath@def{acos}{366}{68.53086}		\pgfmath@def{acos}{367}{68.46928}
\pgfmath@def{acos}{368}{68.40767}		\pgfmath@def{acos}{369}{68.34604}
\pgfmath@def{acos}{370}{68.28438}		\pgfmath@def{acos}{371}{68.22269}
\pgfmath@def{acos}{372}{68.16098}		\pgfmath@def{acos}{373}{68.09924}
\pgfmath@def{acos}{374}{68.03748}		\pgfmath@def{acos}{375}{67.97568}
\pgfmath@def{acos}{376}{67.91386}		\pgfmath@def{acos}{377}{67.85202}
\pgfmath@def{acos}{378}{67.79014}		\pgfmath@def{acos}{379}{67.72824}
\pgfmath@def{acos}{380}{67.66631}		\pgfmath@def{acos}{381}{67.60436}
\pgfmath@def{acos}{382}{67.54237}		\pgfmath@def{acos}{383}{67.48036}
\pgfmath@def{acos}{384}{67.41832}		\pgfmath@def{acos}{385}{67.35626}
\pgfmath@def{acos}{386}{67.29416}		\pgfmath@def{acos}{387}{67.23204}
\pgfmath@def{acos}{388}{67.16988}		\pgfmath@def{acos}{389}{67.10770}
\pgfmath@def{acos}{390}{67.04550}		\pgfmath@def{acos}{391}{66.98326}
\pgfmath@def{acos}{392}{66.92099}		\pgfmath@def{acos}{393}{66.85870}
\pgfmath@def{acos}{394}{66.79637}		\pgfmath@def{acos}{395}{66.73402}
\pgfmath@def{acos}{396}{66.67164}		\pgfmath@def{acos}{397}{66.60923}
\pgfmath@def{acos}{398}{66.54679}		\pgfmath@def{acos}{399}{66.48432}
\pgfmath@def{acos}{400}{66.42182}		\pgfmath@def{acos}{401}{66.35929}
\pgfmath@def{acos}{402}{66.29673}		\pgfmath@def{acos}{403}{66.23414}
\pgfmath@def{acos}{404}{66.17152}		\pgfmath@def{acos}{405}{66.10887}
\pgfmath@def{acos}{406}{66.04619}		\pgfmath@def{acos}{407}{65.98348}
\pgfmath@def{acos}{408}{65.92074}		\pgfmath@def{acos}{409}{65.85796}
\pgfmath@def{acos}{410}{65.79516}		\pgfmath@def{acos}{411}{65.73233}
\pgfmath@def{acos}{412}{65.66946}		\pgfmath@def{acos}{413}{65.60657}
\pgfmath@def{acos}{414}{65.54364}		\pgfmath@def{acos}{415}{65.48068}
\pgfmath@def{acos}{416}{65.41769}		\pgfmath@def{acos}{417}{65.35467}
\pgfmath@def{acos}{418}{65.29161}		\pgfmath@def{acos}{419}{65.22853}
\pgfmath@def{acos}{420}{65.16541}		\pgfmath@def{acos}{421}{65.10226}
\pgfmath@def{acos}{422}{65.03908}		\pgfmath@def{acos}{423}{64.97586}
\pgfmath@def{acos}{424}{64.91261}		\pgfmath@def{acos}{425}{64.84933}
\pgfmath@def{acos}{426}{64.78602}		\pgfmath@def{acos}{427}{64.72267}
\pgfmath@def{acos}{428}{64.65929}		\pgfmath@def{acos}{429}{64.59588}
\pgfmath@def{acos}{430}{64.53244}		\pgfmath@def{acos}{431}{64.46896}
\pgfmath@def{acos}{432}{64.40544}		\pgfmath@def{acos}{433}{64.34190}
\pgfmath@def{acos}{434}{64.27832}		\pgfmath@def{acos}{435}{64.21470}
\pgfmath@def{acos}{436}{64.15105}		\pgfmath@def{acos}{437}{64.08737}
\pgfmath@def{acos}{438}{64.02365}		\pgfmath@def{acos}{439}{63.95990}
\pgfmath@def{acos}{440}{63.89611}		\pgfmath@def{acos}{441}{63.83229}
\pgfmath@def{acos}{442}{63.76844}		\pgfmath@def{acos}{443}{63.70455}
\pgfmath@def{acos}{444}{63.64062}		\pgfmath@def{acos}{445}{63.57666}
\pgfmath@def{acos}{446}{63.51266}		\pgfmath@def{acos}{447}{63.44863}
\pgfmath@def{acos}{448}{63.38456}		\pgfmath@def{acos}{449}{63.32045}
\pgfmath@def{acos}{450}{63.25631}		\pgfmath@def{acos}{451}{63.19213}
\pgfmath@def{acos}{452}{63.12792}		\pgfmath@def{acos}{453}{63.06367}
\pgfmath@def{acos}{454}{62.99938}		\pgfmath@def{acos}{455}{62.93506}
\pgfmath@def{acos}{456}{62.87070}		\pgfmath@def{acos}{457}{62.80630}
\pgfmath@def{acos}{458}{62.74187}		\pgfmath@def{acos}{459}{62.67740}
\pgfmath@def{acos}{460}{62.61289}		\pgfmath@def{acos}{461}{62.54834}
\pgfmath@def{acos}{462}{62.48376}		\pgfmath@def{acos}{463}{62.41913}
\pgfmath@def{acos}{464}{62.35447}		\pgfmath@def{acos}{465}{62.28977}
\pgfmath@def{acos}{466}{62.22504}		\pgfmath@def{acos}{467}{62.16026}
\pgfmath@def{acos}{468}{62.09545}		\pgfmath@def{acos}{469}{62.03059}
\pgfmath@def{acos}{470}{61.96570}		\pgfmath@def{acos}{471}{61.90077}
\pgfmath@def{acos}{472}{61.83580}		\pgfmath@def{acos}{473}{61.77079}
\pgfmath@def{acos}{474}{61.70574}		\pgfmath@def{acos}{475}{61.64065}
\pgfmath@def{acos}{476}{61.57552}		\pgfmath@def{acos}{477}{61.51035}
\pgfmath@def{acos}{478}{61.44514}		\pgfmath@def{acos}{479}{61.37988}
\pgfmath@def{acos}{480}{61.31459}		\pgfmath@def{acos}{481}{61.24926}
\pgfmath@def{acos}{482}{61.18389}		\pgfmath@def{acos}{483}{61.11847}
\pgfmath@def{acos}{484}{61.05302}		\pgfmath@def{acos}{485}{60.98752}
\pgfmath@def{acos}{486}{60.92199}		\pgfmath@def{acos}{487}{60.85641}
\pgfmath@def{acos}{488}{60.79078}		\pgfmath@def{acos}{489}{60.72512}
\pgfmath@def{acos}{490}{60.65941}		\pgfmath@def{acos}{491}{60.59367}
\pgfmath@def{acos}{492}{60.52787}		\pgfmath@def{acos}{493}{60.46204}
\pgfmath@def{acos}{494}{60.39616}		\pgfmath@def{acos}{495}{60.33025}
\pgfmath@def{acos}{496}{60.26428}		\pgfmath@def{acos}{497}{60.19828}
\pgfmath@def{acos}{498}{60.13223}		\pgfmath@def{acos}{499}{60.06613}
\pgfmath@def{acos}{500}{60.00000}		\pgfmath@def{acos}{501}{59.93381}
\pgfmath@def{acos}{502}{59.86759}		\pgfmath@def{acos}{503}{59.80132}
\pgfmath@def{acos}{504}{59.73500}		\pgfmath@def{acos}{505}{59.66864}
\pgfmath@def{acos}{506}{59.60224}		\pgfmath@def{acos}{507}{59.53579}
\pgfmath@def{acos}{508}{59.46929}		\pgfmath@def{acos}{509}{59.40275}
\pgfmath@def{acos}{510}{59.33617}		\pgfmath@def{acos}{511}{59.26953}
\pgfmath@def{acos}{512}{59.20285}		\pgfmath@def{acos}{513}{59.13613}
\pgfmath@def{acos}{514}{59.06936}		\pgfmath@def{acos}{515}{59.00254}
\pgfmath@def{acos}{516}{58.93568}		\pgfmath@def{acos}{517}{58.86876}
\pgfmath@def{acos}{518}{58.80180}		\pgfmath@def{acos}{519}{58.73480}
\pgfmath@def{acos}{520}{58.66774}		\pgfmath@def{acos}{521}{58.60064}
\pgfmath@def{acos}{522}{58.53349}		\pgfmath@def{acos}{523}{58.46629}
\pgfmath@def{acos}{524}{58.39905}		\pgfmath@def{acos}{525}{58.33175}
\pgfmath@def{acos}{526}{58.26441}		\pgfmath@def{acos}{527}{58.19702}
\pgfmath@def{acos}{528}{58.12957}		\pgfmath@def{acos}{529}{58.06208}
\pgfmath@def{acos}{530}{57.99454}		\pgfmath@def{acos}{531}{57.92695}
\pgfmath@def{acos}{532}{57.85931}		\pgfmath@def{acos}{533}{57.79162}
\pgfmath@def{acos}{534}{57.72388}		\pgfmath@def{acos}{535}{57.65608}
\pgfmath@def{acos}{536}{57.58824}		\pgfmath@def{acos}{537}{57.52035}
\pgfmath@def{acos}{538}{57.45240}		\pgfmath@def{acos}{539}{57.38441}
\pgfmath@def{acos}{540}{57.31636}		\pgfmath@def{acos}{541}{57.24826}
\pgfmath@def{acos}{542}{57.18010}		\pgfmath@def{acos}{543}{57.11190}
\pgfmath@def{acos}{544}{57.04364}		\pgfmath@def{acos}{545}{56.97533}
\pgfmath@def{acos}{546}{56.90697}		\pgfmath@def{acos}{547}{56.83855}
\pgfmath@def{acos}{548}{56.77008}		\pgfmath@def{acos}{549}{56.70156}
\pgfmath@def{acos}{550}{56.63298}		\pgfmath@def{acos}{551}{56.56435}
\pgfmath@def{acos}{552}{56.49567}		\pgfmath@def{acos}{553}{56.42693}
\pgfmath@def{acos}{554}{56.35813}		\pgfmath@def{acos}{555}{56.28928}
\pgfmath@def{acos}{556}{56.22038}		\pgfmath@def{acos}{557}{56.15141}
\pgfmath@def{acos}{558}{56.08240}		\pgfmath@def{acos}{559}{56.01333}
\pgfmath@def{acos}{560}{55.94420}		\pgfmath@def{acos}{561}{55.87501}
\pgfmath@def{acos}{562}{55.80577}		\pgfmath@def{acos}{563}{55.73647}
\pgfmath@def{acos}{564}{55.66712}		\pgfmath@def{acos}{565}{55.59770}
\pgfmath@def{acos}{566}{55.52823}		\pgfmath@def{acos}{567}{55.45871}
\pgfmath@def{acos}{568}{55.38912}		\pgfmath@def{acos}{569}{55.31947}
\pgfmath@def{acos}{570}{55.24977}		\pgfmath@def{acos}{571}{55.18001}
\pgfmath@def{acos}{572}{55.11019}		\pgfmath@def{acos}{573}{55.04030}
\pgfmath@def{acos}{574}{54.97036}		\pgfmath@def{acos}{575}{54.90036}
\pgfmath@def{acos}{576}{54.83030}		\pgfmath@def{acos}{577}{54.76018}
\pgfmath@def{acos}{578}{54.69000}		\pgfmath@def{acos}{579}{54.61976}
\pgfmath@def{acos}{580}{54.54945}		\pgfmath@def{acos}{581}{54.47909}
\pgfmath@def{acos}{582}{54.40866}		\pgfmath@def{acos}{583}{54.33817}
\pgfmath@def{acos}{584}{54.26762}		\pgfmath@def{acos}{585}{54.19701}
\pgfmath@def{acos}{586}{54.12633}		\pgfmath@def{acos}{587}{54.05559}
\pgfmath@def{acos}{588}{53.98479}		\pgfmath@def{acos}{589}{53.91392}
\pgfmath@def{acos}{590}{53.84299}		\pgfmath@def{acos}{591}{53.77199}
\pgfmath@def{acos}{592}{53.70093}		\pgfmath@def{acos}{593}{53.62981}
\pgfmath@def{acos}{594}{53.55862}		\pgfmath@def{acos}{595}{53.48736}
\pgfmath@def{acos}{596}{53.41604}		\pgfmath@def{acos}{597}{53.34466}
\pgfmath@def{acos}{598}{53.27320}		\pgfmath@def{acos}{599}{53.20168}
\pgfmath@def{acos}{600}{53.13010}		\pgfmath@def{acos}{601}{53.05844}
\pgfmath@def{acos}{602}{52.98672}		\pgfmath@def{acos}{603}{52.91494}
\pgfmath@def{acos}{604}{52.84308}		\pgfmath@def{acos}{605}{52.77115}
\pgfmath@def{acos}{606}{52.69916}		\pgfmath@def{acos}{607}{52.62710}
\pgfmath@def{acos}{608}{52.55497}		\pgfmath@def{acos}{609}{52.48276}
\pgfmath@def{acos}{610}{52.41049}		\pgfmath@def{acos}{611}{52.33815}
\pgfmath@def{acos}{612}{52.26574}		\pgfmath@def{acos}{613}{52.19326}
\pgfmath@def{acos}{614}{52.12070}		\pgfmath@def{acos}{615}{52.04808}
\pgfmath@def{acos}{616}{51.97538}		\pgfmath@def{acos}{617}{51.90261}
\pgfmath@def{acos}{618}{51.82976}		\pgfmath@def{acos}{619}{51.75685}
\pgfmath@def{acos}{620}{51.68386}		\pgfmath@def{acos}{621}{51.61080}
\pgfmath@def{acos}{622}{51.53766}		\pgfmath@def{acos}{623}{51.46445}
\pgfmath@def{acos}{624}{51.39117}		\pgfmath@def{acos}{625}{51.31781}
\pgfmath@def{acos}{626}{51.24437}		\pgfmath@def{acos}{627}{51.17086}
\pgfmath@def{acos}{628}{51.09728}		\pgfmath@def{acos}{629}{51.02361}
\pgfmath@def{acos}{630}{50.94987}		\pgfmath@def{acos}{631}{50.87606}
\pgfmath@def{acos}{632}{50.80216}		\pgfmath@def{acos}{633}{50.72819}
\pgfmath@def{acos}{634}{50.65414}		\pgfmath@def{acos}{635}{50.58001}
\pgfmath@def{acos}{636}{50.50580}		\pgfmath@def{acos}{637}{50.43152}
\pgfmath@def{acos}{638}{50.35715}		\pgfmath@def{acos}{639}{50.28270}
\pgfmath@def{acos}{640}{50.20818}		\pgfmath@def{acos}{641}{50.13357}
\pgfmath@def{acos}{642}{50.05888}		\pgfmath@def{acos}{643}{49.98411}
\pgfmath@def{acos}{644}{49.90926}		\pgfmath@def{acos}{645}{49.83432}
\pgfmath@def{acos}{646}{49.75930}		\pgfmath@def{acos}{647}{49.68420}
\pgfmath@def{acos}{648}{49.60902}		\pgfmath@def{acos}{649}{49.53375}
\pgfmath@def{acos}{650}{49.45839}		\pgfmath@def{acos}{651}{49.38296}
\pgfmath@def{acos}{652}{49.30743}		\pgfmath@def{acos}{653}{49.23182}
\pgfmath@def{acos}{654}{49.15613}		\pgfmath@def{acos}{655}{49.08035}
\pgfmath@def{acos}{656}{49.00448}		\pgfmath@def{acos}{657}{48.92852}
\pgfmath@def{acos}{658}{48.85248}		\pgfmath@def{acos}{659}{48.77634}
\pgfmath@def{acos}{660}{48.70012}		\pgfmath@def{acos}{661}{48.62381}
\pgfmath@def{acos}{662}{48.54741}		\pgfmath@def{acos}{663}{48.47092}
\pgfmath@def{acos}{664}{48.39434}		\pgfmath@def{acos}{665}{48.31767}
\pgfmath@def{acos}{666}{48.24091}		\pgfmath@def{acos}{667}{48.16405}
\pgfmath@def{acos}{668}{48.08710}		\pgfmath@def{acos}{669}{48.01006}
\pgfmath@def{acos}{670}{47.93293}		\pgfmath@def{acos}{671}{47.85570}
\pgfmath@def{acos}{672}{47.77838}		\pgfmath@def{acos}{673}{47.70096}
\pgfmath@def{acos}{674}{47.62345}		\pgfmath@def{acos}{675}{47.54585}
\pgfmath@def{acos}{676}{47.46814}		\pgfmath@def{acos}{677}{47.39034}
\pgfmath@def{acos}{678}{47.31244}		\pgfmath@def{acos}{679}{47.23445}
\pgfmath@def{acos}{680}{47.15635}		\pgfmath@def{acos}{681}{47.07816}
\pgfmath@def{acos}{682}{46.99987}		\pgfmath@def{acos}{683}{46.92147}
\pgfmath@def{acos}{684}{46.84298}		\pgfmath@def{acos}{685}{46.76439}
\pgfmath@def{acos}{686}{46.68569}		\pgfmath@def{acos}{687}{46.60690}
\pgfmath@def{acos}{688}{46.52800}		\pgfmath@def{acos}{689}{46.44899}
\pgfmath@def{acos}{690}{46.36989}		\pgfmath@def{acos}{691}{46.29068}
\pgfmath@def{acos}{692}{46.21136}		\pgfmath@def{acos}{693}{46.13194}
\pgfmath@def{acos}{694}{46.05241}		\pgfmath@def{acos}{695}{45.97278}
\pgfmath@def{acos}{696}{45.89304}		\pgfmath@def{acos}{697}{45.81319}
\pgfmath@def{acos}{698}{45.73323}		\pgfmath@def{acos}{699}{45.65317}
\pgfmath@def{acos}{700}{45.57299}		\pgfmath@def{acos}{701}{45.49271}
\pgfmath@def{acos}{702}{45.41231}		\pgfmath@def{acos}{703}{45.33180}
\pgfmath@def{acos}{704}{45.25118}		\pgfmath@def{acos}{705}{45.17045}
\pgfmath@def{acos}{706}{45.08961}		\pgfmath@def{acos}{707}{45.00865}
\pgfmath@def{acos}{708}{44.92757}		\pgfmath@def{acos}{709}{44.84638}
\pgfmath@def{acos}{710}{44.76508}		\pgfmath@def{acos}{711}{44.68366}
\pgfmath@def{acos}{712}{44.60212}		\pgfmath@def{acos}{713}{44.52046}
\pgfmath@def{acos}{714}{44.43869}		\pgfmath@def{acos}{715}{44.35680}
\pgfmath@def{acos}{716}{44.27478}		\pgfmath@def{acos}{717}{44.19265}
\pgfmath@def{acos}{718}{44.11039}		\pgfmath@def{acos}{719}{44.02802}
\pgfmath@def{acos}{720}{43.94552}		\pgfmath@def{acos}{721}{43.86289}
\pgfmath@def{acos}{722}{43.78014}		\pgfmath@def{acos}{723}{43.69727}
\pgfmath@def{acos}{724}{43.61427}		\pgfmath@def{acos}{725}{43.53115}
\pgfmath@def{acos}{726}{43.44790}		\pgfmath@def{acos}{727}{43.36452}
\pgfmath@def{acos}{728}{43.28101}		\pgfmath@def{acos}{729}{43.19737}
\pgfmath@def{acos}{730}{43.11360}		\pgfmath@def{acos}{731}{43.02970}
\pgfmath@def{acos}{732}{42.94567}		\pgfmath@def{acos}{733}{42.86151}
\pgfmath@def{acos}{734}{42.77721}		\pgfmath@def{acos}{735}{42.69278}
\pgfmath@def{acos}{736}{42.60821}		\pgfmath@def{acos}{737}{42.52351}
\pgfmath@def{acos}{738}{42.43867}		\pgfmath@def{acos}{739}{42.35370}
\pgfmath@def{acos}{740}{42.26858}		\pgfmath@def{acos}{741}{42.18333}
\pgfmath@def{acos}{742}{42.09793}		\pgfmath@def{acos}{743}{42.01240}
\pgfmath@def{acos}{744}{41.92672}		\pgfmath@def{acos}{745}{41.84090}
\pgfmath@def{acos}{746}{41.75493}		\pgfmath@def{acos}{747}{41.66882}
\pgfmath@def{acos}{748}{41.58257}		\pgfmath@def{acos}{749}{41.49617}
\pgfmath@def{acos}{750}{41.40962}		\pgfmath@def{acos}{751}{41.32292}
\pgfmath@def{acos}{752}{41.23607}		\pgfmath@def{acos}{753}{41.14908}
\pgfmath@def{acos}{754}{41.06193}		\pgfmath@def{acos}{755}{40.97463}
\pgfmath@def{acos}{756}{40.88717}		\pgfmath@def{acos}{757}{40.79956}
\pgfmath@def{acos}{758}{40.71180}		\pgfmath@def{acos}{759}{40.62388}
\pgfmath@def{acos}{760}{40.53580}		\pgfmath@def{acos}{761}{40.44756}
\pgfmath@def{acos}{762}{40.35916}		\pgfmath@def{acos}{763}{40.27061}
\pgfmath@def{acos}{764}{40.18189}		\pgfmath@def{acos}{765}{40.09300}
\pgfmath@def{acos}{766}{40.00396}		\pgfmath@def{acos}{767}{39.91474}
\pgfmath@def{acos}{768}{39.82537}		\pgfmath@def{acos}{769}{39.73582}
\pgfmath@def{acos}{770}{39.64611}		\pgfmath@def{acos}{771}{39.55622}
\pgfmath@def{acos}{772}{39.46617}		\pgfmath@def{acos}{773}{39.37594}
\pgfmath@def{acos}{774}{39.28554}		\pgfmath@def{acos}{775}{39.19496}
\pgfmath@def{acos}{776}{39.10421}		\pgfmath@def{acos}{777}{39.01328}
\pgfmath@def{acos}{778}{38.92218}		\pgfmath@def{acos}{779}{38.83089}
\pgfmath@def{acos}{780}{38.73942}		\pgfmath@def{acos}{781}{38.64777}
\pgfmath@def{acos}{782}{38.55594}		\pgfmath@def{acos}{783}{38.46392}
\pgfmath@def{acos}{784}{38.37171}		\pgfmath@def{acos}{785}{38.27932}
\pgfmath@def{acos}{786}{38.18673}		\pgfmath@def{acos}{787}{38.09396}
\pgfmath@def{acos}{788}{38.00100}		\pgfmath@def{acos}{789}{37.90784}
\pgfmath@def{acos}{790}{37.81448}		\pgfmath@def{acos}{791}{37.72093}
\pgfmath@def{acos}{792}{37.62719}		\pgfmath@def{acos}{793}{37.53324}
\pgfmath@def{acos}{794}{37.43909}		\pgfmath@def{acos}{795}{37.34474}
\pgfmath@def{acos}{796}{37.25019}		\pgfmath@def{acos}{797}{37.15542}
\pgfmath@def{acos}{798}{37.06046}		\pgfmath@def{acos}{799}{36.96528}
\pgfmath@def{acos}{800}{36.86989}		\pgfmath@def{acos}{801}{36.77429}
\pgfmath@def{acos}{802}{36.67848}		\pgfmath@def{acos}{803}{36.58245}
\pgfmath@def{acos}{804}{36.48621}		\pgfmath@def{acos}{805}{36.38974}
\pgfmath@def{acos}{806}{36.29305}		\pgfmath@def{acos}{807}{36.19615}
\pgfmath@def{acos}{808}{36.09901}		\pgfmath@def{acos}{809}{36.00165}
\pgfmath@def{acos}{810}{35.90406}		\pgfmath@def{acos}{811}{35.80625}
\pgfmath@def{acos}{812}{35.70820}		\pgfmath@def{acos}{813}{35.60991}
\pgfmath@def{acos}{814}{35.51139}		\pgfmath@def{acos}{815}{35.41263}
\pgfmath@def{acos}{816}{35.31364}		\pgfmath@def{acos}{817}{35.21440}
\pgfmath@def{acos}{818}{35.11491}		\pgfmath@def{acos}{819}{35.01518}
\pgfmath@def{acos}{820}{34.91520}		\pgfmath@def{acos}{821}{34.81497}
\pgfmath@def{acos}{822}{34.71449}		\pgfmath@def{acos}{823}{34.61375}
\pgfmath@def{acos}{824}{34.51276}		\pgfmath@def{acos}{825}{34.41150}
\pgfmath@def{acos}{826}{34.30999}		\pgfmath@def{acos}{827}{34.20821}
\pgfmath@def{acos}{828}{34.10616}		\pgfmath@def{acos}{829}{34.00385}
\pgfmath@def{acos}{830}{33.90126}		\pgfmath@def{acos}{831}{33.79840}
\pgfmath@def{acos}{832}{33.69526}		\pgfmath@def{acos}{833}{33.59184}
\pgfmath@def{acos}{834}{33.48814}		\pgfmath@def{acos}{835}{33.38416}
\pgfmath@def{acos}{836}{33.27989}		\pgfmath@def{acos}{837}{33.17533}
\pgfmath@def{acos}{838}{33.07047}		\pgfmath@def{acos}{839}{32.96532}
\pgfmath@def{acos}{840}{32.85988}		\pgfmath@def{acos}{841}{32.75413}
\pgfmath@def{acos}{842}{32.64807}		\pgfmath@def{acos}{843}{32.54171}
\pgfmath@def{acos}{844}{32.43504}		\pgfmath@def{acos}{845}{32.32806}
\pgfmath@def{acos}{846}{32.22076}		\pgfmath@def{acos}{847}{32.11314}
\pgfmath@def{acos}{848}{32.00520}		\pgfmath@def{acos}{849}{31.89693}
\pgfmath@def{acos}{850}{31.78833}		\pgfmath@def{acos}{851}{31.67939}
\pgfmath@def{acos}{852}{31.57012}		\pgfmath@def{acos}{853}{31.46051}
\pgfmath@def{acos}{854}{31.35056}		\pgfmath@def{acos}{855}{31.24026}
\pgfmath@def{acos}{856}{31.12961}		\pgfmath@def{acos}{857}{31.01860}
\pgfmath@def{acos}{858}{30.90724}		\pgfmath@def{acos}{859}{30.79551}
\pgfmath@def{acos}{860}{30.68341}		\pgfmath@def{acos}{861}{30.57095}
\pgfmath@def{acos}{862}{30.45811}		\pgfmath@def{acos}{863}{30.34489}
\pgfmath@def{acos}{864}{30.23128}		\pgfmath@def{acos}{865}{30.11729}
\pgfmath@def{acos}{866}{30.00291}		\pgfmath@def{acos}{867}{29.88813}
\pgfmath@def{acos}{868}{29.77294}		\pgfmath@def{acos}{869}{29.65736}
\pgfmath@def{acos}{870}{29.54136}		\pgfmath@def{acos}{871}{29.42494}
\pgfmath@def{acos}{872}{29.30810}		\pgfmath@def{acos}{873}{29.19084}
\pgfmath@def{acos}{874}{29.07315}		\pgfmath@def{acos}{875}{28.95502}
\pgfmath@def{acos}{876}{28.83645}		\pgfmath@def{acos}{877}{28.71743}
\pgfmath@def{acos}{878}{28.59796}		\pgfmath@def{acos}{879}{28.47803}
\pgfmath@def{acos}{880}{28.35763}		\pgfmath@def{acos}{881}{28.23677}
\pgfmath@def{acos}{882}{28.11542}		\pgfmath@def{acos}{883}{27.99360}
\pgfmath@def{acos}{884}{27.87128}		\pgfmath@def{acos}{885}{27.74847}
\pgfmath@def{acos}{886}{27.62516}		\pgfmath@def{acos}{887}{27.50134}
\pgfmath@def{acos}{888}{27.37700}		\pgfmath@def{acos}{889}{27.25214}
\pgfmath@def{acos}{890}{27.12675}		\pgfmath@def{acos}{891}{27.00082}
\pgfmath@def{acos}{892}{26.87434}		\pgfmath@def{acos}{893}{26.74731}
\pgfmath@def{acos}{894}{26.61973}		\pgfmath@def{acos}{895}{26.49157}
\pgfmath@def{acos}{896}{26.36283}		\pgfmath@def{acos}{897}{26.23351}
\pgfmath@def{acos}{898}{26.10359}		\pgfmath@def{acos}{899}{25.97306}
\pgfmath@def{acos}{900}{25.84193}		\pgfmath@def{acos}{901}{25.71017}
\pgfmath@def{acos}{902}{25.57778}		\pgfmath@def{acos}{903}{25.44475}
\pgfmath@def{acos}{904}{25.31106}		\pgfmath@def{acos}{905}{25.17671}
\pgfmath@def{acos}{906}{25.04169}		\pgfmath@def{acos}{907}{24.90598}
\pgfmath@def{acos}{908}{24.76958}		\pgfmath@def{acos}{909}{24.63247}
\pgfmath@def{acos}{910}{24.49464}		\pgfmath@def{acos}{911}{24.35608}
\pgfmath@def{acos}{912}{24.21678}		\pgfmath@def{acos}{913}{24.07672}
\pgfmath@def{acos}{914}{23.93588}		\pgfmath@def{acos}{915}{23.79427}
\pgfmath@def{acos}{916}{23.65185}		\pgfmath@def{acos}{917}{23.50863}
\pgfmath@def{acos}{918}{23.36457}		\pgfmath@def{acos}{919}{23.21967}
\pgfmath@def{acos}{920}{23.07391}		\pgfmath@def{acos}{921}{22.92728}
\pgfmath@def{acos}{922}{22.77975}		\pgfmath@def{acos}{923}{22.63132}
\pgfmath@def{acos}{924}{22.48195}		\pgfmath@def{acos}{925}{22.33164}
\pgfmath@def{acos}{926}{22.18036}		\pgfmath@def{acos}{927}{22.02810}
\pgfmath@def{acos}{928}{21.87483}		\pgfmath@def{acos}{929}{21.72053}
\pgfmath@def{acos}{930}{21.56518}		\pgfmath@def{acos}{931}{21.40876}
\pgfmath@def{acos}{932}{21.25124}		\pgfmath@def{acos}{933}{21.09260}
\pgfmath@def{acos}{934}{20.93281}		\pgfmath@def{acos}{935}{20.77185}
\pgfmath@def{acos}{936}{20.60969}		\pgfmath@def{acos}{937}{20.44630}
\pgfmath@def{acos}{938}{20.28165}		\pgfmath@def{acos}{939}{20.11570}
\pgfmath@def{acos}{940}{19.94844}		\pgfmath@def{acos}{941}{19.77982}
\pgfmath@def{acos}{942}{19.60981}		\pgfmath@def{acos}{943}{19.43837}
\pgfmath@def{acos}{944}{19.26546}		\pgfmath@def{acos}{945}{19.09105}
\pgfmath@def{acos}{946}{18.91509}		\pgfmath@def{acos}{947}{18.73754}
\pgfmath@def{acos}{948}{18.55835}		\pgfmath@def{acos}{949}{18.37748}
\pgfmath@def{acos}{950}{18.19487}		\pgfmath@def{acos}{951}{18.01047}
\pgfmath@def{acos}{952}{17.82423}		\pgfmath@def{acos}{953}{17.63609}
\pgfmath@def{acos}{954}{17.44598}		\pgfmath@def{acos}{955}{17.25385}
\pgfmath@def{acos}{956}{17.05962}		\pgfmath@def{acos}{957}{16.86322}
\pgfmath@def{acos}{958}{16.66457}		\pgfmath@def{acos}{959}{16.46359}
\pgfmath@def{acos}{960}{16.26020}		\pgfmath@def{acos}{961}{16.05430}
\pgfmath@def{acos}{962}{15.84580}		\pgfmath@def{acos}{963}{15.63459}
\pgfmath@def{acos}{964}{15.42057}		\pgfmath@def{acos}{965}{15.20360}
\pgfmath@def{acos}{966}{14.98357}		\pgfmath@def{acos}{967}{14.76033}
\pgfmath@def{acos}{968}{14.53374}		\pgfmath@def{acos}{969}{14.30364}
\pgfmath@def{acos}{970}{14.06986}		\pgfmath@def{acos}{971}{13.83221}
\pgfmath@def{acos}{972}{13.59049}		\pgfmath@def{acos}{973}{13.34447}
\pgfmath@def{acos}{974}{13.09392}		\pgfmath@def{acos}{975}{12.83856}
\pgfmath@def{acos}{976}{12.57811}		\pgfmath@def{acos}{977}{12.31225}
\pgfmath@def{acos}{978}{12.04060}		\pgfmath@def{acos}{979}{11.76278}
\pgfmath@def{acos}{980}{11.47834}		\pgfmath@def{acos}{981}{11.18676}
\pgfmath@def{acos}{982}{10.88748}		\pgfmath@def{acos}{983}{10.57984}
\pgfmath@def{acos}{984}{10.26309}		\pgfmath@def{acos}{985}{9.93636}
\pgfmath@def{acos}{986}{9.59863}		\pgfmath@def{acos}{987}{9.24870}
\pgfmath@def{acos}{988}{8.88512}		\pgfmath@def{acos}{989}{8.50614}
\pgfmath@def{acos}{990}{8.10961}		\pgfmath@def{acos}{991}{7.69281}
\pgfmath@def{acos}{992}{7.25224}		\pgfmath@def{acos}{993}{6.78328}
\pgfmath@def{acos}{994}{6.27958}		\pgfmath@def{acos}{995}{5.73196}
\pgfmath@def{acos}{996}{5.12640}		\pgfmath@def{acos}{997}{4.43922}
\pgfmath@def{acos}{998}{3.62430}		\pgfmath@def{acos}{999}{2.56255}
\pgfmath@def{acos}{1000}{0.00000}

==> pgfmathutil.code.tex <==
% This file defines utilities common to the \pgfmath files.
%
% (c) 2007 Mark Wibrow
%
% but subject to the LaTeX Project Public License 
% (http://www.latex-project.org/lppl.txt)
%
% and the GNU Public License 
% (http://www.gnu.org/licenses/gpl.txt)
%
% Version 0.0 08/03/2007

% Alias some pgf stuff, just in case it needs replacing later.
%
\let\pgfmath@x\pgf@x
\let\pgfmath@xa\pgf@xa
\let\pgfmath@xb\pgf@xb
\let\pgfmath@xc\pgf@xc

\let\pgfmath@y\pgf@y
\let\pgfmath@ya\pgf@ya
\let\pgfmath@yb\pgf@yb
\let\pgfmath@yc\pgf@yc

\let\c@pgfmath@counta\c@pgf@counta
\let\c@pgfmath@countb\c@pgf@countb
\let\c@pgfmath@countc\c@pgf@countc

\let\pgfmath@ifnextchar\pgfutil@ifnextchar

\let\pgfmath@tonumber\pgf@sys@tonumber

\let\pgfmath@ifundefined\pgfutil@ifundefined

\newif\ifpgfmath@in@
\def\pgfmath@in@#1#2{%
 \def\pgfmath@in@@##1#1##2##3\pgfmath@in@@{%
  \ifx\pgfmath@in@##2\pgfmath@in@false\else\pgfmath@in@true\fi}%
 \pgfmath@in@@#2#1\pgfmath@in@\pgfmath@in@@}
 
% Need to redefine to something more appropriate...?
%
\def\pgfmath@error#1#2{\PackageError{PGF Math}{#1}{#2}}
\def\pgfmath@warning#1#2{\PackageWarning{PGF Math}{#1}{#2}}

% \pgfmath@pt
%
% Needed to test for 'pt' resulting from 
% expansion using \the.
%
{\catcode`\p=12\catcode`\t=12\gdef\PgfmaTh@PT{pt}}		
\edef\pgfmath@pt{\PgfmaTh@PT}%

% \pgfmath@ifin@
%
% Interface for \pgfutil@in@
%
\def\pgfmath@ifin@#1#2{%
	\pgfutil@in@{#1}{#2}%
	\ifpgfutil@in@%
		\expandafter\pgfmath@firstoftwo%
	\else%
		\expandafter\pgfmath@secondoftwo%
	\fi%
}

% \pgfmath@empty
%
% A handy macro.
%
\def\pgfmath@empty{}


% \ifpgfmath@empty
%
% Has #1 been let to \pgf@empty?
%
\def\ifpgfmath@empty#1{%
	\ifx#1\pgfmath@empty\relax
		\expandafter\pgfmath@firstoftwo%
	\else%
		\expandafter\pgfmath@secondoftwo%
	\fi%
}
\def\pgfmath@firstoftwo#1#2{#1}
\def\pgfmath@secondoftwo#1#2{#2}

% \ifpgfmath@ifletto
%
% Has #1 been let to #2?
%
\def\pgfmath@ifletto#1#2{%
	\ifx#1#2\relax%
		\expandafter\pgfmath@firstoftwo%
	\else%
		\expandafter\pgfmath@secondoftwo%
	\fi%
}

% \ifpgfmath@iflettoeither
%
% Has #1 been let to #2 or #3?
%
\def\pgfmath@iflettoeither#1#2#3{%
	\ifx#1#2\relax%
		\let\pgfmath@equaltoeithernext\pgfmath@firstoftwo%
	\else%
		\ifx#1#3\relax%
			\let\pgfmath@equaltoeithernext\pgfmath@firstoftwo%
		\else%
			\let\pgfmath@equaltoeithernext\pgfmath@secondoftwo%
		\fi%
	\fi%
	\pgfmath@equaltoeithernext%
}

% \pgfmath@gobbletilpgfmath@
%
% Gobble stream until \pgfmath@ {which is undefined}.
% 
\def\pgfmath@gobbletilpgfmath@#1\pgfmath@{}
\def\pgfmath@gobbleone#1{}%


% \pgfmathloop
%
% A version of the standard TeX and LaTeX
% \loop, with an additional macro \pgfmathcounter
% (which is *not* a TeX counter) which keeps
% track of the iterations.
%
\newif\ifpgfmathcontinueloop
\def\pgfmathloop#1\repeatpgfmathloop{%
	\def\pgfmathcounter{1}%
	\def\pgfmath@iterate{%
		#1\relax%
		{% Do this inside a group, just in case...
			\c@pgfmath@counta=\pgfmathcounter%
			\advance\c@pgfmath@counta by1\relax%
			\xdef\pgfmathloop@temp{\the\c@pgfmath@counta}%
		}%	
		\edef\pgfmathcounter{\pgfmathloop@temp}%
		\expandafter\pgfmath@iterate\fi}%
	\pgfmath@iterate\let\pgfmath@iterate=\relax}
\let\repeatpgfmathloop=\fi


% \pgfmath@returnone
%
% \edef \pfgmathresult to the value of #1 after the end
% of a group.
%
% #1 - a dimension/count/skip register or a macro
%      representing a number or dimension.
%
\def\pgfmath@returnone#1{%
	\afterassignment\pgfmath@gobbletilpgfmath@%
	\pgfmath@x#1pt\relax\pgfmath@%
	\xdef\pgfmath@resulttemp{\pgf@sys@tonumber{\pgfmath@x}}%
	\gdef\pgfmath@returnone@{%
		\edef\pgfmathresult{\pgfmath@resulttemp}%
	}%
	\aftergroup\pgfmath@returnone@}


% \pgfmath@returntwo
%
% \edef \pfgmathresultx to the value of #1, and
% \pgfmathresulty to the value of #2, after the end
% of a group.
%
% #1 - a dimension/count/skip register or a macro
%      representing a number or dimension.
%
% #2 - a dimension/count/skip register or a macro
%      representing a number or dimension.
%	
\def\pgfmath@returntwo#1#2{%
	\afterassignment\pgfmath@gobbletilpgfmath@%
	\pgfmath@x#1pt\relax\pgfmath@%
	\xdef\pgfmath@resulttempx{\pgf@sys@tonumber{\pgfmath@x}}%
	\afterassignment\pgfmath@gobbletilpgfmath@%
	\pgfmath@x#2pt\relax\pgfmath@%
	\xdef\pgfmath@resulttempx{\pgf@sys@tonumber{\pgfmath@x}}%
	\gdef\pgfmath@returntwo@{%
		\edef\pgfmathresultx{\pgfmath@resulttempx}%
		\edef\pgfmathresulty{\pgfmath@resulttempy}%
	}%
	\aftergroup\pgfmath@returntwo@}

% \pgfmath@smuggleone
%
% Summgle a macro outside a group.
%
\def\pgfmath@smuggleone#1{%
	\xdef\pgfmath@smuggleditem{#1}%
	\gdef\pgfmath@@smuggleone{\edef#1{\pgfmath@smuggleditem}}%
	\aftergroup\pgfmath@@smuggleone}

==> pgfrcs.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



% The purpose of this file is to define the command
% \ProvidesPackageRCS, which should be followed by an RCS id
% string. This command will also be available in plain TeX, where it
% prints out a message to the log.


\def\pgfversion{1.18}


\ifx\pgfrcsloaded\undefined
\def\pgfrcsloaded{}

\edef\pgfrcsatcode{\the\catcode`\@}
\catcode`\@=11

% Get date and version from RCS Ids
\def\pgf@parseid $#1: #2.#3,v #4 #5/#6/#7 #8${%
  \pgf@parsercsfile$#2/$
  \def\pgf@rcssuffix{#3}
  \def\pgf@rcsrevision{#4}
  \def\pgf@rcsdate{#5/#6/#7}
}
\def\pgf@parsercsfile$#1/#2${
  \def\pgf@temp{#2}
  \ifx\pgf@temp\pgfutil@empty
    \def\pgf@rcsfile{#1}
  \else
    \pgf@parsercsfile$#2$
  \fi}

\def\ProvidesFileRCS{%
  \def\pgfrcs@marshal{\ProvidesFile{\pgf@rcsfile.\pgf@rcssuffix}}%
  \pgfrcs@parserest%
}

\def\ProvidesPackageRCS{%
  \def\pgfrcs@marshal{\ProvidesPackage{\pgf@rcsfile}}%
  \pgfrcs@parserest%
}

\def\pgfrcs@parserest{%
  \def\pgf@rcsadditional{}%
  \afterassignment\pgfrcs@checkforoptional\let\next=}

\def\pgfrcs@checkforoptional{%
  \ifx\next[%
    \let\next=\pgfrcs@getoptional%
  \else
    \let\next=\pgfrcs@package%
  \fi%
  \next}%}

\def\pgfrcs@getoptional#1] ${%
  \def\pgf@rcsadditional{#1}%
  \pgfrcs@package%
}

\def\pgfrcs@package#1${
  \pgf@parseid $#1$
  \pgfrcs@marshal[\pgf@rcsdate\space\pgf@rcsadditional\space(rcs-revision \pgf@rcsrevision)]
}

\def\ProvidesClassRCS $#1$ [#2]{%
  \pgf@parseid $#1$
  \ProvidesClass{\pgf@rcsfile}[\pgf@rcsdate\space#2\space (rcs-revision \pgf@rcsrevision)]
}

\ifx\ProvidesPackage\@undefined
  % plain tex
  \def\ProvidesPackage#1[#2]{\wlog{Loading package #1 version #2.}}
\fi

\ifx\ProvidesFile\@undefined
  % plain tex
  \def\ProvidesFile#1[#2]{\wlog{Loading file #1 version #2.}}
\fi

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/utilities/pgfrcs.code.tex,v 1.16 2007/06/08 11:24:59 tantau Exp $

\catcode`\@=\pgfrcsatcode

\fi



==> pgfsys.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/systemlayer/pgfsys.code.tex,v 1.24 2007/06/07 07:41:11 tantau Exp $


%
% The following conversion functions are used to convert from TeX
% dimensions to postscript/pdf points.
% 
{\catcode`\p=12\catcode`\t=12\gdef\Pgf@geT#1pt{#1}}

\def\pgf@sys@tonumber#1{\expandafter\Pgf@geT\the#1}

\def\pgf@sys@bp@correct#1{#1=0.99627#1}

\def\pgf@sys@bp#1{%
  {%
    \pgf@x=#1\relax%
    \pgf@x=0.99627\pgf@x%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\toks@}%
  }%
}
\def\pgf@sys@pt#1{%
  {%
    \pgf@x=#1\relax%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\toks@}%
  }%
}


% internal dimensions that are always present when pgsys is loaded.
\newdimen\pgf@x
\newdimen\pgf@y
\newdimen\pgf@xa
\newdimen\pgf@ya
\newdimen\pgf@xb
\newdimen\pgf@yb
\newdimen\pgf@xc
\newdimen\pgf@yc

% internal counters that are alwyas present when pgfsys is loaded
\newcount\c@pgf@counta
\newcount\c@pgf@countb
\newcount\c@pgf@countc
\newcount\c@pgf@countd


% The following \if decides, whether even-odd filling and clipping is
% to be used or normal the non-zero winding number rule. See the
% pdf-documentation for details on what these rules are.

\newif\ifpgfsys@eorule



% In the following dummy definitions of the pgf system commands are
% given. The individual drivers must overwrite these definitions,
% preferably all of them. If some system command is used that has not
% been overwritten, the command fails with a warning.
%
% In some cases, some pgf system commands are just shorthands for a
% series of more complicated commands. In this case, a default
% implementation is given in this file, but a driver may choose to
% overwrite this default implementation with a more effecient
% version. For example, a closestroke is the same as a closepath
% followed by a stroking, but in pdf there is a special shorthand for
% this. So, the pdf driver overwrites \pgfsys@closestroke, while the
% postscript driver does not.
%
% The commands for which default implementations are available are
% given at the end.

\def\pgf@sys@fail#1{%
  \expandafter\ifx\csname pgf@sys@fail@#1\endcsname\pgfutil@empty%
  \else%
    \expandafter\global\expandafter\let\csname pgf@sys@fail@#1\endcsname=\pgfutil@empty%
    \PackageWarning{pgf}{%
      Your graphic driver \pgfsysdriver\space does not supported #1. This warning is given only once}%
  \fi%
}



\def\pgfsys@invoke{\pgf@sys@fail{invoking specials}}
% This command is used whenever some literal text needs to be inserted
% into the resulting .pdf, .ps, or .dvi file. Note that most
% \pgfsys@xxxx commands will not directly call this command, but,
% rather, use the protocolling mechanism to record their literal
% text. It is then left to the discretion of the protocolling
% mechansim to insert the literal text at some appropriate, later
% time. 
%
% This command should only be called when \pgfsys@beginpicture has
% been called previously and when the picture has not been suspended
% using \pgfsys@beginhbox.


\def\pgfsys@outerinvoke{\pgfsys@invoke}
% This command can be used to insert protocolled graphic commands
% outside any picture. This is extremely dangerous, but sometimes
% useful. By default, this command does the same as inside pictures. 



%
%
% Path construction commands
%
%

\def\pgfsys@moveto#1#2{\pgf@sys@fail{path constructions}}
% This command is used to start a path at a specific point (#1bp,#2bp)
% or to move the current point of the current path to (#1bp,#2bp)
% without drawing anything upon stroking (the current path is
% `interrupted'). 
%
% Here (and in the following) the coordinates are in TeX's big points
% (bp), unless the coordinate system has been scaled. A big point is
% 1/72 inches. Note that TeX's point pt is 1/72.27 inches.
%
% Example:
%
% \pgfsys@moveto{10}{10}
% \pgfsys@lineto{0}{0}
% \pgfsys@stroke
%
% This will draw a line from (10bp,10bp) to the origin of the picture.

\def\pgfsys@lineto#1#2{\pgf@sys@fail{path constructions}}
% Continue the current path to (#1bp,#2bp) with a line.

\def\pgfsys@curveto#1#2#3#4#5#6{\pgf@sys@fail{path constructions}}
% Continue the current path with a bezier curver to (#5bp,#6bp). The
% control points of the curve are at (#1bp,#2bp) and (#3bp,#4bp).

\def\pgfsys@rect#1#2#3#4{\pgf@sys@fail{path constructions}}
% Append a rectangle to the current path whose lower left corner is at
% (#1bp,#2bp) and whose width/height is given by (#3bp,#4bp).
%
% This command can be `mapped back' to moveto and lineto commands, but
% it is included since pdf has a special, quick version of this command.

\def\pgfsys@closepath{\pgf@sys@fail{path constructions}}
% Close the current path. This results in joining the current point of
% the path with the point specified by the last moveto
% operation. Typically, this is preferable over using lineto to the
% last point specified by a moveto, since the line starting at this
% point and the line ending at this point will be smoothly joined by
% closepath. 
%
% Example:
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@closepath
% \pgfsys@stroke
%
% versus
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@lineto{0}{0}
% \pgfsys@stroke
% 
% The difference between the above will be that in the second triangle
% the corner at the origin will be wrong; it will just be the overlay
% of two lines going in different directions, not a sharp pointed
% corner.






%
%
% Stroking and filling commands
%
%

\def\pgfsys@stroke{\pgf@sys@fail{path usage}}
% Stroke the current path (as if it were drawn with a pen). A number
% of so-called graphic state parameters influence this, which can be
% set in different ways:
%
% - linewidth
%   The `thickness' of the line. A width of 0 is the thinnest width
%   renderable on the device. On a high-resolution printer this may
%   become invisible and should be avoided. A good choice is 0.4pt,
%   which is the default.
%
% - stroke color
%   This special color is used for stroking. If it is not set, the
%   current color is used.
%
% - cap
%   The cap describes how the endings of lines a drawn. A round cap
%   adds a little half circle to these endings. A butt cap ends the
%   lines exactly at the end (or start) point without anything
%   added. A rectangular cap ends the lines like the butt cap, but the
%   lines protrude over the endpoint by the line thickness. (See also
%   the pdf or postscript manual). If the path has been closed, no cap
%   is drawn.
%
% - join
%   This describes how a bend (a join) in a path is rendered. A round
%   join draws bends using small arcs. A bevel join just draws the two
%   lines and then fills the join minimally so that it becomes
%   convex. A miter join extends the lines so that they form a single
%   sharp corner, but only up to a certain miter limit. (See the pdf
%   or postscript manual once more).
%
% - dash
%   The line may be dashed according to a dashing pattern.
%
% - clipping area
%   If a clipping area is established, only those parts of the path
%   that are inside the clipping area will be drawn.
%
% In addition to stroking a path, the path may also be used for
% clipping after it has been stroked. This will happen if the
% \pgfsys@clipnext is used prior to this command, see there for
% details.

\def\pgfsys@fill{\pgf@sys@fail{path usage}}
% This command fills the area surrounded by the current path. If the
% path has not yet been closed, it is closed prior to filling. The
% path itself is not stroked. For self-intersecting paths or paths
% consisting of multiple parts, the nonzero winding number rule is
% used to determine whether a point is inside or outside the
% path, except if \ifpgfsys@eorule holds -- in which case the even-odd
% rule should be used. (See the pdf or postscript manual for details.) 
%
% The following graphic state parameters influence the filling:
%
% - fill color
%   If the fill color is not especially set, the current color is
%   used. 
%
% - clipping area
%   If a clipping area is established, only those parts of the filling
%   area that are inside the clipping area will be drawn.
%
% In addition to filling the path, the path will also be used for
% clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@fillstroke{\pgf@sys@fail{path usage}}
% First, the path is filled, then the path is stroked. If the fill and
% stroke colors are the same (or if they are not specified and the
% current color is used), this yields almost the same as a
% \pgfsys@fill. However, due to the line thickness of the stroked
% path, the fillstroked area will be slightly larger.
%
% In addition to stroking and filling the path, the path will also be
% used for clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@clipnext{\pgf@sys@fail{path usage}}
% This command should be issued after a path has been constructed, but
% before it has been stroked and/or filled or discarded. When the
% command is used, the next stroking/filling/discarding command will
% first be executed normally. Then, afterwards, the just-used path
% will be used for subsequent clipping. If there has already been a
% clipping region, this region is intersected with the new clipping
% path (the clipping cannot get bigger). The nonzero winding number
% rule is used to determine whether a point is inside or outside the
% clipping area or the even-odd rule, depending on whether
% \ifpgfsys@eorule holds.

\def\pgfsys@discardpath{\pgf@sys@fail{path usage}}
% Normally, this command should `throw away' the current path.
% However, after \pgfsys@clipnext has been called, the current path
% should subsequently be used for clipping. See \pgfsys@clipnext for
% details. 





%
%
% Stroking options
%
%
\def\pgfsys@setlinewidth#1{\pgf@sys@fail{setting the line width}}
% Sets the width of lines, when stroked, to #1bp.

\def\pgfsys@buttcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a butt cap. See \pgfsys@stroke.

\def\pgfsys@roundcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a round cap. See \pgfsys@stroke.

\def\pgfsys@rectcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a rectangular cap. See \pgfsys@stroke.

\def\pgfsys@miterjoin{\pgf@sys@fail{setting the line join}}
% Sets the join to a miter join. See \pgfsys@stroke.

\def\pgfsys@setmiterlimit#1{\pgf@sys@fail{setting the line cap}}
% Sets the miter limit of lines to #1. See the pdf or postscript
% documentation.

\def\pgfsys@roundjoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a round join. See \pgfsys@stroke.

\def\pgfsys@beveljoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a bevel join. See \pgfsys@stroke.

\def\pgfsys@setdash#1#2{\pgf@sys@fail{setting the dashing pattern}}
% Sets the dashing patter. #1 should be a list of lengths given in big
% points (bp) separated by spaces. #2 should be a single value given
% in bp.
%
% The list of values in #1 is used to determine the lengths of the
% `on' phases of the dashing and of the `off' phases. For example, if
% #1 is `3 4', then the dashing pattern is `3bp on followed by 4bp
% off, followed by 3bp on, followed by 4bp off, and so on'. A pattern
% of `.5 4 3 1.5' means `.5bp on, 4bp off, 3bp on, 1.5bp off, .5bp on,
% ...'. If the number of entries is odd, the last one is used twice,
% so `3' means `3bp on, 3bp off, 3bp on, 3bp off,...'. An empty list
% means `always on'.
%
% The second argument determines the `phase' of the pattern. For
% example, for a pattern of `3 4' and a phase of `1', the pattern
% would start: `2bp on, 4bp off, 3bp on, 4bp off, 3bp on, 4bp off...'.




%
%
% Opacity stuff
%
%

\def\pgfsys@stroke@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of stroking operations. 1 means fully opaque, 0
% means fully transparent.

\def\pgfsys@fill@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of filling operations. 1 means fully opaque, 0
% means fully transparent.




%
%
% Color stuff
%
%

\def\pgfsys@color@rgb@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given rgb tuple
% (numbers between 0 and 1). 
%
% Example: Make stroked text dark red: \pgfsys@color@rgb@stroke{0.5}{0}{0}
%
% The special stroking color is only used if the stroking color has
% been set since the last \pgfutil@color command. Thus, each \pgfutil@color command
% should reset both the stroking and filling colors.

\def\pgfsys@color@rgb@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given rgb tuple
% (numbers between 0 and 1). This color may be different from the
% stroking color.

\def\pgfsys@color@rgb#1#2#3{\pgfsys@color@rgb@stroke{#1}{#2}{#3}\pgfsys@color@rgb@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations. This is a
% ``low-level'' version of the \pgfutil@color command. It is currently only
% used by the plain tex version to support colors.

\def\pgfsys@color@cmyk@stroke#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cymk tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmyk@fill#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cymk tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmyk#1#2#3#4{\pgfsys@color@cmyk@stroke{#1}{#2}{#3}{#4}\pgfsys@color@cmyk@fill{#1}{#2}{#3}{#4}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@cmy@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cym tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmy@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cym tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmy#1#2#3{\pgfsys@color@cmy@stroke{#1}{#2}{#3}\pgfsys@color@cmy@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@gray@stroke#1{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given gray level 
% (number between 0 and 1). 

\def\pgfsys@color@gray@fill#1{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given gray level 
% (number between 0 and 1). 

\def\pgfsys@color@gray#1{\pgfsys@color@gray@stroke{#1}\pgfsys@color@gray@fill{#1}}
% Sets the color used for filling and stroking operations.

\newif\ifpgfsys@color@reset@inorder
% This if decides whether the color resetting of the
% \pgfsys@color@reset command may assume that all color commands are
% given ``in order.'' This means that this command will not be called,
% say, at the beginning of a box that is later inserted at a point
% where a fill color was actively set. This may allow the command to
% produce more compact code when it ``knows'' that no special fill or
% stroke color has been set.
\pgfsys@color@reset@inordertrue


\def\pgfsys@color@reset{}
% This command will be called when the \pgfutil@color command is used. It
% should purge any internal settings of stroking and filling
% color. After this call, till the next use of a command like
% \pgfsys@color@rgb@fill, the current color installed by the \pgfutil@color
% command should be used.

\def\pgfsys@color@unstacked#1{}
% This slightly obscure command causes the color stack to be
% tricked. When called, this command should set the current color to
% #1 without causing any change in the color stack. 



%
%
% Coordinate system transformations
%
%

\def\pgfsys@transformcm#1#2#3#4#5#6{\pgf@sys@fail{transformations}}
% Perform a concatenation of the low-level current transformation
% matrix with the matrix given by the values #1 to #6. The
% transformation matrix is a transformation on a homogeneous
% 2D-coordinate system. See the pdf or postscript manual for details. 




%
%
% Graphic state saving and restoring.
%
%

\def\pgfsys@beginscope{\pgf@sys@fail{scoping}}
% Saves the current graphic state on a graphic state stack. All
% changes to the graphic state parameters mentioned for \pgfsys@stroke
% and \pgfsys@fill will be local to the current graphic state and will
% the old values will be restored after endscope is used.
%
% WARNING: pdf and postscript differ with respect to the question of
% whether the current path is part of the graphic state or not. For
% this reason, you should never use this command unless the path is
% currently empty. For example, it might be a good idea to use
% discardpath prior to calling this command. 

\def\pgfsys@endscope{\pgf@sys@fail{scoping}}
% Restores the last saved graphic state.




%
%
% Special commands
%
%

\def\pgfsys@imagesuffixlist{}
% A list of suffixes, separated by `:', that will be tried when
% searching for an image.



%
%
% Special commands
%
%


\def\pgfsys@definemask{\pgf@sys@fail{masking}}
% This command declares a mask for usage with images. It works similar
% to \pgfsys@defineimage: Certain macros are set when the command is
% called. The result should be to set the macro \pgf@mask to a pdf
% object count that can subsequently be used as a soft mask. The
% following macros will be set when this command is invoked:
%
% - \pgf@filename
%   File name of the mask to be defined.
%
% - \pgf@maskmatte
%   The so-called matte of the mask (see the pdf documentation for
%   details). The matte is a color specification consisting of 1, 3 or
%   4 numbers between 0 and 1. The number of numbers depends on the
%   number of color channels in the image (not in the mask!). It will
%   be assumed that the image has been preblended with this color.




%
%
% Shading commands
%
%

\def\pgfsys@horishading#1#2#3{\pgf@sys@fail{shadings}}
% Declares a horizontal shading for later use. The effect of this
% command should be the definition of a macro called `@pgfshading#1!'
% (or \csname @pdfshading#1!\endcsname, to be precise). When invoked,
% this new macro should insert a shading at the current position.
%
% #1 is the name of the shading, which is also used in the output
% macro name. #2 is the height of the shading and must be given as a
% TeX dimension like `2cm' or `10pt'. #3 is a shading color
% specification as specified in the pgfuserguide. The shading
% specification implicitly fixes the width of the shading. 
%
% When `@pgfshading#1!' is invoked, it should insert a box of height
% #2 and the width implicit in the shading declaration.

\def\pgfsys@vertshading#1#2#3{\pgf@sys@fail{shadings}}
% Like horishading, only for vertical shadings. This time, the height
% of the shading is implicit in #3 and the width is given as #2.

\def\pgfsys@radialshading#1#2#3{\pgf@sys@fail{shadings}}
% Declares a radial shading. Like the previous macros, this command
% should setup the macro `@pgfshading#1!', which upon invocation
% should insert a radial shading whose size is implicit in #3. 
%
% The parameter #2 is a pgf point specification if the starting point
% of the shading. See the pgfuserguide for details.





%
%
% Pattern stuff
%
%

\def\pgfsys@declarepattern#1#2#3#4#5#6#7#8#9{\pgf@sys@fail{patterns}}
% This command declares a new colored or uncolored pattern. Uncolored
% patterns have no inherent color, the color is provided when they are
% set. Colored patters have an inherent color.
% #1       = name of the pattern (must be a plain suffix for use in
%            postscript/pdf/etc.) 
% #2 to #5 = four coordinates describing the corners of a bounding box
%            of pattern cells
% #6       = x-step
% #7       = y-step
% #8       = pattern code
% #9       = 0 if uncolored patter, 1 if colored pattern.

\def\pgfsys@setpatternuncolored#1#2#3#4{\pgf@sys@fail{patterns}}
% Sets an uncolored pattern #1 as filling color. The numbers #2, #3,
% #4 must be an rgb-value to be used as the color of the pattern.

\def\pgfsys@setpatterncolored#1{\pgf@sys@fail{patterns}}
% Sets an colored pattern #1 as filling color.


%
%
% Page size stuff
%
%
\def\pgfsys@papersize#1#2{\pgf@sys@fail{papersize}}
% This command sets the paper size in a portable way.
% #1 = width
% #2 = height



%
%
% Position tracking commands
%
%

% Marks the current position on the page. This position can later be
% referenced using \pgfsys@getposition
\def\pgfsys@markposition#1{\pgf@sys@fail{marking the current position}}

% Sets #2 to a pgfpoint macro that returns the position #1 is
% returned in a coordinate system where the x-axis goes right and the
% y-axis goes up. The origin of this coordinate system may or may not
% lie in the lower left corner; you should shift the coordinate system
% to the position "pgfpageorigin" to make sure that the origin is at
% the lower left corner. Typically, getting this position
% requires two runs of TeX. On the first run, the macro will be set to
% \relax, indicating that the position is not available. 
%
% If #1 is set to the special position "pgfpageorigin", the position
% of the the lower left page corner is returned. 

\def\pgfsys@getposition#1#2{\let#2=\relax}



%
%
% Commands having a default implementation. These commands only need
% not be implemented by drivers if this results in a better
% preformance. 
%
%


\def\pgfsys@shadingoutsidepgfpicture#1{%
  #1%
}
% This command gets the definition of a shading (@pgfshadingxxxx!) as
% an argument and should insert this shading into the normal text.
%
% This command has a default implementation.


\def\pgfsys@shadinginsidepgfpicture#1{%
  \pgf@makehbox{#1}%
  \setbox\pgf@hbox=\hbox{\hskip-.5\wd\pgf@hbox\lower.5\ht\pgf@hbox\hbox{\box\pgf@hbox}}%
  \pgfqbox{\pgf@hbox}%
}
% This command works like \pgfsys@shadingoutsidepgfpicture, only it is
% called when a shading should be inserted inside a picture. This
% command should insert the shading centered on the origin (which will
% typically have been low-level translated somewhere else.)
%
% This command has a default implementation.





\def\pgfsys@closestroke{\pgfsys@closepath\pgfsys@stroke}
% This command should have the same effect as first closing the path
% and then stroking it.


\def\pgfsys@transformshift#1#2{\pgfsys@transformcm{1}{0}{0}{1}{#1}{#2}}
% This command will change the origin of the low-level coordinate
% system to (#1bp,#2bp).

\def\pgfsys@transformxyscale#1#2{\pgfsys@transformcm{#1}{0}{0}{#2}{0bp}{0bp}}
% This command will scale the low-level coordinate system (and
% everything that is drawn) by a factor of #1 in x-directed and #2 in
% y-direction. Note that this applies to everything, including
% lines. So a scaled line will have a different width and may even
% have a different width when going along the x-axis and when going
% along the y-axis, if the scaling is different in these directions.

\def\pgfsys@hbox#1{%
  \pgfsys@beginscope%
    \setbox#1=\hbox{\box#1}%
    \wd#1=0pt%
    \ht#1=0pt%
    \dp#1=0pt%
    \box#1%
  \pgfsys@endscope%
}
% Called to insert a TeX hbox into a pgfpicture. 

\def\pgfsys@hboxsynced#1{%
  {\pgfsys@beginscope\pgflowlevelsynccm\pgfsys@hbox#1\pgfsys@endscope}%
}
% Called to insert a TeX hbox into a pgfpicture, but with the current
% coordinate transformation matrix synced with the canvas
% transformation matrix. 
%
% In essence, this command does the same as if you first said
% \pgflowlevelsynccm and then \pgfsys@hbox. However, a driver may
% choose to use a ``TeX-translation'' for the translation part of the
% transformation cm. This will ensure that hyperlinks ``survive'' at
% least translations. 

\def\pgfsys@beginpicture{}
% Called at the beginning of a pgfpicture. Used to setup things.

\def\pgfsys@endpicture{}
% Called at the end of a pgfpicture. 

\def\pgfsys@typesetpicturebox#1{%
  \pgfmathsetlength\pgf@x{\pgf@shift@baseline}%
  \advance\pgf@x by-\pgf@picminy\relax%
  \advance\pgf@picmaxy by-\pgf@picminy\relax% maxy is now the height
  \advance\pgf@picmaxx by-\pgf@picminx\relax% maxx is now the width
  \setbox#1=\hbox{\hskip-\pgf@picminx\lower\pgf@picminy\box#1}%
  \ht#1=\pgf@picmaxy%
  \wd#1=\pgf@picmaxx%
  \dp#1=0pt%
  \leavevmode\raise-\pgf@x\box#1%
}
% Called after a picture has been typeset in box #1. This
% command should insert the box into the normal TeX code. The box #1
% will still be a ``raw'' box that contains only the \special's. The
% job of this command is to resize and shift this box according to the
% baseline shift and the size of the box.
%
% This command has a default implementation.

\def\pgfsys@beginpurepicture{\pgfsys@beginpicture}
% This version of the beginpicture command can be used for pictures
% that are guaranteed not to contain any hboxes. In this case, a
% driver might provide a more compact version of the command.

\def\pgfsys@endpurepicture{\pgfsys@endpicture}
% Called at the end of a ``pure'' pgfpicture.

\def\pgfsys@defineimage{%
  \ifx\pgf@imagewidth\pgfutil@empty\else\edef\pgf@imagewidth{width=\pgf@imagewidth,}\fi%
  \ifx\pgf@imageheight\pgfutil@empty\else\edef\pgf@imageheight{height=\pgf@imageheight,}\fi%
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepage{page=\pgf@imagepage,}\fi%
  \edef\pgf@image{\noexpand\includegraphics[\pgf@imageheight\pgf@imagewidth]{\pgf@filename}}%
}
% Called, when an image should be defined. 
%
% This command does not take any parameters. Instead, certain macros
% will be preinstalled with appropriate values when this command is
% invoked. These are:
%
% - \pgf@filename
%   File name of the image to be defined.
%
% - \pgf@imagewidth
%   Will be set to the desired (scaled) width of the image.
%
% - \pgf@imageheight
%   Will be set to the desired (scaled) height of the image.
%
%   If this macro and also the height macro are empty, the image
%   should have its `natural' size.
%
%   If exactly only of them is specified, the undefined value the
%   image is scaled so that the aspect ratio is kept.
%
%   If both are set, the image is scaled in both directions
%   independently, possibly changing the aspect ratio.
%
%
% The following macros presumable mostly make sense for drivers that
% can handle pdf: 
%
% - \pgf@imagepage
%   The desired page number to be extracted from a multi-page
%   `image'. 
%
% - \pgf@imagemask
%   If set, it will be set to `/SMask x 0 R', where x is the pdf
%   object number of a soft mask to be applied to the image.
%
% - \pgf@imageinterpolate
%   If set, it will be set to `/Interpolate true' or  `/Interpolate
%   false', indicating whether the image should be interpolated in
%   pdf. 
%
%
% The command should now setup the macro \pgf@image such that calling
% this macro will result in typesetting the image. Thus, \pgf@image is
% the `return value' of the command.


\def\pgfsys@defobject#1#2#3#4{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedtrue%
    #4%
    \pgfsysprotocol@getcurrentprotocol\pgfsys@@temp%
    \expandafter\global\expandafter\let\csname #1\endcsname=\pgfsys@@temp%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Declares an object for later use. The idea is that the object can be
% precached in some way and then be rendered more quickly when used
% several times. For example, an arrow head might be defined and
% prerendered in this way.
%
% The parameter #1 is the name for later use. #2 and #3 are pgf points
% specifying a bounding box for the object. #4 is the code for the
% object. The code may only contain protocollable code.


\def\pgfsys@useobject#1#2{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedfalse%
    #2%
    \expandafter\pgfsysprotocol@setcurrentprotocol\csname #1\endcsname%
    \pgfsysprotocol@invokecurrentprotocol%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Renders a previously declared object. The first parameter is the
% name of the the object. The second parameter is extra code that
% should be executed right *before* the object is rendered. Typically,
% this will be some transformation code. 


\def\pgfsys@begininvisible{\pgfsys@transformcm{1}{0}{0}{1}{2000bp}{2000bp}}
% Between this command and the closing endinvisible, all output should
% be suppressed. Nothing should be drawn at all, which includes all
% paths, images and shadings.

\def\pgfsys@endinvisible{\pgfsys@transformcm{1}{0}{0}{1}{-2000bp}{-2000bp}}
% Ends the invisibilty section, unless invisibility blocks have been
% nested. In this case, only the `last' one restores visibility.


\def\pgfsys@atbegindocument{}
% This command will be executed at the begin of the document. If for
% whatever reason this is not done, you may wish to execute this
% command yourself. It will setup certain specials that need to be
% inserted into the resulting .pdf/.ps/.xxx file.





% Discern the driver:
\input pgf.cfg

\PackageInfo{pgfsys}{Driver file for pgf: \pgfsysdriver}
\pgfutil@InputIfFileExists{\pgfsysdriver}{}{%
  \PackageError{pgfsys}{Driver file ``\pgfsysdriver'' not found.}{}}



% This will insert always-present-specials at the beginning of the
% code. 
\AtBeginDocument{
  \pgfsys@atbegindocument
  \let\pgfsys@atbegindocument=\pgfutil@empty
}



% Read aux file in plain and context mode:

\pgfutil@aux@read@hook


\endinput


==> pgfsysprotocol.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/systemlayer/pgfsysprotocol.code.tex,v 1.4 2006/10/16 22:32:59 tantau Exp $



% This package provides the pgf system protcol layer. Protocolling is
% used to record a bunch of graphic operations so that they can be
% reused quickly at a later point.
%
% Basically, all ``recordable'' \pgfsys@xxxx commands call
% \pgfsysprotocol@protocol for their protocolable literal
% specials. The literal text will either be stored in the current
% protocol. At a later point (actually, normally this happens
% immediately afterwards), the accumulated protocolled text is invoked
% using pgfsys@invokeprotocol.



\let\pgfsysprotocol@currentprotocol=\pgfutil@empty
\newif\ifpgfsysprotocol@buffered


% Add to the protocol buffered
\def\pgfsysprotocol@literalbuffered#1{%
  \edef\pgfsysprotocol@temp{{#1\space}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfsysprotocol@currentprotocol\pgfsysprotocol@temp%
}

% Add to the protocol
\def\pgfsysprotocol@literal#1{%
  \pgfsysprotocol@literalbuffered{#1}%
  \ifpgfsysprotocol@buffered%
  \else%
    \pgfsysprotocol@flushcurrentprotocol%
  \fi%
}

% Getting and setting the current protocol
\def\pgfsysprotocol@getcurrentprotocol#1{%
  \let#1=\pgfsysprotocol@currentprotocol%
}

\def\pgfsysprotocol@setcurrentprotocol#1{%
  \global\let\pgfsysprotocol@currentprotocol=#1%
}


% Invoking the current protocol
\def\pgfsysprotocol@invokecurrentprotocol{%
  \ifx\pgfsysprotocol@currentprotocol\pgfutil@empty%
  \else%
    \expandafter\pgfsys@invoke\expandafter{\pgfsysprotocol@currentprotocol}%
  \fi%
}

\def\pgfsysprotocol@flushcurrentprotocol{%
  \pgfsysprotocol@invokecurrentprotocol%
  \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
}


\endinput


==> pgfsyssoftpath.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/systemlayer/pgfsyssoftpath.code.tex,v 1.5 2007/02/19 13:18:57 tantau Exp $


% This package provides the pgf system path abstraction layer. This
% layer is used to construct paths first ``abstractly.'' These
% abstract paths can still be modified, before they are ``made
% concrete.'' 
%
% An abstract path consists of a sequence of basic building blocks,
% each of which is a tuple consisting of two numbers (specifying a
% coordinate) and a token. Possible tokens are:
%
% 1. moveto
% 2. lineto
% 3. rectcorner
% 4. rectsize
% 5. curvetosupporta
% 6. curvetosupportb
% 7. curveto
% 8. closepath
% 9. specialround
%
% A curveto must always be preceeded by a curvetosupporta and a
% curvetosupportb. A non-empty path must always begin with a
% moveto. The coordinates of a closepath are non-specified, currently, 
% but they might be set to the coordinate of the path segment start,
% in the future.



\let\pgfsyssoftpath@currentpath=\pgfutil@empty
% The current path

\def\pgfsyssoftpath@lastmoveto{{0pt}{0pt}}

\newif\ifpgfsyssoftpathmovetorelevant
\pgfsyssoftpathmovetorelevanttrue

% Add a moveto element to the current path
\def\pgfsyssoftpath@moveto#1#2{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@movetotoken{#1}{#2}%
  }}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfsyssoftpath@currentpath\pgfsyssoftpath@temp%
  \ifpgfsyssoftpathmovetorelevant%
    \xdef\pgfsyssoftpath@lastmoveto{{#1}{#2}}%
  \fi%
}

% Add a lineto element to the current path
\def\pgfsyssoftpath@lineto#1#2{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@linetotoken{#1}{#2}%
  }}%
 \expandafter\pgfutil@g@addto@macro\expandafter\pgfsyssoftpath@currentpath\pgfsyssoftpath@temp%
}

% Add curveto elements to the current path
\def\pgfsyssoftpath@curveto#1#2#3#4#5#6{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@curvetosupportatoken{#1}{#2}%
    \noexpand\pgfsyssoftpath@curvetosupportbtoken{#3}{#4}%
    \noexpand\pgfsyssoftpath@curvetotoken{#5}{#6}%
  }}%
 \expandafter\pgfutil@g@addto@macro\expandafter\pgfsyssoftpath@currentpath\pgfsyssoftpath@temp%
}

% Add rectanlge elements to the current path
\def\pgfsyssoftpath@rect#1#2#3#4{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@rectcornertoken{#1}{#2}%
    \noexpand\pgfsyssoftpath@rectsizetoken{#3}{#4}%
  }}%
 \expandafter\pgfutil@g@addto@macro\expandafter\pgfsyssoftpath@currentpath\pgfsyssoftpath@temp%
}

% Add closepath element to the current path
\def\pgfsyssoftpath@closepath{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@closepathtoken\pgfsyssoftpath@lastmoveto%
  }}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfsyssoftpath@currentpath\pgfsyssoftpath@temp%
}

% Add special element to the current path
\def\pgfsyssoftpath@specialround#1#2{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@specialroundtoken{#1}{#2}%
  }}%
 \expandafter\pgfutil@g@addto@macro\expandafter\pgfsyssoftpath@currentpath\pgfsyssoftpath@temp%
}


% Getting and setting the current path
\def\pgfsyssoftpath@getcurrentpath#1{%
  \let#1=\pgfsyssoftpath@currentpath%
}

\def\pgfsyssoftpath@setcurrentpath#1{%
  \global\let\pgfsyssoftpath@currentpath=#1%
}


% Invoking the current path
\def\pgfsyssoftpath@invokecurrentpath{%
  \pgfsyssoftpath@currentpath%
}

\def\pgfsyssoftpath@flushcurrentpath{%
  \pgfsyssoftpath@invokecurrentpath%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
}

% Marshallers
\def\pgfsyssoftpath@movetotoken#1#2{\pgfsys@moveto{#1}{#2}}
\def\pgfsyssoftpath@linetotoken#1#2{\pgfsys@lineto{#1}{#2}}
\def\pgfsyssoftpath@rectcornertoken#1#2#3#4#5{\pgfsys@rect{#1}{#2}{#4}{#5}} % #3 = \pgfsyssoftpath@rectsizetoken
\def\pgfsyssoftpath@curvetosupportatoken#1#2#3#4#5#6#7#8{\pgfsys@curveto{#1}{#2}{#4}{#5}{#7}{#8}}
\def\pgfsyssoftpath@closepathtoken#1#2{\pgfsys@closepath}
\let\pgfsyssoftpath@specialroundtoken=\pgfutil@gobbletwo


\endinput

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> pgfutil-common.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% 
% This file provides utitiliy commands that are used throughout pgf.
%
% For most commands, the definition of these commands is just given
% below. We cannot use the LaTeX definition of these commands since
% LaTeX may not be the current format and since LaTeX packages tend to
% redefine these commands.
%
% For some commands the actual definition of the format (like latex or
% context) is to be preferred over the generic definition below. In
% this case, the definition of the format is installed when the file
% pgfutil-XXXX.tex is read, where XXXX is the format name (latex,
% plain, or context). 



\catcode`\@=11\relax


% Simple stuff

\long\def\pgfutil@ifundefined#1{%
  \expandafter\ifx\csname#1\endcsname\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}
\def\pgfutil@firstofone#1{#1}
\def\pgfutil@firstoftwo#1#2{#1}
\def\pgfutil@secondoftwo#1#2{#2}
\def\pgfutil@empty{}
\def\pgfutil@gobble#1{}
\def\pgfutil@gobbletwo#1#2{}
\def\pgfutil@namedef#1{\expandafter\def\csname #1\endcsname}
\long\def\pgfutil@g@addto@macro#1#2{%
  \begingroup
    \toks@\expandafter{#1#2}%
    \xdef#1{\the\toks@}%
 \endgroup}
\newif\ifpgfutil@tempswa

% pgfutil@ifnextchar

\long\def\pgfutil@ifnextchar#1#2#3{%
  \let\pgfutil@reserved@d=#1%
  \def\pgfutil@reserved@a{#2}%
  \def\pgfutil@reserved@b{#3}%
  \futurelet\pgfutil@let@token\pgfutil@ifnch}
\def\pgfutil@ifnch{%
  \ifx\pgfutil@let@token\pgfutil@sptoken
    \let\pgfutil@reserved@c\pgfutil@xifnch
  \else
    \ifx\pgfutil@let@token\pgfutil@reserved@d
      \let\pgfutil@reserved@c\pgfutil@reserved@a
    \else
      \let\pgfutil@reserved@c\pgfutil@reserved@b
    \fi
  \fi
  \pgfutil@reserved@c}
{%
  \def\:{\global\let\pgfutil@sptoken= } \:
  \def\:{\pgfutil@xifnch} \expandafter\gdef\: {\futurelet\pgfutil@let@token\pgfutil@ifnch}
}

% pgfutil@in@

\newif\ifpgfutil@in@
\def\pgfutil@in@#1#2{%
 \def\pgfutil@in@@##1#1##2##3\pgfutil@in@@{%
  \ifx\pgfutil@in@##2\pgfutil@in@false\else\pgfutil@in@true\fi}%
 \pgfutil@in@@#2#1\pgfutil@in@\pgfutil@in@@}


% pgfutil@for

\def\pgfutil@nnil{\pgfutil@nil}
\def\pgfutil@fornoop#1\@@#2#3{}
\long\def\pgfutil@for#1:=#2\do#3{%
  \expandafter\def\expandafter\pgfutil@fortmp\expandafter{#2}%
  \ifx\pgfutil@fortmp\pgfutil@empty \else
    \expandafter\pgfutil@forloop#2,\pgfutil@nil,\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\pgfutil@nnil \else
       #5\def#4{#2}\ifx #4\pgfutil@nnil \else#5\pgfutil@iforloop #3\@@#4{#5}\fi\fi}
\long\def\pgfutil@iforloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@iforloop\fi#2\@@#3{#4}}
\def\pgfutil@tfor#1:={\pgfutil@tf@r#1 }
\long\def\pgfutil@tf@r#1#2\do#3{\def\pgfutil@fortmp{#2}\ifx\pgfutil@fortmp\space\else
    \pgfutil@tforloop#2\pgfutil@nil\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@tforloop#1#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@tforloop\fi#2\@@#3{#4}}


% pgfutil@IfFileExists

\chardef\pgfutil@inputcheck0
\def\pgfutil@IfFileExists#1#2#3{%
  \openin\pgfutil@inputcheck#1 %
  \ifeof\pgfutil@inputcheck
     #3\relax
  \else
    #2\relax
  \fi
  \closein\pgfutil@inputcheck}

\def\pgfutil@InputIfFileExists#1#2#3{\pgfutil@IfFileExists{#1}{\input #1\relax#2}{#3}}%


% aux-read-hook

\let\pgfutil@aux@read@hook=\relax


\endinput


==> tikz.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz.code.tex,v 1.87 2007/06/07 07:41:10 tantau Exp $


% Always-present libraries:

\usepgflibrary{plothandlers}


\let\tikz@orig@setkeys=\setkeys        % guard against changes, later
\let\tikz@orig@define@key=\define@key  

\newdimen\tikz@lastx
\newdimen\tikz@lasty
\newdimen\tikz@lastxsaved
\newdimen\tikz@lastysaved

\newdimen\tikzleveldistance
\newdimen\tikzsiblingdistance

\newbox\tikz@figbox
\newbox\tikz@tempbox

\newcount\tikztreelevel
\newcount\tikznumberofchildren
\newcount\tikznumberofcurrentchild

\newcount\tikz@fig@count

\newif\iftikz@node@is@a@label
\newif\iftikz@snaked

\let\tikz@options=\pgfutil@empty
\def\tikz@addoption#1{\expandafter\def\expandafter\tikz@options\expandafter{\tikz@options#1}}
\def\tikz@addmode#1{\expandafter\def\expandafter\tikz@mode\expandafter{\tikz@mode#1}}
\def\tikz@addtransform#1{%
  \ifx\tikz@transform\relax%
    #1%
  \else%
    \expandafter\def\expandafter\tikz@transform\expandafter{\tikz@transform#1}%
  \fi%
}



% TikZ options:

\def\tikzoption{\tikz@orig@define@key{tikz}}



% Baseline options
\tikzoption{baseline}[0pt]{\pgfutil@ifnextchar({\tikz@baseline@coordinate}{\tikz@baseline@simple}#1\@nil}%)
\def\tikz@baseline@simple#1\@nil{\pgfsetbaseline{#1}}
\def\tikz@baseline@coordinate#1\@nil{\pgfsetbaselinepointlater{\tikz@scan@one@point\@firstofone#1}}

% Draw options
\tikzoption{line width}{\tikz@semiaddlinewidth{#1}}%

\def\tikz@semiaddlinewidth#1{\tikz@addoption{\pgfsetlinewidth{#1}}\pgfmathsetlength\pgflinewidth{#1}}

\tikzoption{cap}{\tikz@addoption{\csname pgfset#1cap\endcsname}}
\tikzoption{join}{\tikz@addoption{\csname pgfset#1join\endcsname}}
\tikzoption{miter limit}{\tikz@addoption{\pgfsetmiterlimit{#1}}}

\tikzoption{dash pattern}{% syntax: on 2pt off 3pt on 4pt ...
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \def\tikz@dashpattern{}%
    \tikz@addoption{\pgfsetdash{}{0pt}}%
  \else%
    \def\tikz@dashpattern{}%
    \expandafter\tikz@scandashon\pgfutil@gobble#1o\@nil%
    \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
    \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
  \fi}
\tikzoption{dash phase}{%
  \def\tikz@dashphase{#1}%
  \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
  \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
}%
\def\tikz@dashphase{0pt}

\def\tikz@scandashon n#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashoff}}
\def\tikz@scandashoff ff#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashon}}

\tikzoption{draw opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}}}

% Double draw options
\tikzoption{double}[]{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@doublefalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@double@color{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@doubletrue}%
  \fi}
\tikzoption{double distance}{%
  \pgfmathsetlength{\pgf@x}{#1}%
  \edef\tikz@double@width@distance{\the\pgf@x}%
  \tikz@addmode{\tikz@mode@doubletrue}}

\def\tikz@double@width@distance{0.6pt}
\def\tikz@double@color{white}

% Fill options

\tikzoption{even odd rule}[]{\tikz@addoption{\pgfseteorule}}
\tikzoption{nonzero rule}[]{\tikz@addoption{\pgfsetnonzerorule}}

\tikzoption{fill opacity}{\tikz@addoption{\pgfsetfillopacity{#1}}}


% Joined fill/draw options

\tikzoption{opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}\pgfsetfillopacity{#1}}}


% Main color options
\tikzoption{color}{%
  \tikz@addoption{%
    \ifx\tikz@fillcolor\pgfutil@empty%
      \ifx\tikz@strokecolor\pgfutil@empty%
      \else%
        \pgfsys@color@reset@inorderfalse%
        \let\tikz@strokecolor\pgfutil@empty%
        \let\tikz@fillcolor\pgfutil@empty%
      \fi%
    \else%
      \pgfsys@color@reset@inorderfalse%
      \let\tikz@strokecolor\pgfutil@empty%
      \let\tikz@fillcolor\pgfutil@empty%
    \fi%
    \pgfutil@colorlet{tikz@color}{#1}%
    \pgfutil@colorlet{.}{tikz@color}%
    \pgfsetcolor{.}%
    \pgfsys@color@reset@inordertrue%
  }%
  \def\tikz@textcolor{#1}}



% Rounding options
\tikzoption{rounded corners}[4pt]{\pgfsetcornersarced{\pgfpoint{#1}{#1}}}
\tikzoption{sharp corners}[]{\pgfsetcornersarced{\pgfpointorigin}}



% Coordinate options
\tikzoption{x}{\tikz@handle@vec{\pgfsetxvec}{\tikz@handle@x}#1\relax}
\tikzoption{y}{\tikz@handle@vec{\pgfsetyvec}{\tikz@handle@y}#1\relax}
\tikzoption{z}{\tikz@handle@vec{\pgfsetzvec}{\tikz@handle@z}#1\relax}

\def\tikz@handle@vec#1#2{\pgfutil@ifnextchar({\tikz@handle@coordinate#1}{\tikz@handle@single#2}}
\def\tikz@handle@coordinate#1{\tikz@scan@one@point#1}
\def\tikz@handle@single#1#2\relax{#1{#2}}
\def\tikz@handle@x#1{\pgfsetxvec{\pgfpoint{#1}{0pt}}}
\def\tikz@handle@y#1{\pgfsetyvec{\pgfpoint{0pt}{#1}}}
\def\tikz@handle@z#1{\pgfsetzvec{\pgfpoint{#1}{#1}}}


% Transformation options
\tikzoption{scale}{\tikz@addtransform{\pgftransformscale{#1}}}
\tikzoption{xscale}{\tikz@addtransform{\pgftransformxscale{#1}}}
\tikzoption{xslant}{\tikz@addtransform{\pgftransformxslant{#1}}}
\tikzoption{yscale}{\tikz@addtransform{\pgftransformyscale{#1}}}
\tikzoption{yslant}{\tikz@addtransform{\pgftransformyslant{#1}}}
\tikzoption{rotate}{\tikz@addtransform{\pgftransformrotate{#1}}}
\tikzoption{rotate around}{\tikz@addtransform{\tikz@rotatearound{#1}}}
\def\tikz@rotatearound#1{%
  \edef\tikz@temp{#1}% get rid of active stuff
  \expandafter\tikz@rotateparseA\tikz@temp%
}%
\def\tikz@rotateparseA#1:{%
  \def\tikz@temp@rot{#1}%
  \tikz@scan@one@point\tikz@rotateparseB%
}
\def\tikz@rotateparseB#1{%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \pgftransformrotate{\tikz@temp@rot}%
  \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
}

\tikzoption{shift}{\tikz@addtransform{\tikz@scan@one@point\pgftransformshift#1\relax}}
\tikzoption{xshift}{\tikz@addtransform{\pgftransformxshift{#1}}}
\tikzoption{yshift}{\tikz@addtransform{\pgftransformyshift{#1}}}
\tikzoption{cm}{\tikz@addtransform{\tikz@parse@cm#1\relax}}
\tikzoption{reset cm}[]{\tikz@addtransform{\pgftransformreset}}
\tikzoption{shift only}[]{\tikz@addtransform{\pgftransformresetnontranslations}}

\def\tikz@parse@cm#1,#2,#3,#4,{%
  \def\tikz@p@cm{{#1}{#2}{#3}{#4}}%
  \tikz@scan@one@point\tikz@parse@cmA}
\def\tikz@parse@cmA#1{%
  \expandafter\pgftransformcm\tikz@p@cm{#1}%
}



% Grid options
\tikzoption{xstep}{\def\tikz@grid@x{#1}}
\tikzoption{ystep}{\def\tikz@grid@y{#1}}
\tikzoption{step}{\tikz@handle@vec{\tikz@step@point}{\tikz@step@single}#1\relax}
\def\tikz@step@single#1{\def\tikz@grid@x{#1}\def\tikz@grid@y{#1}}
\def\tikz@step@point#1{\pgf@process{#1}\edef\tikz@grid@x{\the\pgf@x}\edef\tikz@grid@y{\the\pgf@y}}

\def\tikz@grid@x{1cm}
\def\tikz@grid@y{1cm}


% Path usage options
\newif\iftikz@mode@double
\newif\iftikz@mode@fill
\newif\iftikz@mode@draw
\newif\iftikz@mode@clip
\newif\iftikz@mode@boundary
\newif\iftikz@mode@shade
\let\tikz@mode=\pgfutil@empty

\def\tikz@nonetext{none}

\tikzoption{path only}[]{\let\tikz@mode=\pgfutil@empty}
\tikzoption{shade}[]{\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{fill}[]{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillcolor{#1}}%
      \def\tikz@fillcolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
}
\tikzoption{draw}[]{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@drawfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetstrokecolor{#1}}%
      \def\tikz@strokecolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@drawtrue}%
  \fi%
}
\tikzoption{clip}[]{\tikz@addmode{\tikz@mode@cliptrue}}
\tikzoption{use as bounding box}[]{\tikz@addmode{\tikz@mode@boundarytrue}}

\tikzoption{save path}{\tikz@addmode{\pgfsyssoftpath@getcurrentpath#1\global\let#1=#1}}

\let\tikz@fillcolor=\pgfutil@empty
\let\tikz@strokecolor=\pgfutil@empty


% Pattern options
\tikzoption{pattern color}{\def\tikz@pattern@color{#1}}
\tikzoption{pattern}[]{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillpattern{#1}{\tikz@pattern@color}}%
      \def\tikz@pattern{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
}
\def\tikz@pattern@color{black}
\def\tikz@pattern{dots}


% Shading options
\tikzoption{shading}{\def\tikz@shading{#1}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{shading angle}{\def\tikz@shade@angle{#1}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{top color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{bottom color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{middle color}{%
  \pgfutil@colorlet{tikz@axis@middle}{#1}%
  \def\tikz@shading{axis}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{left color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{right color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{ball color}{\pgfutil@colorlet{tikz@ball}{#1}\def\tikz@shading{ball}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{inner color}{\pgfutil@colorlet{tikz@radial@inner}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{outer color}{\pgfutil@colorlet{tikz@radial@outer}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}

\def\tikz@shading{axis}
\def\tikz@shade@angle{0}

\pgfdeclareverticalshading[tikz@axis@top,tikz@axis@middle,tikz@axis@bottom]{axis}{100bp}{%
  color(0bp)=(tikz@axis@bottom);
  color(25bp)=(tikz@axis@bottom);
  color(50bp)=(tikz@axis@middle);
  color(75bp)=(tikz@axis@top);
  color(100bp)=(tikz@axis@top)}

\pgfutil@colorlet{tikz@axis@top}{gray}
\pgfutil@colorlet{tikz@axis@middle}{gray!50!white}
\pgfutil@colorlet{tikz@axis@bottom}{white}

\pgfdeclareradialshading[tikz@ball]{ball}{\pgfqpoint{-10bp}{10bp}}{%
 color(0bp)=(tikz@ball!15!white);
 color(9bp)=(tikz@ball!75!white);
 color(18bp)=(tikz@ball!70!black);
 color(25bp)=(tikz@ball!50!black);
 color(50bp)=(black)}

\pgfutil@colorlet{tikz@ball}{blue}

\pgfdeclareradialshading[tikz@radial@inner,tikz@radial@outer]{radial}{\pgfpointorigin}{%
 color(0bp)=(tikz@radial@inner);
 color(25bp)=(tikz@radial@outer);
 color(50bp)=(tikz@radial@outer)}

\pgfutil@colorlet{tikz@radial@inner}{gray}
\pgfutil@colorlet{tikz@radial@outer}{white}


% Pin options
\tikzoption{pin}{\pgfutil@ifnextchar[{\tikz@parse@pin}{\tikz@parse@pin[]}#1\pgf@nil}
\tikzoption{pin distance}{\def\tikz@pin@distance{#1}}
\tikzoption{pin edge}{\def\tikz@pin@edge@style{#1}}

\tikzoption{tikz@pin@post}[]{%
  \tikz@compute@direction{\tikz@label@angle}{\tikz@pin@distance}%
  \global\let\tikz@pin@edge@style@smuggle=\tikz@pin@edge@style%
}
\tikzoption{tikz@pre@pin@edge}[]{\def\pgf@marshal{\tikzstyle{tikz@pin@options}=}
  \expandafter\pgf@marshal\expandafter[\tikz@pin@edge@style@smuggle]%
}

\def\tikz@pin@distance{3ex}
\def\tikz@pin@edge@style{}

\def\tikz@parse@pin[#1]#2:#3\pgf@nil{%
  \tikz@add@after@node@path{\bgroup
    \pgfextra{\let\tikz@save@last@node=\tikzlastnode}%
    node
    [every pin,tikz@label@angle=#2,#1,at=(\tikzlastnode.\tikz@label@angle),%
    after node path={(\tikz@save@last@node) edge[every pin edge,tikz@pre@pin@edge,tikz@pin@options] (\tikzlastnode)},
    tikz@pin@post]
    {#3} \egroup}
}


% Label and pin options

\tikzoption{label}{\pgfutil@ifnextchar[{\tikz@parse@label}{\tikz@parse@label[]}#1\pgf@nil}
\tikzoption{label distance}{\def\tikz@label@distance{#1}}

\tikzoption{tikz@label@angle}{\def\tikz@label@angle{#1}\csname tikz@label@angle@is@#1\endcsname}

\tikzoption{tikz@label@post}[]{\tikz@compute@direction{\tikz@label@angle}{\tikz@label@distance}}

\def\tikz@label@distance{0pt}

\def\tikz@parse@label[#1]#2:#3\pgf@nil{%
  \tikz@add@after@node@path{
    \bgroup
    \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name}%
    node
    [every label,%
    tikz@label@angle=#2,%
    #1,%
    at=(\tikzlastnode.\tikz@label@angle),tikz@label@post]%
    {#3}%
    \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}%
    \egroup%
  }
}

\expandafter\def\csname tikz@label@angle@is@right\endcsname{\def\tikz@label@angle{0}}
\expandafter\def\csname tikz@label@angle@is@above right\endcsname{\def\tikz@label@angle{45}}
\expandafter\def\csname tikz@label@angle@is@above\endcsname{\def\tikz@label@angle{90}}
\expandafter\def\csname tikz@label@angle@is@above left\endcsname{\def\tikz@label@angle{135}}
\expandafter\def\csname tikz@label@angle@is@left\endcsname{\def\tikz@label@angle{180}}
\expandafter\def\csname tikz@label@angle@is@below left\endcsname{\def\tikz@label@angle{225}}
\expandafter\def\csname tikz@label@angle@is@below\endcsname{\def\tikz@label@angle{270}}
\expandafter\def\csname tikz@label@angle@is@below right\endcsname{\def\tikz@label@angle{315}}

\def\tikz@compute@direction#1#2{%
  \let\tikz@do@auto@anchor=\relax
  \c@pgf@counta=#1\relax%
  \ifnum\c@pgf@counta<0\relax
    \advance\c@pgf@counta by 360\relax%
  \fi%
  \ifnum\c@pgf@counta>359\relax
    \advance\c@pgf@counta by-360\relax%
  \fi%
  \ifnum\c@pgf@counta<4\relax%
    \def\tikz@anchor{west}%
  \else\ifnum\c@pgf@counta<87\relax%
    \def\tikz@anchor{south west}%
  \else\ifnum\c@pgf@counta<94\relax%
    \def\tikz@anchor{south}%
  \else\ifnum\c@pgf@counta<177\relax%
    \def\tikz@anchor{south east}%
  \else\ifnum\c@pgf@counta<184\relax%
    \def\tikz@anchor{east}%
  \else\ifnum\c@pgf@counta<267\relax%
    \def\tikz@anchor{north east}%
  \else\ifnum\c@pgf@counta<274\relax%
    \def\tikz@anchor{north}%
  \else\ifnum\c@pgf@counta<357\relax%
    \def\tikz@anchor{north west}%
  \else%
    \def\tikz@anchor{west}%
  \fi\fi\fi\fi\fi\fi\fi\fi%
  \tikz@addtransform{\pgftransformshift{\pgfpointpolar{#1}{#2}}}%  
}



% General shape options
\tikzoption{name}{\edef\tikz@fig@name{#1}}

\tikzoption{at}{\tikz@scan@one@point\tikz@set@at#1}
\def\tikz@set@at#1{\def\tikz@node@at{#1}}%

\tikzoption{shape}{\edef\tikz@shape{#1}}

\tikzoption{nodes}{\tikzstyle{every node}+=[#1]}

\tikzoption{inner sep}{\def\pgfshapeinnerxsep{#1}\def\pgfshapeinnerysep{#1}}
\tikzoption{inner xsep}{\def\pgfshapeinnerxsep{#1}}
\tikzoption{inner ysep}{\def\pgfshapeinnerysep{#1}}

\tikzoption{outer sep}{\def\pgfshapeouterxsep{#1}\def\pgfshapeouterysep{#1}}
\tikzoption{outer xsep}{\def\pgfshapeouterxsep{#1}}
\tikzoption{outer ysep}{\def\pgfshapeouterysep{#1}}

\tikzoption{minimum width}{\def\pgfshapeminwidth{#1}}
\tikzoption{minimum height}{\def\pgfshapeminheight{#1}}
\tikzoption{minimum size}{\def\pgfshapeminwidth{#1}\def\pgfshapeminheight{#1}}

\tikzoption{aspect}{\pgfsetshapeaspect{#1}}

\tikzoption{after node path}{\tikz@add@after@node@path{#1}}%
\def\tikz@add@after@node@path#1{\expandafter\def\expandafter\tikz@after@node\expandafter{\tikz@after@node#1}}

\def\tikzaddafternodepathoption#1{%
  #1%
  \expandafter\def\expandafter\tikz@afternodepathoptions\expandafter{\tikz@afternodepathoptions#1}}

\let\tikz@afternodepathoptions=\pgfutil@empty

\tikzoption{anchor}{\def\tikz@anchor{#1}\let\tikz@do@auto@anchor=\relax}

\tikzoption{left}[]{\def\tikz@anchor{east}\tikz@possibly@transform{x}{-}{#1}}
\tikzoption{right}[]{\def\tikz@anchor{west}\tikz@possibly@transform{x}{}{#1}}
\tikzoption{above}[]{\def\tikz@anchor{south}\tikz@possibly@transform{y}{}{#1}}
\tikzoption{below}[]{\def\tikz@anchor{north}\tikz@possibly@transform{y}{-}{#1}}
\tikzoption{above left}[]%
  {\def\tikz@anchor{south east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{}{#1}}
\tikzoption{above right}[]%
  {\def\tikz@anchor{south west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{}{#1}}
\tikzoption{below left}[]%
  {\def\tikz@anchor{north east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{-}{#1}}
\tikzoption{below right}[]%
  {\def\tikz@anchor{north west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{-}{#1}}

\tikzoption{node distance}{\def\tikz@node@distance{#1}}
\def\tikz@node@distance{1cm}

\tikzoption{above of}{\tikz@of{#1}{90}}%
\tikzoption{below of}{\tikz@of{#1}{-90}}%
\tikzoption{left of}{\tikz@of{#1}{180}}%
\tikzoption{right of}{\tikz@of{#1}{0}}%
\tikzoption{above left of}{\tikz@of{#1}{135}}%
\tikzoption{below left of}{\tikz@of{#1}{-135}}%
\tikzoption{above right of}{\tikz@of{#1}{45}}%
\tikzoption{below right of}{\tikz@of{#1}{-45}}%

\def\tikz@of#1#2{%
  \def\tikz@anchor{center}%
  \let\tikz@do@auto@anchor=\relax%
  \tikz@addtransform{\pgftransformshift{\pgfpointpolar{#2}{\tikz@node@distance}}}%
  \def\tikz@node@at{\pgfpointanchor{#1}{center}}}
  
\tikzoption{transform shape}[true]{%
  \csname tikz@fullytransformed#1\endcsname%
  \iftikz@fullytransformed%
    \pgfresetnontranslationattimefalse%
  \else%
    \pgfresetnontranslationattimetrue%
  \fi%
}

\newif\iftikz@fullytransformed
\pgfresetnontranslationattimetrue%

\def\tikz@anchor{center}%
\def\tikz@shape{rectangle}%

\def\tikz@possibly@transform#1#2#3{%
  \let\tikz@do@auto@anchor=\relax%
  \def\tikz@test{#3}%
  \ifx\tikz@test\pgfutil@empty%
  \else%
    \pgfmathsetlength{\pgf@x}{#3}%
    \pgf@x=#2\pgf@x\relax%
    \edef\tikz@marshal{\noexpand\tikz@addtransform{%
        \expandafter\noexpand\csname  pgftransform#1shift\endcsname{\the\pgf@x}}}% 
    \tikz@marshal%
  \fi%
}


% Inter-picture options
\tikzoption{remember picture}[true]{\csname pgfrememberpicturepositiononpage#1\endcsname}
\tikzoption{overlay}[]{\pgf@relevantforpicturesizefalse}



% Line/curve label placement options
\tikzoption{sloped}[true]{\csname pgfslopedattime#1\endcsname}
\tikzoption{allow upside down}[true]{\csname pgfallowupsidedownattime#1\endcsname}

\tikzoption{pos}{\edef\tikz@time{#1}}

\tikzoption{auto}[]{\csname tikz@install@auto@anchor@#1\endcsname}
\tikzoption{swap}[]{%
  \def\tikz@temp{left}%
  \ifx\tikz@auto@anchor@direction\tikz@temp%
    \def\tikz@auto@anchor@direction{right}%
  \else%
    \def\tikz@auto@anchor@direction{left}%
  \fi%
}

\def\tikz@time{.5}

\def\tikz@install@auto@anchor@{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on}
\def\tikz@install@auto@anchor@false{\let\tikz@do@auto@anchor=\relax}
\def\tikz@install@auto@anchor@left{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{left}}
\def\tikz@install@auto@anchor@right{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{right}}

\let\tikz@do@auto@anchor=\relax%

\def\tikz@auto@anchor@on{\csname tikz@auto@anchor@\tikz@auto@anchor@direction\endcsname}

\def\tikz@auto@anchor@left{\tikz@auto@pre\tikz@auto@anchor\tikz@auto@post}
\def\tikz@auto@anchor@right{\tikz@auto@pre\tikz@auto@anchor@prime\tikz@auto@post}

\def\tikz@auto@anchor@direction{left}

% Text options
\tikzoption{text}{\def\tikz@textcolor{#1}}
\tikzoption{font}{\def\tikz@textfont{#1}}
\tikzoption{text opacity}{\def\tikz@textopacity{#1}}
\tikzoption{text width}{\def\tikz@text@width{#1}}
\tikzoption{text height}{\def\tikz@text@height{#1}}
\tikzoption{text depth}{\def\tikz@text@depth{#1}}
\tikzoption{text ragged}[]%
{\def\tikz@text@action{\raggedright\rightskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}}
\tikzoption{text badly ragged}[]{\def\tikz@text@action{\raggedright\relax}}
\tikzoption{text ragged left}[]%
{\def\tikz@text@action{\raggedleft\leftskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}}
\tikzoption{text badly ragged left}[]{\def\tikz@text@action{\raggedleft\relax}}
\tikzoption{text justified}[]{\def\tikz@text@action{\leftskip\z@\rightskip\z@\relax}}
\tikzoption{text centered}[]{\def\tikz@text@action{%
  \leftskip\z@ plus2em%
  \rightskip\z@ plus2em%
  \spaceskip.3333em \xspaceskip.5em%
  \parfillskip=0pt%
  \let\\=\@centercr% for latex
  \relax}}
\tikzoption{text badly centered}[]%
{\def\tikz@text@action{%
  \let\\=\@centercr% for latex
  \parfillskip=0pt%
  \rightskip\@flushglue%
  \leftskip\@flushglue\relax}}

\let\tikz@text@width=\pgfutil@empty
\let\tikz@text@height=\pgfutil@empty
\let\tikz@text@depth=\pgfutil@empty
\let\tikz@textcolor=\pgfutil@empty
\let\tikz@textfont=\pgfutil@empty
\let\tikz@textopacity=\pgfutil@empty

\def\tikz@text@action{\raggedright\rightskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}





% Arrow options
\tikzoption{arrows}{\tikz@processarrows{#1}}

\tikzoption{>}{%
  \tikz@set@pointed{\csname pgf@arrows@invert#1\endcsname}{#1}%
  \expandafter\tikz@processarrows\expandafter{\tikz@current@arrows}%
}

\tikzoption{shorten <}{\pgfsetshortenstart{#1}}
\tikzoption{shorten >}{\pgfsetshortenend{#1}}

\def\tikz@set@pointed#1#2{%
  \pgfutil@ifundefined{pgf@arrow@code@tikze@>@#2}
  {%
    \pgfarrowsdeclarealias{tikzs@<@#2}{tikze@>@#2}{#1}{#2}%
    \pgfarrowsdeclarereversed{tikzs@>@#2}{tikze@<@#2}{#1}{#2}%
    \pgfarrowsdeclarecombine*{tikz@|<@#2}{tikz@>|@#2}{#1}{#2}{|}{|}%
    \pgfarrowsdeclaredouble[\pgflinewidth]{tikzs@<<@#2}{tikze@>>@#2}{#1}{#2}%
    \pgfarrowsdeclarereversed{tikzs@>>@#2}{tikze@<<@#2}{tikzs@<<@#2}{tikze@>>@#2}%
  }{}%
  \pgfutil@namedef{tikz@special@arrow@start<}{tikzs@<@#2}%
  \pgfutil@namedef{tikz@special@arrow@end>}{tikze@>@#2}%
  \pgfutil@namedef{tikz@special@arrow@start>}{tikzs@>@#2}%
  \pgfutil@namedef{tikz@special@arrow@end<}{tikze@<@#2}%
  \pgfutil@namedef{tikz@special@arrow@start|<}{tikz@|<@#2}%
  \pgfutil@namedef{tikz@special@arrow@end>|}{tikz@>|@#2}%
  \pgfutil@namedef{tikz@special@arrow@start<<}{tikzs@<<@#2}%
  \pgfutil@namedef{tikz@special@arrow@end>>}{tikze@>>@#2}%
  \pgfutil@namedef{tikz@special@arrow@start>>}{tikzs@<<@#2}%
  \pgfutil@namedef{tikz@special@arrow@end<<}{tikze@>>@#2}%
}

\def\tikz@processarrows#1{%
  \def\tikz@current@arrows{#1}%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else%
    \tikz@@processarrows#1\@nil
  \fi%
}
\def\tikz@@processarrows#1-#2\@nil{%
  \expandafter\ifx\csname tikz@special@arrow@start#1\endcsname\relax%
    \pgfsetarrowsstart{#1}
  \else%
    \pgfsetarrowsstart{\csname tikz@special@arrow@start#1\endcsname}%
  \fi%
  \expandafter\ifx\csname tikz@special@arrow@end#2\endcsname\relax%
    \pgfsetarrowsend{#2}
  \else%
    \pgfsetarrowsend{\csname tikz@special@arrow@end#2\endcsname}%
  \fi%
}

\tikz@set@pointed{\pgf@arrows@invertto}{to}
\def\tikz@current@arrows{-}

% Parabola options
\tikzoption{bend}{\tikz@scan@one@point\tikz@set@parabola@bend#1\relax}%
\tikzoption{bend pos}{\def\tikz@parabola@bend@factor{#1}}
\tikzoption{parabola height}{%
  \def\tikz@parabola@bend@factor{.5}%
  \def\tikz@parabola@bend{\pgfpointadd{\pgfpoint{0pt}{#1}}{\tikz@last@position@saved}}}

\def\tikz@parabola@bend{\tikz@last@position@saved}
\def\tikz@parabola@bend@factor{0}

\def\tikz@set@parabola@bend#1{\def\tikz@parabola@bend{#1}}

% Axis options
\tikzoption{domain}{\def\tikz@plot@domain{#1}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}
\tikzoption{range}{\def\tikz@plot@range{#1}}

% Plot options
\tikzoption{smooth}[]{\let\tikz@plot@handler=\pgfplothandlercurveto}
\tikzoption{smooth cycle}[]{\let\tikz@plot@handler=\pgfplothandlerclosedcurve}
\tikzoption{sharp plot}[]{\let\tikz@plot@handler\pgfplothandlerlineto}

\tikzoption{tension}{\pgfsetplottension{#1}}

\tikzoption{xcomb}[]{\let\tikz@plot@handler=\pgfplothandlerxcomb}
\tikzoption{ycomb}[]{\let\tikz@plot@handler=\pgfplothandlerycomb}
\tikzoption{polar comb}[]{\let\tikz@plot@handler=\pgfplothandlerpolarcomb}

\tikzoption{raw gnuplot}[true]{\csname tikz@plot@raw@gnuplot#1\endcsname}
\tikzoption{prefix}{\def\tikz@plot@prefix{#1}}
\tikzoption{id}{\def\tikz@plot@id{#1}}

\tikzoption{samples}{\def\tikz@plot@samples{#1}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}
\tikzoption{samples at}{\def\tikz@plot@samplesat{#1}}
\tikzoption{parametric}[true]{\csname tikz@plot@parametric#1\endcsname}

\tikzoption{variable}{\def\tikz@plot@var{#1}}

\tikzoption{only marks}[]{\let\tikz@plot@handler\pgfplothandlerdiscard}

\tikzoption{mark}{\def\tikz@plot@mark{#1}}
\tikzoption{mark options}{\def\tikz@plot@mark@options{#1}}
\tikzoption{mark size}{\pgfsetplotmarksize{#1}}

\tikzoption{mark indices}{\def\tikz@mark@list{#1}}
\tikzoption{mark phase}{\pgfsetplotmarkphase{#1}}
\tikzoption{mark repeat}{\pgfsetplotmarkrepeat{#1}}

\let\tikz@mark@list=\pgfutil@empty

\let\tikz@plot@mark@options=\pgfutil@empty

\let\tikz@plot@handler=\pgfplothandlerlineto
\let\tikz@plot@mark=\pgfutil@empty

\def\tikz@plot@samples{25}
\def\tikz@plot@domain{-5:5}
\def\tikz@plot@var{\x}
\def\tikz@plot@samplesat{-5,-4.6,...,5}
\def\tikz@plot@samples@recalc#1:#2\relax{%
  \pgfmathparse{#1}%
  \let\tikz@temp@start=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\tikz@temp@end=\pgfmathresult%
  \pgfmathparse{\tikz@temp@start+(\tikz@temp@end-\tikz@temp@start)/\tikz@plot@samples}%
  \edef\tikz@plot@samplesat{\tikz@temp@start,\pgfmathresult,...,\tikz@temp@end}%
}


\def\tikz@plot@prefix{\jobname.}
\def\tikz@plot@id{pgf-plot}

\newif\iftikz@plot@parametric
\newif\iftikz@plot@raw@gnuplot


% To options
\tikzoption{to path}{\def\tikz@to@path{#1}}

\def\tikz@to@path{-- (\tikztotarget) \tikztonodes}



% Tree options
\tikzoption{edge from parent path}{\def\tikz@edge@to@parent@path{#1}}

\tikzoption{parent anchor}{\def\tikzparentanchor{.#1}\ifx\tikzparentanchor\tikz@border@text\let\tikzparentanchor\pgfutil@empty\fi}
\tikzoption{child anchor}{\def\tikzchildanchor{.#1}\ifx\tikzchildanchor\tikz@border@text\let\tikzchildanchor\pgfutil@empty\fi}

\tikzoption{level distance}{\pgfmathsetlength\tikzleveldistance{#1}}
\tikzoption{sibling distance}{\pgfmathsetlength\tikzsiblingdistance{#1}}

\tikzoption{growth function}{\let\tikz@grow=#1}
\tikzoption{growth parent anchor}{\def\tikz@growth@anchor{#1}}
\tikzoption{grow}{\tikz@set@growth{#1}\edef\tikz@special@level{\the\tikztreelevel}}%
\tikzoption{grow'}{\tikz@set@growth{#1}\tikz@swap@growth\edef\tikz@special@level{\the\tikztreelevel}}%

\def\tikz@growth@anchor{center}

\def\tikz@special@level{-1}% never

\def\tikz@swap@growth{%
  % Swap left and right
  \let\tikz@temp=\tikz@angle@grow@right%
  \let\tikz@angle@grow@right=\tikz@angle@grow@left%
  \let\tikz@angle@grow@left=\tikz@temp%
}%

\def\tikz@set@growth#1{%
  \let\tikz@grow=\tikz@grow@direction%
  \expandafter\ifx\csname tikz@grow@direction@#1\endcsname\relax%
    \c@pgf@counta=#1\relax%
  \else%
    \c@pgf@counta=\csname tikz@grow@direction@#1\endcsname%
  \fi%
  \edef\tikz@angle@grow{\the\c@pgf@counta}%
  \advance\c@pgf@counta by-90\relax%
  \edef\tikz@angle@grow@left{\the\c@pgf@counta}%
  \advance\c@pgf@counta by180\relax%
  \edef\tikz@angle@grow@right{\the\c@pgf@counta}%
}

\def\tikz@border@text{.border}
\let\tikzparentanchor=\pgfutil@empty
\let\tikzchildanchor=\pgfutil@empty
\def\tikz@edge@to@parent@path{(\tikzparentnode\tikzparentanchor) -- (\tikzchildnode\tikzchildanchor)}

\tikzleveldistance=15mm
\tikzsiblingdistance=15mm

\def\tikz@grow@direction@down{-90}
\def\tikz@grow@direction@up{90}
\def\tikz@grow@direction@left{180}
\def\tikz@grow@direction@right{0}

\def\tikz@grow@direction@south{-90}
\def\tikz@grow@direction@north{90}
\def\tikz@grow@direction@west{180}
\def\tikz@grow@direction@east{0}

\expandafter\def\csname tikz@grow@direction@north east\endcsname{45}
\expandafter\def\csname tikz@grow@direction@north west\endcsname{135}
\expandafter\def\csname tikz@grow@direction@south east\endcsname{-45}
\expandafter\def\csname tikz@grow@direction@south west\endcsname{-135}

\def\tikz@grow@direction{%
  \pgftransformshift{\pgfpointpolar{\tikz@angle@grow}{\tikzleveldistance}}%
  \ifnum\tikztreelevel=\tikz@special@level%
  \else%
    \pgf@xc=.5\tikzsiblingdistance%
    \c@pgf@counta=\tikznumberofchildren%
    \advance\c@pgf@counta by1\relax%
    \pgfutil@tempdima=\c@pgf@counta\pgf@xc%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@left}{\pgfutil@tempdima}}%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@right}{\tikznumberofcurrentchild\tikzsiblingdistance}}%
  \fi%
}

\tikz@orig@setkeys{tikz}{grow=down}




% Snake options
\tikzoption{snake}[]{%
  \def\tikz@@snake{#1}%
  \ifx\tikz@@snake\pgfutil@empty%
    \tikz@snakedtrue%
  \else%
    \ifx\tikz@@snake\tikz@nonetext%
      \tikz@snakedfalse%
    \else%
      \tikz@snakedtrue%
      \let\tikz@snake=\tikz@@snake%
    \fi%
  \fi}

\tikzoption{segment amplitude}{\pgfmathsetlength{\pgfsnakesegmentamplitude}{#1}}
\tikzoption{segment length}{\pgfmathsetlength{\pgfsnakesegmentlength}{#1}}
\tikzoption{segment angle}{\pgfmathparse{#1}\let\pgfsnakesegmentangle=\pgfmathresult}
\tikzoption{segment aspect}{\pgfmathparse{#1}\let\pgfsnakesegmentaspect=\pgfmathresult}

\tikzoption{segment object length}{\pgfmathparse{#1}\edef\pgfsnakesegmentobjectlength{\pgfmathresult pt}}

\tikzoption{raise snake}{\def\pgf@snake@raise{\pgftransformyshift{#1}}}
\tikzoption{mirror snake}[true]{%
  \csname if#1\endcsname
    \def\pgf@snake@mirror{\pgftransformyscale{-1}}%
  \else%
    \let\pgf@snake@mirror=\pgfutil@empty%
  \fi
}

\tikzoption{gap before snake}{\def\tikz@presnake{{moveto}{#1}}}
\tikzoption{line before snake}{\def\tikz@presnake{{lineto}{#1}}}

\tikzoption{gap after snake}{\def\tikz@postsnake{{moveto}{#1}}\def\tikz@mainsnakelength{\pgfsnakeremainingdistance+-#1}}
\tikzoption{line after snake}{\def\tikz@postsnake{{lineto}{#1}}\def\tikz@mainsnakelength{\pgfsnakeremainingdistance+-#1}}

\tikzoption{gap around snake}{%
  \def\tikz@presnake{{moveto}{#1}}%
  \def\tikz@postsnake{{moveto}{#1}}%
  \def\tikz@mainsnakelength{\pgfsnakeremainingdistance+-#1}%
}
\tikzoption{line around snake}{%
  \def\tikz@presnake{{lineto}{#1}}%
  \def\tikz@postsnake{{lineto}{#1}}%
  \def\tikz@mainsnakelength{\pgfsnakeremainingdistance+-#1}%
}
\let\pgf@snake@mirror=\pgfutil@empty
\let\pgf@snake@raise=\pgfutil@empty

\pgfsetsnakesegmenttransformation{\pgf@snake@mirror\pgf@snake@raise}

\def\tikz@snake{zigzag}

\let\tikz@presnake=\pgfutil@empty
\let\tikz@postsnake=\pgfutil@empty
\def\tikz@mainsnakelength{\pgfsnakeremainingdistance}


% Matrix options
\tikzoption{matrix}[true]{\csname tikz@is@matrix#1\endcsname}

\tikzoption{matrix anchor}{\def\tikz@matrix@anchor{#1}}

\tikzoption{column sep}{\def\pgfmatrixcolumnsep{#1}}
\tikzoption{row sep}{\def\pgfmatrixrowsep{#1}}

\tikzoption{cells}{\tikzstyle{every cell}+=[#1]}

\tikzoption{ampersand replacement}{\def\tikz@ampersand@replacement{#1}}

\newif\iftikz@is@matrix
\let\tikz@matrix@anchor=\pgfutil@empty
\let\tikz@ampersand@replacement=\pgfutil@empty

% Execute option

\tikzoption{execute at begin picture}{\expandafter\def\expandafter\tikz@atbegin@picture\expandafter{\tikz@atbegin@picture#1}}
\tikzoption{execute at end picture}{\expandafter\def\expandafter\tikz@atend@picture\expandafter{\tikz@atend@picture#1}}
\tikzoption{execute at begin scope}{\expandafter\def\expandafter\tikz@atbegin@scope\expandafter{\tikz@atbegin@scope#1}}
\tikzoption{execute at end scope}{\expandafter\def\expandafter\tikz@atend@scope\expandafter{\tikz@atend@scope#1}}
\tikzoption{execute at begin to}{\expandafter\def\expandafter\tikz@atbegin@to\expandafter{\tikz@atbegin@to#1}}
\tikzoption{execute at end to}{\expandafter\def\expandafter\tikz@atend@to\expandafter{\tikz@atend@to#1}}
\tikzoption{execute at begin node}{\expandafter\def\expandafter\tikz@atbegin@node\expandafter{\tikz@atbegin@node#1}}
\tikzoption{execute at end node}{\expandafter\def\expandafter\tikz@atend@node\expandafter{\tikz@atend@node#1}}
\tikzoption{execute at begin cell}{\expandafter\def\expandafter\tikz@atbegin@cell\expandafter{\tikz@atbegin@cell#1}}
\tikzoption{execute at end cell}{\expandafter\def\expandafter\tikz@atend@cell\expandafter{\tikz@atend@cell#1}}
\tikzoption{execute at empty cell}{\expandafter\def\expandafter\tikz@at@emptycell\expandafter{\tikz@at@emptycell#1}}

\let\tikz@atbegin@picture=\pgfutil@empty
\let\tikz@atend@picture=\pgfutil@empty
\let\tikz@atbegin@scope=\pgfutil@empty
\let\tikz@atend@scope=\pgfutil@empty
\let\tikz@atbegin@to=\pgfutil@empty
\let\tikz@atend@to=\pgfutil@empty
\let\tikz@atbegin@node=\pgfutil@empty
\let\tikz@atend@node=\pgfutil@empty
\let\tikz@atbegin@cell=\pgfutil@empty
\let\tikz@atend@cell=\pgfutil@empty
\let\tikz@at@emptycell=\pgfutil@empty




% Styles
\tikzoption{set style}{\tikzstyle#1}

% Handled in a special way.
\def\tikzstyle{\pgfutil@ifnextchar\bgroup\tikz@style@parseA\tikz@style@parseB}
\def\tikz@style@parseB#1={\tikz@style@parseA{#1}=}
\def\tikz@style@parseA#1#2=#3[#4]{% #2 and #3 are dummy
  \pgfutil@in@+{#2}%
  \ifpgfutil@in@%
    \tikz@style{#1}{#4}%
  \else%
    \expandafter\def\csname tikz@st@#1\endcsname{#4}%
  \fi}
\def\tikz@style#1#2{%
  \iftikzstyleempty{#1}
  {\expandafter\def\csname tikz@st@#1\endcsname{#2}}%
  {%
    \edef\tikz@marshal{\def\expandafter\noexpand\csname tikz@st@#1\endcsname}%
    \expandafter\expandafter\expandafter\tikz@marshal\expandafter\expandafter\expandafter{\csname
      tikz@st@#1\endcsname,#2}%
  }%
}

\def\iftikzstyleempty#1#2#3{%
  \expandafter\ifx\csname tikz@st@#1\endcsname\pgfutil@empty%
    \let\pgf@next=\pgfutil@firstoftwo%
  \else%
    \expandafter\ifx\csname tikz@st@#1\endcsname\relax%
      \let\pgf@next=\pgfutil@firstoftwo%
    \else
      \let\pgf@next=\pgfutil@secondoftwo%
    \fi%
  \fi%
  \pgf@next{#2}{#3}}


%
%
% Predefined styles
%
%

\tikzstyle{help lines}=              [color=gray,line width=0.2pt]

\tikzstyle{every picture}=           []
\tikzstyle{every path}=              []
\tikzstyle{every scope}=             []
\tikzstyle{every plot}=              []
\tikzstyle{every node}=              []
\tikzstyle{every child}=             []
\tikzstyle{every child node}=        []
\tikzstyle{every to}=                []
\tikzstyle{every cell}=              []
\tikzstyle{every matrix}=            []
\tikzstyle{every edge}=              [draw]
\tikzstyle{every label}=             [draw=none,fill=none]
\tikzstyle{every pin}=               [draw=none,fill=none]
\tikzstyle{every pin edge}=          [help lines]

\tikzstyle{ultra thin}=              [line width=0.1pt]
\tikzstyle{very thin}=               [line width=0.2pt]
\tikzstyle{thin}=                    [line width=0.4pt]
\tikzstyle{semithick}=               [line width=0.6pt]
\tikzstyle{thick}=                   [line width=0.8pt]
\tikzstyle{very thick}=              [line width=1.2pt]
\tikzstyle{ultra thick}=             [line width=1.6pt]

\tikzstyle{solid}=                   [dash pattern=]
\tikzstyle{dotted}=                  [dash pattern=on \pgflinewidth off 2pt]
\tikzstyle{densely dotted}=          [dash pattern=on \pgflinewidth off 1pt]
\tikzstyle{loosely dotted}=          [dash pattern=on \pgflinewidth off 4pt]
\tikzstyle{dashed}=                  [dash pattern=on 3pt off 3pt]
\tikzstyle{densely dashed}=          [dash pattern=on 3pt off 2pt]
\tikzstyle{loosely dashed}=          [dash pattern=on 3pt off 6pt]

\tikzstyle{transparent}=             [opacity=0]
\tikzstyle{ultra nearly transparent}=[opacity=0.05]
\tikzstyle{very nearly transparent}= [opacity=0.1]
\tikzstyle{nearly transparent}=      [opacity=0.25]
\tikzstyle{semitransparent}=         [opacity=0.5]
\tikzstyle{nearly opaque}=           [opacity=0.75]
\tikzstyle{very nearly opaque}=      [opacity=0.9]
\tikzstyle{ultra nearly opaque}=     [opacity=0.95]
\tikzstyle{opaque}=                  [opacity=1]

\tikzstyle{at start}=                [pos=0]
\tikzstyle{very near start}=         [pos=0.125]
\tikzstyle{near start}=              [pos=0.25]
\tikzstyle{midway}=                  [pos=0.5]
\tikzstyle{near end}=                [pos=0.75]
\tikzstyle{very near end}=           [pos=0.875]
\tikzstyle{at end}=                  [pos=1]

\tikzstyle{bend at start}=           [bend pos=0,bend={+(0,0)}]
\tikzstyle{bend at end}=             [bend pos=1,bend={+(0,0)}]

\tikzstyle{edge from parent}=        [draw]

\tikzstyle{snake triangles 45}=      [snake=triangles,segment object length=2.41421356\pgfsnakesegmentamplitude]
\tikzstyle{snake triangles 60}=      [snake=triangles,segment object length=1.73205081\pgfsnakesegmentamplitude]
\tikzstyle{snake triangles 90}=      [snake=triangles,segment object length=\pgfsnakesegmentamplitude]


%
% Setting keys
%

\let\tikz@late@keys=\pgfutil@empty%

\def\tikz@set@one@key#1{%
  \tikz@orig@setkeys*{tikz}{#1}%
  \ifx\XKV@rm\pgfutil@empty%
    % fine
  \else%
    \expandafter\pgfutil@in@\expandafter!\expandafter{\XKV@rm}%
    \ifpgfutil@in@%
      % this is a color!
      \expandafter\tikz@addoption\expandafter{\expandafter\pgfutil@color\expandafter{\XKV@rm}}%
      \edef\tikz@textcolor{\XKV@rm}%
    \else%
      \pgfutil@doifcolorelse{\XKV@rm}
      { %     
        \expandafter\tikz@addoption\expandafter{\expandafter\pgfutil@color\expandafter{\XKV@rm}}%
        \edef\tikz@textcolor{\XKV@rm}%
      }%
      {%
        % Ok, second chance: This might be an arrow specification:
        \expandafter\pgfutil@in@\expandafter-\expandafter{\XKV@rm}
        \ifpgfutil@in@%
          % Ah, an arrow spec!
          \expandafter\tikz@processarrows\expandafter{\XKV@rm}%
        \else%
          % Ok, third chance: A shape!
          \expandafter\ifx\csname pgf@sh@s@\XKV@rm\endcsname\relax%
            \PackageError{tikz}{I do not know what to do with the option ``\XKV@rm''}{}
          \else%
            \edef\tikz@shape{\XKV@rm}%
          \fi%
        \fi%
      }%
    \fi%
  \fi%  
}

\def\tikz@setkeys#1{\tikz@@setkeys#1,\pgf@stop}

\def\tikz@@setkeys#1,#2\pgf@stop{%
  \def\tikz@key@test{#1}%
  \def\tikz@key@rest{#2}%
  \ifx\tikz@key@test\pgfutil@empty%
  \else%
    \pgfutil@ifnextchar s{\tikz@parse@key}{\tikz@parse@key}#1==\pgf@stop%
  \fi%
  \ifx\tikz@key@rest\pgfutil@empty%
  \else%
    \expandafter\expandafter\expandafter\tikz@@setkeys\expandafter\tikz@key@rest\expandafter\pgf@stop%
  \fi%
}

\def\tikz@style@text{style}

\def\tikz@parse@key#1=#2=#3\pgf@stop{
  \def\tikz@key@test{#1}%
  \ifx\tikz@key@test\tikz@style@text%
    % Ok, style!
    \pgfutil@ifundefined{tikz@st@#2}%
    {\PackageError{tikz}{Unknown style ``#2}''{}}
    {%
      \expandafter\let\expandafter\tikz@temp\expandafter=\csname tikz@st@#2\endcsname%
      \expandafter\expandafter\expandafter\def
      \expandafter\expandafter\expandafter\tikz@key@rest
      \expandafter\expandafter\expandafter{\expandafter\tikz@temp\expandafter,\tikz@key@rest}%
    }%
  \else%
    \expandafter\ifx\csname tikz@st@#1\endcsname\relax%
      % Ok, normal!
      \def\tikz@test{#3}%
      \ifx\tikz@test\pgfutil@empty%
        \tikz@set@one@key{#1}%
      \else%
        \tikz@set@one@key{#1={#2}}%
      \fi%
    \else%
      % Ok, style!
      \expandafter\let\expandafter\tikz@temp\expandafter=\csname tikz@st@#1\endcsname%
      \expandafter\expandafter\expandafter\def
      \expandafter\expandafter\expandafter\tikz@key@rest
      \expandafter\expandafter\expandafter{\expandafter\tikz@temp\expandafter,\tikz@key@rest}%
    \fi%
  \fi%  
}

\def\tikz@every@style#1{%
  \expandafter\ifx\csname tikz@st@#1\endcsname\relax%
  \else%
    \expandafter\expandafter\expandafter\tikz@setkeys
    \expandafter\expandafter\expandafter{\csname tikz@st@#1\endcsname}%
  \fi%
}





%
% Main TikZ Environment
%

\def\tikzpicture{\pgfutil@ifnextchar[\tikz@picture{\tikz@picture[]}}%}
\def\tikz@picture[#1]{%
  \pgfpicture%
  \let\tikz@atbegin@picture=\pgfutil@empty%
  \let\tikz@atend@picture=\pgfutil@empty%
  \let\tikz@transform=\relax%
  \tikz@installcommands\scope[style=every picture,#1]%
  \tikz@atbegin@picture%
}
\def\endtikzpicture{%
    \tikz@atend@picture%
    \global\let\pgf@shift@baseline=\pgf@baseline%
    \global\let\pgf@remember@smuggle=\ifpgfrememberpicturepositiononpage%
    \endscope%
    \let\pgf@baseline=\pgf@shift@baseline%
    \let\ifpgfrememberpicturepositiononpage=\pgf@remember@smuggle%
  \endpgfpicture}

  

% Inlined picture
%
% #1 - some code to be put in a tikzpicture environment.
%
% If the command is not followed by braces, everything up to the next
% semicolon is used as argument.
%
% Example:
%
% The rectangle \tikz{\draw (0,0) rectangle (1em,1ex)} has width 1em and
% height 1ex.

\def\tikz{\pgfutil@ifnextchar[{\tikz@opt}{\tikz@opt[]}}
\def\tikz@opt[#1]{\pgfutil@ifnextchar\bgroup{\tikz@[#1]}{\tikz@@[#1]}}
\def\tikz@[#1]#2{\tikzpicture[#1]#2\endtikzpicture}
\def\tikz@@{%
  \let\tikz@next=\tikz@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@collectactivesemicolon%
  \fi%
  \tikz@next}
\def\tikz@collectnormalsemicolon[#1]#2;{\tikzpicture[#1]#2;\endtikzpicture}
{
  \catcode`\;=\active
  \gdef\tikz@collectactivesemicolon[#1]#2;{\tikzpicture[#1]#2;\endtikzpicture}
}



%
% Environment for scoping graphic state settings
%
\def\tikz@scope@env{\pgfutil@ifnextchar[\tikz@@scope@env{\tikz@@scope@env[]}}
\def\tikz@@scope@env[#1]{%
  \pgfscope%
  \begingroup%
  \let\tikz@atbegin@scope=\pgfutil@empty%
  \let\tikz@atend@scope=\pgfutil@empty%
  \let\tikz@options=\pgfutil@empty%
  \let\tikz@mode=\pgfutil@empty%
  \tikz@every@style{every scope}%
  \tikz@setkeys{#1}%
  \tikz@options%
  \tikz@atbegin@scope%
}
\def\endtikz@scope@env{%
  \tikz@atend@scope%
  \endgroup%
  \endpgfscope%
}


%
% Install the abbreviated commands
%
\def\tikz@installcommands{%
  \ifnum\the\catcode`\;=\active\relax\expandafter\let\expandafter\tikz@origsemi\expandafter=\tikz@activesemicolon\fi%
  \ifnum\the\catcode`\:=\active\relax\expandafter\let\expandafter\tikz@origcolon\expandafter=\tikz@activecolon\fi%
  \ifnum\the\catcode`\|=\active\relax\expandafter\let\expandafter\tikz@origbar\expandafter=\tikz@activebar\fi%
  \let\tikz@origscope=\scope%
  \let\tikz@origendscope=\endscope%
  \let\tikz@origstartscope=\startscope%
  \let\tikz@origstopscope=\stopscope%
  \let\tikz@origpath=\path%
  \let\tikz@origagainpath=\againpath%
  \let\tikz@origdraw=\draw%
  \let\tikz@origpattern=\pattern%
  \let\tikz@origfill=\fill%
  \let\tikz@origfilldraw=\filldraw%
  \let\tikz@origshade=\shade%
  \let\tikz@origshadedraw=\shadedraw%
  \let\tikz@origclip=\clip%
  \let\tikz@origuseasboundingbox=\useasboundingbox%
  \let\tikz@orignode=\node%
  \let\tikz@origcoordinate=\coordinate%
  \let\tikz@origmatrix=\matrix%
  \let\tikz@origcalendar=\calendar%
  %
  \tikz@deactivatthings%
  %
  \let\scope=\tikz@scope@env%
  \let\endscope=\endtikz@scope@env%
  \let\startscope=\scope%
  \let\stopscope=\endscope%
  \let\path=\tikz@command@path%
  \let\againpath=\tikz@command@againpath%
  %
  \def\draw{\path[draw]}
  \def\pattern{\path[pattern]}
  \def\fill{\path[fill]}
  \def\filldraw{\path[fill,draw]}
  \def\shade{\path[shade]}
  \def\shadedraw{\path[shade,draw]}
  \def\clip{\path[clip]}
  \def\useasboundingbox{\path[use as bounding box]}
  \def\node{\path node}
  \def\coordinate{\path coordinate}
  \def\matrix{\path node[matrix]}
  \def\calendar{\tikz@lib@cal@calendar}%
}
\ifx\tikz@lib@cal@calendar\@undefined
\def\tikz@lib@cal@calendar{\PackageError{tikz}{You need to load the calendar library}{}}
\fi

\def\tikz@uninstallcommands{%
  \ifnum\the\catcode`\;=\active\relax\expandafter\let\tikz@activesemicolon=\tikz@origsemi\fi%
  \ifnum\the\catcode`\:=\active\relax\expandafter\let\tikz@activecolon=\tikz@origcolon\fi%
  \ifnum\the\catcode`\|=\active\relax\expandafter\let\tikz@activebar=\tikz@origbar\fi%
  \let\scope=\tikz@origscope%
  \let\endscope=\tikz@origendscope%
  \let\startscope=\tikz@origstartscope%
  \let\stopscope=\tikz@origstopscope%
  \let\path=\tikz@origpath%
  \let\againpath=\tikz@origagainpath%
  \let\draw=\tikz@origdraw%
  \let\pattern=\tikz@origpattern%
  \let\fill=\tikz@origfill%
  \let\filldraw=\tikz@origfilldraw%
  \let\shade=\tikz@origshade%
  \let\shadedraw=\tikz@origshadedraw%
  \let\clip=\tikz@origclip%
  \let\useasboundingbox=\tikz@origuseasboundingbox%
  \let\node=\tikz@orignode%
  \let\coordinate=\tikz@origcoordinate%
  \let\matrix=\tikz@origmatrix%
  \let\calendar=\tikz@origcalendar%
}


{
  \catcode`\;=12
  \gdef\tikz@nonactivesemicolon{;}
  \catcode`\:=12
  \gdef\tikz@nonactivecolon{:}
  \catcode`\|=12
  \gdef\tikz@nonactivebar{|}
  \catcode`\;=\active
  \catcode`\:=\active
  \catcode`\|=\active
  \catcode`\"=\active
  \gdef\tikz@activesemicolon{;}%
  \gdef\tikz@activecolon{:}%
  \gdef\tikz@activebar{|}%
  \gdef\tikz@activequotes{"}%
  \gdef\tikz@deactivatthings{%
    \def;{\tikz@nonactivesemicolon}
    \def:{\tikz@nonactivecolon}
    \def|{\tikz@nonactivebar}
  }
}





% Constructs a path and draws/fills them according to the current
% settings.  

\def\tikz@command@path{%
  \let\tikz@signal@path=\tikz@signal@path% for detection at begin of matrix cell
  \pgfutil@ifnextchar[{\tikz@check@earg}%]
  {\pgfutil@ifnextchar<{\tikz@doopt}{\tikz@@command@path}}}
\def\tikz@signal@path{\tikz@signal@path}%
\def\tikz@check@earg[#1]{%
  \pgfutil@ifnextchar<{\tikz@swap@args[#1]}{\tikz@@command@path[#1]}}
\def\tikz@swap@args[#1]<#2>{\tikz@command@path<#2>[#1]}

\def\tikz@doopt{%
  \let\tikz@next=\tikz@eargnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@eargactivesemicolon%
  \fi%
  \tikz@next}
\long\def\tikz@eargnormalsemicolon<#1>#2;{\only<#1>{\tikz@@command@path#2;}}
{
  \catcode`\;=\active
  \long\global\def\tikz@eargactivesemicolon<#1>#2;{\only<#1>{\tikz@@command@path#2;}}
}

\def\tikz@@command@path{%
  \edef\tikzscope@linewidth{\the\pgflinewidth}%
  \begingroup%
    \let\tikz@options=\pgfutil@empty%
    \let\tikz@mode=\pgfutil@empty%
    \let\tikz@moveto@waiting=\relax%
    \let\tikz@timer=\relax%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \tikz@snakedfalse%
    \tikz@node@is@a@labelfalse%
    \tikz@expandcount=1000\relax%
    \tikz@lastx=0pt%
    \tikz@lasty=0pt%
    \tikz@lastxsaved=0pt%
    \tikz@lastysaved=0pt%
    \tikz@every@style{every path}%
    \tikz@scan@next@command%
}
\def\tikz@scan@next@command{%
  \ifx\tikz@collected@onpath\pgfutil@empty%
  \else%
    \tikz@invoke@collected@onpath%
  \fi%
  \afterassignment\tikz@handle\let\@let@token=%
}
\newcount\tikz@expandcount

% Central dispatcher for commands
\def\tikz@handle{%
  \let\@next=\tikz@expand%
    \ifx\@let@token(%)
      \let\@next=\tikz@movetoabs%
    \else%
      \ifx\@let@token+%
        \let\@next=\tikz@movetorel%
      \else%
        \ifx\@let@token-%
          \let\@next=\tikz@lineto%
        \else%
          \ifx\@let@token.%
            \let\@next=\tikz@dot%
          \else%
            \ifx\@let@token r%
              \let\@next=\tikz@rect%
            \else%
              \ifx\@let@token a%
                \let\@next=\tikz@arcA%
              \else%
                \ifx\@let@token[%]
                  \let\@next=\tikz@parse@options%
                \else%
                  \ifx\@let@token n%
                    \let\@next=\tikz@fig%
                  \else%
                    \ifx\@let@token\bgroup%
                      \let\@next=\tikz@beginscope%
                    \else%
                      \ifx\@let@token\egroup%
                        \let\@next=\tikz@endscope%
                      \else%
                        \ifx\@let@token;%
                          \let\@next=\tikz@finish%
                        \else%
                          \ifx\@let@token c%
                            \let\@next=\tikz@cchar%
                          \else%
                            \ifx\@let@token e%
                              \let\@next=\tikz@e@char%
                            \else%
                              \ifx\@let@token g%
                                \let\@next=\tikz@grid%
                              \else%
                                \ifx\@let@token s%
                                   \let\@next=\tikz@sine%
                                \else%
                                  \ifx\@let@token |%
                                     \let\@next=\tikz@vh@lineto%
                                  \else%
                                    \ifx\@let@token p%
                                      \let\@next=\tikz@pchar%
                                      \pgfsetmovetofirstplotpoint%
                                    \else%
                                      \ifx\@let@token t%
                                        \let\@next=\tikz@to%
                                      \else%
                                        \ifx\@let@token\pgfextra%
                                          \let\@next=\tikz@extra%
                                        \else%
                                          \ifx\@let@token\foreach%
                                            \let\@next=\tikz@foreach%
                                          \else%
                                            \ifx\@let@token\pgf@stop%
                                              \let\@next=\relax%
                                            \else%
                                              \ifx\@let@token\par%
                                                \let\@next=\tikz@scan@next@command%
                                              \fi%      
                                            \fi%      
                                          \fi%      
                                        \fi%      
                                      \fi%      
                                    \fi%  
                                  \fi%  
                                \fi%
                              \fi%
                            \fi%
                          \fi%
                        \fi%
                      \fi%  
                    \fi%  
                  \fi%  
                \fi%  
              \fi%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \@next%
}

\def\tikz@pchar{\pgfutil@ifnextchar l{\tikz@plot}{\tikz@parabola}}
\def\tikz@cchar{%
  \pgfutil@ifnextchar i{\tikz@circle}%
  {\pgfutil@ifnextchar h{\tikz@children}{\tikz@cochar}}}%
\def\tikz@cochar o{%
  \pgfutil@ifnextchar o{\tikz@coordinate}{\tikz@cosine}}
\def\tikz@e@char{%
  \pgfutil@ifnextchar l{\tikz@ellipse}{\tikz@@e@char}}%
\def\tikz@@e@char dge{%
  \pgfutil@ifnextchar f{\tikz@edgetoparent}{\tikz@edge@plain}}%


\def\tikz@finish{%
  \tikz@mode@fillfalse%
  \tikz@mode@drawfalse%
  \tikz@mode@doublefalse%
  \tikz@mode@clipfalse%
  \tikz@mode@boundaryfalse%
  \edef\tikz@pathextend{%
    {\noexpand\pgfqpoint{\the\pgf@pathminx}{\the\pgf@pathminy}}%
    {\noexpand\pgfqpoint{\the\pgf@pathmaxx}{\the\pgf@pathmaxy}}%
  }%
  \tikz@mode% installs the mode settings
  % Rendering pipeline:  
  % 
  % Step 1: Setup options
  % 
  \ifx\tikz@options\pgfutil@empty%
  \else%
    \pgfsys@beginscope%
      \begingroup%
      \tikz@options%
  \fi%
  % 
  % Step 2: Do a fill if shade follows.
  %
  \iftikz@mode@fill%
    \iftikz@mode@shade%
      \pgfprocessround{\pgfsyssoftpath@currentpath}{\pgfsyssoftpath@currentpath}% change the current path
      \pgfsyssoftpath@invokecurrentpath%
      \pgfsys@fill%
      \tikz@mode@fillfalse% no more filling...
    \fi%
  \fi%
  % 
  % Step 3: Do a shade if necessary.
  %
  \iftikz@mode@shade%
    \pgfprocessround{\pgfsyssoftpath@currentpath}{\pgfsyssoftpath@currentpath}% change the current path
    \pgfshadepath{\tikz@shading}{\tikz@shade@angle}%
    \tikz@mode@shadefalse% no more shading...
  \fi%
  % 
  % Step 4: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
      % Change line width
      \begingroup%
        \pgfsys@beginscope%
          \pgf@x=2\pgflinewidth%
          \advance\pgf@x by\tikz@double@width@distance%
          \pgflinewidth=\pgf@x%
          \pgfsetlinewidth{\the\pgflinewidth}%
    \fi%
  \fi%
  % 
  % Step 5: Do stroke/fill/clip as needed
  %
  \edef\tikz@temp{\noexpand\pgfusepath{%
    \iftikz@mode@fill fill,\fi%
    \iftikz@mode@draw draw,\fi%
    \iftikz@mode@clip clip,\fi%
    }}%
  \tikz@temp%
  \tikz@mode@fillfalse% no more filling
  % 
  % Step 6: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
          \pgfsyssoftpath@setcurrentpath\pgf@last@used@path% reinstall
          \pgf@x=\tikz@double@width@distance%
          \pgfsetlinewidth{\the\pgf@x}%
          \pgfsetstrokecolor{\tikz@double@color}%
          \pgfsyssoftpath@flushcurrentpath%
          \pgfsys@stroke%
        \pgfsys@endscope%
        \pgf@add@arrows@as@needed
      \endgroup%
    \fi%
  \fi%
  \tikz@mode@drawfalse% no more stroking
  % 
  % Step 7: Add labels and nodes
  %
  \copy\tikz@figbox%
  \setbox\tikz@figbox=\box\voidb@x%
  %
  % Step 8: Close option brace
  %
  \ifx\tikz@options\pgfutil@empty%
  \else%
      \endgroup%
    \pgfsys@endscope%
    \iftikz@mode@clip%
      \PackageError{tikz}{Extra options not allowed for clipping path command.}{}%
    \fi%
  \fi%
  \iftikz@mode@clip%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \iftikz@mode@boundary%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \endgroup%
  \global\pgflinewidth=\tikzscope@linewidth%
}




\def\tikz@skip#1{\tikz@scan@next@command#1}
\def\tikz@expand{%
  \advance\tikz@expandcount by -1%
  \ifnum\tikz@expandcount<0\relax%
    \PackageError{tikz}{Giving up on this path. Did you forget a semicolon?}{}%
    \let\@next=\tikz@finish%
  \else%
    \let\@next=\tikz@@expand
  \fi%
  \@next}

\def\tikz@@expand{%
  \expandafter\tikz@scan@next@command\@let@token}



% Syntax for scopes: 
% {scoped path commands}

\def\tikz@beginscope{\begingroup\tikz@scan@next@command}
\def\tikz@endscope{%
  \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \tikz@scan@next@command}


% Syntax for pgfextra: 
% \pgfextra {normal tex text}
% \pgfextra normal tex text \endpgfextra

\def\tikz@extra{\pgfutil@ifnextchar\bgroup\tikz@@extra\relax}
\long\def\tikz@@extra#1{#1\tikz@scan@next@command}
\let\endpgfextra=\tikz@scan@next@command

\def\pgfextra{pgfextra}


% Syntax for \foreach: 
% \foreach \var in {list} {path text}
%
% Example:
%
% \draw (0,0) \foreach \x in {1,2,3} {-- (\x,0) circle (1cm)} -- (5,5);

\def\tikz@foreach{%
  \def\pgffor@beginhook{\setbox\tikz@figbox=\box\tikz@tempbox\expandafter\tikz@scan@next@command\@firstofone}%
  \def\pgffor@endhook{\pgfextra{%
      \xdef\tikz@foreach@save@lastx{\the\tikz@lastx}%
      \xdef\tikz@foreach@save@lasty{\the\tikz@lasty}%
      \xdef\tikz@foreach@save@lastxsaved{\the\tikz@lastxsaved}%
      \xdef\tikz@foreach@save@lastysaved{\the\tikz@lastysaved}%
      \global\setbox\tikz@tempbox=\copy\tikz@figbox\pgfutil@gobble}}%
  \def\pgffor@afterhook{%
    \tikz@lastx=\tikz@foreach@save@lastx%
    \tikz@lasty=\tikz@foreach@save@lasty%
    \tikz@lastxsaved=\tikz@foreach@save@lastxsaved%
    \tikz@lastysaved=\tikz@foreach@save@lastysaved%
    \setbox\tikz@figbox=\box\tikz@tempbox\tikz@scan@next@command}%
  \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \foreach}

  
% Syntax for againpath: 
% \againpath \somepathname

\def\tikz@command@againpath#1{%
  \pgfextra{%
    \pgfsyssoftpath@getcurrentpath\tikz@temp%
    \expandafter\pgfutil@g@addto@macro\expandafter\tikz@temp\expandafter{#1}%
    \pgfsyssoftpath@setcurrentpath\tikz@temp%
  }
}




%
% When this if is set, a just-scanned point is a shape and its border
% position still needs to be determined, depending on subsequent
% commands. 
%

\newif\iftikz@shapeborder


% Syntax for moveto: 
% <point>
\def\tikz@movetoabs{\tikz@moveto(}
\def\tikz@movetorel{\tikz@moveto+}
\def\tikz@moveto{%
  \tikz@scan@one@point{\tikz@@moveto}}
\def\tikz@@moveto#1{%
  \tikz@make@last@position{#1}%
  \iftikz@shapeborder%
    % ok, the moveto will have to wait. flag that we have a moveto in
    % wainting:
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \pgfpathmoveto{\tikz@last@position}%
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \tikz@scan@next@command%
}

\let\tikz@moveto@waiting=\relax % normally, nothing is waiting...

\def\tikz@flush@moveto{%
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \pgfpathmoveto{\tikz@last@position}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}


\def\tikz@flush@moveto@toward#1#2#3{%
  % #1 = a point towards which the last moveto should be corrected
  % #2 = a dimension to which the corrected x-coordinate should be stored
  % #3 = a dimension for the corrected y-coordinate
  \ifx\tikz@moveto@waiting\relax%
    % do nothing
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{#1}}%
    #2=\pgf@x%
    #3=\pgf@y%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \pgfpathmoveto{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}


%
% Collecting labels on the path 
%

\def\tikz@collect@coordinate@onpath#1coordinate{%
  \pgfutil@ifnextchar[{\tikz@@collect@coordinate@opt#1}{\tikz@@collect@coordinate@opt#1[]}}%}
\def\tikz@@collect@coordinate@opt#1[#2]{%
  \pgfutil@ifnextchar({\tikz@@collect@coordinate#1[#2]}{%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2]{}}}%}
\def\tikz@@collect@coordinate#1[#2](#3){%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2](#3){}}

\def\tikz@collect@label@onpath#1node{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath node}%
  \tikz@collect@label@scan#1}

\def\tikz@collect@label@scan#1{%  
  \pgfutil@ifnextchar({\tikz@collect@paran#1}%
  {\pgfutil@ifnextchar[{\tikz@collect@options#1}%
    {\pgfutil@ifnextchar\bgroup{\tikz@collect@arg#1}%
      {#1}}}%
}%}}

\def\tikz@collect@paran#1(#2){%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath(#2)}%
  \tikz@collect@label@scan#1%
}
\def\tikz@collect@options#1[#2]{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath[#2]}%
  \tikz@collect@label@scan#1%
}
\def\tikz@collect@arg#1#2{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#2}}%
  #1%
}


\def\tikz@invoke@collected@onpath{%
  \tikz@node@is@a@labeltrue%
  \let\tikz@temp=\tikz@collected@onpath%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \expandafter\tikz@scan@next@command\tikz@temp\pgf@stop%
  \tikz@node@is@a@labelfalse%
}




% Syntax for lineto: 
% -- <point>

\def\tikz@lineto{%
  \pgfutil@ifnextchar |%
  {\expandafter\tikz@hv@lineto\pgfutil@gobble}%
  {\expandafter\pgfutil@ifnextchar\tikz@activebar{\expandafter\tikz@hv@lineto\pgfutil@gobble}%
    {\expandafter\tikz@lineto@mid\pgfutil@gobble}}}
\def\tikz@lineto@mid{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@lineto@mid}%
  {%
    \pgfutil@ifnextchar c{\tikz@close}{%
      \pgfutil@ifnextchar p{\pgfsetlinetofirstplotpoint\expandafter\tikz@plot\pgfutil@gobble}%
        {\tikz@scan@one@point{\tikz@@lineto}}}}}
\def\tikz@@lineto#1{%
  % Record the starting point for later labels on the path:
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate end
    \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@last@position}}%
    \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \tikz@make@last@position{#1}%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    % target is a reasonable point...
    % Record the starting point for later labels on the path:
    \tikz@make@last@position{#1}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@line%
  \tikz@scan@next@command%
}

% snake or lineto?
\def\tikz@path@lineto#1{%
  \iftikz@snaked%
    {
      \pgfsyssoftpathmovetorelevantfalse%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength},\tikz@postsnake}{#1}%
    }
  \else%
    \pgfpathlineto{#1}%
  \fi%
}

% snake or lineto?
\def\tikz@path@close#1{%
  \iftikz@snaked%
    {%
      \pgftransformreset%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength},\tikz@postsnake}{#1}%
    }%
    \pgfpathclose%
  \else%
    \pgfpathclose%
  \fi%
}


% Syntax for lineto horizontal/vertical: 
% -| <point>

\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar n
  {\tikz@collect@label@onpath\tikz@hv@lineto}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@hv@lineto}%
    {\tikz@scan@one@point{\tikz@@hv@lineto}}}}
\def\tikz@@hv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@yc=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@x\pgf@yc%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yc}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
  \fi%
  \let\tikz@timer=\tikz@timer@hvline%
  \tikz@scan@next@command%
}

% Syntax for lineto vertical/horizontal: 
% |- <point>

\def\tikz@vh@lineto-{\tikz@vh@lineto@next}
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar n
  {\tikz@collect@label@onpath\tikz@vh@lineto@next}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@vh@lineto@next}%
    {\tikz@scan@one@point\tikz@@vh@lineto}}}
\def\tikz@@vh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx%
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@y%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xc}{\tikz@lasty}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@vhline%
  \tikz@scan@next@command%
}

% Syntax for cycle: 
% -- cycle
\def\tikz@close c{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@lineto@mid c}% oops, a coordinate
  {\tikz@@close c}}%
\def\tikz@@close cycle{%
  \tikz@flush@moveto%
  \tikz@path@close{\expandafter\pgfpoint\pgfsyssoftpath@lastmoveto}%
  \def\pgfstrokehook{}%
  \let\tikz@timer=\@undefined%
  \tikz@scan@next@command%
}


% Syntax for options: 
% [options]
\def\tikz@parse@options#1]{%
  \tikz@setkeys{#1}%
  \tikz@scan@next@command%
}

% Syntax for edges:
% edge [options] (coordinate)
% edge [options] node {node text} (coordinate)
\def\tikz@edge@plain{%
  \begingroup%
    \tikz@to@use@whom%
    \let\tikz@to@or@edge@function=\tikz@do@edge%
    \tikz@to@or@edge}

% Syntax for to paths:
% to [options] (coordinate)
% to [options] node {node text} (coordinate)
\def\tikz@to o{%
  \tikz@to@use@last@coordinate%
  \let\tikz@to@or@edge@function=\tikz@do@to%
  \tikz@to@or@edge}
  
\def\tikz@to@or@edge{\pgfutil@ifnextchar[\tikz@@to@or@edge{\tikz@@to@or@edge[]}}%}
\def\tikz@@to@or@edge[#1]{%
  \def\tikz@@to@local@options{[#1]}%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@@to@collect%
}
\def\tikz@@to@collect{%
  \pgfutil@ifnextchar(\tikz@@to@or@edge@coordinate
  {\pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@to@collect}%
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@to@collect}
      {\PackageError{tikz}{( expected}{}%}
        \tikz@@to@or@edge@coordinate()}}}%
}

\def\tikz@@to@or@edge@coordinate(#1){%
  \def\tikztotarget{#1}%
  \tikz@to@or@edge@function%
}

\def\tikz@do@edge{%
  \setbox\tikz@figbox=\hbox\bgroup%
    \unhbox\tikz@figbox%
    \hbox\bgroup
      \bgroup%
        \pgfinterruptpath%
          \pgfscope%
            \let\tikz@transform=\pgfutil@empty%
            \let\tikz@options=\pgfutil@empty%
            \let\tikz@tonodes=\tikz@collected@onpath%
            \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
            \let\tikz@collected@onpath=\pgfutil@empty%
            \tikz@options%
            \tikz@transform%            
            % Typeset node:
            \tikz@atbegin@to%
            \path[style=every edge]\tikz@@to@local@options(\tikztostart)\tikz@to@path;%
            \tikz@atend@to%
          \endpgfscope%
        \endpgfinterruptpath%
      \egroup
    \egroup%
  \egroup%
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%  
  \tikz@scan@next@command%  
}

\def\tikz@do@to{%
  \let\tikz@tonodes=\tikz@collected@onpath%
  \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@scan@next@command%
  \pgfextra{\tikz@atbegin@to}%
  [style=every to]\tikz@@to@local@options\tikz@to@path%
  \pgfextra{\tikz@atend@to}%
}


\def\tikz@to@use@last@coordinate{%
  \iftikz@shapeborder%
    \edef\tikztostart{\tikz@shapeborder@name}%
  \else%
    \edef\tikztostart{\the\tikz@lastx,\the\tikz@lasty}%
  \fi%
}
\def\tikz@to@use@last@fig@name{%
  \edef\tikztostart{\tikz@to@last@fig@name}%
}



% Syntax for edge from parent: 
% edge from parent [options]
\def\tikz@edgetoparent from parent{\pgfutil@ifnextchar[\tikz@@edgetoparent{\tikz@@edgetoparent[]}}%}
\def\tikz@@edgetoparent[#1]{%
  \let\tikz@edge@to@parent@needed=\pgfutil@empty%
  \tikz@node@is@a@labeltrue%
  \tikz@scan@next@command [style=edge from parent,#1] \tikz@edge@to@parent@path%
}


% Syntax for bezier curves
% .. controls(point) and (point) .. (target)
% .. controls(point) .. (target) 
% .. (target) % currently not supported

\def\tikz@dot.{\tikz@@dot}%
\def\tikz@@dot{%
  \pgfutil@ifnextchar n%
  {\tikz@collect@label@onpath\tikz@@dot}%
  {\pgfutil@ifnextchar c{\tikz@curveto@double}{\tikz@curveto@auto}}}

\def\tikz@curveto@double co{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@@dot co}
  {\tikz@cureveto@@double}}
\def\tikz@cureveto@@double ntrols#1{%
  \tikz@scan@one@point\tikz@curveA#1%
}
\def\tikz@curveA#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@make@last@position{#1}%
    \xdef\tikz@curve@first{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  \pgfutil@ifnextchar a
  {\tikz@curveBand}%
  {\let\tikz@curve@second\tikz@curve@first\tikz@curveCdots}%
}
\def\tikz@curveBand and{%
  \tikz@scan@one@point\tikz@curveB%
}
\def\tikz@curveB#1{%
  \def\tikz@curve@second{#1}%
  \tikz@curveCdots}
\def\tikz@curveCdots{%
  \afterassignment\tikz@curveCdot\let\@next=}
\def\tikz@curveCdot.{%
  \ifx\@next.%
  \else%
    \PackageError{tikz}{Dot expected}{}%
  \fi%
  \tikz@updatecurrenttrue%
  \tikz@curveCcheck%
}
\def\tikz@curveCcheck{%
  \pgfutil@ifnextchar n%
  {\tikz@collect@label@onpath\tikz@curveCcheck}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@curveCcheck}
    {\tikz@scan@one@point\tikz@curveC}}%
}
\def\tikz@curveC#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@lastxsaved=\tikz@lastx%
    \tikz@lastysaved=\tikz@lasty%
    \tikz@make@last@position{\tikz@curve@second}%
    \xdef\tikz@curve@second{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  %
  % Start recalculating things in case start and end are shapes.
  %
  % First, the start:
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{\tikz@curve@first}}%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \pgfpathmoveto{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@timer@cont@one=\tikz@curve@first%
  \let\tikz@timer@cont@two=\tikz@curve@second%    
  % Second, the end:
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate third
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@curve@second}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
      \global\let\tikz@timer@end@temp=\tikz@curve@third% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
    \let\tikz@timer@end=\tikz@curve@third
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \let\tikz@timer=\tikz@timer@curve%  
  \tikz@scan@next@command%
}


% Syntax for rectangles: 
% rectangle <corner point> 
\def\tikz@rect ectangle{%
  \tikz@flush@moveto%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \tikz@@rect}%
\def\tikz@@rect{%
  \pgfutil@ifnextchar n
  {\tikz@collect@label@onpath\tikz@@rect}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@rect}%
    {
      \pgf@xa=\tikz@lastx\relax%
      \pgf@ya=\tikz@lasty\relax%
      \tikz@scan@one@point\tikz@rectB}}}
\def\tikz@rectB#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \let\tikz@timer=\tikz@timer@line%  
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@ya}}%
  \iftikz@snaked% 
    \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \fi%
  \pgfpathclose%
  \pgfpathmoveto{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \def\pgfstrokehook{}%
  \tikz@scan@next@command%
}



% Syntax for grids: 
% grid <corner point> 
\def\tikz@grid rid{%
  \tikz@flush@moveto%
  \pgf@xa=\tikz@lastx\relax%
  \pgf@ya=\tikz@lasty\relax%
  \pgfutil@ifnextchar[{\tikz@gridA}{\tikz@gridA[]}}%}
\def\tikz@gridA[#1]{%
  \def\tikz@grid@options{#1}%
  \tikz@scan@one@point\tikz@gridB}%
\def\tikz@gridB#1{%
  \tikz@make@last@position{#1}%
  {%
    \expandafter\tikz@setkeys\expandafter{\tikz@grid@options}
    \tikz@checkunit{\tikz@grid@x}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{\tikz@grid@x}{0pt}}%
    \else%
      \pgf@process{\pgfpointxy{\tikz@grid@x}{0}}%
    \fi%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \tikz@checkunit{\tikz@grid@y}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{0pt}{\tikz@grid@y}}%
    \else%
      \pgf@process{\pgfpointxy{0}{\tikz@grid@y}}%
    \fi%
    \advance\pgf@xb by\pgf@x%
    \advance\pgf@yb by\pgf@y%
    \pgfpathgrid[stepx=\pgf@xb,stepy=\pgf@yb]%
      {\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  }
  \tikz@scan@next@command%
}



% Syntax for plot: 
% plot [local options] ...    % starts with a moveto
% -- plot [local options] ... % starts with a lineto
\def\tikz@plot lot{%
  \tikz@flush@moveto%
  \pgfutil@ifnextchar[{\tikz@@plot}{\tikz@@plot[]}}%}
\def\tikz@@plot[#1]{%
  \begingroup%
    \let\tikz@options=\pgfutil@empty%
    \tikz@every@style{every plot}%
    \tikz@setkeys{#1}%
    \pgfutil@ifnextchar f{\tikz@plot@f}%
    {\pgfutil@ifnextchar c{\tikz@plot@scan@points}%
      {\pgfutil@ifnextchar ({\tikz@plot@expression}{%
      \PackageError{tikz}{Cannot parse this plotting data}{}%
       \endgroup}}}}
\def\tikz@plot@f f{\pgfutil@ifnextchar i{\tikz@plot@file}{\tikz@plot@function}}

\def\tikz@plot@file ile#1{\def\tikz@plot@data{\pgfplotxyfile{#1}}\tikz@@@plot}%
\def\tikz@plot@scan@points coordinates#1{%
  \pgfplothandlerrecord\tikz@plot@data%
  \pgfplotstreamstart%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}
  {\tikz@scan@one@point\tikz@plot@next@point}%
  #1\pgf@stop%
}
\def\tikz@plot@next@point#1{%
  \pgfplotstreampoint{#1}%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}%
  {\tikz@scan@one@point\tikz@plot@next@point}%
}  
\def\tikz@plot@function unction#1{%
  \def\tikz@plot@filename{\tikz@plot@prefix\tikz@plot@id}%  
  \iftikz@plot@raw@gnuplot%
    \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{#1}}%
  \else%
    \iftikz@plot@parametric%   
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          set parametric;
          plot [t=\tikz@plot@domain] #1}}%
    \else%
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          plot [x=\tikz@plot@domain] #1}}%
    \fi%
  \fi%
  \tikz@@@plot%
}

\def\tikz@plot@no@resample{%
  \pgfutil@IfFileExists{\tikz@plot@filename.table}%
  {\def\tikz@plot@data{\pgfplotxyfile{\tikz@plot@filename.table}}}%
  {}%
}

\def\tikz@plot@expression(#1){%
  \edef\tikz@plot@data{\noexpand\pgfplotfunction{\expandafter\noexpand\tikz@plot@var}{\tikz@plot@samplesat}}%
  \expandafter\def\expandafter\tikz@plot@data\expandafter{\tikz@plot@data{\tikz@scan@one@point\pgfutil@firstofone(#1)}}%
  \tikz@@@plot%
}

\def\tikz@@@plot{%
    \def\pgfplotlastpoint{\pgfpointorigin}%
    \tikz@plot@handler%
    \tikz@plot@data%
    \global\let\tikz@@@temp=\pgfplotlastpoint%
    \ifx\tikz@plot@mark\pgfutil@empty%
    \else%
      % Marks are drawn after the path.
      \setbox\tikz@figbox=\hbox{%
        \unhbox\tikz@figbox%
        \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \let\tikz@options=\pgfutil@empty%
              \let\tikz@transform=\pgfutil@empty%
              \expandafter\tikz@setkeys\expandafter{\tikz@plot@mark@options}%
              \tikz@options%
              \ifx\tikz@mark@list\pgfutil@empty%
                \pgfplothandlermark{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}%
              \else
                \pgfplothandlermarklisted{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}{\tikz@mark@list}%
              \fi
              \tikz@plot@data%
            \endpgfscope
          \endpgfinterruptpath%
        }}%
      }%
    \fi%
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%  
  \tikz@make@last@position{\tikz@@@temp}%  
  \tikz@scan@next@command%
}


\pgfdeclareplotmark{ball}
{%
  \def\tikz@shading{ball}%
  \shade (0,0) circle (\pgfplotmarksize);%
}




% Syntax for cosine curves:
% cos <end of quarter-period>
\def\tikz@cosine s{\tikz@scan@one@point\tikz@@cosine}
\def\tikz@@cosine#1{%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathcosine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}

% Syntax for sine curves:
% sin <end of quarter-period>
\def\tikz@sine in{\tikz@scan@one@point\tikz@@sine}
\def\tikz@@sine#1{%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathsine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}

% Syntax for parabolas: 
% parabola[options] bend <coordinate> <coordinate>
\def\tikz@parabola arabola{%
  \pgfutil@ifnextchar[{\tikz@parabola@options}{\tikz@parabola@options[]}}%}

\def\tikz@parabola@options[#1]{%
  \def\tikz@parabola@option{#1}%
  \pgfutil@ifnextchar b{\tikz@parabola@scan@bend}{\tikz@scan@one@point\tikz@parabola@semifinal}}
\def\tikz@parabola@scan@bend bend{\tikz@scan@one@point\tikz@parabola@scan@bendB}
\def\tikz@parabola@scan@bendB#1{%
  \def\tikz@parabola@bend{#1}%
  \tikz@scan@one@point\tikz@parabola@semifinal%
}
\def\tikz@parabola@semifinal#1{%
  \tikz@flush@moveto%
  % Save original start:
  \pgf@xb=\tikz@lastx%
  \pgf@yb=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \pgf@xc=\tikz@lastx%
  \pgf@yc=\tikz@lasty%
  \begingroup% now calculate bend:
    \expandafter\tikz@setkeys\expandafter{\tikz@parabola@option}%
    \tikz@lastxsaved=\tikz@parabola@bend@factor\tikz@lastx%
    \tikz@lastysaved=\tikz@parabola@bend@factor\tikz@lasty%
    \advance\tikz@lastxsaved by\pgf@xb%
    \advance\tikz@lastysaved by\pgf@yb%
    \advance\tikz@lastxsaved by-\tikz@parabola@bend@factor\pgf@xb%
    \advance\tikz@lastysaved by-\tikz@parabola@bend@factor\pgf@yb%
    \expandafter\tikz@make@last@position\expandafter{\tikz@parabola@bend}%
    % Calculate delta from bend
    \advance\pgf@xc by-\tikz@lastx%
    \advance\pgf@yc by-\tikz@lasty%
    % Ok, now calculate delta to bend
    \advance\tikz@lastx by-\pgf@xb%
    \advance\tikz@lasty by-\pgf@yb%
    \xdef\tikz@parabola@b{{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}}%
  \endgroup%
  \expandafter\pgfpathparabola\tikz@parabola@b%
  \tikz@scan@next@command%
}


% Syntax for circles:
% circle (radius)
%
% Syntax for ellipses:
% ellipse (x-radius and y-radius)
%
% radii can be dimensionless, then they are in the xy-system
\def\tikz@circle ircle{\tikz@flush@moveto\tikz@@circle}
\def\tikz@ellipse llipse{\tikz@flush@moveto\tikz@@circle}
\def\tikz@@circle{%
  \pgfutil@ifnextchar(\tikz@@@circle{%)
    \advance\tikz@expandcount by -1%
    \ifnum\tikz@expandcount<0\relax%
      \let\@next=\tikz@@circle@scangiveup%
    \else%
      \let\@next=\tikz@@circle@scanexpand%
    \fi%
    \@next%
  }%
}
\def\tikz@@circle@scanexpand{\expandafter\tikz@@circle}
\def\tikz@@circle@scangiveup#1{\PackageError{tikz}{Cannot parse this radius}{}#1{\tikz@scan@next@command}}
\def\tikz@@@circle(#1){%
  \pgfutil@in@{ and }{#1}%
  \ifpgfutil@in@%
    \tikz@@ellipseB(#1)%
  \else%
    \tikz@@ellipseB(#1 and #1)%
  \fi%
  \tikz@scan@next@command%
}
\def\tikz@@ellipseB(#1 and #2){%
  \tikz@checkunit{#1}%
  \iftikz@isdimension%
    \pgfpathellipse{\tikz@last@position}{\pgfpoint{#1}{0pt}}{\pgfpoint{0pt}{#2}}%
  \else%
    \pgfpathellipse{\tikz@last@position}{\pgfpointxy{#1}{0}}{\pgfpointxy{0}{#2}}%
  \fi%
}

% Syntax 1 for arcs:
% arc (start angle:end angle:radius)
%
% Syntax 2 for arcs:
% arc (start angle:end angle:x-radius and y-radius)
%
% radius can be dimensionless, then the arc is in the xy-coordinate system
\def\tikz@arcA rc{%
  \tikz@flush@moveto%
  \pgfutil@ifnextchar({\tikz@@arcto}{\expandafter\tikz@arcA\expandafter r\expandafter c}}

\def\tikz@@arcto(#1){%
  \edef\tikz@temp{(#1)}%
   \expandafter\tikz@@@arcto@check@slashand\tikz@temp%
}

\def\tikz@@@arcto@check@slashand(#1:#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@% 
    \tikz@parse@arc@and(#1:#2:#3)%
  \else%
    \tikz@parse@arc@and(#1:#2:#3 and #3)%
  \fi%
}

\def\tikz@parse@arc@and(#1:#2:#3 and #4){%
  \tikz@checkunit{#3}%
  \iftikz@isdimension%
    \tikz@@@arcfinal{\pgfpatharc{#1}{#2}{#3 and #4}}
    {\pgfpointpolar{#1}{#3 and #4}}
    {\pgfpointpolar{#2}{#3 and #4}}%
  \else%
    \tikz@@@arcfinal{\pgfpatharcaxes{#1}{#2}{\pgfpointxy{#3}{0}}{\pgfpointxy{0}{#4}}}
    {\pgfpointpolarxy{#1}{#3 and #4}}{\pgfpointpolarxy{#2}{#3 and #4}}%
  \fi%
}

\def\tikz@@@arcfinal#1#2#3{%
  #1%
  \pgf@process{#2}%
  \advance\tikz@lastx by-\pgf@x%
  \advance\tikz@lasty by-\pgf@y%
  \pgf@process{#3}%
  \advance\tikz@lastx by\pgf@x%
  \advance\tikz@lasty by\pgf@y%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@scan@next@command%
}


% Syntax for coordinates:
% coordinate[options] (coordinate name) at (point)
% where ``at (point)'' is optional
\def\tikz@coordinate ordinate{%
  \pgfutil@ifnextchar[{\tikz@@coordinate@opt}{\tikz@@coordinate@opt[]}}
\def\tikz@@coordinate@opt[#1]{%
  \pgfutil@ifnextchar({\tikz@@coordinate[#1]}
  {\tikz@fig ode[shape=coordinate,#1]{}}}%}
\def\tikz@@coordinate[#1](#2){%
  \pgfutil@ifnextchar a{\tikz@@coordinate@at[#1](#2)}
  {\tikz@fig ode[shape=coordinate,#1](#2){}}}
\def\tikz@@coordinate@at[#1](#2)at#3(#4){%
  \tikz@fig ode[shape=coordinate,#1](#2)at(#4){}}
  


% Syntax for nodes:
% node[options] (node name) {label text}
%
% all of [options], (node name) and {label text} are optional. There
% can be multiple options before the label text as in
% node[draw] (a) [rotate=10] {text}
%
% A label text always ``ends'' the node.
\def\tikz@fig ode{%
  \edef\tikz@save@line@width{\the\pgflinewidth}%
  \begingroup%
  \let\tikz@fig@name=\pgfutil@empty%
    \begingroup%
      \tikz@is@matrixfalse%
      \let\nodepart=\tikz@nodepart%
      \let\tikz@options=\pgfutil@empty%
      \let\tikz@after@node=\pgfutil@empty%
      \let\tikz@afternodepathoptions=\pgfutil@empty%
      \let\tikz@transform=\pgfutil@empty%
      \let\tikz@mode=\pgfutil@empty%
      \def\tikz@node@at{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \iftikz@node@is@a@label%
      \else%
        \let\tikz@time=\pgfutil@empty%
      \fi%
      \tikz@every@style{every node}%
      \tikz@@scan@fig}%
\def\tikz@@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
  {\pgfutil@ifnextchar({\tikz@fig@scan@name}
    {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
      {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
      {\PackageError{tikz}{A node must have a (possibly empty) label text}{}%
       \tikz@fig@main{}}}}}}%}}
\def\tikz@fig@scan@at at{%
  \tikz@scan@one@point\tikz@@fig@scan@at}
\def\tikz@@fig@scan@at#1{%
  \def\tikz@node@at{#1}\tikz@@scan@fig}%
\def\tikz@fig@scan@name(#1){\edef\tikz@fig@name{#1}\tikz@@scan@fig}%
\def\tikz@fig@scan@options[#1]{\tikz@setkeys{#1}\def\test{#1}\tikz@@scan@fig}%
\def\tikz@fig@main{\afterassignment\tikz@@fig@main\let\next=}
\def\tikz@@fig@main{%
    \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
    {\PackageError{tikz}%
      {Unknown shape ``\tikz@shape.'' Using ``rectangle'' instead}{}%
      \def\tikz@shape{rectangle}}%
    {}%
    \tikz@every@style{every \tikz@shape\space node}%
    \iftikz@is@matrix%
      \let\tikz@next=\tikz@do@matrix%
    \else%
      \let\tikz@next=\tikz@do@fig%
    \fi%
    \tikz@next%  
}
\def\tikz@do@fig{%  
    \setbox\pgfnodeparttextbox=\hbox%
      \bgroup%
        \tikz@every@style{every text node part}%
        \ifx\tikz@textopacity\pgfutil@empty%
        \else%
          \pgfsetfillopacity{\tikz@textopacity}%
          \pgfsetstrokeopacity{\tikz@textopacity}%
        \fi%
        \pgfinterruptpicture%
          \tikz@textfont%  
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
            \begingroup%
              \pgfutil@minipage[t]{\tikz@text@width}%
                \tikz@text@action%
          \fi%
          \tikz@atbegin@node%
          \bgroup%
            \aftergroup\unskip%
            \ifx\tikz@textcolor\pgfutil@empty%
            \else%
              \pgfutil@colorlet{.}{\tikz@textcolor}%
            \fi%
            \pgfsetcolor{.}%
            \setbox\tikz@figbox=\box\voidb@x%
            \tikz@uninstallcommands%
            \aftergroup\tikz@fig@collectresetcolor%
            \ignorespaces%
}
\def\tikz@fig@collectresetcolor{%
  \pgfutil@ifnextchar\reset@color%
  {\reset@color\afterassignment\tikz@fig@collectresetcolor\let\tikz@temp=}%
  {\tikz@fig@boxdone}%
}
\def\tikz@fig@boxdone{%
            \tikz@atend@node%
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
              \pgfutil@endminipage%
            \endgroup%
          \fi%
        \endpgfinterruptpicture%
      \egroup%
    \pgfutil@ifnextchar c{\tikz@fig@mustbenamed\tikz@fig@continue}%
    {\pgfutil@ifnextchar[{\tikz@fig@mustbenamed\tikz@fig@continue}%
      {\pgfutil@ifnextchar t{\tikz@fig@mustbenamed\tikz@fig@continue}
        {\pgfutil@ifnextchar e{\tikz@fig@mustbenamed\tikz@fig@continue}
          {\ifx\tikz@after@node\pgfutil@empty\expandafter\tikz@fig@continue\else\expandafter\tikz@fig@mustbenamed\expandafter\tikz@fig@continue\fi}}}}}%}

\def\tikz@do@matrix{%
    \tikz@every@style{every matrix}%
    \tikz@node@transformations%
    \tikz@fig@mustbenamed%
    \setbox\tikz@figbox=\hbox\bgroup%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox\bgroup\bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\voidb@x%
              \let\tikzmatrixname=\tikz@fig@name%
              \edef\tikz@m@anchor{\ifx\tikz@matrix@anchor\pgfutil@empty\tikz@anchor\else\tikz@matrix@anchor\fi}%
              \expandafter\pgfutil@in@\expandafter{\expandafter.\expandafter}\expandafter{\tikz@m@anchor}%
              \ifpgfutil@in@%
                \expandafter\tikz@matrix@split\tikz@m@anchor\relax%
              \else%
                \def\tikz@matrix@shift{\pgfpointorigin}%  
              \fi%
              \let\tikz@transform=\relax%
              \pgfmatrix%
              {\tikz@shape}%
              {\tikz@m@anchor}%
              {\tikz@fig@name}%
              {%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
              {\tikz@matrix@shift}%
              {%
                \tikz@matrix@make@active@ampersand%
                \def\pgfmatrixbegincode{%
                  \pgfsys@beginscope%
                  \tikz@common@matrix@code%
                  \tikz@atbegin@cell%
                }%
                \def\tikz@common@matrix@code{%
                  \let\tikz@options=\pgfutil@empty%
                  \let\tikz@mode=\pgfutil@empty%
                  \tikz@every@style{every cell}%
                  \tikz@every@style{column \the\pgfmatrixcurrentcolumn}%
                  \ifodd\pgfmatrixcurrentcolumn%
                    \tikz@every@style{every odd column}%
                  \else%
                    \tikz@every@style{every even column}%
                  \fi%
                  \tikz@every@style{row \the\pgfmatrixcurrentrow}%
                  \ifodd\pgfmatrixcurrentrow%
                    \tikz@every@style{every odd row}%
                  \else%
                    \tikz@every@style{every even row}%
                  \fi%
                  \tikz@every@style{row \the\pgfmatrixcurrentrow\space column \the\pgfmatrixcurrentcolumn}%
                  \tikz@options%
                }%
                \def\pgfmatrixendcode{%
                  \tikz@atend@cell%
                  \pgfsys@endscope%
                }%
                \def\pgfmatrixemptycode{%
                  \pgfsys@beginscope%
                  \tikz@common@matrix@code%
                  \tikz@at@emptycell%
                  \pgfsys@endscope%
                }%
                \aftergroup\tikz@do@matrix@cont}%
              \bgroup%
}
\def\tikz@do@matrix@cont{%            
            \endpgfscope
          \endpgfinterruptpath%
      \egroup\egroup%
    \egroup%
    %
    \tikz@node@finish%
}

{%
  \catcode`\&=13
  \gdef\tikz@matrix@make@active@ampersand{%
    \ifx\tikz@ampersand@replacement\pgfutil@empty%
      \catcode`\&=13%
      \let&=\pgfmatrixnextcell%
    \else%
      \expandafter\let\tikz@ampersand@replacement=\pgfmatrixnextcell%
    \fi%
  }%
}%


\def\tikz@matrix@split#1.#2\relax{%
  \def\tikz@m@anchor{text}%
  \def\tikz@matrix@shift{\pgfpointanchor{#1}{#2}}%
}
  
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@node@finish%
}


\def\tikz@fig@mustbenamed{%
  \ifx\tikz@fig@name\pgfutil@empty%
    % Assign a dummy name
    \global\advance\tikz@fig@count by1\relax
    \edef\tikz@fig@name{tikz@f@\the\tikz@fig@count}%
  \fi%
}

\def\tikz@node@transformations{
  % 
  % Possibly, we are ``online''
  % 
  \ifx\tikz@time\pgfutil@empty%
    \pgftransformshift{\tikz@node@at}%
    \iftikz@fullytransformed%
    \else%
      \pgftransformresetnontranslations%
    \fi%
  \else%
    \tikz@do@auto@anchor%
    \tikz@timer%
  \fi%
  % Invoke local transformations
  \tikz@transform%
}

\def\tikz@node@finish{%  
    \global\let\tikz@last@fig@name=\tikz@fig@name%
    \global\let\tikz@after@node@smuggle=\tikz@after@node%
    \global\let\tikz@afternodepathoptions@smuggle=\tikz@afternodepathoptions%
    % shift box outside group
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup\endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \pgflinewidth=\tikz@save@line@width%
  \let\tikz@to@last@fig@name=\tikz@last@fig@name%
  \let\tikz@to@use@whom=\tikz@to@use@last@fig@name%
  \let\tikzlastnode=\tikz@last@fig@name%
  \ifx\tikz@after@node@smuggle\pgfutil@empty%
  \else%
    \tikz@scan@next@command{\pgfextra{\tikz@afternodepathoptions@smuggle}\tikz@after@node@smuggle}\pgf@stop%
  \fi%
  \tikz@scan@next@command%
}
\let\tikz@fig@continue@orig=\tikz@fig@continue



% Syntax for parts of  nodes:
% node ... {... \nodepart{name} ... \nodepart{name} ...}

\def\tikz@nodepart#1{%
  \tikz@atend@node%
  \unskip%
  \gdef\tikz@nodepart@name{#1}%
  \global\let\tikz@fig@continue=\tikz@nodepart@continue%
  \pgfutil@ifnextchar x{\egroup\relax}{\egroup\relax}% gobble spaces
}
\def\tikz@nodepart@continue{%
  \global\let\tikz@fig@continue=\tikz@fig@continue@orig%
  % Now start new box:
   \expandafter\setbox\csname pgfnodepart\tikz@nodepart@name box\endcsname=\hbox%
      \bgroup%
        \tikz@every@style{every \tikz@nodepart@name\space node part}%
        \pgfinterruptpicture%
          \tikz@textfont%  
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
            \begingroup%
              \pgfutil@minipage[t]{\tikz@text@width}%
                \tikz@text@action%
          \fi%
          \bgroup%
            \aftergroup\unskip%
            \ifx\tikz@textcolor\pgfutil@empty%
            \else%
              \pgfutil@colorlet{.}{\tikz@textcolor}%
            \fi%
            \pgfsetcolor{.}%
            \setbox\tikz@figbox=\box\voidb@x%
            \tikz@uninstallcommands%
            \tikz@atbegin@node%
            \aftergroup\tikz@fig@collectresetcolor%
            \ignorespaces%
}


% Auto placement

\def\tikz@auto@pre{%
  \begingroup
    \pgfresetnontranslationattimefalse
    \pgfslopedattimetrue%
    \pgfallowupsidedownattimetrue%
    \tikz@timer%
    \pgf@x=\pgf@pt@aa pt% 
    \pgf@y=\pgf@pt@ab pt%
    \pgfpointnormalised{}%
}

\def\tikz@auto@post{%
    \global\let\tikz@anchor@smuggle=\tikz@anchor%
  \endgroup%
  \let\tikz@anchor=\tikz@anchor@smuggle%
}

\def\tikz@auto@anchor{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south west}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north west}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{east}%
      \else%
        \def\tikz@anchor{west}%
      \fi%
    \fi\fi%
}

\def\tikz@auto@anchor@prime{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north east}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south east}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{west}%
      \else%
        \def\tikz@anchor{east}%
      \fi%
    \fi\fi%
}




% Syntax for trees:
% node {...} child [options] {...} child [options] {...} ...
% node {...} child [options] foreach \var in {list} [options] {...} ...

\def\tikz@children{%
  % Start collecting the children:
  \let\tikz@children@list=\pgfutil@empty%
  \tikznumberofchildren=0\relax%
  \tikz@collect@children c}

\def\tikz@collect@children{\pgfutil@ifnextchar c{\tikz@collect@children@cchar}{\tikz@children@collected}}
\def\tikz@collect@children@cchar c{\pgfutil@ifnextchar h{\tikz@collect@child}{\tikz@children@collected c}}
\def\tikz@collect@child hild{\pgfutil@ifnextchar[{\tikz@collect@childA}{\tikz@collect@childA[]}}%}
\def\tikz@collect@childA[#1]{\pgfutil@ifnextchar f{\tikz@collect@children@foreach[#1]}{\tikz@collect@childB[#1]}}
\def\tikz@collect@childB[#1]{%
  \advance\tikznumberofchildren by1\relax
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list \tikz@childnode[#1]}%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@child@code}{\tikz@collect@child@code{}}}
\def\tikz@collect@child@code#1{%
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list{#1}}%
  \tikz@collect@children%
}
\def\tikz@collect@children@foreach[#1]foreach#2in#3{%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@children@foreachA{#1}{#2}{#3}}{\tikz@collect@children@foreachA{#1}{#2}{#3}{}}}
\def\tikz@collect@children@foreachA#1#2#3#4{%
  \expandafter\def\expandafter\tikz@children@list\expandafter
    {\tikz@children@list\tikz@childrennodes[#1]{#2}{#3}{#4}}%
  \c@pgf@counta=\tikznumberofchildren%
  \foreach#2in{#3}%
  {%
    \global\advance\c@pgf@counta by1\relax%
  }%
  \tikznumberofchildren=\c@pgf@counta%
  \tikz@collect@children%
}
\long\def\tikz@children@collected{%
  \begingroup%
    \advance\tikztreelevel by 1\relax%
    \let\tikz@options=\pgfutil@empty%
    \let\tikz@transform=\pgfutil@empty%
    \tikz@every@style{level \the\tikztreelevel}%
    \tikz@transform%            
    \let\tikzparentnode=\tikz@last@fig@name%
    % Transform to center of node
    \pgftransformshift{\pgfpointanchor{\tikzparentnode}{\tikz@growth@anchor}}%
    \tikznumberofcurrentchild=0\relax%
    \tikz@children@list%
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%  
  \tikz@scan@next@command%
}


% Syntax for children:
%
% child [all children options] foreach \var in {values} [child options] {...}
\def\tikz@childrennodes[#1]#2#3#4{%
  \c@pgf@counta=\tikznumberofcurrentchild\relax%
  \setbox\tikz@tempbox=\box\tikz@figbox%
  \foreach#2in{#3}{%
    \tikznumberofcurrentchild=\c@pgf@counta\relax%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \tikz@childnode[#1]{#4}%
    % we must now make the current child number and the figbox survive
    % the group
    \global\c@pgf@counta=\tikznumberofcurrentchild\relax%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
  }%
  \tikznumberofcurrentchild=\c@pgf@counta\relax%
  \setbox\tikz@figbox=\box\tikz@tempbox%
}


% Syntax for child:
%
% child
%
% child[options]
%
% child[options] {node (name) {child node text} ...
%   edge from parent[options] node {label text} node {label text}}

\def\tikz@childnode[#1]#2{%
  \advance\tikznumberofcurrentchild by1\relax%
  \setbox\tikz@figbox=\hbox\bgroup%
    \unhbox\tikz@figbox%
    \hbox\bgroup\bgroup%
        \pgfinterruptpath%
          \pgfscope%
            \let\tikz@transform=\pgfutil@empty%
            \tikz@every@style{every child}%
            \tikz@setkeys{#1}%
            \tikz@options%
            \tikz@transform%            
            \tikz@grow%
            % Typeset node:
            \edef\tikz@parent@node@name{[name=\tikzparentnode-\the\tikznumberofcurrentchild,style=every child node]}%
            \def\tikz@child@node@text{[shape=coordinate]{}}
            \tikz@parse@child@node#2\pgf@stop%
            \expandafter\expandafter\expandafter\node
            \expandafter\tikz@parent@node@name
              \tikz@child@node@text
              \pgfextra{\global\let\tikz@childnode@name=\tikz@last@fig@name};%
            \let\tikzchildnode=\tikz@childnode@name%
            {%
              \def\tikz@edge@to@parent@needed{edge from parent}
              \ifx\tikz@child@node@rest\pgfutil@empty%
                \path edge from parent;%
              \else%
                \path (0,0) \tikz@child@node@rest \tikz@edge@to@parent@needed;%
              \fi%
            }%
        \endpgfscope%
      \endpgfinterruptpath%
    \egroup\egroup%
  \egroup%
}

\def\tikz@parse@child@node{%
  \pgfutil@ifnextchar n{\tikz@parse@child@node@n}%
  {\pgfutil@ifnextchar c{\tikz@parse@child@node@c}%
    {\tikz@parse@child@node@rest}}}
\def\tikz@parse@child@node@rest#1\pgf@stop{\def\tikz@child@node@rest{#1}}
\def\tikz@parse@child@node@c c{\pgfutil@ifnextchar o{\tikz@parse@child@node@co}{\tikz@parse@child@node@rest c}}
\def\tikz@parse@child@node@co o{\pgfutil@ifnextchar o{\tikz@parse@child@node@coordinate}{\tikz@parse@child@node@rest co}}
\def\tikz@parse@child@node@coordinate ordinate{%
  \pgfutil@ifnextchar ({\tikz@@parse@child@node@coordinate}{%
    \def\tikz@child@node@text{[shape=coordinate]{}}%
    \tikz@parse@child@node@rest}}%}
\def\tikz@@parse@child@node@coordinate(#1){%
  \pgfutil@ifnextchar a{\tikz@p@c@n@c@at(#1)}{%
    \def\tikz@child@node@text{[shape=coordinate,name=#1]{}}%
    \tikz@parse@child@node@rest}}
\def\tikz@p@c@n@c@at(#1)at#2(#3){%
  \def\tikz@child@node@text{[shape=coordinate,name=#1]at(#3){}}%
  \tikz@parse@child@node@rest}%
\def\tikz@parse@child@node@n node{%
  \let\tikz@child@node@text=\pgfutil@empty%
  \tikz@p@c@s}%
\def\tikz@p@c@s{%
  \pgfutil@ifnextchar a{\tikz@p@c@s@at}
  {\pgfutil@ifnextchar ({\tikz@p@c@s@paran}
    {\pgfutil@ifnextchar [{\tikz@p@c@s@bra}
      {\pgfutil@ifnextchar \bgroup{\tikz@p@c@s@group}
        {\PackageError{tikz}{Cannot parse this node}{}}}}}}%}}
\def\tikz@p@c@s@at at#1(#2){%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text at(#2)}
  \tikz@p@c@s}
\def\tikz@p@c@s@paran(#1){%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text(#1)}
  \tikz@p@c@s}
\def\tikz@p@c@s@bra[#1]{%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text[#1]}
  \tikz@p@c@s}
\def\tikz@p@c@s@group#1{%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text{#1}}
  \tikz@parse@child@node@rest}


%
% Timers
% 

\def\tikz@timer@line{%
  \pgftransformlineattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@end}%
}

\def\tikz@timer@vhline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%    
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}

\def\tikz@timer@hvline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%    
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}

\def\tikz@timer@curve{%
  \pgftransformcurveattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@cont@one}{\tikz@timer@cont@two}{\tikz@timer@end}%
}



%
% Coordinate systems
% 

\def\tikzdeclarecoordinatesystem#1#2{%
  \expandafter\def\csname tikz@parse@cs@#1\endcsname(##1){%
    \pgf@process{%
      #2%
      % Smuggle outside:
      \iftikz@shapeborder%
        \global\let\tikz@smuggle@a=\tikz@shapebordertrue%
      \else%
        \global\let\tikz@smuggle@a=\tikz@shapeborderfalse%
      \fi%
      \global\let\tikz@smubble@b=\tikz@shapeborder@name%
    }%
    \tikz@smuggle@a%
    \let\tikz@shapeborder@name=\tikz@smubble@b%
    \edef\tikz@return@coordinate{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
}
\def\tikzaliascoordinatesystem#1#2{%
  \edef\pgf@marshal{\noexpand\let\expandafter\noexpand\csname
    tikz@parse@cs@#1\endcsname=\expandafter\noexpand\csname
    tikz@parse@cs@#2\endcsname}%
  \pgf@marshal%
}


% Default coodinate systems:

\tikzdeclarecoordinatesystem{canvas}
{%
  \tikz@orig@setkeys{tikzcskeys}{x=0pt,y=0pt,#1}%
  \pgfpoint{\tikz@cs@x}{\tikz@cs@y}%
}

\tikzdeclarecoordinatesystem{canvas polar}
{%
  \tikz@orig@setkeys{tikzcskeys}{angle=0,radius=0cm,#1}%
  \pgfpointpolar{\tikz@cs@angle}{\tikz@cs@xradius/\tikz@cs@yradius}%
}

\tikzdeclarecoordinatesystem{xyz}
{%
  \tikz@orig@setkeys{tikzcskeys}{x=0,y=0,z=0,#1}%
  \pgfpointxyz{\tikz@cs@x}{\tikz@cs@y}{\tikz@cs@z}%
}

\tikzdeclarecoordinatesystem{xyz polar}
{%
  \tikz@orig@setkeys{tikzcskeys}{angle=0,radius=0,#1}%
  \pgfpointpolarxy{\tikz@cs@angle}{\tikz@cs@xradius and \tikz@cs@yradius}%
}
\tikzaliascoordinatesystem{xy polar}{xyz polar}


\tikzdeclarecoordinatesystem{node}
{%
  \tikz@orig@setkeys{tikzcskeys}{name=,anchor=none,angle=none,#1}%
  \ifx\tikz@cs@anchor\tikz@nonetext%
    \ifx\tikz@cs@angle\tikz@nonetext%
      \expandafter\ifx\csname pgf@sh@ns@\tikz@cs@node\endcsname\tikz@coordinate@text%
      \else
        \tikz@shapebordertrue%
        \edef\tikz@shapeborder@name{\tikz@cs@node}%
      \fi%
      \pgfpointanchor{\tikz@cs@node}{center}%
    \else%
      \pgfpointanchor{\tikz@cs@node}{\tikz@cs@angle}%
    \fi%
  \else%
    \pgfpointanchor{\tikz@cs@node}{\tikz@cs@anchor}%
  \fi%
}

\tikzdeclarecoordinatesystem{intersection}
{%
  \tikz@orig@setkeys{tikzcskeys}{#1}%
  \expandafter\tikz@@@scan@@absolute\expandafter\tikz@parse@intersection@a\tikz@cs@line@a@begin%
  \expandafter\tikz@@@scan@@absolute\expandafter\tikz@parse@intersection@b\tikz@cs@line@a@end%
  \expandafter\tikz@@@scan@@absolute\expandafter\tikz@parse@intersection@c\tikz@cs@line@b@begin%
  \expandafter\tikz@@@scan@@absolute\expandafter\tikz@parse@intersection@d\tikz@cs@line@b@end%
  \edef\pgf@marshal{%
    {\noexpand\pgfpointintersectionoflines%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}}%
  \pgf@marshal%
}

\tikzdeclarecoordinatesystem{perpendicular}
{%
  \tikz@orig@setkeys{tikzcskeys}{#1}%
  \expandafter\tikz@@@scan@@absolute\expandafter\tikz@parse@intersection@a\tikz@cs@hori@line%
  \expandafter\tikz@@@scan@@absolute\expandafter\tikz@parse@intersection@b\tikz@cs@vert@line%
  \pgfqpoint{\the\pgf@xb}{\the\pgf@ya}
}

\tikzdeclarecoordinatesystem{barycentric}
{%
  {%
    \pgf@xa=0pt% point
    \pgf@ya=0pt%
    \pgf@xb=0pt% sum
    \tikz@bary@dolist#1,=,%
    \pgfmathparse{1/\the\pgf@xb}%
    \global\pgf@x=\pgfmathresult\pgf@xa%
    \global\pgf@y=\pgfmathresult\pgf@ya%
  }%
}

\def\tikz@bary@dolist#1=#2,{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else
    \pgf@process{\pgfpointanchor{#1}{center}}%
    \pgfmathparse{#2}%
    \advance\pgf@xa by\pgfmathresult\pgf@x%
    \advance\pgf@ya by\pgfmathresult\pgf@y%
    \advance\pgf@xb by\pgfmathresult pt%
    \expandafter\tikz@bary@dolist%
  \fi%
}


\tikz@orig@define@key{tikzcskeys}{x}{\def\tikz@cs@x{#1}}
\tikz@orig@define@key{tikzcskeys}{y}{\def\tikz@cs@y{#1}}
\tikz@orig@define@key{tikzcskeys}{z}{\def\tikz@cs@z{#1}}
\tikz@orig@define@key{tikzcskeys}{angle}{\def\tikz@cs@angle{#1}}
\tikz@orig@define@key{tikzcskeys}{radius}{\def\tikz@cs@xradius{#1}\def\tikz@cs@yradius{#1}}
\tikz@orig@define@key{tikzcskeys}{x radius}{\def\tikz@cs@xradius{#1}}
\tikz@orig@define@key{tikzcskeys}{y radius}{\def\tikz@cs@yradius{#1}}
\tikz@orig@define@key{tikzcskeys}{name}{\def\tikz@cs@node{#1}}
\tikz@orig@define@key{tikzcskeys}{anchor}{\def\tikz@cs@anchor{#1}}

\tikz@orig@define@key{tikzcskeys}{first line}{\tikz@parse@cs@line{tikz@cs@line@a}#1}
\tikz@orig@define@key{tikzcskeys}{second line}{\tikz@parse@cs@line{tikz@cs@line@b}#1}

\def\tikz@parse@cs@line#1(#2)--(#3){%
  \expandafter\def\csname #1@begin\endcsname{(#2)}%
  \expandafter\def\csname #1@end\endcsname{(#3)}%
}

\tikz@orig@define@key{tikzcskeys}{horizontal line through}{\def\tikz@cs@hori@line{#1}}
\tikz@orig@define@key{tikzcskeys}{vertical line through}{\def\tikz@cs@vert@line{#1}}




%
% Coordinate management
%


% Last position visited
\def\tikz@last@position{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}
\def\tikz@last@position@saved{\pgfqpoint{\tikz@lastxsaved}{\tikz@lastysaved}}

% Make given point the last position visited
\def\tikz@make@last@position#1{%
  \pgf@process{#1}%
  \tikz@lastx=\pgf@x\relax%
  \tikz@lasty=\pgf@y\relax%
  \iftikz@updatecurrent%
    \tikz@lastxsaved=\pgf@x\relax%
    \tikz@lastysaved=\pgf@y\relax%
  \fi%
  \tikz@updatecurrenttrue%
}

\newif\iftikz@updatecurrent
\tikz@updatecurrenttrue



% Scanner: Scans a point or a relative point. 
% It then calls the first parameter with the argument set to an
% appropriate pgf command representing that point.

\def\tikz@scan@one@point#1{%
  \let\tikz@to@use@whom=\tikz@to@use@last@coordinate%
  \tikz@shapeborderfalse%
  \pgfutil@ifnextchar+{\tikz@scan@relative#1}{\tikz@scan@absolute#1}}
\def\tikz@scan@absolute#1{%
  \pgfutil@ifnextchar({\tikz@scan@@absolute#1}%)
  {%
    \advance\tikz@expandcount by -1%
    \ifnum\tikz@expandcount<0\relax%
      \let\@next=\tikz@@scangiveup%
    \else%
      \let\@next=\tikz@@scanexpand%
    \fi%
    \@next{#1}%
  }%
}
\def\tikz@@scanexpand#1{\expandafter\tikz@scan@one@point\expandafter#1}
\def\tikz@@scangiveup#1{\PackageError{tikz}{Cannot parse this coordinate}{}#1{\pgfpointorigin}}
\def\tikz@scan@@absolute#1(#2){%
  \edef\tikz@temp{(#2)}%
  \expandafter\tikz@@scan@@absolute\expandafter#1\tikz@temp%
}
\def\tikz@@scan@@absolute#1({%
  \pgfutil@ifnextchar[% uhoh... options!
  {\def\tikz@scan@point@recall{#1}\tikz@scan@options}%
  {\tikz@@@scan@@absolute#1(}%
}

\def\tikz@scan@options[#1]#2{%
  \def\tikz@scan@point@options{#1}%
  \tikz@@@scan@@absolute\tikz@scan@handle@options(#2%
}

\def\tikz@scan@handle@options#1{%
  {%
    % Ok, compute point with options set and zero transformation
    % matrix:
    \pgftransformreset%
    \let\tikz@transform=\pgfutil@empty%
    \expandafter\tikz@setkeys\expandafter{\tikz@scan@point@options}%
    \tikz@transform%
    \pgf@process{\pgfpointtransformed{#1}}%
    \xdef\tikz@marshal{\expandafter\noexpand\tikz@scan@point@recall{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  }%
  \tikz@marshal%  
}

\def\tikz@@@scan@@absolute#1(#2){%
  \pgfutil@in@{intersection of}{#2}%
  \ifpgfutil@in@%
    \let\@next\tikz@parse@intersection%
  \else%
    \pgfutil@in@|{#2}%
    \ifpgfutil@in@
      \pgfutil@in@{-|}{#2}%
      \ifpgfutil@in@
        \let\@next\tikz@parse@hv%
      \else%
        \let\@next\tikz@parse@vh%
      \fi%
    \else%
      \pgfutil@in@{cs:}{#2}%
      \ifpgfutil@in@%
        \let\@next\tikz@parse@coordinatesystem%
      \else%
        \pgfutil@in@:{#2}%
        \ifpgfutil@in@
          \let\@next\tikz@parse@polar%
        \else%
          \pgfutil@in@,{#2}%
          \ifpgfutil@in@%      
            \let\@next\tikz@parse@regular%
          \else%
            \let\@next\tikz@parse@node%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \@next#1(#2)%
}

\def\tikz@parse@coordinatesystem#1(#2 cs:#3){%
  \let\tikz@return@coordinate=\pgfpointorigin%
  \pgfutil@ifundefined{tikz@parse@cs@#2}
  {\PackageError{tikz}{Unknown coordinate system '#2'}{}}
  {\csname tikz@parse@cs@#2\endcsname(#3)}%
  \expandafter#1\expandafter{\tikz@return@coordinate}%
}


\newif\iftikz@isdimension
\def\tikz@checkunit#1{%
  \pgfmathparse{#1}%
  \let\iftikz@isdimension=\ifpgfmathunitsdeclared%
}
\def\tikz@@checkunit{\pgfutil@ifnextchar\tikz@unique{\tikz@checkunit@number}{\tikz@checkunit@dimension}}
\def\tikz@checkunit@number\tikz@unique{\tikz@isdimensionfalse}
\def\tikz@checkunit@dimension#1\tikz@unique{\tikz@isdimensiontrue}

\def\tikz@parse@polar#1(#2:#3){%
  \pgfutil@ifundefined{tikz@polar@dir@#2}
  {\tikz@@parse@polar#1(#2:#3)}
  {\tikz@@parse@polar#1(\csname tikz@polar@dir@#2\endcsname:#3)}%
}
\def\tikz@@parse@polar#1(#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@%
    \edef\tikz@args{(#2:#3)}%
  \else%
    \edef\tikz@args{(#2:#3 and #3)}%
  \fi%
  \expandafter\tikz@@@parse@polar\expandafter#1\tikz@args%
}
\def\tikz@@@parse@polar#1(#2:#3 and #4){%
  \tikz@checkunit{#3}%
  \iftikz@isdimension%
    \def\tikz@next{#1{\pgfpointpolar{#2}{#3 and #4}}}%
  \else%
    \def\tikz@next{#1{\pgfpointpolarxy{#2}{#3 and #4}}}%
  \fi%
  \tikz@next%
}
\def\tikz@polar@dir@up{90}
\def\tikz@polar@dir@down{-90}
\def\tikz@polar@dir@left{180}
\def\tikz@polar@dir@right{0}
\def\tikz@polar@dir@north{90}
\def\tikz@polar@dir@south{-90}
\def\tikz@polar@dir@east{0}
\def\tikz@polar@dir@west{180}
\expandafter\def\csname tikz@polar@dir@north east\endcsname{45}
\expandafter\def\csname tikz@polar@dir@north west\endcsname{135}
\expandafter\def\csname tikz@polar@dir@south east\endcsname{-45}
\expandafter\def\csname tikz@polar@dir@south west\endcsname{-135}

\def\tikz@parse@regular#1(#2,#3){%
  \pgfutil@in@,{#3}%
  \ifpgfutil@in@%  
    \tikz@parse@splitxyz{#1}{#2}#3,%
  \else%
    \tikz@checkunit{#2}%
    \iftikz@isdimension%
      \def\@next{#1{\pgfpoint{#2}{#3}}}%
    \else%
      \def\@next{#1{\pgfpointxy{#2}{#3}}}%
    \fi%
  \fi%
  \@next%
}

\def\tikz@parse@splitxyz#1#2#3,#4,{%
  \def\@next{#1{\pgfpointxyz{#2}{#3}{#4}}}%
}

\def\tikz@coordinate@text{coordinate}

\def\tikz@parse@node#1(#2){%
  \pgfutil@in@.{#2}% Ok, flag this
  \ifpgfutil@in@
    \tikz@calc@anchor#2\tikz@stop%
  \else%
    \tikz@calc@anchor#2.center\tikz@stop% to be on the save side, in
                                % case iftikz@shapeborder is ignored...
    \expandafter\ifx\csname pgf@sh@ns@#2\endcsname\tikz@coordinate@text%
    \else
      \tikz@shapebordertrue%
      \def\tikz@shapeborder@name{#2}%
    \fi%
  \fi%
  \edef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \tikz@marshal%
}

\def\tikz@calc@anchor#1.#2\tikz@stop{%
  \pgfpointanchor{#1}{#2}%
}


\def\tikz@parse@hv#1(#2){%
  \pgfutil@in@{ -| }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@hvboth%
  \else%
    \pgfutil@in@{ -|}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@hvleft%
    \else%
      \pgfutil@in@{-| }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@hvright%
      \else%
        \let\tikz@next=\tikz@parse@hvdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}
\def\tikz@parse@hvboth#1(#2 -| #3){\tikz@parse@vhdone#1(#3|-#2)}
\def\tikz@parse@hvleft#1(#2 -|#3){\tikz@parse@vhdone#1(#3|-#2)}
\def\tikz@parse@hvright#1(#2-| #3){\tikz@parse@vhdone#1(#3|-#2)}
\def\tikz@parse@hvdone#1(#2-|#3){\tikz@parse@vhdone#1(#3|-#2)}

\def\tikz@parse@vh#1(#2){%
  \pgfutil@in@{ |- }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@vhboth%
  \else%
    \pgfutil@in@{ |-}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@vhleft%
    \else%
      \pgfutil@in@{|- }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@vhright%
      \else%
        \let\tikz@next=\tikz@parse@vhdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}
\def\tikz@parse@vhboth#1(#2 |- #3){\tikz@parse@vhdone#1(#2|-#3)}
\def\tikz@parse@vhleft#1(#2 |-#3){\tikz@parse@vhdone#1(#2|-#3)}
\def\tikz@parse@vhright#1(#2|- #3){\tikz@parse@vhdone#1(#2|-#3)}
\def\tikz@parse@vhdone#1(#2|-#3){%
  {%
    \tikz@@@scan@@absolute\tikz@parse@vh@mid(#2)%
    \tikz@@@scan@@absolute\tikz@parse@vh@end(#3)%
    \xdef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  }%
  \tikz@shapeborderfalse%
  \tikz@marshal%
}
\def\tikz@parse@vh@mid#1{\pgf@process{#1}\pgf@xa=\pgf@x}
\def\tikz@parse@vh@end#1{\pgf@process{#1}\pgf@ya=\pgf@y}

\def\tikz@parse@intersection#1(intersection of #2--#3 and #4--#5){%
  {%
    \tikz@@@scan@@absolute\tikz@parse@intersection@a(#2)%
    \tikz@@@scan@@absolute\tikz@parse@intersection@b(#3)%
    \tikz@@@scan@@absolute\tikz@parse@intersection@c(#4)%
    \tikz@@@scan@@absolute\tikz@parse@intersection@d(#5)%
    \xdef\tikz@marshal{\noexpand#1{\noexpand\pgfpointintersectionoflines%
        {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
        {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}}%
  }%
  \tikz@shapeborderfalse%
  \tikz@marshal%  
}

\def\tikz@parse@intersection@a#1{\pgf@process{#1}\pgf@xa=\pgf@x\pgf@ya=\pgf@y}
\def\tikz@parse@intersection@b#1{\pgf@process{#1}\pgf@xb=\pgf@x\pgf@yb=\pgf@y}
\def\tikz@parse@intersection@c#1{\pgf@process{#1}\pgf@xc=\pgf@x\pgf@yc=\pgf@y}
\def\tikz@parse@intersection@d#1{\pgf@process{#1}}

\def\tikz@scan@relative#1+{%
  \pgfutil@ifnextchar+{\tikz@scan@plusplus#1}{\tikz@scan@oneplus#1}}

\def\tikz@scan@plusplus#1+{%
  \def\tikz@doafter{#1}%
  \tikz@scan@absolute\tikz@add%
}
\def\tikz@add#1{%
  \tikz@doafter{\pgfpointadd{#1}{\tikz@last@position@saved}}%
}
\def\tikz@scan@oneplus#1{%
  \def\tikz@doafter{#1}%
  \tikz@updatecurrentfalse%
  \tikz@scan@absolute\tikz@add%
} 



% Loading further libraries

% Include a library file.
%
% #1 = List of names of library file.
%  
% Description:
%
% This command includes a list of TikZ library files. For each file X in the
% list, the file pgflibrarytikzX.code.tex is included, provided this has
% not been done earlier. 
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usetikzlibrary{arrows}
% \usetikzlibrary[patterns,topaths]

\def\usetikzlibrary{\pgfutil@ifnextchar[{\use@tikzlibrary}{\use@@tikzlibrary}}%}
\def\use@tikzlibrary[#1]{\use@@tikzlibrary{#1}}
\def\use@@tikzlibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname tikz@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikz@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikz@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikz@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \input pgflibrarytikz\pgf@temp.code.tex
      \catcode`\@=\csname tikz@library@#1@atcode\endcsname
      \catcode`\|=\csname tikz@library@#1@barcode\endcsname
    \fi%
  }%
}


% Always-present libraries:

\usetikzlibrary{topaths}




\endinput


==> xkeyval.tex <==
%%
%% This is file `xkeyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvtex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2005 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, pst-xkey.tex, pst-xkey.sty, xkveca.cls, xkvecb.cls,
%% xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex, xkvex2.tex,
%% xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValLoaded\endcsname
\let\XKeyValLoaded\endinput
\edef\XKVcatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \catcode`\noexpand\=\the\catcode`\=\relax
  \catcode`\noexpand\,\the\catcode`\,\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \let\noexpand\XKVcatcodes\relax
}
\catcode`\@11\relax
\catcode`\=12\relax
\catcode`\,12\relax
\catcode`\:12\relax
\newtoks\XKV@toks
\newcount\XKV@depth
\newif\ifXKV@st
\newif\ifXKV@sg
\newif\ifXKV@pl
\newif\ifXKV@knf
\newif\ifXKV@rkv
\newif\ifXKV@inpox
\newif\ifXKV@preset
\let\XKV@rm\@empty
\ifx\ProvidesFile\@undefined
  \message{2005/11/25 v2.5e key=value parser (HA)}
  \input xkvtxhdr
\else
  \ProvidesFile{xkeyval.tex}[2005/11/25 v2.5e key=value parser (HA)]
  \@addtofilelist{xkeyval.tex}
\fi
\long\def\@firstoftwo#1#2{#1}
\long\def\@secondoftwo#1#2{#2}
\long\def\XKV@afterfi#1\fi{\fi#1}
\long\def\XKV@afterelsefi#1\else#2\fi{\fi#1}
\ifx\ifcsname\@undefined\XKV@afterelsefi
  \def\XKV@ifundefined#1{%
    \begingroup\expandafter\expandafter\expandafter\endgroup
      \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\@firstoftwo
    \else
      \expandafter\@secondoftwo
    \fi
  }
\else
  \def\XKV@ifundefined#1{%
    \ifcsname#1\endcsname
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }
\fi
\XKV@ifundefined{ver@keyval.sty}{
  \input keyval
  \expandafter\def\csname ver@keyval.sty\endcsname{1999/03/16}
}{}
\long\def\@ifnextcharacter#1#2#3{%
  \@ifnextchar\bgroup
  {\@ifnextchar{#1}{#2}{#3}}%
  {\@ifncharacter{#1}{#2}{#3}}%
}
\long\def\@ifncharacter#1#2#3#4{%
  \if\string#1\string#4%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#2}{#3}#4%
}
\long\def\XKV@for@n#1#2#3{%
  \def#2{#1}%
  \ifx#2\@empty
    \XKV@for@break
  \else
    \expandafter\XKV@f@r
  \fi
  #2{#3}#1,\@nil,%
}
\long\def\XKV@f@r#1#2#3,{%
  \def#1{#3}%
  \ifx#1\@nnil
    \expandafter\@gobbletwo
  \else
    #2\expandafter\XKV@f@r
  \fi
  #1{#2}%
}
\long\def\XKV@for@break #1\@nil,{\fi}
\long\def\XKV@for@o#1{\expandafter\XKV@for@n\expandafter{#1}}
\long\def\XKV@for@en#1#2#3{\XKV@f@r#2{#3}#1,\@nil,}
\long\def\XKV@for@eo#1#2#3{%
  \def#2{\XKV@f@r#2{#3}}\expandafter#2#1,\@nil,%
}
\long\def\XKV@whilist#1#2#3\fi#4{%
  #3\expandafter\XKV@wh@list#1,\@nil,\@nil\@@#2#3\fi{#4}{}\fi
}
\long\def\XKV@wh@list#1,#2\@@#3#4\fi#5#6{%
  \def#3{#1}%
  \ifx#3\@nnil
    \def#3{#6}\expandafter\XKV@wh@l@st
  \else
    #4%
      #5\expandafter\expandafter\expandafter\XKV@wh@list
    \else
      \def#3{#6}\expandafter\expandafter\expandafter\XKV@wh@l@st
    \fi
  \fi
  #2\@@#3#4\fi{#5}{#1}%
}
\long\def\XKV@wh@l@st#1\@@#2#3\fi#4#5{}
\def\XKV@addtomacro@n#1#2{%
  \expandafter\def\expandafter#1\expandafter{#1#2}%
}
\def\XKV@addtomacro@o#1#2{%
  \expandafter\expandafter\expandafter\def
    \expandafter\expandafter\expandafter#1\expandafter
    \expandafter\expandafter{\expandafter#1#2}%
}
\def\XKV@addtolist@n#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@n#1{#2}%
  \else
    \XKV@addtomacro@n#1{,#2}%
  \fi
}
\def\XKV@addtolist@o#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@o#1#2%
  \else
    \XKV@addtomacro@o#1{\expandafter,#2}%
  \fi
}
\def\XKV@addtolist@x#1#2{\edef#1{#1\ifx#1\@empty\else,\fi#2}}
\def\@selective@sanitize{\@testopt\@s@lective@sanitize\@M}
\def\@s@lective@sanitize[#1]#2#3{%
  \begingroup
    \count@#1\relax\advance\count@\@ne
    \XKV@toks\expandafter{#3}%
    \def#3{#2}\@onelevel@sanitize#3%
    \edef#3{{#3}{\the\XKV@toks}}%
    \expandafter\@s@l@ctive@sanitize\expandafter#3#3%
  \expandafter\endgroup\expandafter\def\expandafter#3\expandafter{#3}%
}
\def\@s@l@ctive@sanitize#1#2#3{%
  \def\@i{\futurelet\@@tok\@ii}%
  \def\@ii{%
    \expandafter\@iii\meaning\@@tok\relax
    \ifx\@@tok\@s@l@ctive@sanitize
      \let\@@cmd\@gobble
    \else
      \ifx\@@tok\@sptoken
        \XKV@toks\expandafter{#1}\edef#1{\the\XKV@toks\space}%
        \def\@@cmd{\afterassignment\@i\let\@@tok= }%
      \else
        \let\@@cmd\@iv
      \fi
    \fi
    \@@cmd
  }%
  \def\@iii##1##2\relax{\if##1\@backslashchar\let\@@tok\relax\fi}%
  \def\@iv##1{%
    \toks@\expandafter{#1}\XKV@toks{##1}%
    \ifx\@@tok\bgroup
      \advance\count@\m@ne
      \ifnum\count@>\z@
        \begingroup
          \def#1{\expandafter\@s@l@ctive@sanitize
            \csname\string#1\endcsname{#2}}%
          \expandafter#1\expandafter{\the\XKV@toks}%
          \XKV@toks\expandafter\expandafter\expandafter
            {\csname\string#1\endcsname}%
          \edef#1{\noexpand\XKV@toks{\the\XKV@toks}}%
        \expandafter\endgroup#1%
      \fi
      \edef#1{\the\toks@{\the\XKV@toks}}%
      \advance\count@\@ne
      \let\@@cmd\@i
    \else
      \edef#1{\expandafter\string\the\XKV@toks}%
      \expandafter\in@\expandafter{#1}{#2}%
      \edef#1{\the\toks@\ifin@#1\else
              \ifx\@@tok\@sptoken\space\else\the\XKV@toks\fi\fi}%
      \edef\@@cmd{\noexpand\@i\ifx\@@tok\@sptoken\the\XKV@toks\fi}%
    \fi
    \@@cmd
  }%
  \let#1\@empty\@i#3\@s@l@ctive@sanitize
}
\def\XKV@checksanitizea#1#2{%
  \XKV@ch@cksanitize{#1}#2=%
  \ifin@\else\XKV@ch@cksanitize{#1}#2,\fi
  \ifin@\@selective@sanitize[0]{,=}#2\fi
}
\def\XKV@checksanitizeb#1#2{%
  \XKV@ch@cksanitize{#1}#2,%
  \ifin@\@selective@sanitize[0],#2\fi
}
\def\XKV@ch@cksanitize#1#2#3{%
  \def#2{#1}%
  \@onelevel@sanitize#2%
  \@expandtwoargs\in@#3{#2}%
  \ifin@
    \def#2##1#3##2\@nil{%
      \def#2{##2}%
      \ifx#2\@empty\else\in@false\fi
    }%
    #2#1#3\@nil
  \fi
  \def#2{#1}%
}
\def\XKV@sp@deflist#1#2{%
  \let#1\@empty
  \XKV@for@n{#2}\XKV@resa{%
    \expandafter\KV@@sp@def\expandafter\XKV@resa\expandafter{\XKV@resa}%
    \XKV@addtomacro@o#1{\expandafter,\XKV@resa}%
  }%
  \ifx#1\@empty\else
    \def\XKV@resa,##1\@nil{\def#1{##1}}%
    \expandafter\XKV@resa#1\@nil
  \fi
}
\def\XKV@merge#1#2#3{%
  \XKV@checksanitizea{#2}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@pltrue
    #3\XKV@tempa\XKV@tempb
    \let\XKV@tempc#1%
    \let#1\@empty
    \XKV@for@o\XKV@tempc\XKV@tempc{%
      #3\XKV@tempc\XKV@tempd
      \ifx\XKV@tempb\XKV@tempd
        \XKV@plfalse
        \XKV@addtolist@o#1\XKV@tempa
      \else
        \XKV@addtolist@o#1\XKV@tempc
      \fi
    }%
    \ifXKV@pl\XKV@addtolist@o#1\XKV@tempa\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@delete#1#2#3{%
  \XKV@checksanitizeb{#2}\XKV@tempa
  \let\XKV@tempb#1%
  \let#1\@empty
  \XKV@for@o\XKV@tempb\XKV@tempb{%
    #3\XKV@tempb\XKV@tempc
    \@expandtwoargs\in@{,\XKV@tempc,}{,\XKV@tempa,}%
    \ifin@\else\XKV@addtolist@o#1\XKV@tempb\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@warn#1{\message{xkeyval warning: #1}}
\def\XKV@err#1{\errmessage{xkeyval error: #1}}
\def\KV@errx{\XKV@err}
\let\KV@err\KV@errx
\def\XKV@ifstar#1{\@ifnextcharacter*{\@firstoftwo{#1}}}
\def\XKV@ifplus#1{\@ifnextcharacter+{\@firstoftwo{#1}}}
\def\XKV@makepf#1{%
  \KV@@sp@def\XKV@prefix{#1}%
  \def\XKV@resa{XKV}%
  \ifx\XKV@prefix\XKV@resa
    \XKV@err{`XKV' prefix is not allowed}%
    \let\XKV@prefix\@empty
  \else
    \edef\XKV@prefix{\ifx\XKV@prefix\@empty\else\XKV@prefix @\fi}%
  \fi
}
\def\XKV@makehd#1{%
  \expandafter\KV@@sp@def\expandafter\XKV@header\expandafter{#1}%
  \edef\XKV@header{%
    \XKV@prefix\ifx\XKV@header\@empty\else\XKV@header @\fi
  }%
}
\def\XKV@srstate#1#2{%
  \ifx\@empty#2\@empty\advance\XKV@depth\@ne\fi
  \XKV@for@n{XKV@prefix,XKV@fams,XKV@na,ifXKV@st,ifXKV@pl,ifXKV@knf}%
    \XKV@resa{\expandafter\let\csname\XKV@resa#1\expandafter
      \endcsname\csname\XKV@resa#2\endcsname
  }%
  \ifx\@empty#1\@empty\advance\XKV@depth\m@ne\fi
}
\def\XKV@testopta#1{%
  \XKV@ifstar{\XKV@sttrue\XKV@t@stopta{#1}}%
    {\XKV@stfalse\XKV@t@stopta{#1}}%
}
\def\XKV@t@stopta#1{\XKV@ifplus{\XKV@pltrue#1}{\XKV@plfalse#1}}
\def\XKV@testoptb#1{\@testopt{\XKV@t@stoptb#1}{KV}}
\def\XKV@t@stoptb#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@makehd{#3}%
  \KV@@sp@def\XKV@tfam{#3}%
  #1%
}
\def\XKV@testoptc#1{\@testopt{\XKV@t@stoptc#1}{KV}}
\def\XKV@t@stoptc#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@checksanitizeb{#3}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \@testopt#1{}%
}
\def\XKV@testoptd#1#2{%
  \XKV@testoptb{%
    \edef\XKV@tempa{#2\XKV@header}%
    \def\XKV@tempb{\@testopt{\XKV@t@stoptd#1}}%
    \expandafter\XKV@tempb\expandafter{\XKV@tempa}%
  }%
}
\def\XKV@t@stoptd#1[#2]#3{%
  \@ifnextchar[{\XKV@sttrue#1{#2}{#3}}{\XKV@stfalse#1{#2}{#3}[]}%
}
\def\XKV@ifcmd#1#2#3{%
  \def\XKV@@ifcmd##1#2##2##3\@nil##4{%
    \def##4{##2}\ifx##4\@nnil
      \def##4{##1}\expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \XKV@@ifcmd#1#2{\@nil}\@nil#3%
}
\def\XKV@getkeyname#1#2{\expandafter\XKV@g@tkeyname#1=\@nil#2}
\def\XKV@g@tkeyname#1=#2\@nil#3{%
  \XKV@ifcmd{#1}\savevalue#3{\XKV@rkvtrue\XKV@sgfalse}{%
    \XKV@ifcmd{#1}\gsavevalue#3%
      {\XKV@rkvtrue\XKV@sgtrue}{\XKV@rkvfalse\XKV@sgfalse}%
  }%
}
\def\XKV@getsg#1#2{%
  \expandafter\XKV@ifcmd\expandafter{#1}\global#2\XKV@sgtrue\XKV@sgfalse
}
\def\XKV@define@default#1#2{%
  \expandafter\def\csname\XKV@header#1@default\expandafter
    \endcsname\expandafter{\csname\XKV@header#1\endcsname{#2}}%
}
\def\define@key{\XKV@testoptb\XKV@define@key}
\def\XKV@define@key#1{%
  \@ifnextchar[{\XKV@d@fine@k@y{#1}}{%
    \expandafter\def\csname\XKV@header#1\endcsname####1%
  }%
}
\def\XKV@d@fine@k@y#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \expandafter\def\csname\XKV@header#1\endcsname##1%
}
\def\define@cmdkey{\XKV@testoptd\XKV@define@cmdkey{cmd}}
\def\XKV@define@cmdkey#1#2[#3]#4{%
  \ifXKV@st\XKV@define@default{#2}{#3}\fi
  \def\XKV@tempa{\expandafter\def\csname\XKV@header#2\endcsname####1}%
  \begingroup\expandafter\endgroup\expandafter\XKV@tempa\expandafter
    {\expandafter\def\csname#1#2\endcsname{##1}#4}%
}
\def\define@cmdkeys{\XKV@testoptd\XKV@define@cmdkeys{cmd}}
\def\XKV@define@cmdkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \edef\XKV@tempa{\noexpand\XKV@define@cmdkey{#1}{\XKV@tempa}}%
    \XKV@tempa[#3]{}%
  }%
}
\def\define@choicekey{\XKV@testopta{\XKV@testoptb\XKV@define@choicekey}}
\def\XKV@define@choicekey#1{\@testopt{\XKV@d@fine@choicekey{#1}}{}}
\def\XKV@d@fine@choicekey#1[#2]#3{%
  \toks@{#2}%
  \XKV@sp@deflist\XKV@tempa{#3}\XKV@toks\expandafter{\XKV@tempa}%
  \@ifnextchar[{\XKV@d@fine@ch@icekey{#1}}{\XKV@d@fine@ch@ic@key{#1}}%
}
\def\XKV@d@fine@ch@icekey#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \XKV@d@fine@ch@ic@key{#1}%
}
\def\XKV@d@fine@ch@ic@key#1{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@ch@ic@k@y
  \else\XKV@afterfi
    \expandafter\XKV@d@f@ne@ch@ic@key
  \fi
  \csname\XKV@header#1\endcsname
}
\def\XKV@d@f@ne@ch@ic@key#1#2{\XKV@d@f@n@@ch@ic@k@y#1{{#2}}}
\def\XKV@d@f@ne@ch@ic@k@y#1#2#3{\XKV@d@f@n@@ch@ic@k@y#1{{#2}{#3}}}
\def\XKV@d@f@n@@ch@ic@k@y#1#2{%
  \edef#1##1{%
    \ifXKV@st\noexpand\XKV@sttrue\else\noexpand\XKV@stfalse\fi
    \ifXKV@pl\noexpand\XKV@pltrue\else\noexpand\XKV@plfalse\fi
    \noexpand\XKV@checkchoice[\the\toks@]{##1}{\the\XKV@toks}%
  }%
  \def\XKV@tempa{\def#1####1}%
  \expandafter\XKV@tempa\expandafter{#1{##1}#2}%
}
\def\define@boolkey{\XKV@t@stopta{\XKV@testoptd\XKV@define@boolkey{}}}
\def\XKV@define@boolkey#1#2[#3]{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@boolkey
  \else\XKV@afterfi
    \expandafter\XKV@d@fine@boolkey
  \fi
  \csname\XKV@header#2\endcsname{#2}{#1#2}{#3}%
}
\def\XKV@d@fine@boolkey#1#2#3#4#5{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}}%
}
\def\XKV@d@f@ne@boolkey#1#2#3#4#5#6{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}{#6}}%
}
\def\XKV@d@f@ne@b@olkey#1#2#3#4#5{%
  \expandafter\newif\csname if#3\endcsname
  \ifXKV@st\XKV@define@default{#2}{#4}\fi
  \ifXKV@pl
    \def#1##1{\XKV@pltrue\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \else
    \def#1##1{\XKV@plfalse\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \fi
}
\def\define@boolkeys{\XKV@plfalse\XKV@testoptd\XKV@define@boolkeys{}}
\def\XKV@define@boolkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \expandafter\XKV@d@fine@boolkeys\expandafter{\XKV@tempa}{#1}{#3}%
  }%
}
\def\XKV@d@fine@boolkeys#1#2#3{%
  \expandafter\XKV@d@f@ne@b@olkey\csname\XKV@header#1\endcsname
    {#1}{#2#1}{#3}{{\csname#2#1\XKV@resa\endcsname}}%
}
\def\XKV@cc{\XKV@testopta{\@testopt\XKV@checkchoice{}}}
\def\XKV@checkchoice[#1]#2#3{%
  \def\XKV@tempa{#1}%
  \ifXKV@st\lowercase{\fi
  \ifx\XKV@tempa\@empty
    \def\XKV@tempa{\XKV@ch@ckch@ice\@nil{#2}{#3}}%
  \else
    \def\XKV@tempa{\XKV@ch@ckchoice#1\@nil{#2}{#3}}%
  \fi
  \ifXKV@st}\fi\XKV@tempa
}
\def\XKV@ch@ckchoice#1#2\@nil#3#4{%
  \def\XKV@tempa{#2}%
  \ifx\XKV@tempa\@empty\XKV@afterelsefi
    \XKV@ch@ckch@ice#1{#3}{#4}%
  \else\XKV@afterfi
    \XKV@@ch@ckchoice#1#2{#3}{#4}%
  \fi
}
\def\XKV@ch@ckch@ice#1#2#3{%
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
  \in@{,#2,}{,#3,}%
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}
\def\XKV@@ch@ckchoice#1#2#3#4{%
  \edef\XKV@tempa{\the\count@}\count@\z@
  \def\XKV@tempb{#3}%
  \def\XKV@tempc##1,{%
    \def#1{##1}%
    \ifx#1\@nnil
      \def#1{#3}\def#2{-1}\count@\XKV@tempa
      \ifXKV@pl
        \let\XKV@tempd\@secondoftwo
      \else
        \XKV@toks{#3}%
        \XKV@err{value `\the\XKV@toks' is not allowed}%
        \let\XKV@tempd\@gobble
      \fi
    \else
      \ifx#1\XKV@tempb
        \edef#2{\the\count@}\count@\XKV@tempa
        \ifXKV@pl
          \let\XKV@tempd\XKV@@ch@ckch@ice
        \else
          \let\XKV@tempd\XKV@@ch@ckch@ic@
        \fi
      \else
        \advance\count@\@ne
        \let\XKV@tempd\XKV@tempc
      \fi
    \fi
    \XKV@tempd
  }%
  \XKV@tempc#4,\@nil,%
}
\def\XKV@@ch@ckch@ice#1\@nil,{\@firstoftwo}
\def\XKV@@ch@ckch@ic@#1\@nil,{\@firstofone}
\def\key@ifundefined{\@testopt\XKV@key@ifundefined{KV}}
\def\XKV@key@ifundefined[#1]#2{%
  \XKV@makepf{#1}%
  \XKV@checksanitizeb{#2}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \XKV@key@if@ndefined
}
\def\XKV@key@if@ndefined#1{%
  \XKV@knftrue
  \KV@@sp@def\XKV@tkey{#1}%
  \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{\XKV@header\XKV@tkey}{}{\XKV@knffalse}%
  }%
  \ifXKV@knf
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\def\disable@keys{\XKV@testoptb\XKV@disable@keys}
\def\XKV@disable@keys#1{%
  \XKV@checksanitizeb{#1}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@ifundefined{\XKV@header\XKV@tempa}{%
      \XKV@err{key `\XKV@tempa' undefined}%
    }{%
      \edef\XKV@tempb{%
        \noexpand\XKV@warn{key `\XKV@tempa' has been disabled}%
      }%
      \XKV@ifundefined{\XKV@header\XKV@tempa @default}{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}}%
      }{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}[]}%
      }%
      \expandafter\XKV@tempc\expandafter{\XKV@tempb}%
    }%
  }%
}
\def\presetkeys{\XKV@stfalse\XKV@testoptb\XKV@presetkeys}
\def\gpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@presetkeys}
\def\XKV@presetkeys#1#2{%
  \XKV@pr@setkeys{#1}{preseth}%
  \XKV@pr@setkeys{#2}{presett}%
}
\def\XKV@pr@setkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@checksanitizea{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname
      XKV@\XKV@header#2\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\delpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@delpresetkeys}
\def\gdelpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@delpresetkeys}
\def\XKV@delpresetkeys#1#2{%
  \XKV@d@lpresetkeys{#1}{preseth}%
  \XKV@d@lpresetkeys{#2}{presett}%
}
\def\XKV@d@lpresetkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\unpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@unpresetkeys}
\def\gunpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@unpresetkeys}
\def\XKV@unpresetkeys{%
  \XKV@ifundefined{XKV@\XKV@header preseth}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header preseth\endcsname\@undefined
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header presett\endcsname\@undefined
  }%
}
\def\savekeys{\XKV@stfalse\XKV@testoptb\XKV@savekeys}
\def\gsavekeys{\XKV@sttrue\XKV@testoptb\XKV@savekeys}
\def\XKV@savekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@checksanitizeb{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname XKV@%
      \XKV@header save\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\delsavekeys{\XKV@stfalse\XKV@testoptb\XKV@delsavekeys}
\def\gdelsavekeys{\XKV@sttrue\XKV@testoptb\XKV@delsavekeys}
\def\XKV@delsavekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\unsavekeys{\XKV@stfalse\XKV@testoptb\XKV@unsavekeys}
\def\gunsavekeys{\XKV@sttrue\XKV@testoptb\XKV@unsavekeys}
\def\XKV@unsavekeys{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header save\endcsname\@undefined
  }%
}
\def\setkeys{\XKV@testopta{\XKV@testoptc\XKV@setkeys}}
\def\XKV@setkeys[#1]#2{%
  \XKV@checksanitizea{#2}\XKV@resb
  \let\XKV@naa\@empty
  \XKV@for@o\XKV@resb\XKV@tempa{%
    \expandafter\XKV@g@tkeyname\XKV@tempa=\@nil\XKV@tempa
    \XKV@addtolist@x\XKV@naa\XKV@tempa
  }%
  \let\XKV@rm\@empty
  \XKV@usepresetkeys{#1}{preseth}%
  \expandafter\XKV@s@tkeys\expandafter{\XKV@resb}{#1}%
  \XKV@usepresetkeys{#1}{presett}%
}
\def\XKV@usepresetkeys#1#2{%
  \XKV@presettrue
  \XKV@for@eo\XKV@fams\XKV@tfam{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{XKV@\XKV@header#2}{}{%
      \XKV@toks\expandafter\expandafter\expandafter
        {\csname XKV@\XKV@header#2\endcsname}%
      \@expandtwoargs\XKV@s@tkeys{\the\XKV@toks}%
        {\XKV@naa\ifx\XKV@naa\@empty\else,\fi#1}%
    }%
  }%
  \XKV@presetfalse
}
\def\XKV@s@tkeys#1#2{%
  \XKV@sp@deflist\XKV@na{#2}%
  \XKV@for@n{#1}\CurrentOption{%
    \expandafter\XKV@s@tk@ys\CurrentOption==\@nil
  }%
}
\def\XKV@s@tk@ys#1=#2=#3\@nil{%
  \XKV@g@tkeyname#1=\@nil\XKV@tkey
  \expandafter\KV@@sp@def\expandafter\XKV@tkey\expandafter{\XKV@tkey}%
  \ifx\XKV@tkey\@empty
    \XKV@toks{#2}%
    \ifcat$\the\XKV@toks$\else
      \XKV@err{no key specified for value `\the\XKV@toks'}%
    \fi
  \else
    \@expandtwoargs\in@{,\XKV@tkey,}{,\XKV@na,}%
    \ifin@\else
      \XKV@knftrue
      \KV@@sp@def\XKV@tempa{#2}%
      \ifXKV@preset\XKV@s@tk@ys@{#3}\else
        \ifXKV@pl
          \XKV@for@eo\XKV@fams\XKV@tfam{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \else
          \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \fi
      \fi
      \ifXKV@knf
        \ifXKV@inpox
          \ifx\XKV@doxs\relax
            \ifx\@currext\@clsextension\else
              \let\CurrentOption\XKV@tkey\@unknownoptionerror
            \fi
          \else\XKV@doxs\fi
        \else
          \ifXKV@st
            \global\XKV@addtolist@o\XKV@rm\CurrentOption
          \else
            \XKV@err{`\XKV@tkey' undefined in families `\XKV@fams'}%
          \fi
        \fi
      \else
        \ifXKV@inpox\ifx\XKV@testclass\XKV@documentclass
          \expandafter\XKV@useoption\expandafter{\CurrentOption}%
        \fi\fi
      \fi
    \fi
  \fi
}
\def\XKV@s@tk@ys@#1{%
  \XKV@ifundefined{\XKV@header\XKV@tkey}{}{%
    \XKV@knffalse
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter{\XKV@tempa}%
    \ifx\@empty#1\@empty\XKV@afterelsefi
      \XKV@ifundefined{\XKV@header\XKV@tkey @default}{%
        \XKV@err{no value specified for key `\XKV@tkey'}%
      }{%
        \expandafter\expandafter\expandafter\XKV@default
          \csname\XKV@header\XKV@tkey @default\endcsname\@nil
      }%
    \else\XKV@afterfi
      \XKV@srstate{@\romannumeral\XKV@depth}{}%
      \csname\XKV@header\XKV@tkey\expandafter
        \endcsname\expandafter{\XKV@tempa}\relax
      \XKV@srstate{}{@\romannumeral\XKV@depth}%
    \fi
  }%
}
\def\XKV@testsavekey#1#2{%
  \ifXKV@rkv\else
    \XKV@for@o#1\XKV@resa{%
      \expandafter\XKV@ifcmd\expandafter{\XKV@resa}\global\XKV@resa{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgtrue
        \fi
      }{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgfalse
        \fi
      }%
    }%
  \fi
}
\def\XKV@replacepointers#1{%
  \let\XKV@tempa\@empty
  \let\XKV@resa\@empty
  \XKV@r@placepointers#1\usevalue\@nil
}
\def\XKV@r@placepointers#1\usevalue#2{%
  \XKV@addtomacro@n\XKV@tempa{#1}%
  \def\XKV@tempb{#2}%
  \ifx\XKV@tempb\@nnil\else\XKV@afterfi
    \XKV@ifundefined{XKV@\XKV@header#2@value}{%
      \XKV@err{no value recorded for key `#2'; ignored}%
      \XKV@r@placepointers
    }{%
      \@expandtwoargs\in@{,#2,}{,\XKV@resa,}%
      \ifin@\XKV@afterelsefi
        \XKV@err{back linking pointers; pointer replacement canceled}%
      \else\XKV@afterfi
        \XKV@addtolist@x\XKV@resa{#2}%
        \expandafter\expandafter\expandafter\XKV@r@placepointers
          \csname XKV@\XKV@header#2@value\endcsname
      \fi
    }%
  \fi
}
\def\XKV@default#1#2\@nil{%
  \expandafter\edef\expandafter\XKV@tempa
    \expandafter{\expandafter\@gobble\string#1}%
  \edef\XKV@tempb{\XKV@header\XKV@tkey}%
  \@onelevel@sanitize\XKV@tempb
  \ifx\XKV@tempa\XKV@tempb
    \begingroup
      \expandafter\def\csname\XKV@header\XKV@tkey\endcsname##1{%
        \gdef\XKV@tempa{##1}%
      }%
      \csname\XKV@header\XKV@tkey @default\endcsname
    \endgroup
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter
      {\XKV@tempa}\XKV@afterelsefi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \expandafter#1\expandafter{\XKV@tempa}\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \else\XKV@afterfi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \csname\XKV@header\XKV@tkey @default\endcsname\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \fi
}
\def\setrmkeys{\XKV@testopta{\XKV@testoptc\XKV@setrmkeys}}
\def\XKV@setrmkeys[#1]{%
  \def\XKV@tempa{\XKV@setkeys[#1]}%
  \expandafter\XKV@tempa\expandafter{\XKV@rm}%
}
\XKVcatcodes
\endinput
%%
%% End of file `xkeyval.tex'.

